Ibn al-\v{S}\=atir, L'ach\`evement de l'enqu\^ete et la correction des fondements / Kit\=ab nih\=aya al-s\=ul f\=i tash\=ih al-'us\=ul. \'Edition, traduction et commentaire math\'ematique par Erwan Pench\`evre

This book is a critical edition of a treatise of astronomy by the Syrian scholar Ibn al-\v{S}\=atir (1304-1375). The Arabic text has been established on the basis of several manuscript copies, and it has been translated into French; a bilingual index is also provided. This treatise is one of the latest and one of the most elaborate medieval work on theoretical astronomy; it is famous today for having provided the first viable lunar model in terms of the distance Moon-Earth. Although demonstrations have been consigned to another manuscript which is now lost, we reconstruct the physical models in our mathematical commentary, and we attempt at a better historical understanding of the nascent concepts of space transformations, solid reference frames, trajectory, etc. Predictions of the models are to be compared to observations and to other contemporary models, as well as theoretical premises; in turn, when records of observations are missing, those have to be recalculated by modern means. Part of our commentary is devoted to the latitudinal movement of the five planets: Ibn al-\v{S}\=atir's work on this problem belongs to a tradition initiated by Ibn al-Haytham three centuries before. Ibn al-\v{S}\=atir addresses a clever criticism to the work of his predecessor Nas\=ir al-D\=in al-T\=us\=i on this problem, thus revealing a better understanding of affine rotations in space. Many other criticisms by Ibn al-\v{S}\=atir, especially to the astronomers working at Mar\=a\.ga during the 13th century, also contribute to a better knowledge of their own work.

==> fichier2a.tex <==
% pour toute l'intro, on a mis des directives \iscomplet et \VARC
% qui permettent de faire disparaître à loisir les mss. B et E

% pour les chapitres 1 à 11, l'apparat critique contient B et E

\begin{arab}
\resetlinenumber\pagewiselinenumbers

\begin{center}
\LARGE kitAb nihAyaT al-sUl fI ta.s.hI.h al-'u.sUl
\end{center}
bism\fol{.z 1 \ma\\.z 21 \md\\.z 1 \mc} al-ll_ah
al-ra.hmn al-ra.hIm al-lahum .sl `l_A m.hmd wa-'Alh
al-.hmd lillah .hmd"aN ylyq bjlAlh, wa-\VAR{.sl_A al-ll_ah}{.sl_A
al-ll_ah wa-salam [\mc]} `l_A sayidnA m.hmd wa-'Alh.

wa-b`d fa-'innahu yaqUl `lI bin 'ibrAhIm bin m.hmd bin al-^sA.tr
al-mu'aqt bi-al-jAmi` al-'ummawI, \VAR{`fA al-ll_ah `nh}{r.hmh
al-ll_ah [\md,\mc]} :

.gr.dnA an nUrid fI h_dh al-maqAlaT hI'aT 'aflAk al-kawAkab `l_A
al-wjh alla_dI ibtakarnAh, wa-hwa al-sAlim min al-^sukUk al-mwAfq
lil-'ir.sAd al-.sa.hI.haT, mjrrdaT"aN `n al-barAhIn, biqawl"iN wjIz
li-yshl al-'i.tlA` `layhA, wa-al-'intifA` bihA. wa-n.dIf il_A _dlika
mA yjb i.dAfath \VARC{mimmA}{famA [\mb]} y.htAj ilayhi
wa-\VAR{nstdll}{ystdll \iscomplet{[\mb,\mc,\md,\me]}{[\md,\mc]}}
`layhi min al-'u.sUl wa-al-masA'il al-.durUriyaT.

wa-h_dA ma.tlab"uN jalIl"uN, i_d y`rf bihi \VAR{'a.hwAl
al-'ajrAm}{\iscomplet{nAq.saT [\mb,\me], }{}a.hwl al-'ajrAm [\ma]}
al-`lwiyaT wa-al-safaliyaT min jihaT \VARC{kmiyAthA}{kmAtihA [\mb]},
wa-maqAdIr al-'ab`Ad wa-al-'ajrAm al-`lwyaT 
wa-al-safaliyaT min jihaT kmyAthA, wa-b`.d kayfiyAthA, wa-'aw.dA`
.harakAthA, wa-mqAdIrhA wa-jihAthA, wa-maqAdIr al-'ab`Ad wa-al-'ajrAm
wa-mA ytfr`u min _dlika mimmA hwa m`lUm"uN ma^shUr"uN.

wa-qd tqddm b.tlmyws wa-.gayrh min al-mtqddmIn wa-al-mta'a_h_hrIn
\VAR{bw.d` 'u.sUl"iN}{biw.d` \iscomplet{[\mb,\mc,\md],
bi-'aw.dA` [\me]}{[\md,\mc]}},
illA annahA lA tf_A \VARC{bi-al-m.tlUb}{bi-al-m.t [\me]}, li-annahA
m_hAlifaT"aN limA \VAR{qad}{nAqi.saT [\mc]} tqrr-r min al-'u.sUl
al-hndsiyyaT wa-al-.tabI`iyyaT. wa-qad awrd jmA`aT"aN min m.hqq-qI
h_dA al-`ilm `l_A tilka al-'u.sUl ^sukUk"aN
\VARC{yqynyh}{byyanaT"aN [\mb,\me]}.
wa-awrdnA na.hnu ^skUk"aN 'A_har wqfnA
\VARC{`layhA}{`layh [\me]} bi-al-ra.sd wa-.gayrh.

wa-lam ymkin man \VARC{kAn}{nAqi.saT [\me]} qblanA w.d` 'u.sUl tf_A
bi-al-maq.sUd min .gayr m_hAlifaT"aN lil-'ir.sAd al-.sa.hI.haT, kamA
_dakarwA fI ktbhm. wa-qd tatabba`nA tilka al-^sukUk al-wArdaT `l_A
tilka al-'u.sUl, wa-^sara.hnA _dlika fI kitAbnA alla_dI smynAh bita`lIq
al-'ir.sAd. wa-nUrdu h_dihi al-^sukUk fI 'awwal h_dihi al-maqAlaT min
.gayr barAhIn `layhA wa-lA ^sr.h lahA, .hatt_A yu`lm `_drnA fImA
qulnAh, wa-`.zm fA'idaT mA 'ibtakarnAh. wa-lA y`lm _dlika illA man
a.hA.t `ilm"aN bimA \VAR{ibtakarth al-mutaqaddimUn
  wa-al-muta'a_h_hirUn}{abkrth al-mtaqaddimUn wa-al-muta'a_h_hirUn
  [\ma]\iscomplet{, ibtakarth al-mtaqaddimIn wa-al-muta'a_h_hirIn [\mb]}{}},
  min m_hAlifaT \VAR{tilk}{slk [\mc]} al-'u.sUl limA yjb min al-'u.sUl,
wa-\VAR{'istifrA.g}{'istiqrA` [\ma]} al-jhd minhm `l_A w.d` 'u.sUl
tf_A bi-al-maq.sUd.

\clearpage
falam ywffqwA li-_dalika, wa-qad wfq al-ll_ah \VAR{ta`Al_A}{nAqi.saT
  \iscomplet{[\ma,\mb,\me]}{[\ma]}}
  wa-lah al-.hmd \VAR{lil-'aml}{lil-'amr [\ma]}
al-ma`jUz `nh, wa-_dakarnA jamI` mqddmAt ha_dihi al-'u.sUl, wa-mA
ytfrr` minhA wa-al-barAhIn `layhA fI \VAR{kitAb}{kitAbnA [\mc]} ta`lIq
al-'ir.sAd. wa-.gr.dnA an njrrd tilka al-u.sUl `n al-barAhIn, wa-nUrd
tilka al-^sukUk kamA qulnA, wa-nas'al al-ll_ah al-twfIq wa-al-`.smaT.
wa-qad j`lthA ta^stml \VAR{`l_A maqAlatayn 'ammA al-maqAlaT al-'awwal
  fa-annahA mu^stamalaT `l_A _talA_tIn bAb"aN wa-_hAtimaT
  fa-al-mqdmaT}{\iscomplet{`l_A mqddmaT wa-_talA_tIn bAb"aN wa-_hAtimaT ammA
  al-mqdmaT [\me], }{}`l_A mqdmaT wa-_hAtimaT 'ammA al-mqdmaT
  \iscomplet{[\ma,\mb,\md]}{[\ma,\md]}. ktb fI
  hAmi^s [\md] >>w _talA_tIn bAb"aN<<}
\VAR{n_dkrhA fI f.slayn}{fI al-hAmi^s [\ma]}.

\clearpage
\begin{center}
  \Large al-mqddmaT

  \large al-fa.sl al-'awwal
\end{center}
i`lam an \textbf{al-`Alam} ism limA .hwAh al-s.t.h al-.zAhir
min al-falak al-'a`l_A al-'awwal al-msm_A mu.hddid al-jihAt i_d bih
wa-bimarkazh \VAR{tat.hddad}{yt.hddad \iscomplet{[\md,\me]}{[\md]}}
jihatA al-`lw wa-al-sfl. wa-hwa al-bsI.t al-m.tlq.

wa-al-'ajsAm tnqsm il_A \textbf{basI.t} wa-\textbf{mrkb}.
fa-al-basI.t mA yata^sAbh
'ajzA'uhu wa-.tbA`uhu, \VARC{'a`nI}{y`nI [\mb,\me]} lA ynqsm il_A
\VARC{ajsAm}{aqsAm [\me]} m_htlfaT al-.sUr wa-al-.tbA` ; bal lahu
.tabI`aT wA.hidaT y.sdr `nhA mA y.sdr `l_A nahj \VARC{wA.hid}{wA.hidaT
[\mb]}. wa-al-mrkb .diddh.

wa-al-basI.t, ynqsm il_A \textbf{a_tIriy}
wa-\textbf{`n.sriy}. fa-al-a_tIriy, hwa al-'aflAk bimA fIhA min
al-kawAkab. wa-\VARC{ysmm_A}{tsmm_A [\me]} al-`Alam al-`lwiy
wa-`Alam al-'aflAk wa-al-samawAt. wa-al-qsm al-_tAniy, hwa al-`nA.sr
al-'arba`aT al-ma^shUraT.
wa-\VAR{ysmm_A}{tsmm_A \iscomplet{[\mc,\md,\me]}{[\md,\mc]}}
\VARC{al-istiq.sAt}{al-is.tqsAt [\me]} bimA fIhA min al-murakkabAt.
wa-\VARC{ysmm_A}{tsmm_A [\me]} bi-al-`Alam al-safliy wa-`Alam al-kwn
wa-al-fsAd wa-makAn al-`nA.sr wa-al-mrkbAt minhA ta.hta falak
al-qamar.

wa-ynqsimu il_A tAmm al-tarkIb .hAfi.z al-.sUraT muddaT"aN wa-il_A .gyr
\VAR{tAmh}{tAm \iscomplet{[\mb,\mc,\me]}{[\mc]}} .gyr .hAfi.z lil-.sUraT.
wa-al-qsm al-'awwal, hwa al-mwAlId \VAR{al-_talA_taT}{al-talataT
[\md]}, wa-hya al-m`dn, wa-al-nabAt, wa-al-.hayawAn. fa-al-m`dn mA
lA yakUn fIhi\fol{w 22 \md} quwwaT nAmyaT, wa-al-nabAt mA fIhi quwwaT
nAmyaT min .gayr idrAk"iN, wa-al-.hayawAn mA fIhi quwwaT nAmyaT ma`a idrAk.
wa-al-qsm al-_tAniy min al-mrkb, hwa al-msmm_A bi-al-a_tAr al-`lwiyaT,
\VAR{ka-al-s.hb wa-al-^shb _dwAt al-a_dnAb}{ka-al-^shb _dwAt al-a_dnAb
wa-al-s.hb [\mc]\iscomplet{, ka-al-s.hb wa-al-^shb wa-_dwAt al-a_dnAb [\me]}{}}
wa-na.hwahA. wa-'amkinaT al-mrkbAt \VARC{'amkinaT}{m` makAn [\me]}
al-juz'i al-.gAlib fIhA, m` `adam al-mjA_dbAt.

wa-al-.harakaT hiya kwn al-^say' al-muta.harrk fImA bayna al-mubtada'i
wa-al-mnth_A, bi.hay_tu yakUn .hAlh fI kull 'An"iN m_hAlif"aN limA b`dh
wa-mA qablah.

\clearpage
\noindent wa-al-.harakaT 'immA `r.diyyaT, 'aw qsriyyaT, 'aw
'irAdiyyaT, 'aw .tabI`iyyaT, 'aw mA ytrkb min al-.tabI`iyaT, ka.harakAt
al-kwAkab fa-annahA mrkkbaT"uN basI.taT wa-`l_A qwl"iN mrkbaT
'irAdiyaT. \textbf{fa-al-.harakaT al-`r.diyaT} hiya ka.harakaT sAkin
al-safInaT. wa-\textbf{al-qsriyaT} hiya \VARC{ka.harakaT}{.harakaT [\me]}
al-safInaT wa-hya mustafAdaT min sabab _hArijy.
\textbf{\VAR{wa-al-'irAdiyaT}{wa-'irAdiyaT
\iscomplet{[\ma,\md,\mb]}{[\ma,\md]}}}
ka.harakaT al-.hayawAn allatI yakUn lahA ^su`Ur.
wa-\textbf{al-.tabI`iyaT} in lA yakUn lahA ^su`Ur bimA y.sdr `nhA,
ka.harakaT al-`nA.sr, \VARC{w al-'aflAk `l_A qwl"iN}{[\me] tzId fI
al-hAmi^s >>`.tf `l_A al-`nA.sr lA al-'aflAk<<}, wa-al-nbAt.

wa-al-.harakaT al-.tabI`iyaT tnqsm il_A \textbf{mA lA yakUn `l_A nahj
wA.hid"iN}, ka.harakaT al-nabAt, wa-il_A \textbf{mA yakUn `l_A nahj
wA.hid}.  wa-hiya tnqsm `l_A mA\fol{.z 2 \mc} ar_A qsmayn:
mustaqImaT wa-mustadIraT.
\textbf{fa-al-mustaqImaT} .tlb al-ws.t wa-t_ht.s bi-al-`nA.sr,
\VARC{wa-al-mrkbAt minhA}{wa-al-mrkbAt minhA `ndI [\mb]}.
wa-\textbf{al-mustadIraT} ka.harakaT\fol{.z 2 \ma} al-'aflAk
\VARC{`ndI}{nAqi.saT [\mb]}.

wa-`nd .tA'ifaT"iN an al-'irAdiyaT tnqsm il_A \textbf{mA lA yakUn `l_A
nahj wA.hid"iN} ka.harakaT al-.hayawAn wa-il_A \textbf{mA yakUn `l_A
nahj wA.hid} ka.harakaT al-'aflAk `l_A marAkazhA. wa-`nd ha_dihi
al-.tA'ifaT an al-'aflAk wa-al-kawAkib lahA ^s`Ur, wa-`nd 'u_hr_A
innahA basA'i.t laysa lahA ^su`Ur. wa-anA ar_A anhA murkbaT .gayr
al-tAsi` minhA, lakin min .gayr al-`nA.sir.

wa-al-.harakaT al-falakiyaT al-mfrdaT mA \VAR{y.sdr}{t.sdr [\ma]} `n
\VAR{m.hrk"iN}{\iscomplet{mt.hrk"iN [\mb,\me], }{}t.hrk [\mc]}
wA.hid"iN basI.t, wa-\VARC{al-mrkbaT}{al-mrkb hwa [\me]} mA
\VARC{t.sdr}{y.sdr [\mb,\me]}
\VAR{min}{`an \iscomplet{[\md,\mb,\me]}{[\md]}} jumlaT
basA'i.t fawqa wA.hidaT"iN. fakull mufardaT"iN basI.taT, wa-kull
m_htalfaT mrkbaT; likawn ba`.d al-.harakAt al-falakiyaT basI.taT
mrkbaT `l_A mA ya't_A \VARC{bayAnh}{bitmAmh [\mb]} in ^sA al-ll_ah ta`Al_A.

wa-al-m.htAj il_A taqdImh min al-.tabI`iyyAt sb` masA'il :

\textbf{al-mas'alaT al-'Ul_A}, an al-_hlA' m.hAl, wa-al-sukUn fI
al-'aflAk m.hAl.

\clearpage
\textbf{al-mas'alaT al-_tAniyaT}, an likull .harakaT mubtada'"uN.
wa-al-mt.hrk
'in \VARC{lam yfArqh}{fArqh [\mb]} mabda'uhu bi-al-w.d`, \VAR{bi.hay_tu
an yakUn}{yjb an yakUn [\md], yjb an takUn [\mc]\iscomplet{, bi.hay_tu an lA
takUn [\mb],}{,} .gayr maqrU' [\ma]} al-i^sAraT al-.hsiyaT ilayhi
wA.hidaT, qIl annahu mt.hrrk binafsihi. wa-'in \VAR{fAraqh bi.hay_tu
y"unsb al-ta.harruk}{\iscomplet{yfAriqh bi.hay_tu ynsb al-t.hrrk [\me], lam
yfAriqh bi.hay_tu ynsb al-t.hrk [\mb], }{}fAraqah binisb
al-ta.hrIk [\ma,\md], fAraqh sbab al-t.hrk [\mc]} ilayh
wa-\VAR{al-ta.hrIk}{al-t.hrk [\mc]} il_A mA fIhi mabda'uhu, qIl annhu
mt.hrrk bi.gayrihi.

\textbf{al-mas'alaT al-_tAli_taT}, .zuhUr .harakaT ajsAm lA
\VARC{takUn}{yakUn [\mb,\me]} mt.hrrkaT binafsihA
bl \VARC{takUn}{yakUn [\me]} min t.hrIk 'ajsAm 'u_har mt.hrrkaT
binafsihA.

\textbf{al-mas'alaT al-rAbi`aT}, kull \VAR{mA fIhi mabda'"uN}{fI
hAmi^s [\ma]} \VAR{.harakaT"iN}{.harakath [\ma]} mustadIraT \VAR{fahwa lA
yqbl}{fahya lA tqbl [\md,\mc]} al-.harakaT al-mustaqImaT,
wa-bi-al-`ks, illA bi-al-qsr.

\textbf{al-mas'alaT al-_hAmisaT}, lA yumkin an ykUn fI mt.harrak
basI.t mabda' .harakatayn m_htalifatayn li-'anna i_htilAf al-.harakAt
\VAR{yqt.d_A}{\iscomplet{tqt.d_A [\mb], _Aqt.d_A [\me], }{}.gayr maqrU' [\ma]}
i_htilAf al-mt.hrkAt. wa-likull m_htlf al-.harakaT min al-falakiyAt
.harakaT min nafsihi wa-'u_hr_A min .gayrihi.

\textbf{al-mas'alaT al-sAdisaT}, al-'aflAk lA tqbl al-.harakaT
al-mustaqImaT, wa-lA yjUz an ykUn .harakaT al-kawkab fI al-samA'
ka.harakaT al-samak fI al-mA'.

\textbf{al-mas'alaT al-sAbi`aT}, an \VAR{.harakAt}{.harakaT [\md,\mc]}
al-'aflAk `l_A nahj wA.hid"iN, falA \VARC{tsr`}{ysr` [\mb,\me]} wa-lA
\VARC{t"ub.ti'}{yb.t_A [\mb,\me]}, wa-lA yakUn lahA rujU`
\VARC{qabla}{qIl [\mb]} tamAm al-dawraT, \VARC{w-lA}{falA [\me]} wuqUf,
wa-lA _hurUj min .hayyiz"iN, wa-lA i_htilAf .hAl"iN. bl abad"aN
mt.harkaT .harakaT"aN basI.taT"aN mustadIraT"aN il_A al-jihaT allat_A
kAnat tmIlu ilayhA. wa-mA wjd fIhA bi-al-ra.sad _hilAf _dalika fahwa
bi-al-`r.d min tarkIb .harakAt basI.taT.

faha_dihi al-'u.sUl lA yjUz al-_hurUj `n mqt.dAhA, wa-mqt.d_A al-hI'aT
allat_A \VARC{wAfaqa}{wqf [\mb], fI [\me] ktb fwq al-s.tr
  >>wAqafa<<}\fol{w 3 \mc} `layhA b.tlmyws wa-wAfaqa `layhA .gayrh lA
\VAR{ywAfq}{twAfq [\mc]} ha_dihi al-'u.sUl, wa-lA mA
\VAR{tkllfUh}{tklfh \iscomplet{[\mc,\me]}{[\mc]}}
afA.dl al-muta'a_h_hirIn `l_A mA .zhr `nhm fI kutubihim.

\clearpage
\begin{center}
\large al-fa.sl al-_tAniy
\end{center}
fI al-^sukUk wa-al-m.hAlAt allat_A waqfnA `layhA fI
\VARC{al-hI'aT}{al-hay'aAt [\mb,\me]} al-ma^shUraT.

famin\fol{w 3 \ma} _dalika \textbf{al-falak al-_hArij al-markaz} i_dA kAna
mu.hI.t"aN bimarkaz al-`Alam mu.hAl, li-annahu ylzm minh an ykUn fI al-'aflAk
al-mu.hI.taT bimarkaz al-`Alam i^skAl .gayr tAmmaT al-istidAraT
wa-.gayr mt.hrrkaT. wa-in \VAR{t.hrrk}{t.harakh [\md]} .hawla markaz
al-`Alam lzm an ykUn hunAk _hilAf ; wa-in t.hrk al-_hArij
al-markaz\fol{.z 22 \md}
.harakaT mustawiyaT `nd markazh lzm an ykUn
\VAR{mu.hI.t"aN}{mu.hI.t \iscomplet{[\ma,\mb,\me]}{[\ma]}}
bimarkaz al-`Alam .harakAt .gayr mutasAwiyaT, fa-in
jAz _dalika \VARC{falA .drUraT liwa.d` al-'aflAk}{famA al-.durUraT
  liwa.d` al-'aflAk lA [\me]} \VARC{bal nqUl an likull kawkab"iN
  falak yu.hrkh .harakaT mu_htalifaT fa-yqf wa-yrj` wa-ysr` wa-yb.t_A
  wa-h_dA mu.hAl}{fI hAmi^s [\me]}. wa-hwa m` .harakaT al-'awj 'a^sd
mu.hAl"aN, wa-lammA kAna al-awj fI rAy b.tlmyws _tAbit"aN a_htAra
al-_hArij al-markaz. wa-'ammA falak al-tadwIr fI al-^sams fahwa jA'iz
illA annahu lam ywAfq daqIq al-ra.sad `l_A mA \VAR{tqf}{tfq [\md]}
`layhi fI _dkr hI'aT al-^sams wa-_dalika annA wjdnA i_htilAf al-^sams
wa-hwa al-ta`dIl .gayr mwAfiq fI 'an.sAf 'arbA` min.tqaT al-burUj
lidaqIq al-ra.sad.

wa-min al-^sukUk fI aflAk al-qamar. al-_hArij al-markaz fIhA mu.hAl.
wa-istiwA' .harakaT \VAR{al-_hArij}{nAqi.saT [\md,\mc]} al-markaz
\VARC{`nd}{fI hAmi^s [\me]} .gayr markazh m.hAl. wa-mu.hA_dAT q.tr
al-tadwIr li.gayr markaz .hAmilh m.hAl ; fa-annahu y.zhr minh an falak
al-tadwIr \VARC{takUn}{yakUn [\mb]} .harakath mu_htalifaT wa-ykUn fIh
.harakatAn mstawiyaT wa-mu_htalifaT wa-al-mu_htalifaT lA tkml
al-dawraT wa-h_dA mu.hAl. wa-_dalika \VAR{y`.t_A}{yqt.d_A [\md],
  al-mqt.d_A [\mc]} an ykUn q.tr al-qamar fI al-trbI`In .d`f q.tr
al-qamar fI al-abdAr, wa-h_dA m.hAl li-annahu lam y"ura k_dalika.

\clearpage
\noindent wa-y.zhr bidaqIq al-ra.sad \VAR{annahu}{li-annahu [\mc]}, i_dA kAna
ba`d al-qamar min al-^sams brj wa-n.sf,
\VAR{m_hAlifaT}{m.hAl \iscomplet{[\mb,\mc,\md,\me]}{[\md,\mc]}}
fI tqwImh bitilka al-u.sUl lmA yqt.dyh
al-ra.sad al-.sa.hI.h. wa-lam y_dkr b.tlmyws wa-lA .gayrh r.sd taqwIm
al-qamar fI tilka al-mwA.d`. wa-\VAR{ta.hdId}{tajdId [\mc]} ws.th
wa-markazh \VAR{min dA'iraT}{fI hAmi^s [\ma]}
\VAR{^sabIhaT}{ta^sbIh-h \iscomplet{[\ma,\mb,\md]}{[\ma,\md]}}
\VARC{min falak}{bifalak [\me]} al-burUj m.hAl
li-annahA lam tu'_h"a_du min dA'iraT wA.hidaT wa-lA nuq.taT wA.hidaT.

wa-al-falak al-_hArij al-markaz fI bAq_A \VARC{al-syAraT}{al-syArAt
  [\me]} mu.hAl, lammA qulnA wa-istiwA' .harkaT al-_hawArij
al-marAkiz `nda \VARC{.gayr marAkizhA}{marAkiz .gayrhA [\mb]} m.hAl.
wa-qawlhm an al-_hArij al-markaz fI s.t.h al-mA'il wa-s.t.h
al-_hArij al-markaz \VAR{tqA.t`}{yqA.t` [\mc,\md]} al-muma_t_tal `l_A
nuq.tatayn mutqAbilatayn (wa-humA al-ra's wa-al-_dnb), m.hAl, li-anna
al-`.zImaT mA \VAR{yq.t`hA}{tq.t`hA [\md]} bin.sfayn \VARC{illA
  `.zImaT}{fI hAmi^s [\me]}, wa-al-_hArij\fol{.z 3 \mc} al-markaz
laysa bi`.zIm~; famu.hAl an yqA.t` al-muma_t_tal `l_A nuq.tatayn
mutaqAbilatayn, wa-fIhi diqqaT, fata'amlihu. wa-mu.hA_dAT q.tr al-tadwIr
\VAR{li.gayr}{li.did [\ma]} markaz .hAmilh, \VAR{m.hAl}{fwq al-s.tr
  [\md]}, kamA w.d`wA _dalika fI aflAk al-kawAkib al-_hamsaT.
wa-al-falak al-m`ddl al-masIr mu.hAl. wa-hwa\fol{.z 3 \ma} tawahhum kA_dib.
wa-tawahhum _h.t.t"iN a.had .trfayh _tAbit fI markaz m`ddl al-masIr,
wa-\VARC{.trfh}{.trfayh [\me]} al-'A_har y.tUl wa-yq.sr wa-ymrr bi-markaz
\VAR{tadAwIr}{tdwAyr [\md]\iscomplet{, dawA'ir [\me]}{}}
al-kawAkib wa-ydIrhA .hwl tilka al-nuq.taT, m.hAl. wa-laysa lil-_ha.t.t jism,
wa-y.htAj il_A _hlA', wa-il_A .gayr _dlika min al-m.hAlAt
\VAR{al-lAzimaT}{al-mulAzimaT ? [\ma]} \VARC{`nh}{minh [\me]}. wa-kwn
'aqrb qrb `.tArd fI .gayr mqAbalaT al-'awj m.hAl bimA t.hqq-q
\VAR{bi-al-ra.sad}{al-ra.sad [\md]}, lA bi-al-ta.sawur. wa-t.swr
'aflAk fI 'aflAk tadAwIr al-kawAkib al-sayyAraT, `l_A al-wjh alla_dI
\VAR{_dkrh}{_dkr [\ma]} b.tlmyws fI \textbf{\VARC{al-iqti.sA.s}{fi al-hAmi^s
    [\me]}}, \VAR{tamIl}{ym_tl [\mc,\md]\iscomplet{, ymIl [\me]}{}}
su.tU.hhA `n s.t.h al-burUj, li-ajl .harakaT `r.d al-kawkab, m.hAl.

al-w.d` alla_dI _dakarah al-n.sIr al-.tUsI fI \textbf{al-ta_dkiraT} fI izAlaT
^skUk aflAk al-qamar m.hAl
\VAR{li-wjd al-_hArij al-markaz wa-li-mu.hA_dAT}{\iscomplet{li-wujUd
    al-_hArij al-markaz [\mb], li-wujUd al-_hArij al-markaz
    wa-li-mu.hA_dAT [\me], }{}li-wujUd al-_hArij wa-li-mu.hA_dAT [\mc,\md]}
q.tr al-tadwIr li.gayr markaz .hAmil al-tadwIr.

\clearpage
al-w.d` alla_dI _dakarah al-na.sIr al-.tUsI fI 'i.slA.h hI'aT
al-kawAkib al-'arba`, z.hl, wa-al-m^strI, wa-al-mari_h, wa-al-zhraT,
m.hAl, libaqA' al-_hawArij \VARC{al-marAkiz}{al-markaz [\mb], nAqi.saT
  [\me]}, wa-m`ddlAt al-masIr, wa-i_htilAf al-_hA.saT
\VAR{li.harakaT}{bi.harakaT [\mc]}
\VAR{_dirwaT}{dwraT \iscomplet{[\mb,\mc,\md,\me]}{[\md,\mc]}}
al-tadAwIr, il_A .gayr _dlika min al-m.hAlAt.
wa-qad a`trf r.hmh \VARC{al-ll_ah}{nAqi.saT [\me]} bi-al-`jz `n
'a.sl yfI bi-al-maq.sUd.

al-w.d` alla_dI \VARC{.hdsh}{a.hd_t [\me]} al-mwyd al-`r.dI fI
\textbf{hI'aT 'aflAk al-qamar} min qlbh lijihaT .harakaT al-_hArij
al-markaz wa-i_htilAf \VAR{_dirwaT}{dwraT [\mc,\md]} al-tadwIr
\VAR{bi-mu.hA_dAtihA}{li-mu.hA_dAtihA \iscomplet{[\mb,\mc,\md,\me]}{[\md,\mc]}}
\VAR{linuq.taT}{al-nuq.taT [\mc]} .gayr markaz .hAmil al-tadwIr, m.hAl.

al-w.d` alla_dI _dkarh al-mwyd al-`r.dI fI 'i.slA.h 'aflAk al-sayyAraT
m.hAl libaqA' al-_hArij al-markaz, wa-m`dlAt al-masIr,\fol{w 23 \md}
wa-.gayr _dlika.

al-w.d` alla_dI _dakarah q.tb al-dIn al-^sIrAzI fI 'i.slA.h hI'aT
'aflAk al-qamar m.hAl, libaqA' al-_hArij al-markaz wa-linuq.taT
al-mu.hA_dAT. wa-al-.hujjaT allatI i.htj bihA, r.hmh al-ll_ah, `l_A jiwAz
nuq.taT al-mu.hA_dAT \VARC{fI}{min [\me]} al-qamar, min
\VARC{am.hal}{nAq.saT [\mb,\me]} al-m.hAlAt wa-tawahhum kA_dib.
wa-qad rj` `n _dalika fI \textbf{al-tu.hfaT}, wa-_dakara fIhA
\VAR{wjh}{wjhA [\md]} 'A_har, wa-hwa m.hAl ay.d"aN.

al-'a.sl alla_dI sammAhu al-abdA`I \VARC{fI}{fI al-hAmi^s [\me]}
fAsid `rU.d al-kawAkib m.hAl.

\VAR{al-w.d`}{w al-w.d` [\mc]} alla_dI _dakarahu fI 'i.slA.h
\VAR{'aflAk}{fwq al-s.tr [\mc]} al-kawAkib \VAR{al-sayyAraT}{fwq
  al-s.t.h [\md]} m.hAl liwujUd
\VARC{al-_hwArij al-marAkiz}{al-_hArij al-markaz [\mb,\me]}
fIhA, wa-m`dlAt al-masIr, wa-i_htilAf
\VAR{_dirwatay}{.gayr maqrU' \iscomplet{[\ma,\mb]}{[\ma]}, dwrt_A
  [\mc,\md]} al-tadwIr.

.harakaT \VAR{al-'iqbAl}{.gayr maqrU' [\ma]} wa-al-'idbAr .gayr
.sa.hI.haT lim_hAlifatihA limA\fol{w 4 \mc} .s.h.h bi-al-'ar.sAd qadIm"aN
wa-.hadI_t"aN. m` annahu ta.sawwur kA_dib ma`a imkAn ta.swr w.d` 'aflAk
ylzm `nhA tilka al-.harakaT. law kAna lahA .haqIqaT, wa-laqad qwwmt
al-^sams \VAR{birA_A}{bir_A [\mc]\iscomplet{, bisiw_A [\mb], siw_A [\me]}{}}
al-zarqAlaT, fawjdthA \VAR{ynq.s}{tnq.s [\mc,\md]} `n al-.sa.hI.h
\VAR{_tl_t}{_tlA_t \iscomplet{[\mb,\mc,\me]}{[\mc]}}
darjAt"iN wa-ak_tar min n.sf
darjaT"iN, h_dA wa-al-.harakaT \VAR{mqblaT}{.gayr maqrU' [\ma]}.
falaw kAnat mudbraT \VAR{kAnat}{lkAnat [\mc]}\fol{w 4 \ma} al-m_hAlifaT
ak_tar min \VARC{i_tn_A `^sar}{i_tnatA `^sar [\me]}
darjaT i_dA kAna fI nihAyaT
al-adbAr.

\clearpage
\noindent wa-qad qwwmt qlb al-asad bitilka al-.harakaT, falam ywAfiq
limA hwa \VARC{`layhi}{`layhA [\me]}, wa-_hAlafa \VARC{sA'ir}{fI
  al-hAmi^s [\me]} mA _dakara min 'ar.sAd _dalika
\VARC{al-kawkab}{al-kawAkib [\mb,\me]} min qadIm il_A yawuminA
h_dA mu_hAlifaT fA.hi^saT tazId \VAR{fI al-.gAlib arba` darjAt"iN
  il_A darjatayn}{`l_A d darjAt il_A darjatayn fI al-.gAlib [\mc]}.
  wa-lam ajd fI al-'u.sUl mA fIhi h_dA al-miqdAr min al-_hl-l. 
% A 4r l. 3-4
wa-qad tu.haqqiqu bi-al-ra.sad
an .harakaT al-_tawAbit .harakaT"uN basI.taT"uN mustawiyaT"uN .hawla
markaz al-`Alam wa-`l_A qu.tbay al-burUj il_A jihaT al-ma^srq.
\VARC{fa_hlAf}{w _hlAf [\mb,\me]} _dalika m.hAl.

qwl \VARC{al-majrI.tI}{fwq al-s.tr [\me]} an .harakAt jamI` 'aflAk
al-kawAkib min al-ma^srq il_A al-m.grib, wa-mA \VARC{tr_A}{y"ur_A
  [\mb,\me]} min al-.harakAt il_A jihaT al-ma^srq
\VARC{fa_dalika}{ka_dalika [\me]} min taq.sIr al-.harakAt
al-^sarqiyyaT min al-l.hUq bi-al-.harakaT al-yawmiyyaT, m.hAl.

wa-qawlh 'anna
\VAR{q.tb}{nAqi.saT \iscomplet{[\mb,\md,\me]}{[\md]}} falak al-burUj
ydUr fI dA'iraT (.hawla q.tb al-`Alam) \VARC{smthA}{fI hAmi^s [\me]
  s`rhA?  s`rathA?} mqdAr al-mIl al-a`.zm, il_A jihaT al-ma^sriq, min
taq.sIr .harakaT al-falak al-_tAmin, m.hAl. wa-_dalika ltbddl 'ajzA'i
m`ddl al-nhAr m`a 'ajzA'i al-burUj. wa-al-ta.hqIq _hlAfah. wa-m_tAl
_dalika, anna q.tb falak al-burUj i_dA t.hrrk, bitq.sIrh, il_A jihaT
al-m^srq, rb` dA'iraT al-mIl, wa-'a_hrajnA dA'iraT `.zImaT tmrr biq.tbay
falak al-burUj wa-q.tbay m`dl al-nahAr wa-bi-al-munqalbayn, marrat
bi-al-juz'i alla_dI kAna y.hA_dI
\VAR{al-'awwal min}{\iscomplet{fI al-hAmi^s [\me], al-'awwal [\mb], }{}
  'awwal [\ma,\mc,\md]} brj al-.haml min
dA'iraT m`ddl al-nahAr. wa-qad t.hqq-q bi-al-ra.sad _tibAt al-nuq.t
al-'arba` min m`ddl al-nahAr~: wa-innamA ytbddl `l_A tilka
\VAR{al-nuq.t}{al-nuq.taT [\mc,\md]} bi-'ajzA'i al-burUj al-mkwkbaT
lA al-burUj
\VAR{al-.haqIqiyyaT}{al-.haqIqaT \iscomplet{[\mb,\md]}{[\md]}}.
famA qAlah m.hAl fI al-tawahhum wa-al-wjUd.

wa-kamA jwwz .harakaT q.tbay \VAR{falak}{fwq al-s.tr [\mc,\md]}
al-burUj il_A jihaT al-ma^srq .hawla q.tbay m`dl al-nahAr, yjUz
.harakaT .gayrh il_A al-ma^srq~; fah_dA .gayr mA \VAR{ankrh}{.gayr
  maqrU' \iscomplet{[\ma,\mb]}{[\ma]}} min wjUd
\VARC{.harakaT}{.harakath [\me]} il_A jihaT al-ma^srq. wa-qwlh an
al-.harakAt allatI il_A jihaT al-ma^srq min taq.sIr
\VARC{al-_tAmin}{al-nAs [\mb]} wa-.gayrh bA.til. wa-qad qAm al-burhAn
`l_A wujUdhA wa-dall `l_A anna\fol{.z 4 \mc} taq.sIr al-falak bimiqdAr
ha_dihi al-.harakaT m.hAl.

\clearpage
qwl man qAl an likull kawkab falak wA.hid yt.harrak bihi .hawla q.tbay
falak al-burUj il_A jihaT al-ma^srq, bitaq.sIrh ay.d"aN, ytwlld min
\VARC{ha_dayni}{hAtayni, fI al-hAmi^s [\me]} al-.harakatyn
\VARC{lil-kawAkib}{nAqi.saT [\mb,\me]} wqUf wa-rujU`, wa-istiqAmaT
wa-mIl il_A al-jihatayn, wa-.gayr _dalika mimmA wjd lil-kawAkib, qwl
bA.til. wa-qad tatb``t _dalika wa-aqmt \VARC{al-burhAn}{al-barAhIn
  [\me]} `l_A ab.tAlihi fI kitAbI al-msmmI \textbf{bita`lIq al-'ar.sAd}.

\VAR{jamI`}{w jamI` [\mc]} mA tklfh al-majrI.tI fI rsAlatihi min
t.gyyr al-.harakAt wa-'i_tbAt falak al-^sms .hwl markaz al-`Alam,
markazh _hArij `n q.tb al-`Alam\fol{.z 4 \ma}, wa-in
\VARC{q.tbay}{q.tb [\mb,\me]} falak al-^sms ydUr `l_A \VAR{tilka
  al-dA'iraT}{\iscomplet{tilka al-dA'ir [\mb], }{} tilka al-dawA'ir
  [\mc,\md]} al-_hArijaT al-markaz il_A jihaT al-m^srq bitaq.sIr
_dlika al-falak, m.hAl. wa-_dlika an m.hwr falak al-^sms i_dA dAra fI
_hArij al-markaz `l_A q.tbay m`ddl al-nahAr, \VARC{rsmt}{w smt [\me]}
al-^sams, bal kll nuq.taT \VARC{tfr.d}{yfr.d [\me]} fI s.t.h falak
al-^sams, falak _hArij al-markaz~; wa-hwa .gyr mA \VAR{a_dkurh}{.gayr
  maqrU' [\ma], ankrUh \iscomplet{[\mb,\mc,\md], _dakarUh
    [\me]}{[\md,\mc]}}. `l_A an mA _dkrUh .gyr m.tAbq al-ra.sd~;
faqad tbyn ab.tAl _dlika.

al-.harakaT \VAR{al-lwlbyaT}{al-.tUliyyaT [\mc,\md]}
allatI\fol{.z 23 \md} _dkrhA
\VAR{aris.twA}{aris.tw \iscomplet{[\mc,\me]}{[\mc]}}
lA y.zhr minhA lil-kwkb sur`aT
wa-lA bu.tw wa-lA wqUf wa-lA rujU`. wa-hya i^sAraT il_A madArihA
\VAR{alla_dI}{allat_A [\mc]} \VARC{trsmh}{yrsmh [\me]}
bi-al-.harakatIn al-ywmyaT wa-al-_hA.s.saT bihA, lA .gyr. wa-bayAn
_dlika an al-^sms i_dA kAnat fI ra's al-jdI _tmm ta.harrakat fI ni.sf
snaT il_A ra's al-sir.tAn, \VAR{fa-in al-^sms}{fa-inhA [\mc]} trsm
madAr"aN .halzawny"aN .hwl markaz al-`Alam. wa-il_A h_dA a^sAra
aris.twA bi-al-.harakaT \VAR{al-lwlbyaT}{al-kwkbyaT [\mc,\md]}, lA
.gyr. f.zn man sm` _dlika an maq.sUd aris.twA anna al-^sams, i_dA
ta.harrakat .harakaT \VAR{lwlbyaT"aN}{kwkbyat"aN [\mc,\md]}, .h.sl
i_htilAf .harakaT al-^sms, wa-`l_A _dlika \VARC{.gyrhA}{.gayr [\mb]} min
al-kwAkb, wa-hwa m.hAl.

kull .harakaT mustawyaT `nd nuq.taT fahya mu_htalifaT `nd 'u_hr_A,
wa-`aksh. fa-`al_A _dlika kull falak .harakath mustawyaT `nd
\VARC{.gyr}{nAqi.saT [\me]} markazh fa.harakath mrkkbaT.

\VAR{min}{fI al-hAmi^s [\md], nAqi.saT
  \iscomplet{[\ma,\mb,\mc,\me]}{[\ma,\mc]}} wjUd 'aflAk .s.gAr
ka'aflAk al-tdAwIr, .gyr m.hI.taT bmrkz al-`Alm, .gayr m-mtn` fI siw_A
al-falak al-tAsi`. wa-ydll `l_A _dlk annah kmA wjd fI kll falak
kawkab"iN, wa-fI al-_tAmin kwAkb"uN ka_tIraT \VARC{kryT}{kraT
  [\mb,\me]}, kll wA.hid minhA 'a`.zam min b`.d tdAwIr b`.d al-kawAkib
\VAR{w al-kawkab}{nAqi.saT [\mc,\md]} m_hAlf"uN lijism al-falak. flA
ymtn` wjUd 'aflAk tdAwIr wa-n.hwhA, wa-min \VAR{hunA}{h_dA
  \iscomplet{[\mb,\mc,\md,\me]}{[\md,\mc]}} yfhm an al-'aflAk
fIhA\fol{w 5 \mc} tarkIb mA~; wa-al-basI.t al-m.tlq, hw al-tAsi`,
wa-lA ymkn an yt.swwr fIh kawkab"uN wa-lA .gayrh.

\clearpage
\VAR{w.d` al-man^sUraT}{w.d` al-man^sUrAt \iscomplet{[\mc,\md,\me]}{[\md,\mc]},
  wa-ktb >>w.d`<< fwq al-s.tr fI [\mc]}
\VAR{alla_dI}{allat_A \iscomplet{[\mb,\mc,\md,\me]}{[\md,\mc]}}
_dkarahA b.tlmyws fI kitAbihi
\VAR{al-ma`rUf}{al-msm_A [\mc]} \textbf{bi-al-iqti.sA.s} bA.til"uN.

mA _dkarah ibn afla.h wa-al-mu'ayyid al-`r.dI min kwn al-zhraT fwq
al-^sms, wa-mA istadalla bihi, m.hAl.

taqArub min.taqaT \VAR{falak}{fwq al-s.tr [\mc]} al-burUj min
min.taqaT m`ddl al-nahAr, wa-tabA`udhA `nhA, m.hAl.

al-mIl al-a`.zm lA y_htalif bi-i_htilAf al-zamAn wa-lA bi-i_htilAf
al-makAn. wa-mA wjd \VARC{fIhi}{nAqi.saT [\me]} min al-i_htilAf
fa_dalika min qbl al-alAt, wa-i_htilAf n.sbhA, wa-min qbl
\VAR{i_htilAf}{fI al-hAmi^s [\mc]} .zl a.trAf al-maqAyIs, wa-min qbl
i_htilAf ^su`A` al-^sams al-dA_hil min
\VAR{jrm}{_hrm \iscomplet{[\mc,\mb,\me]}{[\mc]}}
\VARC{al-hdf}{al-hdb [\mb]}, wa-min kwn markaz .hjm
al-ar.d .gyr m.tAbiq limarkaz al-`Alam, `l_A n.hw mA ^sr.hnAh fI
\VAR{kitAbI}{kitAbinA \iscomplet{[\mc,\me]}{[\mc]}}
al-mawsUm \textbf{bita`lIq al-'ar.sAd}.

\VARC{mA _dkr}{fwq al-s.tr [\me]} \VARC{`n}{min [\mb,\me]} al-hnUd
\VAR{wa-.gyrhm}{fI al-hAmi^s [\mc]},\fol{w 5 \ma} 'an jumlaT mIl
al-^sms 'arba`aT wa-`^srUn darjaT, bA.tl, lA .haqIqaT lah. wa-ka'anna
h_dh \VAR{al-.tA'ifaT}{.gayr maqrU' [\ma]} t^sIr il_A al-jism alla_dI
y.hw_A mIl al-^sms il_A al-jihatayn~; wa-anna `r.dh _tmAnyaT
wa-\VARC{'arba`Un}{'arba`In [\me]} darjaT wa-nu.sfh 'arba`aT wa-`^srUn
darjaT, wa-_dlika il_A muntah_A `r.d al-^sms, \VAR{fayakUn}{fatakUn
  [\mc]} il_A \textbf{markazhA} lA \VAR{yazId}{tazId [\mc,\md]} `l_A
\aemph{kj lA}. fa-in kAna `l_A \VAR{h_dA}{fwq al-s.tr [\mc]} rAy h_dh
al-.tA'ifaT fahwa .s.hI.h wa-illA falA.

\clearpage
\begin{center}
\Large al-bAb al-'awwal

\large fI u.sUl"iN maw.dU`aT musallamaT fI al-hndsaT mttafaq `lyhA
\end{center}
al-nq.taT wa-al-_h.t.t wa-al-zAwyaT wa-al-s.t.h
wa-al-dA'irT wa-al-kuraT mawujUdaT m`lUmaT al-.sUr. wa-inn
kll wA.hd"iN mn al-nq.taT wa-al-_h.t.t al-mstqIm wa-al-s.t.h
al-mstwI wa-al-zAwyaT yn.tbq `l_A m_tlh.
wa-inna al-fa.sl al-mu^starak bayna kull _ha.t.tayn nuq.taT,
wa-bayna kull s.t.hayn _ha.t.t, wa-bayna kull jsmayn s.t.h.

wa-lanA an nfr.d _ha.t.t"aN `l_A ayy s.t.h"iN kAn, 'aw mArr binuq.taT
kyf \VAR{^si'nA}{^si'ta [\me]}, wa-in \VAR{tu`yn}{n`yyn
[\mb,\md,\me]} nq.taT `l_A ay _h.t.t 'aw s.t.h"iN kAn, wa-in
\VAR{n.sl}{itt.sl [\mb], y.sl [\md]} _ha.t.t"aN mustaqIm"aN 
\VAR{m.hdUd"aN}{mj_dUr"aN [\md]} `l_A ay s.t.h"iN 'aw jsm"iN
^si'nA, wa-in \VAR{narsamu}{tarsamu [\ma,\mb]} `l_A kll nq.taT"iN
wa-\VAR{bikull}{likull [\mb]} b`d"iN dA'iraT.

wa-inna al-zwAyA al-qA'imT \VAR{mtsAwyT wa-i_dA qAm 
_h.t.t mstqIm `l_A _h.t mstqIm fa-'immA an y.hd_t zAwytyn}{nAqi.saT 
[\mb,\me], wa-ktb fI hAmi^s [\me]: >>mtsAwyT wa-i_dA qAm _h.t.t mstqIm 
`l_A _h.t mstqIm fa-'imma an y.hd_t<<} \VAR{qAymatayn}{fI al-hAmi^s [\ma]} 
'aw zAwyatayn .hAddaT wa-mnfrjT, \VAR{w}{nAqi.saT [\ma,\mb,\md,\me]} mjmU` 
al-zAwyatIn qAymatayn. wa-inna majmU` ziwAyA kull m_tl_t 
\VAR{qA'imtayn}{qA'imatAn [\mb,\me]}.

\clearpage
\begin{center}
\Large al-bAb al-_tAny

\large fImA \VAR{tqrriru}{nqriru [\ma]} min al-u.sUl
\end{center}
qd tqrrar 'istdAraT al-s.t.h 
al-.zAhr mn al-ar.d wa-al-mA bi-al-taqrIb.

wa-inna istdAraT al-samA' ka-istidAraT al-kuraT.

wa-inna al-ar.d `nd al-samA' kmrkz\fol{.z 5 \mc} al-krT `nd m.hI.thA.

wa-inna lhA \VAR{qdr m.hsUs}{qdr"aN m.hsUs"aN [\mc]} fImA
dUn flk al-marI_h.

wa-inna mrkz _tqlhA \VAR{m.tAbq}{y.tAbq [\mc]} lmrkz al-`Alm,
lA mrkz .hjmhA, sAkinaT \VAR{fIh}{nAqi.saT [\me]}
\VAR{.gyr}{lA [\mc]} mt.harakaT il_A jihaT mn al-jihAt.

wa-inna al-fwq, il_A mA yl_A al-samA' wa-yab`d mn al-mrkz ; wa-al-t.ht 
mA yl_A al-markz. wa-mIl al-a_tqAl jmI`hA il_A al-mrkz, wa-mIl mA hw _hfIf 
il_A al-m.hI.t.

\clearpage
\begin{center}
\Large al-bAb al-_tAl_t

\large fI trtIb al-'aflAk wa-hy \VAR{ts`T}{nAqi.saT [\mb], fI al-hAmi^s [\me]}
\end{center}
'awwalhA wa-hw al-m.hI.t bi-al-_tmAniyyaT, wa-^sklh kurYY, wa-mrkzh
mrkz al-`Alm,\fol{w 24 \md} wa-lh q.tbAn yt.hrrk `lyhmA .hwl mrkzh alla_dI hw mrkz al-`Alm 
wa-mrkz al-kll, .hrkT mstwyT fy al-yawm blaylatihi dwraT wA.hidaT 
\VAR{binfs m.tAl` mA tat.hrkh al-^sms fI yawm bilaylatihi}{fI hAmi^s [\mc], binfs m.tAl` mA 
tat.hrkh al-^sms fI yawm wa-laylaT [\mb], yatanaffas m.tAl` mA _At.harrakh 
al-^sams fI yawm wa-laylatihi [\me], bi^sams m.tAl` mA tat.hrkh al-^sms 
fI yawm bilaylatihi [\md]}, wa-bh_dh al-.harakaT tata.harrak jamI` 
al-AflAk min al-ma^srq il_A al-ma.grb .hwla markazh wa-`l_A q.tbyhi. 
wa-min.taqaT h_dihi al-.harakaT, wa-hy\fol{.z 5 \ma} allatI b`dhA min
\VAR{al-q.tbayn}{.gayr maqrU' [\ma], al-nuq.tatayn [\mb]} `l_A al-sawA',
\VAR{w}{nAqi.saT [\mc]} tusamm_A min.taqaT \textbf{mu`addl al-nhAr}.
\VAR{w al-q.tb alla_dI `al_A ^simAl mustaqbali al-ma^sriq yqAlu lahu q.tb m`ddl
al-nhAr}{fI al-hAmi^s [\me]} al-^simAly, wa-n.zIrh al-q.tb al-jnUby. wa-yfr.d fy
s.t.h \VAR{dA'iraT}{fwq al-s.tr [\mc]} m`ddl al-nhAr dA'iraT
\VAR{_tAnyaT}{_tAbitaT [\me]}, wa-mu.hI.thA mqsUm bi-al-'ajzA'i
wa-ksUrhA allatI hya _tl_tmi'aT wa-\VAR{sittIn}{sittUn [\md]} juz'"aN,
wa-\VAR{tsmm_A}{ysm_A [\mb]} h_dhi \VAR{al-aqsAm}{fI al-hAmi^s [\mc]}
bi-azmAn m`ddl al-nahAr, wa-\VAR{bi-'ajzA'i}{'ajzA'i [\mc]} m`ddl al-nahAr
ay.d"aN; liyqAs bihA al-.harakAt lifr.d _tbAthA. wa-h_dA al-falak, a`n_A
al-'awwal, hwa al-basI.t al-mu.tlaq
\VAR{al-m.hd_A}{m.hddad [\mc,\md,\me]} lil-jihAt al-msmm_A 
\textbf{bi-al-a.tlas}.

wa-al-flk al-_tAny, wa-hw flak al-kwAkb al-musammAh bi-al-_twAbit, wa-^sklh 
kurYY, m.hddbh mumAss limq``r al-tAs`, wa-mq``rh mumAss lim.hddb 
\VAR{al-flk}{nAqi.saT [\mc]} al-sAb` al-m.hI.t bi-aflAk z.hl. wa-lahu q.tbAni 
_tAbitAni \VAR{w}{nAqi.saT [\mc]} yta.harak `alyhumA .hwla markaz al-`Alam 
.harakaT basI.taT mstawiyyaT min jihaT al-ma.grb 'il_A jihaT al-ma^srq, `l_A 
mA t.haqiqu \VAR{bi-al-burhAn}{bi-al-barAhIn [\me]} wa-al-r.sd. wa-min.tqaT 
ha_dihi al-.harakaT, allatI ba`duhA min q.tbay h_dA al-flk `l_A al-sawA', 
marsUmaT `l_A \VAR{s.t.hh}{s.t.h [\me]}, mqsUmaT bi-al-brUj al-i_tn_A `^sr 
wa-drjhA wa-ksUrhA, mubtadi'"aN min al-tqA.t` al-m.hA_dy li.sUraT al-.hml min 
\VAR{al-mukwkab}{al-kawAkib [\me]} `inda 'awwal al-tasmyaT `l_A mA hwa 
ma^shUr.

wa-s.t.h ha_dihi al-min.taqaT mAyl `an s.t.h falak m`ddl al-nahAr 
\aemph{kj lA}, wa-hwa al-mIl al-a`.zam.

\clearpage
\noindent wa-\VAR{nfr.d}{yfr.d [\mc,\md,\me]} 
dA'iraT `.zImaT tmrr biqu.tbay \VAR{m`ddl}{m`tdl [\mb]} al-nahAr\fol{w 6 \mc} wa-bqu.tbay 
flk al-brUj \VAR{fatq.t`}{fayq.t` [\mb]} \VAR{min.taqaT}{minq.a.taT [\me]} 
falak al-brUj `l_A nuq.tatayn, \VAR{w al-taqA.tu`}{fa-al-tqA.t` [\ma]} 
al-qarIb \VAR{min}{fI [\me]} al-q.tb al-^simAly ysmm_A \textbf{al-mnqlb
al-.sayfiyy}, wa-al-_tAnI \textbf{al-mnqlb al-^satawI}. wa-s.t.h al-burUj
yq.t` m`ddl al-nhAr `l_A nq.tatayn, fa-al-nuq.taT allatI qbl al-mnqlb
al-.sayfiyy \VAR{tsmI}{ysmI [\mb,\md]} \textbf{al-i`tidAl al-rabI`iyy},
wa-allatI qbl al-mnqlb al-^stwiyy \VAR{tsm_A}{nAqi.saT
[\ma,\mb,\md,\me]} \textbf{al-i`tidAl al-_hrIfiyy}. wa-h_dhi 
al-nq.t \VAR{al-arba`aT}{al-arba` [\ma,\me]} _tAbtaT .gyr mt.hrkaT `mmA 
\VAR{t.hA_dyh}{y.hA_dyh [\mc]} min dA'iraT m`ddl al-nahAr. fayfr.d mA bayna 
kull nuq.tatayn maqsUm bi_talA_taT 'aqsAm"iN mutasAwyaT, 
wa-\VAR{yatawahhm}{natawahhm [\ma,\mb]} \VAR{st}{sittaT [\mc]} dawA'ir `i.zAm 
mArraT biq.tbay al-burUj \VAR{w bitilka al-aqsAm}{fI al-hAmi^s [\ma]},
\VAR{fayataqasam}{faynqsm [\mb], fatanqsm [\me], fataqsm [\mc,\md]} bihA 
al-min.tqaT \VAR{i_tn_A}{i_tnA [\md]} `^sr qsmaN 
\VAR{mutasAwyaT"aN}{mutasAwyaT sit dawA'ir [\mb] mutasAwiy"aN wa sit 
dawA'ir [\me]},
wa-k_dlika jmlaT basI.t al-_tAmin.
wa-kll qsm"iN minhA ysmm_A \textbf{brj"aN} wa-kll brj maqsUm _tlA_tIn 
qsm"aN \VAR{mustawiyaT}{mustawiy"an [\me]} tsm_A drj al-brUj.

wa-kAna fI 
qdIm al-zmAn \VAR{m.hA_dI lil-qism}{y.ha_dI al-qism [\mb,\me]} all_dI 
'awwalahu al-'i`tidAl al-rabI`iyy .sUraT al-.hml min al-flak al-_tAmn al-mkwkb.
ysamm_A h_dA al-qism bi-al-.hml, wa-al-_tAnI bimA kAn y.hA_dyh wa-hw al-_tawr, 
_tmm al-jawzA', _tmm\fol{w 6 \ma} al-sir.tAn, il_A 'A_hir al-i_tn_A `^sr, `l_A mA hw m^shUr. 
wa-il_A .hdUd _tmAn 
\VAR{mi'aT}{fI al-hAmi^s [\me]} wa-`^srIn min ta'rI_h al-hjraT, y.hA_dI 
al-qsm al-'awwal .sUraT al-.hwt min \VAR{al-mkwkb}{al-kwkb [\mb], al-kawAkib 
[\me]}; \VAR{fayntql}{fatantaqilu [\me]} al-.sawr il_A twAl_A al-brUj 
brj wA.hd, fay.hA_dI al-'aqsAm \VAR{al-_tAbitaT}{al-_tAniyaT [\mc,\me]} 
.gyr mA kAna y.hA_dyhA. fayajUz .haynay_d \VAR{an}{bi-an [\mc]} ysmm_A al-qsm 
al-'awwal al-.hwt wa-al-_tAnI al-.hml wa-al-_tAli_t al-_twr 'il_A 
\VAR{'A_hirhA}{al-'A_hir [\mc]}. 
wa-yajUz baqA' ismAyhA `alayhA, wa-lA yn.zuru il_A mA 
\VAR{y.hA_dI}{y.hA_dyhA [\mc]} min .sUr al-burUj 
\VAR{al-mukwkbaT}{al-kawkabiyyaT [\mb,\me]}. wa-qd t.hqaqa bi-al-r.sd 
an mqdAr h_dhi al-.harakaT fI \VAR{kll}{nAqi.saT [\ma,\mb,\md,\me]} 
sab`In snaT fArisiyyaT drjaT wA.hidaT, wa-`nda b.tulamyUs fI kll mi'aT sanaT 
drjaT \VAR{wA.hidaT}{nAqi.saT [\ma,\mb,\me]}, wa-`nda\fol{.z 24 \md} al-mt'a_h_hrIn
fI kll mi'aT \VAR{sanaT}{nAqi.saT [\mb]} drjaT wa-n.sf, wa-`nda b`.dhum fI kll 
sb`In snaT drjaT min al-sinIn al-fArisiyyaT.

\clearpage

wa-i_dA tqrrara _dlk fa-i`lam anna al-flk al-adn_A wa-hw al-'awwal lil-qmr, 
wa-al-_tAnI li`i.tArd, wa-al-_tAli_t \VAR{lil-zhraT}{lizhraT [\me]}, 
wa-al-rAb` lil-^sms, wa-al-_hAmis lil-marI_h, wa-al-sAdis lil-m^strI, 
wa-al-sAb` liz.hl, wa-al-_tAmn \VAR{mr.s.s` fIh al-kwAkb}{mw.d`
al-kwAkb [\mb,\mc,\me], mr.s.s` bi-al-kwAkb [\md]}
al-_tAbitaT smmyt bi_dlika li_tibAt aw.dA`hA \VAR{b`.dhA}{fI 
al-hAmi^s [\md], b`.d [\me]} min b`.d"iN, _tmm al-tAs` al-mutaqaddm\fol{.z 6 \mc}
_dkrh al-mt.hrrak \VAR{`l_A}{`n [\mc,\md]} q.tbayhi wa-.hwl mrkzh min al-m^srq 
il_A al-m.grb \VAR{al-.harakaT}{bi-al-.harakaT [\md]} al-yawmiyyaT.
wa-\VAR{yt.harrak biha_dhi al-.harakaT}{biha_dhi al-.harakaT tat.hrk [\mc]} 
'aflAk al-kwAkb al-sb`aT `l_A mwAza'aT \VAR{min.tqaT}{fwq al-s.tr [\mc]} 
m`ddl al-nhAr, wa-yl_A flk al-qmr flk al-nAr, _tm al-hwA _tm al-mA' _tm 
al-trAb wa-hw kuraT al-ar.d. wa-qd tqddm tqrIr _dlka, wa-qd bayyanA .d`f dlIl 
min 'istidll \VAR{`l_A an}{bi-an [\mc]} al-zhraT fwq al-^sms, wa-lam 
\VAR{yr}{yr_A [\mb,\me]} _dlika \VAR{min ahl}{ahl"uN [\mb,\md,\me]} 
al-`lm illA qalIl"aN. wa-qd ^sr.hnA _dlika fI .gyr mw.d` min kutubnA,
\VAR{w al-ll_ah 'a`lm}{nAqi.saT [\me]}.

\clearpage
\begin{center}
\Large al-bAb al-rAbi`

\large fI al-dawA'ir al-ma^shUraT wa-`r.d al-bld
\end{center}
a^shr al-dwA'ir al-`i.zAm dA'iraT \textbf{m`ddl al-nhAr}.
wa-hya allatI b`dhA min q.tbay m`ddl al-nahAr sawA', wa-hya min.taqaT
al-.harakaT al-ywmyyaT wa-dA'iraT al-istiwA' wa-al-i`tidAl. wa-yfr.d
s.t.hhA fA.sil"aN li-kuraT al-ar.d, \VAR{faysmm_A}{faysmmA [\mc]}
_h.t.t al-istiwA' li-istiwA' al-lyl wa-al-nahAr `l_A jamI` al-skkAn
`lyh, wa-_dlika likwn al-falak ydUr hunAka \VAR{dUlAbI}{dUlAbiy"aN
[\me]} wa-q.tbay m`ddl al-nahAr `l_A al-ufuq. wa-limA kAnat al-ar.d
kuryaT _tAbitaT fI markaz al-`Alam, kAna al-_dAhb min _h.t.t
al-istiwA' `l_A al-ar.d il_A jihaT al-^simAl, yartafi`u al-q.tb
al-^simAliyy `n ufuqh; wa-al-_dAhib il_A jihaT al-junUb, yartafi`u
al-q.tb al-junUby `n ufuqihi. wa-bimiqdAr irtifA`
a.hdhumA,\fol{.z 6 \ma} \VAR{yan_haf.d}{yan.haf.d [\me]} al-'A_har.

\VAR{faysmm_A}{fatsmm_A [\me]} irtifA`
al-q.tb \textbf{`r.d al-bld}. wa-hwa qws min al-dA'iraT al-mArraT bisamt
al-ra's \VAR{w q.tbay m`ddl al-nahAr}{fImA bayna al-q.tb wa-al-ufuq [\me]},
\VAR{w ha_dA al-qws musAwyaT li-in.hfA.t al-q.tb al-'A_har, wa-hya
  ay.d"aN musAwyaT liba`d dA'iraT m`ddl al-nahAr min samt al-ra's fI
  tilka al-bq`aT}{fI al-hAmi^s [\me], wa-ha_dA al-qws musAwyaT
  li-in_hfA.d al-q.tb al-'A_har, wa-hya ay.d"aN musAwyaT liba`d dA'iraT
  m`ddl al-nahAr min samt al-ra's fI tilka al-bq`aT [\ma,\mc,\md]}
\VAR{fI tilka al-ufuq}{nAqi.saT [\ma,\mb,\mc,\md]}.

\textbf{dA'iraT ni.sf al-nahAr} wa-.tUl al-bld wa-hya al-fA.silaT li-jamI`
al-madArAt al-.zAhiraT binu.sfayn. wa-hya al-mArraT bi-al-qu.tb
al-.zAhir wa-smt al-ra's. wa-hya t_htlf bi-al-ta^srIq wa-al-ta.grIb
wa-lA t_htlf \VAR{bi-al-slUk}{bi-al-^sukUk [\mc], bi-al-^sulUk
  [\md]} ^smAl"aN wa-\VAR{lA}{nAqi.saT [\ma,\mc,\me,\md]}
junUb"aN.

wa-\VAR{nfri.du}{yfri.du [\mc,\md]} likull bld dA'iraT
ni.sf \VAR{nahAr}{al-nahAr [\me,\mc,\md]},
wa-\VAR{natawahhamu}{yatawahham [\mc,\md]} kull wA.hidaT minhA
fA.silaT likuraT al-ar.d 'aw murtasamaT `layhA. \VAR{fImA}{famA [\ma],
  .gayr maqrU' [\mb,\me]} bayna dA'iraT ni.sf al-nahAr al-mArraT
bi-'awwal al-ma`mUr min jihaT al-ma.grb wa-dA'iraT ni.sf
\VAR{al-nahAr}{nahAr [\mb,\mc,\me,\md]} bq`aT"iN mafrU.daT"iN, hwa
\textbf{.tUl al-bld}. wa-.gAyatuha mi'aT wa-_tmAnIn darjaT.
wa-.gAyaT al-`r.d tis`Un darjaT. \VAR{w}{min [\me]} _dlika `nd
kwn \VAR{a.hd}{a.hd_A [\mb,\mc,\md]} q.tbay al-`Alam
`l_A smt al-ra's. wa-yadUru al-falak
hunAka \VAR{ra.hAwiyy"aN}{ra.hawiyy"aN [\mc]}, wa-yadUr fI bAqy\fol{w 7 \mc}
al-`rU.d \VAR{.hamA'iliyy}{.hamA'iliyy"aN [\me,\mc?]}.

\clearpage
\noindent wa-al-maskUn
min .zhr al-ar.d min _h.t.t al-istiwA' il_A .hay_tu irtifA` al-q.tb
al-^smAlI msAw"iN litamAm al-mIl al-a`.zm, wa-hwa \aemph{sw k.t}, wa-fI
al-.tUl min .tUl darjaT"iN il_A tamAm mi'aT wa-_tamAnIn darjaT.

wa-\VAR{i_dA}{i_d [\mb,\md]} tqrrir _dlika, fa-aqUlu an -- min
al-dawA'ir al-ma^shUraT -- ay.d"aN \VAR{dA'iraT}{nAqi.saT [\md]}
min.taqaT al-burUj. wa-hya min.taqaT \VAR{al-falak}{fwq al-s.tr
  [\md]} al-_tAmin wa-tsmm_A bi.tarIqaT al-^sams,
\VAR{limusAmataT}{li-mumAsaT [\mc]} \VAR{al-^sams}{bi-al-^sams
  [\me]} lahA abad"aN. wa-\VAR{natawahhamu}{yatawahhamu [\mc]} h_dh
al-dA'iraT fA.silaT lijamI` al-'aflAk \VAR{fatarsamu}{fayarsamu
  [\mc,\md]} fI kull falak"iN dA'iraT `a.zImaT tsmm_A \textbf{bi-al-falak
al-muma_t_tal}. wa-al-ni.sf min min.taqaT al-burUj alla_dI ibtidA'uhu
nq.taT al-i`tidAl al-rabI`I ^smAliyy"uN `n m`ddl al-nahAr, wa-al-ni.sf
al-'A_har junUbI `nh. wa-kull wA.hid"iN minhumA maqsUm bisittaT aqsAm,
ysmm_A kull qism \textbf{brj"aN} \VAR{`lay mA tqddm}{nAqi.saT [\me]}.

wa-min al-dawA'ir al-`i.zAm \textbf{dA'iraT al-mIl}. wa-hya\fol{w 25 \md}
\VAR{al-`a.zImaT al-mArraT}{dA'iraT `a.zImaT mArraT [\mc], al-`azImaT [\me],
  wa-ktb >>al-mArraT<< fI hAmi^s [\me]} bq.tbay m`ddl al-nahAr
wa-bi-ayy juz'i kAn 'aw \VAR{bikawkab}{kutiba fI [\me] ta.hta
  al-sa.t.h >>bal bi-.trf _h.t.t mArraT bimarkaz al-kawkab _hArij `n
  markaz al-`Alam<<} mafrU.d"iN; \VAR{fayaq.t`}{fataq.t`
  [\mc,\me,\md]} min.taqaT m`ddl al-nahAr. wa-al-qws al-.s.gr_A
al-wAqi`aT minhA bayna _dlika al-juz'i wa-m`ddl al-nahAr hya mIl
_dlika al-juz'i wa-\VAR{ysmm_A}{tsmm_A [\me]} \textbf{al-mIl al-'awwal}.
fa-in kAnat hya al-mArraT bira's al-sir.tAn wa-al-jdy,
\VAR{fatamurru}{fayamurru [\me]} .haynay_d biq.tbay falak al-burUj
ay.d"aN wa-yakUn al-mIl fI nihAyatihi. fa-in furi.dat mArraT bikwkab
kAn mA bayna al-kwkab wa-\VAR{bayna}{nAqi.saT [\ma,\mb,\me,\md]}
m`ddl al-nahAr minhA hwa b`d _dlika al-kwkb `n m`ddl al-nahAr.
wa-nuq.taT \VAR{taqA.tu`hA}{mqA.t`hA [\me,\md]} limu`ddl al-nahAr
hya \textbf{ma.tAli`} darjaT mumrr \VAR{_dlika}{nAqi.saT [\mc]} al-kwkab
bidA'iraT ni.sf al-nahAr; wa-nq.taT \VAR{taqA.tu`hA}{mqA.t`hA [\me]}
limin.taqaT al-burUj \VAR{al-_tAnyaT}{al-_tAbitaT [\me,\mc,\md]}
\VAR{hya}{nAsi_h [\me] kataba ba`dhA >>min.taqaT<<} darjaT mumrr
_dlika al-kawkab.

wa-min \VAR{al-dawA'ir}{nAqi.saT [\ma,\mb,\me,\md]} al-`.zAm,
\textbf{dA'iraT al-`r.d}.\fol{w 7 \ma} wa-hya al-`.zImaT al-mutawahhamaT al-mArraT
biq.tbay falak al-burUj wa-bijuz'"iN mafrU.d"iN min al-burUj 'aw bikwkab.
wa-\VAR{t`rf}{y`rf [\mc,\md]} \textbf{bidA'iraT al-mIl al-_tAnI}. wa-al-qws
al-.s.gr_A al-wAqi`aT minhA bayna min.tqatay al-burUj wa-m`ddl
al-nahAr hya mIl _dlika al-juz'i al-_tAnI, wa-yqAl lahu \textbf{`r.d} _dlika
al-juz'i ay.d"aN.

\clearpage
\noindent fa-in marrat bikwkab, kAna mA bayna al-kwkab
wa-min.tqaT al-burUj minhA min al-jihaT al-aqrab \textbf{`r.d} _dlika al-kwkb;
wa-al-qws al-.s.gr_A minhA allatI fImA
bayna al-kwkb wa-m`ddl al-nahAr
hwa `r.d _dlika al-kwkab al-m`ddl wa-ysmm_A \textbf{\VAR{.h.s.saT}{bi.h.s.saT
  [\mc,\md]} `r.d} al-kwkab ay.d"aN. wa-dA'iraT al-`r.d i_dA marrat
bikwkab mafrU.d"iN\fol{.z 7 \mc} wa-q.t`at min.tqaT al-burUj, q.t`ath \VAR{`l_A}{fwq
  al-s.tr [\md]} darjaT \textbf{.tUl} _dlika al-kwkab. wa-ibtidA a.twAl
\VAR{al-kwkb}{al-kawAkib [\mb,\mc,\md]} min \VAR{nuq.taT}{min.tqaT
  [\mb]} al-i`tidAl al-rabI`I, wa-hya ra's al-.hml, i.s.tilA.h"aN. wa-in
q.t`at \VAR{lim`ddl}{al-m`ddl [\mb]} al-nahAr, kAna _dlika al-taqA.t`
.tUl _dlika al-kwkab al-m`ddl. wa-in kAna \VAR{al-juz'u
  al-mafrU.d}{al-juz'u wa-al-mfrU.d [\mc]} 'a.had al-inqilAbIn,
.tAbaqat lidA'iraT al-mIl al-'awwal: wa-kAnat hya al-mArraT biq.tbay
falak al-burUj wa-biq.tbay m`dl al-nahAr, wa-itt.hd al-mIlAn al-'awwal
wa-al-_tAnI, wa-kAna kull wA.hid"iN minhumA fI nihAyatihi
wa-hwa \aemph{kj lA}.

wa-min al-dawA'ir al-ma^shUraT \textbf{dA'iraT al-ufuq}.
wa-hya al-fA.silaT bayna al-.zAhir wa-al-_hfI min al-falak.
wa-'a.had q.tbayhA \textbf{smt al-ra's}, wa-al-'A_har \textbf{smt al-qdm}.
wa-`l_A h_dh al-dA'iraT yakUn al-.tulU`
wa-al-.grUb. wa-hya trsm min \VAR{al-_h.t.t}{nAqi.saT [\me]}
al-_hArij min \VAR{al-b.sIr}{al-b.sr [\mb,\me,\mc,\md]} al-mumAss
likuraT al-ar.d muntah_A il_A al-tAsi`; fa-inna al-.zAhir
yakUn ak_tr min al-_hfI.

\VAR{w qUl man qAl bi-an al-.zAhir ak_tr min
  al-_hfI}{fI al-hAmi^s [\md]} bimiqdAr arba` daqA'iq wa-sitt
wa-`^srIn _tAnyaT laysa bi.sa.hI.h. \VAR{fa-in}{fa-inny
  [\mb,\me,\mc]} wjdtu bi-al-ra.sd an \VAR{qismay}{qis_A
  [\me,\mc]} al-^sams wa-al-kwAkb al-.zAhiraT ak_tr min al-ma.hsUb
bimiqdAr mu_htalif yazId `l_A \VAR{_tul_tay darjaT}{\aemph{m} daqIqaT
  [\mc]}, wa-_dlika mrkb min \VAR{in.hdAr}{in.h_dAr [\mc]}
\VAR{al-ba.sIr}{al-ba.sr [\mb,\me,\mc]} wa-min
\VAR{in_hfA.s}{in.hfA.z [\mb,\me]} markaz .hjm \VAR{kuraT}{fwq
  al-s.tr [\mc]} al-ar.d `n markaz al-`Alam. wa-_dlika
\VAR{likwn}{li-yakUn [\mb,\mc]} al-m.tAbiq limarkaz al-`Alam hwa
markaz _tql al-ar.d lA markaz .hjmhA. wa-i_htilAf
\VAR{al-markaz}{al-markazayn [\me]} .durUrI, likwnhA murakkabaT min
mA'"iN wa-turAb, wa-markaz al-_tql \VAR{fI}{min [\me,\mc]} jihaT
al-turAb. tqrir \VAR{_dlika}{bi_dlika [\me]}
\VAR{bitawAtur}{bitawA_tur [\mc]} al-imt.hAn, wa-qad afradtu li_dlika
risAlaT"aN.

wa-min al-`i.zAm, \textbf{dA'iraT ni.sf al-nahAr},
wa-qad tqddm b`.d .sifAthA.
wa-hya al-mutwhhamaT al-`.zImaT al-mArraT biq.tbay al-ufuq wa-biq.tbay
m`ddl al-nahAr. fa-in kAn q.tb al-ufuq hwa q.tb
al-m`ddl, \VAR{kAna}{kAnat [\mb,\me,\mc]} \VAR{hya}{fI [\me]}
al-qA'imaT `layhi `l_A qwA'im, wa-hya tf.sl al-.zAhir min al-madArAt
al-yawmiyyaT nu.sfayn.

\clearpage
\noindent wa-tf.sl min.tqaT al-burUj fwq al-ar.d `l_A
nuq.taT tsmm_A al-`A^sir, wa-t.htahA \VAR{`l_A}{nAqi.saT [\me]}
nuq.taT tsmm_A al-rAbi` wa-watad al-ar.d.
% A 7r l. 20 - 7v l. 1
wa-i_dA w.sala al-kwkb
ilayhA, kAna fI .gAyaT \VAR{irtifA`ihi}{al-irtifA` [\me]} i_dA lam
ykun \VAR{abady}{abad [\me]} al-.zuhUr; fa-in kAn abady al-.zuhUr,
falahu `layhA irtifA`An, ni.sf majmU`humA `r.d \VAR{tilka}{nAqi.saT
  [\mc]} al-buq`aT. wa-al-qws al-wAqi`aT min dA'iraT ni.sf al-nhAr
bayna q.tbay m`ddl al-nhAr wa-al-ufuq al-.haqIqI hwa `r.d al-bld.
wa-yq.t` al-ar.d `l_A\fol{w 8 \mc} _h.t.t"iN ysmm_A \textbf{_h.t.t n.sf al-nhAr}.

wa-min \VAR{al-dawA'ir}{nAqi.saT [\ma,\mb,\me]} al-`i.zAm, dA'iraT
al-ma^srq wa-al-ma.grb. wa-hya\fol{.z 25 \md} \VAR{al-`a.zImaT}{dA'iraT `azImaT [\mc]}
al-mtwhhamaT al-mArraT bisamt al-ra's wa-al-qdm wa-biq.tbay dA'iraT
ni.sf al-nhAr, fatqwm `l_A al-ufuq \VAR{`l_A qwA'im}{biqwA'im [\me]},
wa-tsmm_A \textbf{bidA'iraT 'awwal al-smUt}. wa-i_dA marra bihA kwkb"uN 'aw
juz'"uN mafrU.d, kAn .hayna al-murUr lA smt lahu. wa-i_dA tuwuhhmt
qA.ti`aT"aN likuraTi al-ar.d, kAn _dlika al-_ha.t.t _h.t.t
\VAR{al-m^srq wa-al-m.grb}{al-m.grb wa-al-m^srq [\me]} wa-hwa qA'im
`l_A _h.t.t ni.sf al-nahAr. wa-_h.t.t al-m^srq wa-al-m.grb \VAR{lA
  y_htalif}{li-i_htilAfihi [\mb,\me], ya_htalifu [\mc], li-i_htilAf
  [\md]} bi-i_htilAf al-bqA` al-^srqiyyaT wa-al-.grbiyyaT, bal fI
\VAR{al-^smAlyaT wa-al-junUbyaT}{al-^simAl wa-al-junUb [\me]}.

wa-min \VAR{al-dawA'ir}{nAqi.saT [\ma,\mb,\me,\md]} al-`i.zAm
\textbf{dA'iraT `r.d aqlIm al-rwyaT}. wa-hya dA'iraT \VAR{mtwhhmaT
  `.zImaT}{`.zImaT mtwhhmaT [\me]} mArraT biq.tbay falak al-burUj
wa-\VAR{biq.tbay}{nAqi.saT [\ma,\mb,\mc,\md]} al-ufuq,
\VARX{fatakUn}{qA'imaT `l_A al-ufuq, wa-hya tn.sf al-.zAhir
  wa-al-_hfI}{min falak al-burUj}{nAqi.saT [\me]}. wa-al-qws allatI
minhA fImA bayna a.hd q.tbay falak al-burUj wa-al-ufuq ysmm_A
\textbf{`r.d aqlIm al-rwyaT}.

wa-min \VAR{al-dawA'ir}{nAqi.saT [\ma,\mb,\me,\md]} al-`.zAm
\textbf{dA'iraT al-irtifA`}. wa-hya dA'iraT `.zImaT mtwhhmaT mArraT
biq.tbay al-ufuq wa-al-juz'i al-marfU.d, \VAR{fataq.t`}{fayaq.t`
  [\mc,\me,\md]} al-ufuq `l_A qwA'im `l_A nuq.tatayn b`d kull
wA.hidaT"iN min hAtayn al-nuq.tatayn min _ha.t.t al-m^srq wa-al-ma.grb
hwa al-smt li_dlika al-irtifA`. wa-al-qws al-wAqi` minhA bayna al-ufuq
wa-al-juz'i al-mafrU.d hwa \textbf{al-irtifA`}, wa-b`d al-juz'i
\VAR{`layhA}{`nhA [\mb]} min smt al-ra's hwa tamAm al-irtifA`.

wa-min \VAR{al-dawA'ir}{nAqi.saT [\ma,\mb,\me,\md]} al-`i.zAm,
\textbf{dA'iraT al-ufuq al-.hAdi_t}.
% A 7v l. 14
wa-hya dA'iraT `.zImaT tmrr binuq.tatay al-^simAl
wa-al-junUb wa-al-juz'i al-mafrU.d 'aw bikwkb"iN mafrU.d. \textbf{wa-irtifA`
al-ufuq al-.hAdi_t} qws min dA'iraT 'awwal \VAR{al-smUt}{al-smwAt
  [\mb]}, bayna ufuq al-bld wa-al-ufuq al-.hAdi_t.

\clearpage
\noindent \textbf{wa-`r.d al-ufuq
al-.hAdi_t} qws min dA'iraT `.zImaT"iN tamurr biq.tbay m`ddl al-nhAr
wa-\VAR{tqwm}{yqwm [\mc,\me,\md]} `l_A dA'iraT al-ufuq al-.hAdi_t
\VARX{fImA}{bayna q.tb al-`Alam w}{al-ufuq al-.hAdi_t}{fI hAmi^s
  [\me] fq.t}.

wa-min al-dwA'ir \VAR{al-ma^shUraT}{al-ma^shUrAt [\mb]}, \textbf{al-madArAt}.
wa-hya dwA'ir mwAzyaT lim`ddl al-nahAr mArraT bi-al-juz'i al-mafrU.d,
wa-jihatihA \VAR{mutaswyaT}{mansUbaT [\mb,\mc,\me]} il_A jihaT
al-mIl 'aw al-q.tb. wa-a`.zmhA mA qrb min al-min.taqaT. \VAR{w
  i_dA}{fa-i_dA [\mb,\mc,\me,\md]} kAna \VAR{libld}{lil-bilad
  [\mc]} `r.d kAn al-.zAhir min al-madArAt al-^smAliyyaT ak_tr min
al-ni.sf, wa-min al-junUbiyyaT aqll min al-ni.sf, \VAR{w}{nAqi.saT
  [\ma,\mb,\md]} \textbf{qws nahAr} al-kwkb mansUb il_A al-.zAhir min\fol{.z 8 \mc}
madArihi; fa-in ba`d al-madAr min al-q.tb \VAR{yqdr}{biqdr
  [\mb,\mc,\md]} `r.d al-bld 'aw aqll, fa-al-kwkb alla_dI `layhi
abadiyy al-.zhUr in kAn al-kwkb fI jihaT al-q.tb al-.zAhir, wa-illA
fahwa abadiyy al-_hfA'.

wa-min al-dawA'ir al-ma^shUraT, \textbf{madArAt al-`rU.d}.\fol{w 8 \ma}
wa-hya dawA'ir mwAzyaT
limin.tqaT al-burUj mArraT bimA \VAR{nfr.d}{yfr.d [\mb,\mc,\me]}
min \VAR{al-kwAkb}{al-kawkab [\me]}. wa-al-kwAkb al-_tAbitaT tadUr
`l_A q.tbay \VAR{falak}{nAqi.saT [\mb]} al-burUj, il_A jihaT al-m^srq,
fatakUn lAzimaT"aN lidA'iraT min dwA'ir al-`rU.d .gyr zA'ilaT `nhA abad"aN.

wa-min al-ma^shUrAt, \textbf{dwA'ir al-muqan.tarAt}.
\VAR{w hya dwA'ir}{nAqi.saT [\me]}
mwAzyaT lil-ufuq: wa-mA kAn minhA fwq al-ufuq
\VAR{ysmm_A}{tsmm_A [\mc]} muqan.tarAt al-irtifA`, wa-mA
\VAR{kAna}{nAqi.saT [\mb]} minhA t.ht al-ufuq ysmm_A muqan.tarAt
al-in.hi.tA.t. wa-dwA'ir al-irtifA` qA'imaT `layhA. fatf.sl dwA'ir
al-irtifA` bi-'ajzA'"aN mutasAwyaT"aN. wa-\VAR{q.tbayhA}{q.tbhA [\mb],
  q.tbAhA [\mc]} smt al-ra's wa-al-qdm. \VAR{w}{nAqi.saT [\me]}
ta_htalifu a^skAlhA i_dA s.t.hat bi-i_htilAf al-s.t.h \VAR{al-ms.t.haT
  `layhi}{al-ms.t.h `layhA [\mb,\mc,\me]}, wa-al-q.tb ay.d"aN.

\clearpage
\begin{center}
\Large al-bAb al-_hAmis

\large fI .harakaT al-_tawAbit, wa-\VAR{nub_daT}{nub_d"iN [\mb,\mc,\me]}
min i_htilAf aw.dA`ihA bisabab al-.harakatayn al-^sarqiyyaT
wa-al-.garbiyyaT 
\end{center}
al-kawAkab al-ma`rUfaT \textbf{bi-al-_tawAbit} mura.s`aT
\VAR{fI}{`al_A [\mc]} s.t.h \textbf{al-falak al-_tAmin}. wa-hya mu_htalifaT
al-mqAdIr. wa-lA yumkin an yu.h.s_A `adadhA, illA al-llah \VAR{`zz
  wa-jll}{ta`Al_A [\mc]}, illA an min tqAdm `hdh `n ibar_hs
  ra.sudUA\fol{w 26 \md} minhA
alf"aN wa-i_tnayn wa-`^srIn kawkab"aN. wa-'a_tbtUA a.twAlahA
wa-`urU.dahA lita'rI_h mafrU.d. wa-rattabUA aqdArhA \VAR{`l_A}{`an
  [\me]} sittaT mrAtb: al-mrtbaT al-'Ul_A a`.zmhA wa-al-sAdisaT
a.s.grhA. wa-kull mrtbaT mutafAwataT `l_A _tlA_taT anwA`: a`.zm wa-aws.t
wa-a.s.gr. wa-wjdUA \VAR{min}{fI [\me]} al-alf wa-al-i_tnayn
wa-`^srIn kwkb"aN _hmsaT `^sr fI \VAR{al-qdr}{al-miqdAr [\mc,\me]}
al-awwal wa-_hms"aN wa-arba`In fI \VAR{al-qdr}{al-miqdAr [\me]}
al-_tAniy wa-mi'atayn wa-_tamAniyyaT \VAR{fI al-qdr}{`al_A al-miqdAr
  [\me]} al-_tAli_t wa-arba`mi'aT wa-'arba`aT wa-sb`In fI
\VAR{al-rAbi`}{al-qdr al-rAbi` [\me]} wa-mi'atayn wa-sb`aT `^sr fI
al-_hAmis wa-tis`"aN wa-arba`ayn fI al-qdr al-sAdis. wa-_hArij"aN `n
h_dh al-mrAtb 'arba`aT `^sr kwkb"aN, tis`aT _hfyaT tsmm_A \textbf{m.zlmaT},
wa-_hmsaT \textbf{sa.hAbiyyaT} ka-annahA l.t_haT 'aw q.t`aT .gaym.

wa-lammA k_tr
`dadhA \VAR{`srt}{`sr [\mb,\me]} asmA .db.thA wa-kAnat m` _dlika
_tAbitaT al-a^skAl tawahhamUA lita`rIfhA .suwar"aN yakUn al-kawAkab
`layhA 'aw bi-al-qrb minhA. fayuqAl qlb al-`qrb, wa-qrn al-_twr, wa-_dnb
al-db, liy`rf _dlika al-kawkab
wa-lA \VAR{ya^stariku}{ytrk [\mc,\md]}\fol{w 9 \mc}
\VAR{ma`a .gayrihi}{nAqi.saT [\ma,\mb,\mc]} bi-al-asm. fatawahhamUA
lahA _tamAniyyaT wa-arba`In .swraT: minhA ^simAly `n min.tqaT al-burUj
'a.had wa-\VAR{`^srIn}{`i^srUn [\md,\me]} .sUraT, wa-`l_A
al-min.tqaT i_tn_A `^sr .sUraT, wa-fI al-junUb `nhA _hamsaT `^sr .sUraT.

fa-al-.swr al-^simAliyyaT: al-dubb al-a.s.gr wa-al-dubb al-akbar
wa-al-tinIn wa-qayfAws wa-yuqAlu lahu al-mlthb ay.d"aN wa-al-`wA
wa-al-fkaT wa-al-jA_t_A `l_A rakbatayhi wa-ysm_A al-rAqi.s
wa-al-^salyAq wa-yaqAlu lahu al-sl.hf'aT ay.d"aN wa-al-dajAjaT
wa-_dAt\fol{.z 8 \ma} al-kursiy wa-.hAmil ra's al-.gwl wa-yusm_A
br^sAw^s ay.d"aN wa-mamsk al-`nAn wa-al-.hwA wa-.hyaT al-.hwA
wa-al-shm wa-al-`qAb wa-hwa al-nsr al-.tA'ir wa-al-dulfIn wa-q.t`aT
al-frs wa-al-frs al-akbar wa-al-mr'aT al-mslslaT wa-al-m_tl_t.
wa-`layhA min al-kwAkb al-mar.sUdaT _tl_tmi'aT wa-sittUn kwkab"aN.

wa-.sUraT al-burUj: al-.haml wa-al-_twr wa-al-jawzA' wa-al-sir.tAn
wa-al-asad wa-al-sunbulaT wa-al-mIzAn wa-al-`qrab wa-al-qws wa-al-jd_A
wa-al-dAl_A wa-al-.hwt. wa-`alayhA wa-.hwlhA min al-kwAkb al-mar.sUdaT
_tl_tmi'aT wa-sittaT wa-arba`Un kwkb"aN.

\clearpage
wa-al-.swr
al-junUbiyyaT \VAR{qaytus}{qay.tu^s [\me]} wa-al-jabbAr wa-al-nhr
wa-al-arnab w al-kalb al-akbar wa-al-kalb al-a.s.gar wa-al-safInaT
wa-al-^sujA` wa-al-ka's wa-yaqAlu lahu al-bA.tyaT wa-al-.grAb
wa-qan.tUrus wa-al-sb` wa-al-mjmraT wa-al-iklIl al-junUby wa-al-.hwt
al-junUby. wa-`alayhA wa-.hwlahA min al-kwAkb al-mar.sUdaT _tl_tmi'aT
wa-sittaT `^sr kwkb"aN.

wa-'ammA al-s.hAbiyAt fa-i.hdhA `l_A ma`.sam
bar^sAw^s, wa-_tAnyhA ra's al-jabAr, wa-_tAl_thA al-n_traT,
% A 8v l. 9
wa-rAbi`hA \VAR{al-tAly}{al-_tAny [\mb],
al-_tAly [\me]} \VAR{lijmmaT}{lijabhaT [\mb,\me]} al-`qrb,
wa-_hAmishA `ayn al-rAmy.

\textbf{wa-al-majarraT} kwAkb .si.gAr mutaqArabaT
ka_tIraT jidd"aN, .zhrt min .s.grhA wa-k_tratihA wa-tqArubihA ka-annahA
l.t_hAt s.hAbiyaT, wa-li_dalika ^sbht bi-al-lbn lwn"aN, wa-bi_dlika
smAhA b.tulimayUs.

wa-\VAR{minhA}{nAqi.saT [\ma,\mb,\mc]} \textbf{manAzil
al-qmr} _tamAniyaT wa-`^srUn \VAR{w kwAkbhA min jumlaT}{kwkb"aN min
jumlaT [\mb,\me], kawkab"aN min jumlaT al-kawAkb [\mc]}
al-mar.sUdaT \VAR{w}{nAqi.saT [\me]} ismA'uhA ma^shUraT.

\begin{center}
\large f.sl
\end{center}
.harakaT ha_dihi al-kawAkib fI al-.tUl dUna al-`r.d. wa-hya `l_A
q.tbay al-burUj min al-ma.grb il_A al-ma^srq, wa-\VAR{y`rf}{t`rf
  [\me]} \textbf{bi-al-.harakaT \VAR{al-_tAniyaT}{al-_tAbitaT [\mb,\mc]}}.
wa-mqdArhA `nd b.tulamyUs fI kull mi'aT sanaT"iN darjaT, wa-`nd
al-muta'a_h_hirIn fI kull mi'aT sanaT darjaT wa-ni.sf, wa-`nd ba`.dhm
fI kull sb`In sanaT darjaT. wa-qd .haqqaqtu _dlika bi-al-ra.sd
fawajadtuhA tata.hrrk fI \VAR{kull}{nAqi.saT [\me]} sab`In sanaT
fArsyaT\fol{.z 9 \mc} darjaT wA.hidaT.
wa-qad istaw`abtu ar.sAd al-mutaqaddimIn
wa-al-muta'a_h_hirIn liha_dihi al-kawAkib alla_dI wq`t ilaynA;
wa-_dakartu _dlika m` mA ra.sadtuh wa-\VAR{'a_tbattuhu}{'a_tbatatuhu
  [\mc]} fI \VAR{kitAb}{nAqi.saT [\me]} \textbf{ta`lIq al-ar.sAd}
fayk^sf min hunAk.

wa-\VAR{i_d tqarrir}{i_dA naqUlu [\me]} _dlika, fa-i`lam an jamI`
al-kwAkb al-ma`rUfaT bi-al-_tawAbit lA tafArq madArAtahA al-`r.diyaT
al-battaT, wa-lA \VAR{ta_htalf}{ya_htalifu [\me]} aw.dA`ahA
biqiyAs\fol{.z 26 \md}
ba`.dhA il_A b`.d"iN wa-lA biqiyAshA il_A q.tbay al-burUj.
wa-ta_htalifu aw.dA`hA bi-al-qiyAs il_A m`ddl al-nahAr bisabab
al-.harakaT \VAR{al-_tAniyaT}{al-_tAbitaT [\mc]}, wa-ta_htalifu
al-madArAt al-yawmiyaT likull kwkb minhA wa-\VAR{tatazAyd}{yatazAyd
  [\me]} 'ab`AdhA `n m`ddl al-nahAr wa-\VAR{tatanAqi.s}{yatanAqi.s
  [\me]}. wa-ta_htalifu aw.dA`hA bi-al-qiyAs il_A skAn al-aqlIm,
faya.sIr mA hwa ak_tr irtifA`"aN aqall -- wa-_dlika i_dA kAn madArah
al-yawmiy yb`d\fol{w 9 \ma} `n smt al-ra's -- wa-bi-al-`ks.
wa-y.hd_t lib`.dhA murUr
bismt al-ra's ba`d an lam yakun, wa-_dlika `nd .sayrUraT b`dh `n m`dl
al-nahAr \VAR{yqdr}{biqdr [\me]} `r.d al-bld (wa-fI jihath) ba`d an
kAn aqll 'aw ak_tr.

\clearpage
\noindent wa-bi-al-`ks wa-_dlika `nd .sayrUraT ba`dh `n m`dl
al-nahAr aqll min `r.d al-bilad 'aw ak_tr b`d an kAn musAwiy"aN lah
wa-fI jihatihi, wa-`l_A al-awwl ymrr madArahu al-yawmiy fI jihaT
al-q.tb al-_hfiy min samt al-ra's, wa-`l_A al-_tAniy fI jihaT al-q.tb
al-.zAhir. wa-ya.sIr b`.dhA abdiy al-.zhUr 'aw abdiy al-_hafA ba`d an
lam yakun, wa-_dlika `nd .sayrUraT tamAm ba`dh `n m`dl al-nahAr aqll
min `r.d al-bilad 'aw musAwiy"aN lah wa-fI jihaT al-q.tb al-.zAhir 'aw
al-_hafiyy ba`d an kAn ak_tr minh. wa-\VAR{i_d _dAk}{in zAd [\me]}
falahu .tulU` wa-.grUb, wa-`l_A taqdIr al-tasAwy yamAss al-ufuq fI kull
dawraT"iN marraT"aN `l_A dA'iraT ni.sf al-nhAr, wa-lA y.grb in kAn fI
jihaT al-q.tb al-.zAhir, 'aw lA y.tl` in kAn fI jihaT al-q.tb al-_hfiy;
wa-.gAyaT ba`dh `n al-ufuq yakUn biqdr .d`f `r.d al-bilad. wa-in .sAr
aqll, falA yamAssh wa-yakUn ba`dh min al-ufuq i_dA kAn aqrb biqdr fa.dl
`r.d al-bilad `l_A tamAm ba`dh min al-m`dl wa-i_dA kAn ab`d fabiqdr
majmU` `r.d al-bilad wa-tamAm ba`dh minh. wa-y.hd_t lib`.dhA .tlU`
wa-.grUb ba`d an kAn \VAR{abadiy al-.zhUr 'aw al-_hfA wa-_dlika `nd
  ziyAdaT tamAm ba`dh `n m`dl al-nhAr `l_A `r.d al-bilad ba`d an
  kAn}{nAqi.saT [\mb,\mc,\md,\me]} aqll minh 'aw musAwiy"aN lah. w min
`ksh .sayrUraT abadiy\fol{w 10 \mc} al-_hafA \VAR{_dA}{w _dA [\me]} .tulU`
wa-.gurUb. wa-ta`In i.tlAq ism abdiy al-.zuhUr wa-abadiy al-_hafA `l_A
ba`.d ha_dihi al-kawAkib mjAz"uN illA .haqIqaT, \VAR{w al-llahu
  'a`lm}{nAqi.saT [\me]}.

\clearpage
\addcontentsline{toc}{chapter}{\textarab{fI al-.harakAt al-`r.dyyaT
    wa-.gayrihA}}
\begin{center}
\Large al-bAb al-sAds

\large fI al-.harakAt al-`r.dyyaT wa-.gyrhA
\end{center}
i_dA ta.harraka al-tAs`, ta.harraka m`h sA'ir al-'aflAk min al-m^srq
il_A al-m.grb `l_A q.tbyhi wa-.hwl markazh. wa-h_dA \VAR{ysm_A}{yqI.d
  [\mb,\me], yqt.d_A [\mc]} .hrakaT al-.hAw_A lil-m.hw_A.
\VAR{fqd}{w qad [\me]} ittfq al-mutaqaddimUn `l_A ^gawAz .hrakaT
al-m.hw_A b.harakaT al-.hAwI, m` t.hrrk al-m.hw_A il_A ^ghaT .hrkaT
al-.hAwI 'aw il_A _hlAfhA. wa-i_htlfUA fI anna al-m.hw_A i_dA
ta.harraka \textbf{.hrkth al-_hA.s.saT `l_A m.hUr al-.hAwI wa-markazh}: hel
yajUz an yata.harrak b.hrkaT al-.hAwI, 'am \VAR{lA}{nAqi.saT [\mb]}~?

fa_dahaba b`.dhm il_A jawAz _dlk mstdll"aN `lyh, bi-anna t.hrk al-.hAwiy
lil-m.hw_A hwa bimlAzmaT al-mt.hrk limkAnh min al-m.hrk, fayt.hrk
bi-al-`ara.d bi.harakaT makAnihi, ka.harakaT sAkn al-safInaT bi.harakaT
al-safInaT. _tm annh m` _dlk, yt.hrk .hrakath al-_hA.saT bihi, ksAkn
al-safInaT i_dA trddidu fI al-safInaT, tAraT"aN il_A jihaT .harakatihA
wa-tAraT"aN il_A\fol{.z 9 \ma} _hlAf tlk al-jihaT. \VAR{lkn}{lAkin [\mc]} ymtn`
al-idrAk bihi, li-an al-idrAk bi.hrakatayn mu_htlifatayn fI kraT"iN
wA.hidaT"iN `l_A min.tqaT"iN wa-q.tbayn bi-a`yiAnihA mamtn`: bl annamA
y.hassu bi.harakaT"iN wA.hidaT"iN mrkkbaT"iN min ma^gmU`hmA in kAntA
il_A \VAR{jihaT wA.hidaT"iN}{jihatayn [\mb,\me]}, 'aw .hA.silaT min
f.dl 'asr`humA `l_A \VAR{'ab.ta'ihimA}{ab.tAhimA [\ma,\mb,\mc,\me]}
in \VAR{kAnatA}{kAnat [\me]} il_A \VAR{jihatayn}{jihaT wA.hidaT"iN
  [\me]} (wa-k_dlk al-.hkm fImA zAda `l_A _dlika al-tqdIr).
wa-\VAR{yrdd}{yzAd [\mc]} `lyh: annh lA ymtn` al-'i.hsAs i_dA kAna
`l_A al-fawqAn_A kwkab ay.d"aN.

wa-_dhb b`.dhm il_A annh ymtn` mstdl"aN `lIhi, anna t^sbb_t al-m.hw_A
bi-al-.hAwI .hynI_d lA ykUn bi-al-q.tbayn likwnhmA _tAbitayn `l_A
al-m.hUr al-m^strk, wa-lA binuq.tatayn .gyrhmA. \VAR{lw}{i_dA [\me]}
kAna al-ta^sabbu_t dA'im"aN, i_d yU^gib an ykUn al-t^sb_t
\VAR{bijamI`}{lijamI` [\me], il_A jamI` [\mc]} al-s.tU.h, wa-_dlk
ymn` al-m.hw_A min al-.hrakaT al-_hA.saT bih. wa-\VAR{lA yjUz}{ylzm
  [\mb], ilA ylzm [\me]} an ykUn \VAR{nq.t}{nq.taT
  [\mb,\mc,\me]} min al-m.hw_A tlzm \VAR{nq.tA}{naq.taT [\me]}
min al-.hAwy tAraT"aN, wa-tfArqhA \VAR{tAraT"aN}{nAqi.saT
  [\mb,\mc,\me]} 'u_hr_A. wa-t.hrkh aqll min\fol{w 27 \md} .hrkatihi
\textbf{bi-al-ilzAq} lA binafsihi. i_d lA ykUn mt.hrk"aN bi.hrakaT al-.hAwy
kulluhA.

\clearpage
\noindent \VAR{kamA}{lmA [\ma,\mb,\mc,\md,\me]} yUjd
\VAR{fI al-mudAwr}{min al-madArAt [\me], min al-madAwr [\mb]}
al-mw.dU`aT t.ht al-_tql; i_d yUjb an ykUn al-t.hrIk bi.gayr n.zAm"iN
li-anna h_dhi al-.hrakaT lA takUn .tbI`yaT li-'i.hd_A al-kratayn, bl tkUn
.drb"aN\fol{.z 10 \mc} min al-ittfAq, wa-lysa _t"amma ^sy m_htl"uN al-ni.zAm.
wa-ay.d"aN lA ykUn al-ma.hw_A, .hAl t^sb_th bi-al-.hAwI, mut.hrk"aN
bi_dAtihi; wa-lA muta^sb_t"aN .hayna \VAR{.hrkth}{t.hrkh [\ma,\md]}
bi_dAtihi; faylzm an ykUn mt.hrk"aN bi_dAtihi \VAR{w}{fI [\me]
  faqa.t} .gyr \VAR{mt.hrk"iN}{mut.harak"aN [\mc]} bi_dAtihi,
wa-mt^sb_t"aN wa-.gyr mt^sb_t"iN; \VAR{h_dA _hlf}{hf
  [\mb,\mc,\md,\me]}. \VAR{w qAl}{nAqi.saT [\mc]} wa-'ammA imkAn
t.hrk al-m.hw_A `l_A m.hUr al-.hAwI .hrkaT mwAfiqaT lh 'aw
m_hAlifaT"aN, flA ar_A sabab"aN ymn` _dlik. fa-an tasAwat
\VAR{.hrkatAhmA}{.harakAthmA [\me]}, wa-itt.hdt al-jhaT wa-al-zmAn,
falA yu`qal al-inf.sAl falA fA'idaT fIh.

h_dhi hya al-m_dAhb m` al-dlA'il wa-al-^sbh. qAl q.tb al-dIn al-^sIrAzI
dlIl al-jwAz a.zhr wa-aqrb, wlkn `l_A taf.sIl. wa-dlIl al-imtinA` .gyr
sAlim"iN `n al-munU`, \VAR{li-'ibtinA'ihi}{li-abtyAnihi [\ma]} `l_A an
ma`a itt.hAd al-mrkaz lA budda min al-t^sb_t. wa-hw .gyr lAzm.

\begin{center}
\large f.sl
\end{center}
lA ar_A bijwAz .hrkaT \VAR{al-m.hw_A}{al-m.hw_A bi.hAwiy [\ma],
  al-m.hw_A bi.hAw"iN [\me]}, m` .hrkatihi bnafsihi, m`a .hrakatihi
bi.hAw"iN 'A_har `l_A _hlAf q.tbayhi wa-il_A .gyr jhatihi. byAnuhu
'anna al-flk al-muma_t_tal lial-^sms mt.hrk bi-al-.harakaT al-yUmyaT
min al-m^srq il_A al-m.grb, wa-yt.hrk hw binfsihi `l_A q.tbay al-brUj
min al-m.grb il_A al-m^srq, bimqdAr .hrakaT markaz al-^sms 'aw ws.thA.
flA \VAR{yjUz}{tjUz [\md,\mc]} .hrakatihi bi.hrakaT al-_tAmin
\VAR{lit.hrk}{liy.hrk [\me]} al-awj, bl y.htAj il_A flk 'A_har
\VAR{y.hrkh}{bi.harakaT [\mb]} il_A al-m^srq `l_A q.tbay al-brUj bqdr
.hrkaTi al-awj.

\newpage
\noindent wa-lw fur.d jawAz _dlk, wajab an yata.harrak sA'ir
al-'aflAk libAqI al-kwAkb bitilka al-.harakaT, faannah lA yumkin an
yata.harrak muma_t_tal al-^sms m_tAlh wa-lA yata.harak bAq_A 'aflAk
z.hl wa-al-m^striy. wa-fIhi\fol{w 10 \ma} dqaT fataamlh.

\textbf{tanbIh}. lw fr.dnA lial-^sms \VAR{tadwIr"aN wa-muma_t_tal"aN}{tadwIr
  wa-muma_t_tal [\ma,\mb,\md]} `l_A al-m^shUr, kAna muma_t_tal
al-^sms yt.hrk binafsihi `l_A q.tbay al-burUj m_tl markaz al-^sms,
wa-al-tdwIr yta.hrak fI 'a`lAh il_A _hlAf al-twAlI, wa-al-tAsi` y.hrrk
al-flkayn min al-m^srq il_A al-m.grb. \VAR{flA yqw_A al-_tAmin an
y.hrrk}{flA yqw_A al-_tAmin an y.hrk al-falakayn min al-m^srq il_A
al-ma.grb wa-lA yqw_A al-_tAmin an y.hrk [\mc]} al-muma_t_tal min
al-m.grb il_A al-m^srq bmqdAr .hrkaT al-awj lammA qulnA. fay.htAj il_A
flk 'A_har \VAR{t.hrk}{y.hrk [\mb,\mc,\me]} al-muma_t_tal bimqdAr
.hrakaT al-awj. wa-lmmA lam y"aj"idh man qAl bi.hrakaT
al-awj \VAR{w-lA y.hrkh}{w-lA b.hrkaT [\mb,\mc,\md], nAqi.saT
[\me]} fr.d .hrkath m_tl .hrkaT al-_tAmin wa-fr.d al-_tAmin y.hrkh
bi-al-`r.d\fol{w 11 \mc} il_A al-tiwAlI wa-al-tAsi` y.hrkh ilI _hlAf
al-twAly `l_A .gyr q.tbay al-.hrakaT al-awl_A wa-hw m` _dlk yt.hrk
binfsihi, wa-h_dA m.hAl, fy.htAj il_A \VAR{zyAdaT}{.harakaT [\me]}
flk 'A_har y.hrk al-awj bi-al-.drUraT.
% A 10r l. 5-7

\textbf{tnbyh 'A_har}. qd \VAR{twAtrt}{twA_tr [\mc]} al-ar.sAd al-.s.hI.haT
bi-'anna .hrkaT al-awj asr` min .hrakaT al-_tAmin. fawjb .haynay_d"iN
zyAdaT flk 'A_har y.hrk al-awj bimqdAr al-.hrakaT al-mr.sUdaT.

\textbf{tanbIh 'A_har}. lw fr.d lil-^sms muma_t_tal wa-tadwIr \VAR{w
  flk}{nAqi.saT [\mc]} 'A_har y.hrk al-awj, lm ykun al-taqwIm bih_dA
al-a.sl y.tAbiq al-r.sd al-.s.hI.h, faAnnA qd r.sdnA in.sAf arbA`
al-brUj mu.haddad"aN, fawjdnA _dlk m_hAlif"aN lil-taqwIm bi-al-a.sl
al-m_dkUr. wa-qd brhnA `l_A _dlk fI \VAR{kitAb}{fI [\mc] faqa.t}
\textbf{ta`lIq al-ar.sAd}. faa.htjnA il_A a.sl bsI.t"iN ya.tAbq al-mr.sUd;
\VAR{fa-waffaqa al-llah wa-lah}{fawfq al-llah ta`Al_A wa-lah [\mc], fawafaqat ilayhi
  wa-lillah [\me]} al-.hmd wa-al-mnaT li-a.sl yf_A bi-al-mq.sUd,
`l_A mA sataqifu `lIh in ^sA al-llah t`Al_A.
% A 10r l. 12-13

\newpage
\textbf{tnbIh 'A_har}. A_htlfUA fI .hrkAt al-'aflAk al-.s.gAr al-.gyr
\VAR{m.hI.tT}{al-mu.hI.t [\me]} bmrkz al-`Alm, kflk al-tdwIr
wa-n.hwh. fAjm`UA `l_A jUAz .hrkAthA il_A ayy jihaT"iN, fr.dt mustdlayn
bi-an lflk al-tdwIr n.sf"aN 'a`l_A wa-n.sf"aN Asfl; fAn t.hrk fI A`lAh
il_A al-twAl_A, t.hrk fI Asflihi il_A _hlAf al-twAlI, wa-`ksh. flA
\VAR{ykUn}{takUn [\mc]} .hrkth qsryyT, wlA `r.dyT, bl .tbI`yT. wa-ajm`UA
`l_A jUAz al-tdwIr fI .gyr al-flk al-tAs`, lwjUd\fol{.z 27 \md} mA
\VAR{nrAh}{tarAh [\mc,\me]} mn al-kwAkb fI \VAR{al-'aflAk}{'aflAk [\md,\mb]}.
fAn al-kwkb fI al-flk ydll `l_A \textbf{trkIb} mA. wa-man qAl bAn al-AflAk bsAy.t
ymtn` wjUd al-tdwIr fIhA, wAn yakn _tm .hrkaT \VAR{`l_A .gyr
  al-mrkz}{fI al-hAmi^s [\me], `l_A .gayr markaz [\mc]} flyst hY
bsI.tT, qlt qd t`yn wjUd al-tdAwIr w.hrkAthA. fAn Amtn` _dlk bibrhAn"iN
q.t`Y"iN, \VAR{_tbt}{tb_t [\ma]} trkIb al-AflAk. wa-`dm al-bsA.tTi fIhA.
wa-`ndI AnhA mrkbT mn bsAI.t lA mn al-`nA.sr, _hlA al-tAs`, wa-al-lh
'a`lm.

\end{arab}


==> fichier2b.tex <==
\begin{arab}
\resetlinenumber\pagewiselinenumbers

\clearpage
\addcontentsline{toc}{chapter}{\textarab{fI 'aflAk al-^sams
    wa-.harakAtihA `al_A al-.sa.hI.h}}
\begin{center}
\Large al-bAb al-sAbi`

\large fI 'aflAk al-^sams wa-.harakAtihA `l_A al-.sa.hI.h
\end{center}
wa-nUridu madArAt marAkaz\fol{.z 10 \ma} al-akr al-mjsmaT awwal"aN
likwnihA ashal ta.sawwur"aN `l_A
al-bsI.t. \VAR{fanatawahham}{fayatawhm [\md,\mc], .gayr maqrU'
[\mb,\ma]} \VAR{falak}{falak"aN [\me]} fI sa.t.h al-burUj wa-`l_A
markazh wa-nsmmIh \textbf{al-muma_t_tal}.
wa-\VAR{natawahham}{yatawhhm [\md]} \VAR{falak}{falak"aN
[\mb,\me]} 'A_har, markazh `l_A \VAR{m.hI.t}{min.taqaT [\mb]}
al-muma_t_tal, n.sf q.trh arba` darjAt wa-sab` wa-_tl_tUn daqIqaT
bi-al-'ajzA'i allatI yakUn \VAR{bihA}{nAqi.saT [\mc]} ni.sf q.tr
al-muma_t_tal \VAR{sitIn}{sitUn [\mc]} juz'"aN,\fol{.z 11 \mc}
wa-nusmmIh \textbf{bi-al-flak al-.hAmil}. wa-`l_A m.hI.t al-.hAml,
markaz falak 'A_har, ni.sf q.trhu darjatayn wa-ni.sf bitilka
al-'ajzA'i, \VAR{yusmm_A}{tusmm_A [\me]}
\textbf{al-mudIr}. wa-falak 'A_har `l_A markaz al-`Alam, m.hI.t `l_A h_dihi
al-'aflAk. ni.sf q.trh min dA_hl bimiqdAr an.sAf iq.tAr al-'aflAk
al-_tlA_taT al-ma_dkUraT, wa-ziyAdaT ni.sf q.tr kuraT al-^sams ; wa-_dlk
sds juz' min tilka al-'ajzA'i, \VAR{fayakUn}{fatakUn [\mb], .gayr
  maqrU' [\me]} ni.sf q.trh sb`aT wa-sitIn darjaT wa-sb` `^sar
dqIqaT. wa-sumkh bimqdAr"iN yumkin an yata.harak il_A jhaT al-m^srq
m_tl .hrakaT al-awj ; \VAR{fayufri.du}{fanufri.du [\ma]} ni.sf q.trh
_tmAnyaT wa-sittIn darjaT"aN, fayakUn samkuh _tlA_taT wa-arba`In
daqIqaT. \VAR{w yusamm_A \textbf{al-^sAmil}}{fI hAmi^s [\me] faqa.t}.

wa-\VAR{nufri.du}{tufri.du [\mc]} al-'aflAk al-_tlA_taT `l_A al-_h.t
al-_hArij min markaz al-burUj al-mArr bi-al-awj \VAR{`l_A h_dh
  al-.sUraT al-atyaT}{`al_A ha_dihi al-atyaT [\md], haka_dA [\mc]}.
wa-'ammA\fol{w 12 \mc} al-.harakAt, faanna al-falak al-muma_t_tal yta.harak
\VAR{min}{nAqi.saT [\ma,\mb]} .harakaT basI.taT .hwl markaz al-burUj
wa-`l_A q.tbayhi il_A tiwAl_A al-burUj m_tl .harakaT markaz al-^sams,
wa-\VAR{hwa}{hya [\md]} fI al-ywm \aemph{0 n.t .h .t nA mw nz lb j}.
\VARX{fayantaqilu}{markaz al-.hAmil il_A al-twAlI
  bih_dA al-miqdAr. wa-yata.hrrak al-falak al-.hAmil .hrakaT mustawiyaT
  `nd markazhi il_A _hlAf al-tiwAlI fI 'a`lAh mi_tl markaz al-^sms
  ay.d"aN, wa-hwa}{\aemph{0 n.t .h .t nA mw nz lb j}}{fI al-hAmi^s
  [\md], fayantaqilu ... \aemph{0 n.t .h .t nA mw n nh} [\mc]}.
wa-yata.hrrak al-falak al-mudIr .harakaT mustawyaT `nda markazh fI
'a`lAh il_A al-tiwAl_A mi_tl .di`f markaz al-^sms, wa-hwa fI al-yawm
\VAR{\aemph{A n.h _Aw _A.t mj ld}}{\aemph{A n.h nw _A.t mj ld}
  [\md], \aemph{A n.h nw n.t mj ld} [\mc], fI [\me] >>_Aw _A.t<<
  .gayr maqrU'}. fayantqilu markaz jrm al-^sms il_A al-tiwAlI bih_dA
al-mqdAr.

\clearpage
\noindent wa-yta.harrak al-flk al-^sAmil .hrakaT basI.taT .hwla markazh
min al-ma.grb il_A al-ma^srq m_tl .hrakaT al-awj, wa-hwa fI al-yawm
tis`a _twAl_t wa-i.hd_A wa-_hmsUn rAbi`aT wa-sitt wa-arb`Un _hAmisaT
wa-i.hd wa-_hmsUn sAdisaT ; faykml lah fI al-snaT daqIqaT wA.hidaT, wa-fI
kl sttIn sanaT drjaT bi-al-r.sd al-m.haqqaq. \VAR{r.sd wa-nqq.h}{fI
  al-hAmi^s [\mc]}, faya.sIr b`d markaz \VAR{al-tadwIr}{.gayr maqrU'
  [\mb], al-mudIr [\me]} `n al-nuq.taT al-_tAbitaT min al-burUj
bimiqdAr majmU` al-.harakatayn, wa-majmU`uhumA al-ws.t, wa-hwa basI.t
markkab"uN.

fayakUn ab`d b`d al-^sms min markaz al-`Alam a_dA kAnat fI al-awj,
wa-aqrb qrbhA minh \VAR{i_dA}{ilay [\mb]} kAnat fI al-.ha.dI.d,
wa-\VAR{yakUn}{takUn [\ma,\mc]} fI b`dhA al-aws.t i_dA kAna al-markaz
\VAR{\aemph{j z z A w .h _Aj}}{\aemph{j z z A w .h nj} [\mb], \aemph{j
    z A w .h _Aj} [\me]}. wa-\VAR{n_hrj}{y_hrj [\mb]} min markaz
al-burUj _h.t.t"iN mustaqIm il_A markaz al-.hAmil, wa-n_hruj _h.t.t
'A_har\fol{w 11 \ma} min markaz al-burUj il_A jrm al-^sms, fay.hI.tAn bizAwyaT
i_htilAf al-^sms wa-hwa al-ta`dIl. wa-yt.tAbqAn i_dA kAna markaz
al-.hAmil fI al-awj 'aw al-.h.dI.d. wa-ak_tr h_dA al-i_htilAf darjatayn
wa-daqIqatayn wa-sitt _twAnI, wa-_dlk `nd kwn al-markaz
\VAR{_tlA_t}{_talA_taT [\me]} burUj wa-sb` \VAR{drj}{darjAt [\mb]}
'aw _tmAnyaT wa-_talA_t wa-`^srIn darjaT. wa-al-_h.t.t al-mArr
\VAR{bimarkaz al-.hAmil}{bi-al-markaz ay bimarkaz al-.hAmil [\mc]}
yaf.sil min falak al-burUj \textbf{ws.t al-^sms}. wa-ba`d h_dA al-_h.t.t min
al-_h.t.t al-_hArij min al-burUj al-mArr bi-al-i`tidAl al-rabI`_A
wa-hwa ws.t al-^sms; wa-ba`dh min al-_h.t.t al-mArr bi-al-awj hwa
\textbf{markazhA}. wa-b`d al-_h.t.t al-mArr bi-al-awj min al-_h.t.t al-mArr
bi-awwl al-.hml hwa \textbf{al-awj}. wa-majmU` al-awj wa-al-markaz hwa ws.t
al-^sms.

\clearpage
\noindent wa-yakUn ab`d b`d markaz al-^sms min markaz al-`Alam sb`
wa-sittIn darjaT wa-sb` daqA'iq bi-al-'ajzA'i allt_A bihA 
n.sf\fol{.z 11 \ma} q.tr
al-muma_t_tal \VAR{sittIn}{sittUn [\me]} juz'"aN. wa-aqrb qrb markaz
al-^sms min markaz al-`Alam i_tnAn wa-_hamsUn juz'"aN wa-_tl_t
wa-_hmsUn daqIqaT bitilka al-'ajzA'i .

\VAR{w}{aw [\me]} ws.t al-^sms lini.sf nahAr ywm al-_tlA_tA awl
snaT 'i.hd_A wa-sb`mi'aT liyazdjrd \VAR{\aemph{.t _A .t 0}}{\textarab{fI
  hAmi^s [\ma,\mc] >>wa mwAfiqh
  yawm al-_tul_tA 'awl sanaT 'i.hd_A wa-sb`mi'aT liyazdjrd _tAli_t `^srIn rabI`
  al-'awl 732 `nd al-m.slaT min al-hjraT al-m.thraT, wa rAbi` `^srIn rabI` [...]
  sanaT 1131 [...]<<, fI hAmi^s [\me] >>mwAfq lil-_tAli_t
    wa-al-`^srIn min rabI` al-awwl sanaT i_tnayn wa-talatIn
    wa-sb`mi'aT hjriyyaT<<}}
bidami^sq, wa-awj\fol{.z 12 \mc} al-^sms lil-ta'rI_h
al-ma_dkUr \VAR{\aemph{b k.t nb j A}}{\aemph{b k.t nb} [\ma]};
wa-.harakaT al-awj il_A al-tiwAlI fI sittIn sanaT fArisyaT darjaT
wA.hidaT; wa-.harakaT al-^sms fI sanaT fArisyaT \aemph{yA k.t mh m},
wa-fI ^shr"iN wa-hwa _tl_tUn ywm"aN \VAR{\aemph{0 k.t ld .t nA mw n nz
    lb}}{\aemph{0 k.t l.t nA mw n nz lb} [\me]}, wa-fI ywm"iN
\aemph{0 n.t .h y.t mj lj mA nh d w}, wa-fI sA`aT mustawyaT
\VAR{\aemph{0 b kz n m.t y.h nd yd mz}}{\aemph{0 b kz n n.t y.h nd yd
    mz} [\mb]}. fa-i_dA nq.snA \VAR{min al-ws.ti al-awj}{al-awj min
  al-ws.t [\mc]} bq_A al-markaz.

%E20v
\VAR{natawahham}{fi hAmi^s [\mc], yatawahham [\me]}
  al-muma_t_tal flak kurYY mjssm
  mq``rh\fol{w 12 \ma\\.z 28 \md} mumAs lim.hddb al-^sAmil li-'aflAk
  al-zhraT wa-m.hdbh mumAs limq`r al-falak al-^sAml lil-^sms ;
  wa-markazh markaz al-`Alam wa-lah q.tbAn
\VAR{mu.hA_dyAn}{m.hwyAn [\mc], m.hwyAn [\md], m.hA_d_AAn [\me]}
liq.tb_A \VAR{falak al-burUj}{falak [\mb,\mc,\md], wa-ktb fI hAmi^s
  [\mb,\mc,\md] >>falak al-burUj<<} wa-min.tqath fI s.t.h min.taqaT
al-burUj.

wa-sumkh \VAR{arb`}{arb`aT [\me]} `^sr darjaT wa-arba` wa-_tala_tUn
daqIqaT, wa-zyAdaT. bi.hay_tu ytt.sl b`.dh biba`.d"iN i_dA .gms fIhi %B13r
kuraT al-.hAmil, wa-\VAR{nufri.du}{tfr.d [\me]} al-zyAdaT min _hArij
wa-dA_hil _tl_t drjaT, bi-al-'ajzA'i allatI bihA ni.sf q.tr mu.hI.th
sb`aT wa-sittUn juz'"aN wa-sb` `^sr dqIqaT. wa-\VAR{nufri.du}{yfr.d
  [\me]} kuraT q.trhA arb` `^sr \VAR{drjaT}{drj [\mb]} wa-arb`
wa-_tl_tUn daqIqaT, mu.garraqaT fIh, mumAssaT lah min dA_hil wa-_hArij
wa-\VAR{nufri.du}{yfr.d [\me]} kuraT 'u_hr_A ni.sf q.trhA drjatAn
wa-ni.sf wa-sds min \VAR{tilka}{_dlika [\me]} al-'ajzA'i,
mu.garraqaT fI kuraT al-.hAmil bi.hay_t \VAR{tamAssuhA}{yamAssuhA
  [\me]} `l_A nuq.taT"iN. wa-\VAR{nufri.du}{yfr.d [\mc,\me]} jrm
al-^sms \VAR{mu.garraq}{mu.garraq"aN [\me]} fI h_dh al-kuraT.
wa-\VAR{nufri.du}{tfr.d [\mc,\me]} \VAR{manA.tq}{min.taqaT
  [\me]} h_dh \VAR{al-akr}{al-kuraT [\me]} fI s.t.h falak
al-burUj. fa-yakUn .sUrathA `l_A mA \VAR{n.swr}{t.swwr [\mb,\me],
  y.swr [\mc]} `l_A al-basI.t \VAR{hk_dA}{nAqi.saT [\mc]}.

\clearpage

wa-y.hI.t bihA kuraT"aN markazhA markaz al-`Alam, maq``rh mumAss
lim.hddb muma_t_tal \VAR{al-^sms wa-samkh _tlA_t wa-arba`Un daqIqaT
  wa-m.hddbh mumAss limaq``r muma_t_tal}{nAqi.saT [\mc,\md]}
al-mirrI.h, wa-min.tqath fI s.t.h al-burUj, wa-q.tbAh q.tbA al-burUj.
wa-al-.harakAt\fol{w 29 \md} `l_A mA taqaddm. faytmm amr al-^sms
\VAR{bi-'arba`aT}{'arba`aT [\mb], arba` [\md]} 'aflAk"iN : i_tnAn
mu.hI.tAn bimarkaz al-`Alam wa-`l_A markazh wa-fI s.t.h al-burUj,
wa-al-.hAmil wa-al-mudIr. wa-lw wAfq al-tqwIm bi-a.sl al-tdwIr `l_A
hI'aT b.tlmyws fI 'an.sAf al-'arbA`, kAn yjb an yazAd fIh falak 'A_har
y.hrrk al-awj fI kull sittIn sanaT darjaT. %E21v
wlkn \VAR{_hAlif fI
  al-r.sd}{y_hAlif al-r.sd [\me]} wa-lam ywAfiq fI .gyr al-nq.t
al-arba` al-i`tidAlIn wa-al-inqilAbIn lA .gyr. wa-h_dh al-'aflAk `l_A
markaz wA.hd"iN wa-al-markaz wa-al-ws.t wa-al-awj mqddr min dA'iraT"iN
wA.hdaT ; fa-in fI \VAR{al-hI'aT}{al-hay'At [\mb,\me]} al-m^shUraT
yakUn al-ws.t \VAR{mqddr}{mqddr"aN [\mb,\me]} min dA'iraT
wa-al-markaz wa-al-awj \VAR{mqddr}{mqddr"uN [\me], mqdrAn [\mc]}
min dA'iraT 'u_hr_A wa-h_dA lA y.s.h.h wa-j`lUh min qws
\VAR{^sbIh}{^sbIhih? [\ma]} wa-\VAR{hwa}{h_dA [\mb,\me]} m.hAl. 

\begin{center}
\large f.sl\fol{.z 13 \mc}
\end{center}
\textbf{wa-.tarIq tqwIm al-^sms bi-al-jdwl wa-al-.hisAb} in tjm`
al-ws.t lil-ta'rI_h alla_dI turId wa-tajm` al-awj ay.d"aN wa-tsq.t al-awj
min al-ws.t ybq_A al-markaz. 'aw \VAR{tst_hrj}{yst_hrj [\mb,\me],
  ast_hrj [\mc]} al-ws.t wa-al-awj min al-jadwal lil-wqt alla_dI turId.
wa-_dlik in ta'_h_d \VAR{mA y_h.s.s}{fI al-hAmi^s [\me]} al-sinIn
al-tAmmaT al-majmU`aT wa-al-sinIn al-mbsU.taT wa-al-^shUr wa-al-'ayyAm,
wa-lA tad_hul al-ywm alla_dI ant fIh fI al-.hisAb, _tm ujm` kl jns"iN
il_A jinsh wa-irf` mA yjb irtifA`h ; wa-\VAR{u.tr.h}{u_hrj [\me]}
al-adwAr al-tAmmaT, famA bq_A fahwa al-ws.t. wa-`l_A _dlik, ujm` al-awj
_tm usq.t \VAR{al-awj}{nAqi.saT [\me]} min al-ws.t, ybq_A al-markaz.
fa-ud_hul bihi il_A jdwal ta`dIl
al-^sms\fol{.z 12 \ma}. \VAR{famA wjdt bi-izA'ihi min
  al-darj wa-ksUrhA}{famA wjd bi-izAyh min al-darj wa-al-daqA'iq
  [\mc]}, m`dl"aN bif.dl \VAR{mA}{nAqi.saT [\md,\mc]} bayna al-s.trIn,
fahwa ta`dIl al-^sms. fa-in wq` al-markaz fI 'a`l_A al-jadwal, fanqq.s
al-ta`dIl min al-ws.ti, wa-in wq` fI asfl al-jadwal, fazd al-ta`dIl `l_A%E22r
al-ws.t.

\clearpage
\noindent famA .h.sl, fahwa taqwIm al-^sms min falak al-burUj lini.sf
al-nahAr alla_dI .hsbt lah bdami^sq. %B13v

wa-in ^si't .hsAb al-ta`dIl bi-al-.hisAb min .gyr \VAR{jdwl}{al-jdwl [\mc]} :
\VAR{i_dA aradt _dlik}{nAqi.saT [\mc]},
fa-u.drub jIb markaz al-^sms fI
sb` drj wa-sb` daqAyq mun.h.t"aN \VAR{famA}{mimmA [\ma]?} .h.sl, fzdh
`l_A sittIn in kAn al-markaz fI jihaT al-b`d al-ab`d wa-hwa in yakUn
al-markaz aqll min _tlA_t burUj wa-sb` drj wa-sb` daqAyq 'aw ak_tr min
_tmAn burUj wa-i_tnayn wa-`^srIn darjaT wa-_tl_taT wa-_hamsIn daqIqaT,
fa-in kAn .gyr _dlik fahwa fI jihaT al-b`d al-aqrb, fanqq.sh min sittIn.
famA bl.g 'aw bq_A fahwa al-.hA.sl. _tm u.drb jIb al-markaz fI
darjatayn wa-sb` daqAyq, famA .h.sl fasmmyh al-maqsUm. _tmm rbb`
al-mqsUm, wa-rbb` al-.hA.sl, wa-ujm` al-murabbi`ayn, wa-_h_d j_dr _dlik,
fahwa b`d al-^sms min markaz al-`Alam bi-al-'ajzA'i allatI bihA ni.sf
q.tr al-muma_t_tal sittIn juz'"aN. _tmm \VAR{aqsmt}{qsmt [\md], i_dA
  qsmt [\mb,\me]} al-maqsUm `l_A b`d al-^sms min markaz al-`Alam,
ya_hrj jIb ta`dIl al-^sms, qwsh fI jadwal al-jIb, ya_hrj al-ta`dIl.
wa-`l_A _dlika .hsbnA lijuz' juz' wa-'a_tbtnAh fI al-jadwl. fa-in
\VAR{kAn}{fwq al-s.tr [\me]} al-markaz aql min sitt burUj, fanqq.s
al-ta`dIl min al-ws.ti, wa-in kAn ak_tr min sitt burUj"iN, fazd
al-ta`dIl `l_A al-ws.t ; y.h.sl \VAR{maw.d`}{mqwm [\mc]} al-^sms min
flak al-burUj.

\begin{center}
\large fa.sl
\end{center}
\textbf{q.tr al-^sms} fI b`dhA al-aws.t, wa-_dlika `nd kwn b`dhA min
markaz al-`Alam m_tl ni.sf q.tr al-muma_t_tal, wa-_dlika bi-al-far.d
sittIn juz'"aN : \aemph{lb lb}. wa-q.trhA fI b`dhA al-ab`d :
\aemph{k.t h}.\fol{w 14 \mc} wa-fI b`dhA al-aqrb : \aemph{lw nh}.

\clearpage

wa-.trIq al-.hisAb liq.trhA fI .gyr \VAR{h_dh}{h_dA [\mc]} al-mwA.d`,
an tqsm q.trhA fI b`dhA al-aws.t \VARX{`l_A b`dhA}{min markaz al-`Alam
  alla_dI hwa markaz al-burUj.}{wa-q.trhA fI b`dhA al-aws.t}{`l_A b`d
  min markaz al-`Alam alla_dI hwa markaz al-burUj wa-q.trhA fI b`dhA
  al-aws.t [\md], nAqi.saT [\me]} \VAR{`n}{`nd [\mb,\mc,\md],
  hwa `nd [\me]} ibr_hs \aemph{lb mh}, wa-`nd al-hnd \aemph{lb lj},
wa-`nd al-mu.hda_tIn \aemph{lb lh}, wa-`nd b.tlmyws fI \fol{.z 29 \md}
sA'ir al-'ab`Ad
\aemph{lA k}, wa-alla_d_A ta.harrara `ndI bi-al-ra.sd \aemph{lb lb}.
wa-fIhi .tarIq bitaqrIb ysyr, wa-hwa an \VAR{ta.drb}{y.drb
  [\md,\mb], .gayr maqrU' [\mc,\me]} buht ywm al-^sms
fI _tlA_taT wa-\VAR{_talA_tIn}{_tul_tay [\ma,\mc]} drjaT, y_hrj q.trhA
bi-al-taqrIb ; wa-al-awwl mbrhn. \VAR{w al-ll_ah 'a`lm}{nAqi.saT
  [\md,\mb,\me]}.
\end{arab}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\input{soleil.pdf_tex}
\end{minipage}
\textarab{.sUraT 'aflAk al-^sms `l_A annhA mdArAt marAkz al-akr
  al-tAmmaT `l_A .hsb mA yata.sUr `l_A al-basI.t}
\end{figure}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\input{soleil_orbes.pdf_tex}
\end{minipage}
\textarab{.sUraT 'aflAk al-^sams al-mujsmaT wa-hiya kurAt mujsmaT tAmmaT}
\end{figure}

\begin{arab}
\resetlinenumber\pagewiselinenumbers
\clearpage
\begin{center}
\Large al-bAb al-_tAmin

\large fI .hisAb ta`dIl al-'ayyAm bilayAlIhA
\end{center}
wa-hwa tafAwt mA bayna al-'ayyAm bilayAlIhA bi-al-qiyAs il_A
al-yawm al-mar.sUd ws.th wa-mqwwmh. wa-qad ja`alnA al-ywm alla_dI ra.sdnA
lahu al-ws.t\fol{w 13 \ma} wa-al-mqwwm al-i`tidAl al-rabI`I, wa-bihi naqIs
bAqI al-'ayyAm bilayAlIhA. wa-.tarIqu .hisAb h_dA al-ta`dIl an t.hsab
ws.t al-^sams wa-mqwwmhA
\VAR{lil-yawm}{lil-wqt [\mb,\me]} alla_dI turId, wa-zad `l_A ws.t
al-^sams darjatayn wa-daqIqaT wa-sb` \VAR{_tawAn_A}{_tawAn [\me]}.
famA bala.ga _hu_d tafAwt mA baynahu wa-bayna \VAR{m.tAl`}{m.tl`
[\mc,\md]} mqwwm al-^sams (bi-al-m.tAl` al-istiwA'iyyaT al-ma`mUlaT
min awwal al-.haml). famA kAna u.drubhu fI 'arba`aT. y.h.sl %B14r
daqA'iq ta`dIl al-'ayyAm bilayAlIhA. fa-in kAna al-ws.t ma` al-ziyAdaT
ak_tr min m.tAl` mqwwm al-^sms, \VAR{fanaqqi.s}{fa-_Aq.s [\mb],
fa-nq.s [\mc], yanq.s [\md]} al-ta`dIl min al-ta'rI_h, wa-in kAna
aqall fazadhu `l_A al-ta'rI_h. y.h.sl al-ta'rI_h al-mu`addl bita`dIl
al-'ayyAm bilayAlIhA. wa-`layhi ysta_hruju al-awsA.t min
\VAR{al-jdwl}{al-jdAwl [\mc,\md]}.

\textbf{tnbIh}. u.drb bht al-kawkab fI sA`aT \VAR{fI}{min [\mc,\me]}
daqA'iq ta`dIl al-'ayyAm bilayAlIhA. famA .h.sl un.zur, fa-in kAna
al-ws.t m` al-ziyAdaT ak_tar min m.tAl` mqwwm al-^sams fanaqqi.s
al-.hA.sl min mqwwm _dalika al-kawkab, \VAR{w in}{fa-in [\me]} kAna
aqall fazad al-.hA.sil `l_A mqwwm _dlika al-kawkab. y.h.sl mqwwm
al-kawkab lil-wqt al-m.tlUb. wa-qad .hsbnA lahu jdwl"aN yUjd minh
biws.t al-^sams.

\clearpage
\addcontentsline{toc}{chapter}{\textarab{fI 'aflAk al-qmr
    wa-.harakAtihA}}
\begin{center}
\Large al-bAb al-tAsi`

\large fI 'aflAk al-qmr wa-.harakAtihA \VAR{.tUl"aN wa-`r.d"aN}{fI hAmi^s
  [\ma]} `l_A al-wjh al-.s.hI.h al-sAlim min al-^skUk.
\end{center}
lammA ru.sida al-qmr, fawujida muta.harrak"aN `l_A mdAr .gyr mdAr
al-^sms muqA.ti` lahu fI maw.du`ayn mutaqAbilayn mntqlayn fI mdAr
al-^sms il_A _hlAf tiwAlI al-burUj wa-_dlika al-mdAr mA'il `n mdAr
al-^sms, wa-.gAyaT al-mIl fI al-jihatayn bimqdAr"iN wA.hd"iN abd"aN
wa-_dlika _hmsaT 'ajzA' bi.hay_tu yakUn fI\fol{.z 14 \mc} ni.sf
madArihi ^simAliyy"aN `n min.tqaT al-burUj wa-fI al-ni.sf al-'A_har
janUbiyy"aN `nhA. fa-i`lam an lahu \VAR{falak muma_t_tal}{falak"aN
muma_t_tal"aN [\mb,\md,\mc]} bifalak al-burUj wa-\VAR{falak
mA'il}{falak"aN mA'il"aN [\md,\mc], falak"aN mA'il [\mb], wa-ktb
>>falak"aN<< fI hAmi^s [\me] ay.d"aN} `nh \VAR{mutaqA.ti`An `l_A
nuq.tatayn}{mutaqA.ti`ayn `l_A jihatayn [\md,\mc]} mutaqAbilatayn,
fayan.s.sf a.hadhumA lil-'A_har.

wa-lammA wujidat .hrkaT al-qamar `l_A al-falak al-mA'il mu_htalifaT
bi-al-bu.t'i wa-al-sur`aT .hwl markaz al-`Alam alla_dI hwa markaz
al-burUj, `lm anna lahu \VAR{falak}{falak"aN [\mb,\md,\mc]} markazh
`l_A min.tqaT al-mA'il b.hay_tu 'i_dA kAna al-qamar fI 'a`lAh kAna
ab`d `n markaz al-`Alam wa-i_dA kAna fI .h.dI.dh kAna aqrb ilayhi ;
\VAR{`lm}{nAqi.saT [\md,\mc]} _dlika bi-i_htilAf \VAR{miqdAr}{fawqa
  al-s.tr [\mc]} jarimh fI al-_hsUfAt wa-al-ksUfAt wa-.gayrhA.
\VAR{fasmm_A}{sm_A [\md,\mc]} _dlk al-falak \textbf{bi-al-tadwIr} qadIm"aN.

_tmm wujida \VAR{miqdAr}{bimiqdAr [\md,\mc]} \VAR{n.sf q.tr}{fI
  hAmi^s [\ma], n.sf qdr [\md,\mc]} h_dA al-falak fI al-ijtimA`At
\VAR{w al-istiqbAlAt}{fI hAmi^s [\ma]} lA yazId `l_A _hmsaT 'ajzA'
wa-sds abd"aN `ndanA, wa-`nda b.tlmyws wa-\VAR{`nda}{fwq al-s.tr [\ma],
  nAqi.saT [\mc,\me]} ibar_hus _hmsaT
wa-rb`, _tmm wjd \VAR{miqdArh}{bimiqdArh [\mb,\md,\mc]} i_dA kAna b`d
al-qmr `n al-^sms rb` dA'iraT min al-jihatayn, _tmAniyyaT 'ajzA' .
fa-`lmnA anna `l_A \VAR{min.tqaT}{nAqi.saT [\mc]} al-tadwIr falak
'A_har .s.gIr, bi.hay_tu i_dA kAna al-qmr fI al-ijtimA`At
wa-\VAR{al-istiqbAlAt}{al-ijtimA`At [\me]}
yakUn al-qmr fI .h.dI.d _dlika al-falak, wa-i_dA kAna fI al-tarbI`ayn
kAna fI \VAR{_dirwatihi}{dawratihi [\mb]} wa-ykUn b`dh `n markaz
al-tadwIr _tmAnyaT 'ajzA' ; wa-i_dA kAna fI \VAR{.h.dI.dh}{.h.dI.d
  [\ma]}, kAna b`d al-qmr `n markaz al-tadwIr _hmsaT 'ajzA' wa-sds.
wa-anna .harakath .d`f .harakaT .hAmil markaz al-tadwIr bi.hay_tu i_dA
dAra .hAmil al-tadwIr rb` dA'iraT t.hrk .hAmil jrm al-qamar n.sf
dA'iraT.

fa-`lmnA anna lah \VAR{arb` 'aflAk"iN w}{fI al-hAmi^s [\me]} arb`
.harakAt basI.taT.\fol{w 30 \md}

\clearpage

al-falak al-awwl, \VAR{fahwa}{w hwa [\mb,\me,\md,\mc]}
\textbf{al-muma_t_tal bifalak al-burUj}, wa-q.tbAh m.hA_dyAn liqu.tbay falak
al-burUj, wa-m.hddbh mumAss limaq``r 'aflAk `.tArd, wa-maq``rh mumAss
lim.hddb al-falak al-_tAnI min 'aflAkihi, \VAR{w}{nAqi.saT [\me]}
ni.sf q.trh tis`aT wa-sittIn juz'"aN.

wa-al-falak al-_tAnI \VAR{\textbf{falak mA'il}}{al-falak al-mA'il wa-[\mc]},
s.t.hh \VAR{mA'il}{nAqi.saT [\me]} `n s.t.h al-muma_t_tal mIl"aN
_tAbit"aN .gAyath _hmsaT 'ajzA' . wa-markazh markaz al-`Alam all_dI hwa
markaz al-muma_t_tal, wa-m.hddbh mumAss limaq``ar al-muma_t_tal,
wa-mq``arh mumAss lifalak al-nAr `l_A al-ma^shUr. ni.sf q.trh
bi-al-far.d sittIn juz'"aN . wa-min.tqatuh alltI `l_A m.hddbh tq.t`
min.tqaT al-muma_t_tal alltI fI maq``rh `l_A nuq.tatayn mutaqAbilatayn,
ysmyAn \textbf{bi-al-`uqdatayn wa-al-jwzharayn}. \VAR{'i.hdAhumA}{'a.hadhumA
  [\me]}, i_dA \VAR{jAzhA}{jAwizhA [\me,\mc]} al-qamar, mAl il_A
al-^simAl `n al-muma_t_tal, \VAR{tsmA}{tsmyA [\mb,\md,\mc], ysm_A
  [\me]} \textbf{al-ra's}\fol{w 15 \mc} wa-al-jwzhar wa-al-mujAz
  al-^simAliyy; wa-al-'A_har
al-muqAbil lahu \VAR{ysmA}{tsmyAn [\mb], ysm_A [\me,\mc]} \textbf{al-_dnb}
wa-al-mujAz al-junUbiyy. wa-q.tbA al-mA'il mulAzamAn linuq.tatayn min
maq``r al-muma_t_tal abad"aN. wa-ba`dhumA `n q.tbay al-muma_t_tal
bmqdAr .gAyaT mIl al-mA'il, alla_dI hwa nihAyaT `r.d al-qamar, wa-_dlika
_hmsaT 'ajzA'. wa-maq``r \VAR{al-falak}{falak [\me]} al-mAyl, markazh
markaz al-`Alam, wa-ni.sf q.trh a.hd wa-_hmsIn juz'"aN.

\VAR{wa-'ammA al-falak al-_tAli_t}{fI hAmi^s [\ma], wa-al-falak
  al-_tAli_t [\me], al-falak al-_tAli_t [\mc]},
\VAR{fanatawahham}{fayatawahham [\md,\mc]} kuraT n.sf q.trhA
_tmAniyaT 'ajzA' wa-sittaT `^sr dqIqaT wa-sb`aT wa-`^srIn _tAnyaT min
al-'ajzA' allatI bihA ni.sf q.tr min.tqaT al-mA'il sittIn juz'"aN.
wa-nufri.dhA mu.garraqaT fI al-mA'il tmAss limin.tqatihi `l_A nuq.taT.
\VAR{fanusmIhA}{nsmmIhA [\me]} bikuraT \textbf{al-tadwIr}.

\VAR{wa-'ammA al-falak al-rAbi`}{fI hAmi^s [\ma], al-falak al-rAbi`
  [\mc]}, \VAR{fanatawahham}{fayatawahham [\me,\md,\mc]} kuraT
\VAR{nu.sf}{fwq al-s.tr [\ma]} q.trhA juz'"aN wa-a.hd wa-arba`In
daqIqaT wa-\VAR{sb`}{ts` [\me,\mb]} wa-`^srIn _tAnyaT min tilka
al-'ajzA'. wa-\VAR{nufri.dhA}{tfr.dhA [\md,\mc]} m.grraqaT fI jsm
al-tadwIr, wa-\VAR{tamAs}{yamAss [\me]} limin.tqatihi allatI fI
s.t.h al-mA'il `l_A nq.taT, wa-hya allatI yamAss `layhA al-tadwIr
limin.taqaT al-mA'il. wa-yusmm_A h_dA al-falak \textbf{bi-al-mudIr}.
wa-\VAR{nufri.du}{yfri.du [\mb,\me,\md,\mc]} jrm al-qamar
m.grrq"aN fI jsm al-mudIr. yamAssu nuq.taT m.hddb al-qamar limin.tqaT
al-mudIr allatI hya fI s.t.h al-mA'il. wa-q.tr kuraT al-qmr wjd
bir.sdnA i_tnayn wa-_tla_tIn daqIqaT wa-'arba`aT wa-_hamsIn _tAnyaT"aN
min tilka al-'ajzA'.

\clearpage

wa-'ammA al-.harakAt, \VAR{fa-al-.harakaT al-'Ul_A}{fa-al-'Ul_A [\mc]},
.harakaT al-muma_t_tal: .harakaT"aN basI.taT .hwl markazh all_dI hwa
markaz al-`Alam wa-\VAR{`l_A q.tbayhi il_A _hilAf}{il_A q.tbayhi `l_A
  _hilAf [\md,\mc]} al-tiwAlI, bimiqdAr .harakaT al-jwzhr, wa-hya
\VAR{\aemph{0 j _A l.h kz}}{\aemph{0 j _A l.h kw lz m.h k.t lw}
  [\me]}. \VAR{fayantaqilu}{yanqilu [\md,\mc]} bih_dhi al-.harakaT
al-ra's, wa-al-_dnb, wa-mw.d` nihAyaT `r.d al-qamar, wa-jamI` 'aflAk
al-qamar. wa-h_dhi al-.harakaT, fI al-.haqIqaT, f.dl .harakaT al-jwzhar
`l_A\fol{w 14 \ma} .harakaT al-kwAkab al-_tAbitaT `l_A qwl"iN.

wa-al-.harakaT al-_tAnyaT .harakaT al-falak al-mA'il .hwl markazh 
alla_dI hwa markaz al-muma_t_tal wa-markaz al-`Alam, wa-.hwl q.tbayhi
al-_tAbitayn al-mutqddm _dkrhumA, .harakaT basI.taT mustawiyaT taf`lu
fI al-azmAn al-mutasAwiyaT qsiyy"aN mutasAwyaT il_A tiwAlI al-burUj
\aemph{_Aj _Aj mh l.t m}. wa-hya bqdr majmU` ws.t al-qamar wa-.harakaT
al-jwzhar, wa-tsmm_A \textbf{.harakaT al-`r.d} qadIm"aN. fayantaqilu markaz
al-tadwIr il_A al-tiwAlI `n \VAR{al-min.taqaT}{al-nuq.taT [\ma]}
al-mutawhhm _tibAtahA min falak al-burUj, bimiqdAr ws.t al-qmr, wa-hwa
\VAR{\aemph{_Aj _A lh A _Aj nj}}{\aemph{_Aj _A lh A lj nj}
  [\mb,\me]}.

wa-al-.harakaT al-_tAli_taT .harakaT al-tadwIr .hwl markazh, wa-`l_A
q.tbayhi al-qA'imayn `l_A s.t.h al-mA'il, fI al-ywm bilaylatihi
\VAR{\aemph{_Aj j nj mw _A.h}}{\aemph{_Aj j nj mw n.h} [\me]}, fI
'a`lAh il_A _hilAf al-tiwAlI. wa-\VAR{t`rf}{y`rf [\mb,\md,\mc], _A`rf
  [\me]}\fol{.z 15 \mc} qadIm"aN \textbf{bi.harakaT _hA.saT al-qamar}.
wa-ibtidA'uhA min _dirwaT al-tadwIr al-mar'iyy.

wa-al-.harakaT al-rAbi`aT, .harakaT al-mudIr, wa-hya .harakaT basI.taT
.hwl markazh, \VAR{fayata.haraka}{_Aa_Aa.harak [\mb], yata.harak
  [\me], .gayr maqrU' [\md], wa-yata.harrak [\mc]} al-qamar
bi.harakatihi `l_A min.taqatihi allatI fI s.t.h min.taqaT al-mA'il, fI
'a`lAh il_A al-tiwAlI. fI al-ywm bilaylatihi \aemph{kd kb nj kj}. wa-hya
bimiqdAr \VAR{.d`f}{fwq al-s.tr [\mc]} f.dl ws.t al-qmr `l_A ws.t
al-^sms. wa-ibtadA' h_dh al-.harakaT fI al-ijtimA`At wa-al-istiqbAlAt
al-ws.tI min .h.dI.d al-mudIr wa-\VAR{ta.sIru}{ya.sIru
  [\mb,\me,\md,\mc]} fI al-tarbI`In min
\VAR{_dirwatihi}{dawratihi [\mb]}.\fol{.z 30 \md}

wa-lanfr.d libiyAn _dlika anna al-^sms wa-al-qamar
\VAR{mujtami`An}{yajtami`An [\mc]} bi-al-ws.t fI nuq.taT _tAbitaT min
falak al-burUj; wa-nfr.d markaz al-tadwIr wa-markaz al-mudIr `l_A
al-_h.t.t al-mustaqIm al-mArr bimarkaz al-`Alam wa-bitilka al-nuq.taT
al-mutawhham _tibAtahA min falak al-burUj; wa-nufri.d al-qamar fI
.h.dI.d al-mudIr, fI _dlika al-wqt, `l_A _dlika al-_h.t.t, fI aqrb qurbh
min markaz al-tadwIr, wa-_dlika _hamsaT 'ajzA' wa-sds juz'.

\clearpage
\noindent _tmma yta.harraka kl falak bimA fara.dnA lahu min
al-.harakaT al-basI.taT al-mar.sUdaT.

-- \VAR{fayata.harrak}{fant.hrk [\md], f_At.harrak [\mc]}
al-^sms fI al-ywm bilaylatihi \aemph{0 n.t .h k} il_A al-tiwAlI.

-- wa-yata.harraka al-muma_t_tal fI al-ywm bilaylatihi il_A _hlAf
al-tiwAlI \aemph{0 j _A l.h kz} \VAR{fayantaqilu al-mA'il wa-al-tadwIr
  wa-al-mudIr bih_dhi al-.hrkaT il_A _hlAf al-tiwAlI}{fI hAmi^s
  [\ma]}.

-- \VAR{_tm}{w [\mb,\me,\md,\mc]} yata.haraka al-mA'il il_A
al-tiwAl_A fI _dlika al-zmAn \aemph{_Aj _Aj mh l.t m}. faya.sIr b`d
markaz al-tadwIr \VAR{`l_A m.hAdAh}{`n m.hArAh? [\ma], `n mu.hA_dAT
  [\md,\mc], `l_A m.hA_dAh [\me]}
al-nuq.taT al-_tAbitaT min falak al-burUj all_dI \VAR{kAnA al-nIrayn
  ijtima`A}{kAn al-nIrAn ijtima`A [\me], kAnA ijtima`A al-nIrayn
  [\mc]} fIhA, \VAR{fI}{min [\mb,\me,\md,\mc]} al-ywm bilaylatihi,
\aemph{_Ab _AA kw mA l}; wa-_dlika bimiqdAr f.dl .harakaT ws.t al-qamar
`l_A ws.t al-^sms, wa-\VAR{ysmm_A}{ysmA? [\mb]} _dlika
\textbf{bu`d mA bayna al-nIrayn bi-al-ws.t}.

-- wa-yata.harraka al-mudIr .hwl markazh,
\VAR{fayntqlu}{faynql [\md]} al-qamar min .ha.dI.d al-mudIr, il_A
_hlAf al-tiwAl_A, fI al-ywm bilaylatihi, .d`f al-ba`d, wa-hwa \aemph{kd
  kb nj kj}.

fayab`d jrm al-qmar `n markaz al-tadwIr wa-ysmm_A _dlk
al-ba`d n.sf \textbf{q.tr al-tadwIr al-mar'iyy}.

fa-i_dA \VAR{t.harrak}{yata.harrak [\mc]} al-mA'il bimAlh min
al-.harakaT rb` dA'iraT\fol{.z 14 \ma} fI sb` 'ayyAm wa-_tmAnyaT `^sr dqIqaT
wa-arba`aT `a^sar _tAniyaT wa-'i_tnayn wa-_hamsIn _tAli_taT wa-_hamsaT
`a^sar rAbi`aT min yawm bilaylatihi, \VAR{t.harka}{.gayr maqrU'
  [\md], yata.harrak [\mc]} al-mudIr fI _dalika al-zamAn ni.sf
dA'iraT, likawn .harakatihi .d`f .harakaT al-bu`d, fayantaqil al-qamar
min .h.dI.d al-tadwIr il_A _dirwatihi, wa-ya.sIr b`d markaz jrm
al-qamar min markaz al-tadwIr _tmAnyaT 'ajzA', wa-_dlika ni.sf q.tr
al-tadwIr al-mar'iyy fI al-tarbI`ayn al-awwl wa-al-_tAnI.

\VAR{fa-i_dA}{w i_dA [\me]} ta.harraka al-mA'il bitilka al-.harakaT,
fI .d`f tilka al-muddaT, n.sf dA'iraT, .sAr markaz\fol{w 16 \mc} al-tadwIr fI
muqAbilaT tilka al-nuq.taT \VAR{al-_tAbitaT}{al-_tAniyaT [\mb]} `l_A
al-_ha.t.t al-mArr bitilka al-nuq.taT \VAR{al-_tAbitaT}{al-_tAniyaT
  [\md]} wa-\VAR{bimarkaz}{markaz [\mb,\me]} al-`Alam min jihaT
muqAbilaT juz'i al-ijtimA`. fayakUn fI _dlika al-wqt
\VAR{.haqIqaT}{`mIqaT [\ma]?} istiqbAl al-^sms wa-al-qamar bi-al-ws.t.
wa-yat.hrk al-mudIr .d`f mA \VAR{ta.hrak}{yt.harrak [\mc]} al-mA'il,
wa-_dlika dA'iraT tAmmaT, \VAR{faynql}{fayantaqilu [\mb,\me,\mc]}
al-qamar il_A .h.dI.d al-mudIr. 

\clearpage
\noindent wa-ya.sIr al-qamar fI aqrab qurbh min
markaz al-tadwIr wa-ya.sIr n.sf q.tr al-tadwIr al-mar'iyy \VAR{fI
  _dlika al-wqt _hmsaT 'ajzA' wa-sds \aemph{h _A}, m_tl mA kAna fI
  al-ijtimA`. falA yazAl n.sf q.tr al-tadwIr al-mr'iyy}{fI al-hAmi^s
  [\mc]} fI kll ijtimA` wa-kll istiqbAl \aemph{h _A}, wa-fI kll tarbI`
_tmAnyaT 'ajzA', wa-\VAR{k_dlika}{_dlika [\mc]} wujida bi-al-r.sd fI
kll zmAn.

_tm yta.harak al-tadwIr bi.harakaT al-_hA.saT. fayadUr markaz
\VAR{jrm}{fI hAmi^s [\ma], nAqi.saT [\mb,\me,\md,\mc]} al-qamar
.hwl markaz al-tadwIr fI madAr"iN n.sf q.trh \aemph{h _A}, kmA qulnA, fI
kll ijtimA` wa-\VAR{kll}{nAqi.saT [\mc]} istiqbAl. wa-yakUn qws _dlika
\aemph{d nw kd}. wa-\VAR{hwa .gAyaT}{hwa fI .gAyaT [\md,\mc]}
al-ta`dIl fI kll ijtimA` wa-istiqbAl, wa-_dlika `nda .sIrUraT al-qamar
`l_A al-_ha.t.t al-mumAss lil-tadwIr al-mr'iyy min al-jAnbayn. fa-i_dA
kAna markaz al-tadwIr fI al-tarbI`ayn kAna ba`d markaz jrm al-qamar
min markaz al-tadwIr _tmAnyaT 'ajzA'"iN, wa-hwa \VAR{n.sf}{fI al-hAmi^s
  [\me]} q.tr al-tadwIr al-mr'iyy fI kll al-tarbI`. wa-yakUn qws
_dlika i_dA fr.d jIb"aN sb` 'ajzA' wa-_tl_t_A juz'. wa-hwa kamA wajadnA
\VAR{bi-al-ra.sd fI al-tarbI`}{fI al-ra.sd bi-al-tarbI`
  [\mb,\me]}, wa-_dlika `nd kwn al-qamar `l_A al-_h.t.t al-mumAss
lil-tadwIr al-mar'iyy min al-jAnbayn fI \VAR{al-tarbI`An}{al-tarbI`At
  [\ma]}.

wa-likwn nsbaT .harakaT _hA.saT al-qamar il_A .harakaT ws.th a.s.gr
min nisbaT al-_h.t.t al-wA.sl bayna markaz al-`Alam wa-.h.dI.d
al-tadwIr al-mar'iyy il_A ni.sf q.tr al-tadwIr al-mar'iyy, lA yakUn
lil-qamar wqUf wa-\VAR{lA}{nAqi.saT [\me]} rjU`, bal
\VAR{ta.sIr}{ya.sIr [\ma]} .harakath bi.tI'aT\fol{w 31 \md}
fI n.sf \VAR{al-_dirwaT}{al-dawraT [\mb]} \VAR{w}{fI [\me]
  fq.t} sarI`aT fI n.sf al-.h.dI.d, wa-lA yr_A lahu \VAR{rjU`h}{rujU`
  [\mb,\me,\mc]} il_A _hlAf al-tiwAlI \VAR{li.s.gr}{a.s.gr
  [\md,\mc]} al-tadwIr al-mar'iyy wa-qllaT .harakatihi
\VAR{bi-al-nisbaT}{linisbaT [\mb]} il_A \VAR{.harakaT
  mA'ilh}{.harakaT"iN mAylaT [\mb]}.

wa-kwn n.sf q.tr al-tadwIr al-mar'iyy y_htalif fImA bayn _hmsaT wa-sds
il_A _tmAnyaT 'ajzA',\fol{w 15 \ma} ka'anna aqdAr al-bu.t' wa-al-sur`aT \VAR{.gyr
  muta^sAbhih bal t_htalif}{nAqi.saT [\mb,\me,\md,\mc]}
bi.hy_t y`Ud al-bu.t' wa-al-sur`aT 'aw
.gyrhumA min al-i_htilAf tAraT"aN il_A al-aql wa-tAraT"aN il_A
al-ak_tr.

\VAR{fah_dh hya}{w h_dh hya [\mc], h_dh fI [\mb,\me?]} al-'aflAk
al-mt.hrkaT \VAR{lil-.harakAt}{al-.harakAt [\mb,\me,\md,\mc]}
al-basI.taT allatI yantaj `nhA al-.harakAt al-m_htalifaT al-mwAfiqaT
lil-ra.sd fI sA'ir al-azmAn.

wa-'ammA al-i_htilAfAt al-.tUlyaT al-basI.taT allatI \VAR{ylzim}{_Alzm
  [\ma], taltazimu [\mb], talzm [\md,\mc]} bisabab h_dihi
al-.harakAt fahya 'arba`aT wa-tu`rif \textbf{bi-al-ta`AdIl}.

\clearpage

fa-al-i_htilAf al-awwl, hwa mA y.h.sl lah bisabab n.sf q.tr al-tadwIr
fI\fol{.z 16 \mc} al-ijtimA`At wa-al-istiqbAlAt. wa-hwa zAwyaT \VAR{y.hd_t}{t.hd_t
  [\mb,\me,\md,\mc]} `nd markaz al-`Alam min _hurUj .h.t.tayn
\VAR{minhu}{minhumA [\md], minhA [\mc]}, a.hdhumA il_A markaz
al-tadwIr wa-al-'A_har il_A markaz jrm al-qamar. wa-\VAR{yakUn}{takUn
  [\md,\mc]} .gAyatuhu i_dA kAna al-_ha.t.t al-mArr
\VAR{bi-al-qamar}{fwq al-s.tr [\md,\mc]} yamAss al-tadwIr al-mar'iyy
il_A ayy al-jihatayn kAna wa-lA yaq.t`h. wa-.gAyaT tilka al-zAwyaT fI
al-ijtimA`At wa-al-istiqbAlAt \aemph{d nw kd}, `l_A an n.sf q.tr
al-mA'il sittUn juz'"aN. wa-yn`dm fI al-_dirwaT wa-al-.h.dI.d, wa-_dlika
`nda t.tAbq al-.h.t.tayn al-ma_dkUrayn. wa-h_dA al-i_htilAf yanq.s min
ws.t al-qmr mA dAm al-qamar hAb.t"aN min al-_dirwaT il_A al-.h.dI.d fI
al-ni.sf al-ayman, liwuqU` al-_h.t.t al-mArr bi-al-qamar `n
\VAR{al-_ha.t.t}{fI [\md] fq.t wa-hwa fawqa al-s.tr} al-mArr
\VAR{bimarkaz}{bi-al-markaz [\mb,\md,\mc]} al-tadwIr, il_A _hilAf
al-tiwAlI. wa-yazAd `l_A ws.th mA dAm al-qamar .sA`id"aN min al-.h.dI.d
il_A al-_dirwaT fI al-ni.sf al-aysar liwuqU` al-_h.t.t \VAR{`n}{`l_A
  [\mb,\me]} al-_h.t.t, il_A al-tiwAlI. wa-ysmm_A al-ta`dIl al-mfrd
\textbf{wa-al-awwal} ay.d"aN.

wa-al-i_htilAf al-_tAnI, \VAR{fahwa}{hwa [\me,\md,\mc]} all_dI
ykUn bisabab zyAdaT al-i_htilAf al-awwl al-ma_dkUr `nda kwn markaz
al-tadwIr fI .gyr al-ijtimA`At wa-al-istiqbAlAt. wa-hwa mu_htala.t
bi-al-awwl, lA yUjadu bidUnihi. wa-.gAyath `nda \VAR{kwn}{fawqa al-sa.tr
  [\mc]} markaz al-tadwIr fI al-tarbI`ayn, ayy `nda rb`
\VAR{dA'iraT}{al-dA'iraT [\mc]} min al-juz'i alla_dI yq` \VAR{fI}{fIhi
  [\mc]} al-ijtimA` wa-al-istiqbAl bi-al-ws.t. \VAR{w .gAyath}{w hwa ay
  .gAyath [\mc]} \aemph{b md}, wa-m` al-awwl \VAR{\aemph{z m}. wa-hwa m`
  al-awwl}{nAqi.saT [\me]}
abd"aN, fI al-zyAdaT wa-al-nuq.sAn. wa-ysmm_A
\textbf{bi-al-ta`dIl al-_tAnI} wa-bi-i_htilAf al-bu`d al-aqrb qdIm"aN.

\textbf{tanbIh.} qd qdmnA an ni.sf q.tr al-tadwIr al-mar'iyy \VAR{ykn}{ykr
  [\mb], ykUn [\me]} fI al-ijtimA`At wa-al-istiqbAlAt \aemph{h _A}
abd"aN, wa-fI al-tarbI`At \aemph{.h 0}. wa-fI mA bayna _dlika
yatadarraju bi-al-zyAdaT min al-aqall il_A al-ak_tr. faya.sIr
al-i_htilAf al-awwl, bisabab i_htilAf ni.sf al-q.tr, bqdr majmU`
al-i_htilAfayn. wa-h_dA \VAR{m.d"aN}{m`n_A [\mb,\me,\md,\mc]}
daqIq fata'ammalh.

wa-al-i_htilAf al-_tAli_t, wa-y`rf \textbf{bta`dIl al-_hA.saT}, wa-hwa zAwyaT
`nda markaz al-tadwIr min _hurUj _h.t.tayn minh, ymrr a.hdhmA bmarkaz
\VAR{al-mudIr}{al-tadwIr [\md,\mc]}
wa-al-'A_har bimarkaz al-qamar.

\clearpage
\noindent fa-in kAn
alla_dI ymrr bmarkaz al-qamar ymAss al-mudIr, fa-al-ta`dIl fI
nihAyatihi, wa-hwa br.sdnA \aemph{_Ab kw}. wa-yn`dm fI kwn al-qamar fI
al-_dirwaT wa-al-.ha.dI.d \VAR{limarkaz al-tadwIr}{in kAna
al-tadwIr [\mb,\mc,\md], nAqi.saT [\me]}.\fol{.z 15 \ma} wa-yazAd `l_A
al-_hA.saT i_dA kAn b`d markaz al-tadwIr min ws.t al-^sms aqall min
rb` \VAR{dA'iraT}{al-dA'iraT [\mc]} 'aw ak_tr min ni.sf wa-rb` dA'iraT,
ay ak_tr min\fol{w 17 \mc} ts` burUj"iN 'aw aqall min _tlA_t burUj. wa-ynq.s i_dA kAn
al-b`d ak_tr min rb` dA'iraT wa-aqall min ni.sf wa-rb` dA'iraT, \VAR{ay
  aqll min tis` burUj}{fI hAmi^s [\mc] faqa.t}.

\VAR{al-i_htilAf al-rAbi`}{w al-i_htilAf al-rAbi` [\mc]}, wa-y`rf
\textbf{bita`dIl al-nql}. fa-inna mqwwm al-qamar y.h.sl min al-falak al-mA'il
\VAR{bi.gayr h_dA al-ta`dIl}{fI hAmi^s [\md] faqa.t}; wa-al-.gara.d
maw.di`h min al-muma_t_tal ly`rf maw.di`h min n.tAq al-burUj. wa-h_dA
al-ta`dIl hwa al-tafAwt bayna \VAR{ba`d}{nAqi.saT [\mc]} maw.d`h min
min.tqatay al-muma_t_tal wa-al-mA'il `n al-`qdaT. wa-y`tbr _dlika i_dA
urId t.hwIl a.hadhumA il_A al-'A_har. wa-ysm_A h_dA al-ta`dIl nql
al-qamar \VAR{fI}{min [\mc]}\fol{.z 31 \md} al-mA'il il_A al-burUj. wa-.gAyath
fI 'an.sAf 'arbA` al-mA'il, wa-_dlika \VAR{qarIb}{.gayr maqrU' [\ma]} stt
daqA'iq. wa-yn`dm fI al-`qdatayn wa-`nda nihAyaT `r.d al-qamar fI
al-jihatayn. wa-qll an \VAR{ista`malah}{tasta`miluhu [\mb]}
al-muta'a_h_hrUn.

wa-'ammA \textbf{\VAR{daqA'iq}{al-daqA'iq [\me]} al-nsb}, fahya `dad
\VAR{nisbatihi}{.gayr maqrU' [\ma]} il_A \VAR{sittIn}{al-sittIn
  [\me]} \VAR{kanisbaT}{.gayr maqrU' [\ma]} \VAR{al-lAzim}{al-ilzAm
  [\ma], al-azm ? illA z m ? [\mb]} min i_htilAf al-b`d min al-^sms,
li-annah w.d` litashIl .hsAb mqwwm al-qamar bi-al-jadAwl.

\textbf{tanbIh}. lw .hsbnA min n.sf q.tr al-tadwIr al-mr'iyy bi.tarIq .hsAb
al-ta`dIl al-awwl, .h.sl jmlaT al-ta`dIl \VAR{al-awwal}{fI al-hAmi^s
  [\mb,\me]} wa-al-_tAnI \VAR{al-lAzim}{.gayr maqrU' [\ma], al-azm
  ? illa z m ? [\mb]} fI al-b`d al-m.hsUb lh. wa-hwa m`n_A la.tIf
\VAR{fatanabbah lh}{fatanahhah ilayhi [\mb,\me,\md], fanisbath
  ilayhi [\mc]}.

al-kalAm fI `r.d al-qamar. wa-qd \VAR{ubayyin}{tubayyin
  [\mb,\me,\mc], byn? [\md]} fImA taqaddm annh mtsAwI al-.gAyaT
fI al-^smAl wa-al-junUb. wa-hwa `l_A mA wjd \VAR{bi-al-r.sd}{fI al-r.sd
  [\me]} _hmsaT 'ajzA'. wa-ykUn ^simAly"aN min al-ra's il_A al-_dnb,
wa-junUby"aN min al-_dnb il_A al-ra's. wa-.sA`id"aN min .gAyaT `r.dh fI
al-junUb il_A .gAyaT `r.dh fI al-^simAl, wa-hAb.t"aN min .gAyaT `r.dh
fI al-^simAl il_A .gAyaT `r.dh fI al-junUb.

\clearpage
\noindent wa-al-mrAd min al-.s`Ud qrb
al-qamar min al-q.tb al-.zAhr, wa-min al-hbU.t b`dh minh.
wa-i_htilAf al-man.zr \VAR{w i_htilAf}{fI al-hAmi^s [\me]} t^skkulAtihi
al-nUriyyaT \VAR{b.hsb}{_A.hsb [\ma]} w.d`h min al-^sms
\VAR{y_dkr}{t_dkr [\md], _A_dkr [\mc]} fI bAb"iN mfrd min b`d, in ^sA
al-ll_ah t`Al_A.

wa-'ammA i_htilAf 'ajzA' s.t.hh min qbUl al-nUr al-musammI bi-al-m.hw
fa-al-a^sbh anna b`.dh qAbil lil-nUr dUn b`.d"iN 'aw li-i_htilAf w.d`h
min al-^sms. wa-qIl min wjUd 'ajrAm m_htalifaT"iN m`h fI tadwIrh .gyr
qAbilaT lil-inAraT `l_A al-tasAwI. wa-qIl an sbabh in`kAs al-i^s`aT min
al-b.hr al-m.hI.t, li.sqAlatihi, il_A al-qamar, wa-`dm in`kAsh
\VAR{fI}{min [\mb,\me,\md,\mc]} s.t.h al-rb` al-m`mUr wa-.gyrh
\VAR{li.h^swnath}{li_h^swnath [\me,\mc]} ilayhi.
\VAR{fatakUn}{fayakUn [\me]} al-mwA.d`
\VAR{al-mstnIraT}{al-mstatiraT (?) [\mb,\me], al-mstadIraT
[\md,\mc]} min wjhih\fol{.z 17 \mc} bi-al-i^s`aT al-mstaqImaT al-wA.silaT
ilyh min al-^sms \VAR{al-mun`akasaT min s.t.h al-b.hr a.dwA min al-mwA.d`
al-mstnIraT bi-al-i^s`aT al-mustaqImaT min al-^sms}{fI al-hAmi^s [\md,\mc]}
fq.t.

\begin{center}
\large f.sl
\end{center}
wa-'ammA b`d al-qamar min markaz al-ar.d:
`l_A h_dh al-hI'aT, fa-anna b`d al-qamar,
fI\fol{w 16 \ma} \VAR{kull}{fI [\md] wa-[\mc] faqa.t} al-ijtimA`At
wa-al-istiqbAlAt, aws.th sittIn juz'"aN, wa-ak_trh \aemph{sh _A},
wa-aqllh \aemph{nd n}. wa-fI al-tarbI`At, ak_trh \aemph{s.h 0} wa-aqllh
\aemph{nb 0}. wa-\VAR{ab`d}{ab`dh [\md]} b`d 'aflAkh \aemph{s.t 0},
wa-aqrb qrbhA \aemph{nA 0}. al-jamI` bi-al-'ajzA'i allatI bihA ni.sf
q.tr al-mA'il sittIn juz'"aN.

wa-i`lam an markaz al-tadwIr b`dh min markaz al-ar.d sittIn juz'"aN lA
yzId wa-lA yanq.s. fa-i_dA aradti b`d al-qmr bi-al-'ajzA'i allatI
\VAR{bihA}{nAqi.saT [\md], fI al-hAmi^s [\mb], fawqa al-s.tr
  [\ma,\me], walakin fI [\mb,\me] ktb >>bihA<< ba`da >>ni.sf
  q.tr al-ar.d<<} ni.sf q.tr al-ar.d \VAR{aw a.hd 'aw h_dA}{wA.hid
  wa-h_dA [\mb,\me], wA.hid"aN wa-h_dA [\md,\mc]} hwa al-msta`ml
fI al-'ab`Ad wa-al-'ajrAm, fa.tarIqh `l_A r.sdnA, an \VAR{tsq.t}{nsq.t
  [\mb], _Asq.t [\me,\md]} min kl drjaT"iN daqIqatayn ybqI
al-ma.tlUb, wa-`l_A m_dhb b.tlmyws \VAR{talqI}{nAqi.saT [\mc]} min kl
darjaT daqIqaT. li-anna ba`d markaz al-tadwIr min markaz al-`Alam
br.sdnA _tmAnyaT wa-_hamsIn m_tl"aN lini.sf q.tr al-ar.d, wa-hwa `nd
b.tlmyws ts`aT wa-_hmsIn m_tl"aN lini.sf q.tr al-ar.d.

\clearpage

wa-tfsIr \VAR{a^syA}{a^syA a^syA [\md]} tata`laq bi-al-qamar.

-- \textbf{ws.t al-jwzhr} hwa mA bayna 'awwal al-.hml wa-nq.taT al-ra's min
\VAR{al-muma_t_tal}{muma_t_tal [\ma]} il_A _hilAf al-tiwAlI.

-- \textbf{wa-tqwIm al-jwzhr} hwa mA baynahumA minh `l_A al-tiwAlI.

-- \textbf{ws.t al-qamar} hwa mA
bayna al-nuq.taT al-mu.hA_dyaT li-'awwal al-.hml `l_A annahA _tAbitaT
wa-bayna .trf al-_h.t.t al-_hArij min markaz al-`Alam il_A markaz
al-tadwIr. wa-in qultu b`d markaz al-tadwIr min al-nuq.taT al-ma_dkUraT
`l_A al-tiwAlI kAn .sawAb"aN ay.d"aN.

-- wa-i_dA \VAR{usq.tnA}{usq.tnAh
  [\mb]} ws.t al-^sms min ws.t al-qamar bq_A \textbf{b`d} markaz al-tadwIr min
ws.t al-^sms, wa-.d`f h_dA al-b`d ysmm_A \textbf{al-b`d al-m.dA`f}, wa-hwa
bimqdAr .harakaT mudIr al-qamar.

-- \textbf{wa-_hA.s.saT al-qamar} mA bayna
_dirwaT al-tadwIr al-ws.t_A wa-markaz jrmh min min.taqaT al-tadwIr
`l_A al-tiwAlI al-mafrU.d minh, wa-hwa in yakUn fI \VAR{al-nu.sf}{ni.sf
  [\mb,\me,\md,\mc]} al-'a`l_A il_A _hilAf al-tiwAlI.

wa-h_dh al-qs_A lA \VAR{t_htalif}{_A_htalif [\ma,\me,\md]} muqAdIrhA.
\VAR{w mA ya_htalifu muqAdIrhA}{fI al-hAmi^s [\ma], wa-mA ta_htalifu
  muqAdIrhA [\md], wa-ammA mA ya_htalifu muqAdIrhA [\mb,\me],
  walakin ktb >>mA<< fwq al-s.tr fI [\mb]} bi-al-zyAdaT wa-al-nuq.sAn faminhA~:

-- \textbf{_hA.sath al-m`dlaT} wa-hya mA bayna markaz jrm al-qamar
wa-\VAR{_dirwatihi}{dawratihi [\mb]} al-mar'iyyaT\fol{w 32 \md} min min.taqaT
tadwIrh wa-hya al-_hA.s.saT \VAR{al-.haqIqaT}{al-.haqIqiyyaT
  [\mb,\me]} b`d ta`dIlhA bi-al-ta`dIl al-'awwal,

-- \textbf{wa-tqwIm al-qamar} hwa mA bayna 'awwal al-.hml wa-al-nuq.taT
allatI ytqA.t` `lyhA dA'iraT
`r.dh min al-muma_t_tal `l_A al-tiwAl_A,

-- \textbf{wa-.hi.s.saT `r.dh} hya f.dl mqwwm al-qamar `l_A mqwwm al-jwzhr.

\clearpage
\addcontentsline{toc}{chapter}{\textarab{fI taqyId .harakAt al-qamar
    lita'rI_h mafrU.d"iN}}
\begin{center}
\Large al-bAb al-`A^sr\fol{.z 18 \mc}

\large fI \VAR{taqyId}{ta`Id [\mc]} .harakAt al-qamar lita'rI_h mafrU.d"iN
\end{center}
qad katabnA fI al-jadAwil an wasa.t al-qamar lini.sf nahAr yawm
al-_tl_tA 'awwal sanaT i.hd_A wa-sb`mi'aT liyazdajard
wa-sb`mi'aT\fol{.z 32 \md\\.z 16 \ma} \VAR{\aemph{r j lh n}}{\aemph{r j lh nh} [\mb],
  kutiba fI hAmi^s [\mc] 'ay.d"aN >> i`lam an ws.t al-qamar hwa
  biziyAdaT `i^srIn daqIqaT allatI minhu al-m.sn_d fI al-zIj `l_A
  nq.shA fahwa ... fatanq.s fI mwA.dfhA wa-ra.sad wa-`ilm <<}.
wa-.harakaT was.t al-qamar fI `i^srIn sanaT fArsiyyaT \VAR{\aemph{b r
    m m.t m.h kA}}{\aemph{b r m _A.t m.h kA} [\mb]}, wa-fI sanaT
wA.hidaT \VAR{\aemph{d .t kj b k.t kh A}}{\aemph{w .t kj b k.t kh A}
  [\mb,\md,\me], \aemph{d .t kj b k.t kh j} [\mc]}, wa-fI
_talA_tIn yawm"aN \aemph{A h _Ar l lw nw _A.h .t}, wa-fI yawm
bilaylatihi \VAR{\aemph{0 _Aj _A lh A _Aj nb lw _A.h _Aw r}}{\aemph{0
    _Aj _A lh A _Aj b lw _A.h _Aw r} [\mb,\me]}, wa-fI sA`aT
\VAR{mutasawiyaT}{mustawiyaT [\md,\me,\mc]} \VAR{\aemph{0 0 lb nw
    kz lj d mA l mh}}{\aemph{0 0 lb nw kz _Aj mA lA} [\mb,\me],
  \aemph{0 0 lb nw kz lj mA lA} [\ma,\md]}.

wa-katabnA an \VAR{_hA.s.saT}{_hA.siyaT [\md]} al-qamar lil-ta'rI_h
al-ma_dkUr \aemph{d _A.h lb kr}. wa-.harakatuhA fI `^srIn sanaT
fArisiyaT \VAR{\aemph{_AA d kb l}}{\aemph{_AA d lb l} [\mb,\me]},
wa-fI sanaT wA.hidaT \aemph{b k.h mj r}, wa-fI ^shr \aemph{A A nw n.h},
wa-fI yawm \aemph{0 _Aj j nj nw} wa-fI sA`aT \aemph{0 0 lb l.t mh}.

wa-\VAR{a_tbatnA}{ay.d"aN [\mb,\me]} ws.t al-jawzhar lil-ta'rI_h
al-ma_dkUr \aemph{.t h r lh}. wa-.harakatuhA il_A _hilAf al-twAl_A fI
kull `^srIn sanaT\fol{w 17 \ma}
\VAR{\aemph{0 kw ld lr
    k}}{\aemph{0 kw ld lr kh} [\mb,\me]}, wa-\VAR{fI sanaT wA.hidaT
  \aemph{0 _A.t _A.t mj nb}}{fI ^shr wA.hid \aemph{0 _A.t _A.t mj nb}
  [\mb]}, wa-fI ^shr wA.hid \aemph{0 A lh _A.t _Aj _A.h nd _Ah}, wa-fI
yawm \aemph{0 0 j _A l.h kw lr m.h k.t lw}, wa-fI sA`aT \aemph{0 0 r nw
  lw wa-lh}.

\clearpage

wa-i_d tqddm _dalika, fa-i`lam an al-sanaT al-qamariyaT `l_A
al-.sa.hI.h \VAR{\aemph{^snd kb A lh .h n kd}}{nAqi.saT [\mb]},
wa-al-^shr\fol{.z 33 \md} al-qamariyy al-wasa.t \VAR{\aemph{k.t lA
  n r nh md _Ab}}{\aemph{k.t lA nh r nh md _Ab} [\mb,\me]}, wa-sanaT
al-^sams al-.sa.hI.haT \VAR{_tlA_tmi'aT wa-_hmsaT wa-sittUn yawm"aN
  wa-_hms sA`At"iN wa-ts` wa-arba`Un daqIqaT wa-_tlA_taT a_hmAs
  _tAli_taT wa-hya}{nAqi.saT [\mc]} \aemph{^ssh} \aemph{h m.t 0 lw lb}.

wa-i_dA fr.dnA al-yawm bilaylatihi sittIn juz'"aN, kAnat al-sanaT
al-^samsiyaT 365 \aemph{_Ad lb lA lA k} wa-yakUn f.dl \VAR{al-dawraT
  \aemph{w _Ah .t .h}}{al-dawr \aemph{_Aw _Ah .t .h} [\mb,\me],
  al-dawwar \aemph{fw _Ah .t .h} [\md,\mc]}.

wa-i_d\fol{.z 17 \ma} tqddm _dlika, fa-i`lam anna q.tr al-qamar fI b`dihi al-awsa.t
min al-ar.d, \VAR{w _dalika `nda kawn b`d al-qamar min al-ar.d sittIn
  juz"aN min ajzA' ni.sf q.tr .hAmil al-tadwIr}{\aemph{0 lb nd lj}
  wa-_dalika `nd kawn b`d al-qamar min al-ar.d 60 juz"aN min ajzA'
  qi.tr .hAmil al-tadwIr [\mc]} \VAR{\aemph{0 lb nd lj}}{\aemph{0 lb
    nd l.h} [\me], nAqi.saT [\mc]}. wa-qad kuntu waqaftu `l_A
_dalika min .tarIq 'A_hr fawajadtuhu \aemph{lb kb}, wa-a`tmAdiy `l_A
al-'awwal. wa-q.tr al-qamar `nd ibar_hus \aemph{lj _Ah}, wa-`nda
b.tulamiyUs \aemph{lj h}, wa-`nda ahl al-hind \aemph{lb 0}, wa-`nda
al-jumhUr \aemph{lb k}, wa-`nda al-a_tIr wa-kw^siyAr wa-al-.tUsI
\aemph{lb j}.

wa-i_dA aradnA qi.tr al-qamar fI .gayr b`dh al-awsa.t, qsmnA qi.trh fI
b`dh al-awsa.t `l_A b`dh min markaz al-`Alam, bi-ajzA' qi.tr
al-muma_t_tal, y.h.sl qi.tr al-qamar fI _dalika al-b`d.

wa-buht sA`aT al-qamar huwa qi.trh ay.d"aN, wa-\VAR{bi-al-wajh}{al-wajh
  [\mc]} al-'awwal a.s.h.h fa-a`rfh.

wa-ammA qi.tr al-.zill, \VAR{fa-annahu}{fahwa [\mc]} `nda b.tulamiyUs
mi_tl qi.tr al-qamar marratayn wa-_tlA_taT a_hmAs marraT. wa-qad
wjadtuhu bi-ar.sAd"iN _husUfAt ka_tIraT qadImaT wa-.hadI_taT,
\VAR{marratayn wa-ni.sf wa-_hms marraT}{\aemph{b l _Ab} [\mc]} i_dA
\VAR{`amalnA `l_A}{`alamnA [\md,\mc], `alamnA `l_A [\me]} an
nihAyaT `r.d al-qamar _hams\fol{w 19 \mc} darjAt"iN ; wa-i_d \VAR{`amalnA
  `l_A}{`alamnA `l_A [\md,\me], `alamnA [\mc]} annah \VAR{arba`
  darj wa-_tl_t_A wa-rb` darjaT}{\aemph{d m _Ah} [\mc]}, kAna mi_tl
qi.tr al-qamar \VAR{marratayn wa-_tl_t_A marraT}{\aemph{b m} [\mc]}.
wa-_dalika anA wajadnA mk_t al-_husUfAt bi-al-ra.sad ak_tar mA
yqt.diyh al-.hisAb `l_A far.d an qi.tr al-.zll mi_tl qi.tr al-qamar
marratayn wa-_tl_taT a_hmAs.
\end{arab}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\input{lune.pdf_tex}
\end{minipage}
\textarab{w h_dh .sUraT aflAk al-qamar w hya madArAt marAkiz al-akr
  al-tAmmaT `l_A .hsb mA yata.swr `l_A al-basI.t li-iqAmaT al-barAhIn
  w .hisAb al-ta`AdIl `l_A anA .sawarnA falak al-tadwIr w al-mudIr fI
  _tamAniyyaT amAkin w tilka al-amAkin hya al-ijtimA` w al-istiqbAl w
  al-tarbI`ayn w fI an.sAf al-arbA` liyshl t.swr _dlika fI kull makAn}
\end{figure}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\input{lune_orbes.pdf_tex}
\end{minipage}
\textarab{w h_dh .sUraT aflAk al-qamar al-mjsmaT `l_A annahA krrAt
  tAmmaT mt.hrkAt .harakAt basI.taT mustawiyaT `nd marAkzhA .hsb mA
  yt.swr fI al-basI.t alla_dI hwa s.t.h al-mA'il w qad tqdm an s.t.h
  al-mA'il mA'il `n s.t.h al-burUj ayy al-mum_t_tl mIlaN wA.hidaN
  nihAyath m_tl `r.d al-qamar}
\end{figure}

\begin{arab}
\resetlinenumber\pagewiselinenumbers
\clearpage
\addcontentsline{toc}{chapter}{\textarab{fI taqwIm al-qamar,
    bi-al-jadwal wa-al-.hisAb}}
\begin{center}
\Large al-bAb al-.hAdI `^sr\fol{.z 19 \mc}

\large fI taqwIm al-qmr bi-al-jadwal wa-al-.hsAb
\end{center}
'i_dA 'ardt _dlk, fa-a.hsb min al-jadAwl ws.t al-qmr wa-_hA.s.satahu
wa-ws.t al-^sms `l_A n.hw mA 'aw.d.htu laka fI al-^sms. _tmm unq.s ws.t
al-^sms min ws.t al-qmr; famA bq_A a.d`fh fahwa markaz al-qmr, wa-hwa
b`d markaz al-tadwIr min al-b`d al-'ab`d. fa-ud_hl bihi 'il_A jadwl
ta`AdIl \VAR{al-qmr}{fawqa al-s.tr [\mc]}, wa-_h_d bihi ta`dIl
al-_hA.s.saT. fa-'in kAna al-markaz 'aqall min sitt burUj, fazid
al-ta`dIl `l_A al-_hA.s.saT, wa-'in kAna al-markaz 'ak_tr min sitt
burUj, fanaqqi.sh min al-_hA.s.saT. \VAR{t.h.sl}{y.h.sl [\md,\me]}
al-_hA.s.saT al-mu`addlaT. _tmm ud_hl bi-al-_hA.s.saT al-mu`addlaT
'il_A jadwl \VAR{t`AdIl}{nAqi.saT [\mb]} al-qmr, wa-_h_d mA bi-'izA'i
_dlk min al-t`dIl al-_tAli_t wa-al-rAb`. _tmm ud_hl bi-al-markaz 'il_A
jdwl t`AdIl al-qmr, wa-_h_d bihi al-t`dIl al-_tAnI, \VAR{fa-u.drbh}{w
  u.drbh [\mc]} fI al-rAb`, famA .h.sl fazidh `l_A al-_tAli_t ; y.h.sl
al-t`dIl \VAR{al-_tAli_t}{nAqi.saT [\me]} \textbf{al-mu.hkm}. _tmm un.zr,
\VAR{'in}{an in [\ma]} kAnat \VAR{al-_hA.s.saT}{al-.hA.silaT [\mb]}
al-m`addlaT 'aqll min sitt burUj, fanaqqi.s al-m.hakam min ws.t al-qmr,
wa-'in kAnat 'ak_tr min sitt burUj, fazid al-m.hkam `l_A ws.t al-qmr.
y.h.sl muqawwamu al-qmr min min.tqaT al-mA'il. _tmm unq.s al-jwzhr
al-mqwm\fol{w 18 \ma} min \VAR{al-qmr al-mqwm}{al-qamar bi-al-mqawwm [\mb,\me],
  al-qamar [\md], muqawwam al-mA'il [\mc]}. \VAR{ybq_A}{tabq_A
  [\mb,\mc], _Abq_A [\me]} .hi.s.saT \VAR{`r.d al-qmr}{al-`r.d
  [\mc]}. ud_hl bihA 'il_A jadwal ta`dIl nql al-qmr, famA wjdt
bi-'izA'ihA, fanaqqi.sh min mqwm al-qmr 'in kAnat .h.s.saT \VAR{`r.d
  al-qmr}{al-`r.d [\mc]} min darjaT 'il_A ts`In 'aw min mi'aT"iN
wa-_tmAnyn 'il_A mi'atayn wa-sb`In, wa-\VAR{'in}{'i_dA [\me]} kAnat
.gyr _dlk fazdh `l_A mqwm al-qmr.

\clearpage
\noindent y.h.sl mqwm al-qmr min flk al-burUj
lil-wqt alla_dI .hsbt lah, lini.sf nhAr, dami^sq. fa-in lam ykn
al-ta'rI_h m`ddl"aN bit`dIl al-'ayyAm bilayAlIhA, fayujib 'an
\VAR{tu`dl}{y`dl [\mc], _A`dl [\me]} `l_A na.hw mA `rftuk fI
al-^sms.

wa-'i_dA 'aradta `r.d al-qamar, fa-ud_hl bi.h.s.saT al-`r.d 'il_A jadwl
`r.d al-qamar, tjd bi-'izA'ihA `r.d al-qamar wa-jihatihi.

wa-.tarIqh bi-al-.hisAb, 'an ta.drb jIb al-.hi.s.saT fI .zll `r.d
al-qamar al-kullI, y.h.sl .zll `r.d al-qamar al-juz'iyy.
\VAR{faqawwish}{tqUsh [\ma]} fI jdwl al-.zll al-m`kUs al-sittIniyy, tjd
al-`r.d. wa-qd tqdm `lm jihath.

\begin{center}
\large f.sl

\normalsize fI m`rfaT ta`dIl _hA.s.saT al-qamar bi-al-.hisAb
\end{center}
i`rif markaz al-qamar wa-u.drub jIbh fI ni.sf q.tr .hAmil al-jrm, wa-hwa \aemph{A
  kh}. famA .h.sl fahwa \textbf{al-maqsUm}. _tmm u.drub jIb tamAm al-markaz fI
\aemph{A kh}. famA .h.sl naqqi.sh min ni.sf q.tr\fol{w 20 \mc} al-tadwIr, wa-hwa
\aemph{w lh}, i_dA kAn al-markaz min darjaT il_A ts`In 'aw min mi'atayn
wa-sb`In 'il_A _tl_tmi'aT wa-sittIn. wa-in kAn al-markaz _hlAf _dlik,
fazdh `l_A n.sf q.tr al-tadwIr \VAR{alla_dI hwa \aemph{w lh}}{nAqi.saT
  [\mc]}. famA .h.sl, ujm` murabb`h wa-murabb` al-maqsUm. famA kAn, _h_d
j_drh, fahwa n.sf q.tr al-tadwIr al-mr'iyy. fa-i.hfa.zh, fa-innaka
ta.htAj 'ilayhi fI h_dA al-`ml wa-.gyrh. _tmm iqsim `l_A ni.sf q.tr
al-tadwIr al-mr'iyy al-maqsUm, y_hrj \VAR{jIb}{.hsb [\mb]} ta`dIl
al-_hA.s.saT ; 'a_tbith bi-'izA' tlk al-darjaT.

\clearpage

\begin{center}
\large f.sl

\normalsize fI .hsAb ta`dIl al-qamar al-_tAnI
\end{center}
u.drb jIb al-_hA.s.saT
al-mu`addlaT wa-jIb tamAmihA fI ni.sf q.tr al-tadwIr al-mr'iyy fI
\VAR{waqt}{fI [\mc] faqa.t} al-ijtimA` wa-al-istiqbAl, wa-hwa f.dl n.sf
q.tr al-tadwIr `l_A n.sf q.tr al-mdIr, wa-hwa \aemph{h _A}. famA\fol{.z 33 \md}
.h.sl min jIb al-tamAm, fazidh `l_A \VAR{sittIn}{90 [\me]} abad"aN 'in
kAnat al-_hA.s.saT \VAR{al-mu`addalaT}{fawqa al-s.tr [\md,\mc]} fI
al-n.sf \VAR{al-'a`l_A min al-tadwIr wa-naqqi.sh in kAnat al-_hA.saT
  fI al-ni.sf}{fI hAmi^s [\mc,\md], al-'a`l_A min al-tadwIr wa-b`.dh
  in kAnat al-_hA.saT fI al-ni.sf [\mb], al-'a`l_A min al-tadwIr
  wa-naqqi.sh in kAnat fI al-ni.sf [\me]} al-'asfl minh. famA .h.sl
fazid mrbb`h `l_A mrbb` al-mt.h.s.sl min .drb jIb al-_hA.s.saT fI
\aemph{h _A}, wa-hwa al-maqsUm. famA bl.g _h_d j_drh. famA kAn iqsim
`alayh al-maqsUm. y.h.sl jIb al-ta`dIl al-_tAnI lil-darjaT allatI .hsbt
lahA. \VAR{tqwwsh}{faqawwsh [\mc]} fI jdwl al-jIb : tjd ta`dIl _dlika
al-juz'i.

wa-.tarIq .hsAb al-t`dIl al-_tAli_t 'an \VAR{tafr.d}{_A`iwa.d? (.gayr
  maqrU') [\mb], nfr.d [\md]} \VAR{ni.sf}{nAqi.saT [\me]} q.tr
al-tadwIr al-mr'iyy _tmAn darjAt, wa-hwa jIb sb`aT wa-_tl_tay, \VAR{w
  usluk}{fa-usluk [\md,\mc]} mA `rftuka fI al-ta`dIl al-_tAnI. famA
.h.sl likull juz'"iN, fa-unqu.s minhu al-ta`dIl al-_tanI\fol{.z 18 \ma}
li_dlika al-juz'i. famA bq_A fa-'a_tbith bi-'izA' _dlika al-juz'i.

\textbf{tanbIh}. 'i_dA ista`malt ni.sf q.tr al-tadwIr al-mr'iyy
\VAR{lijuz'"iN}{bijuz'"iN [\me]} mafrU.d"iN `iwa.d \aemph{h _A},
wa-slkt al-.tarIq al-ma_dkUr, _hrj al-ta`dIl al-mu.hakkam, wa-hwa
\VAR{jIb}{fI [\mc] faqa.t, fawqa al-s.tr} al-ta`dIl
\VAR{al-_tAniy}{kutiba >>~al-_tAli_t~<< fI hAmi^s [\md], al-_tAli_t
  [\mc]} mu`addal"aN.

\clearpage

\begin{center}
\large fa.sl

\normalsize fI .hisAb daqA'iq al-nisb lil-qamar
\end{center}
'i_dA 'aradt \VAR{_dlika}{nAqi.saT [\me]} faqws n.sf q.tr al-tadwIr al-mr'iyy fI
jdwl al-jIb ; famA .h.sl fahwa .gAyaT al-i_htilAf fI tilka al-darjaT,
wa-hwa al-ta`dIl al-mu.hakkam litilka al-darjaT. fa-unq.s minh
\VAR{\aemph{d nw kd}}{\aemph{d nw kh} [\mb,\me]} wa-hwa nihAyaT
al-ta`dIl al-_tAnI. \VAR{w mA}{famA [\mb,\me]} baq_A, iqsimh `l_A
\aemph{b mj kA}, wa-hwa fa.dl .gAyaT al-i_htilAf fI al-tarbI`In alla_dI
hwa \aemph{z l.t mh yA} `l_A .gAyaT al-_tAnI. famA _hrj bi-al-qismaT,
fahwa daqA'iq al-nisb ; fa-'a_tbith bi-'izA'i tilka al-darjaT.

\textbf{tanbIh}. i`lam annahu yumkin an \VAR{tuwa.da`a}{yw.d` [\mb], _Aw.d`
  [\me]} jdAwl litaqwIm al-qamar, `l_A aw.dA` 'A_har\fol{.z 20 \mc} .gyr
\VAR{al-ma^shUraT}{al-ma^shUr [\me]}. wa-_dlik bi-an
\VAR{tafr.d}{nfr.d [\md], yfr.d [\me]} tdwIr al-qamar al-tadwIr
al-.haqIqI alla_dI ni.sf q.trh \aemph{w lh}. wa-t.hsb lah i_htilAf
ynq.s minh fI al-b`d al-'ab`ad, wa-i_htilAf \VAR{yzAd}{yzId [\md]}
`lyh fI al-b`d al-'aqrb wa-hwa _tmAnyaT 'ajzA'. wa-\VAR{t.hsb}{y.hsb
  [\mc,\me?]} lh i_htilAf ynq.s minh bidaqA'iq \VAR{nisb}{bisabab
  [\mb,\me]}, `ks al-ma^shUr. wa-ymkin an yw.d` jdwl wA.hd litaqwIm
al-qamar \VAR{bayna}{nAqi.saT [\mc]} li-'An"iN .gAyaT al-i_htilAf fI
'ajzA'i al-.hAmil ma`lUmaT wa-ta`dIl al-_hA.s.saT lAzm fI _dlika
al-juz'i.
% A 18v l. 11

\clearpage

\VAR{w m_tAl}{m_tAlh [\mc]} _dlika, 'i_dA fara.dnA markaz al-qamar,
wa-hwa al-b`d al-mu.dA`f, _tlA_t burUj, kAn ta`dIl al-_hA.s.saT
\aemph{yb kw}. wa-nihAyaT al-i_htilAf, 'i_dA kAn al-markaz _tlA_t burUj,
sittaT 'ajzA' wa-suds juz' ; wa-.hsbnA al-ta`dIl al-_tAnI `l_A 'anna
nihAyath \VAR{al-sittaT}{al-sitt [\mb,\me]} wa-al-suds. wa-'a_tbatnA
_dlika bi-'izA'i \aemph{yb kw}. kAn h_dA al-jdwl mat_A d_hlnA
\VAR{'ilyh}{`layh [\md]} bi-al-_hA.s.saT al-mu.tlqaT, \VAR{a`nI
  al-.gyr m`ddlaT}{nAqi.saT [\mc]}, wjdnA al-ta`dIl al-mu.hakkam min
.gyr ta`dIl"iN zA'id ; wa-'innamA \VAR{n.htAj}{y.htAj
  [\md,\mc,\me]} 'il_A jdAwl ka_tIraT.

\begin{center}
  \large f.sl
\end{center}
\textbf{i_dA 'aradt b`d al-qamar min markaz al-`Alam}, fa-i`rif jIb
_hA.s.saT al-qamar al-m`ddlaT wa-jIb tamAmhA ; wa-u.drub kull wA.hid"iN
min al-jIbayn fI ni.sf q.tr falak al-tadwIr al-mr'iyy, wa-hwa \aemph{h
  _A} fI al-ijtimA` wa-al-istiqbAl, wa-fI .gyrhumA wa-hwa mA 'amartuka
bi.hf.zh fI al-fa.sl al-'awwal min h_dA al-bAb. famA .ha.sala min jIb
al-_hA.s.saT, fahwa \textbf{al-maqsUm} fa-i.hf.zh. wa-zd mA .h.sl min jIb
al-tamAm `l_A sittIn, 'i_dA kAnat al-_hA.s.saT al-m`ddlaT 'aqll min
_tlA_t burUj 'aw 'ak_tr min ts` burUj, wa-'in kAnat .gyr _dlika
fa-unq.sh min sittIn. famA bl.g 'aw bq_A, fa-ujm` mrbb`h wa-mrbb`
al-maqsUm. wa-_h_d j_dr _dlika, famA kAn fahwa b`d al-qamar min markaz
al-`Alam `l_A 'anna ni.sf q.tr al-.hAmil sittIn \VAR{juz'"aN}{'ajzA'
  [\me]}.

\textbf{tanbIh}. 'i_dA qsmnA `l_A h_dA al-b`d q.tr\fol{w 19 \ma} al-qamar fI
b`dh al-'aws.t, wa-hwa \VAR{\aemph{0 lb nd lj}}{\aemph{0 lb nd _Aj} [\me]}, .h.sl
q.trh fI _dlika al-b`d. wa-'i_dA .drbnA bht ywmh fI daqIqatayn wa-ni.sf,
.h.sl q.tr al-qamar, wa-bi-al-.tarIq al-'awwal 'a.db.t. wa-q.tr al-qamar
'aqallh fI al-ijtimA`At wa-al-istiqbAlAt \VAR{\aemph{0 l
    n.h}}{\aemph{0 l n.h A _A} [\md,\mc], \aemph{0 l _A.h A}
  [\me]}, wa-'ak_trh fIhA \aemph{lw 0}. wa-'aqllh fI al-tarbI`ayn
\VAR{\aemph{k.t b yh}}{\aemph{l.t b _Ah} [\me]}, wa-'ak_trh fIhA
\aemph{lz n.h k}. fa-i`rif _dlika.

\textbf{tanbIh _tAn"iN}.\fol{w 34 \md\\w 21 \mc} \VAR{w}{nAqi.saT [\mb,\md,\mc]}
lw qsmnA `l_A h_dA al-b`d al-maqsUm al-ma.hfU.z, _hrj jIb al-ta`dIl
al-mu.hakkam lil-qamar. \VAR{fa-ifham _dlika}{nAqi.saT [\mc]}.

\end{arab}


==> fichier2c.tex <==
\begin{arab}
\resetlinenumber\pagewiselinenumbers

% à partir de maintenant, on ne garde plus que A, C et D.
% (il y avait certaines portions des mss. pour lesquelles on avait édité
% aussi B et E, mais elles seront commented out avec des \iscomplet)
\clearpage
\begin{center}
\Large al-bAb al-_tAniy `^sr

\large fI hI'aT 'aflAk z.hl `l_A al-wajh al-.s.hI.h
\end{center}
\VAR{ntwhm}{ytwhm [\md]} min 'aflAk z.hl :

-- \textbf{falak muma_t_tal} bifalak al-burUj fI s.t.hh
.hawla markazh wa-`l_A q.tbayhi,

-- wa-ntwhm falak _tAn"iN \textbf{mA'il} `n al-muma_t_tal mIl _tAbit
miqdArh juz'An wa-ni.sf, \VAR{mqA.t`}{yuqA.t` [\md,\mc]} lah `l_A
nuq.tatayn mtqAblatayn wa-tsm_A 'i.hdAhumA al-ra's wa-al-'u_hr_A
al-_danb,

-- wa-ntwhm falak _tAli_t markazh `l_A mu.hI.t al-mA'il wa-ni.sf q.trh
_hamsaT 'ajzA' wa-_tmn juz' (bi-al-'ajzA' allatI bihA ni.sf q.tr
al-mA'il sittIn juz'"aN); wa-ysm_A \textbf{al-.hAmil},

-- \VAR{wa-ntwhm}{wa-ytwhm [\md,\mc]} falak rAbi`
markazh `l_A mu.hI.t al-.hAmil wa-ni.sf q.trh darjaT wa-i_tnayn
wa-'arba`In daqIqaT wa-_tala_tIn _tAniyaT; wa-ysm_A \textbf{al-mudIr},

-- wa-ntwhm falak _hAmis markazh `l_A mu.hI.t al-mudIr wa-ni.sf q.trh
sittaT 'ajzA' wa-ni.sf (bitilka al-'ajzA'); wa-ysm_A \textbf{falak
al-tadwIr},

-- wa-markaz jrm z.hl lAzim"uN linuq.taT `l_A min.taqaT al-tadwIr.

fa-'ammA al-.harakAt fa-'inna al-muma_t_tal yata.harrak .harakaT
basI.taT .hawla markazh 'il_A al-twAlI \textbf{.harakaT al-'awjAt}
wa-hwa fI al-yawm \aemph{0 0 .t nb}. fayantaqilu al-taqA.tu` wa-hwa
al-ra's wa-al-_danb wa-tantaqilu .gAyatAn al-mIl 'ay.d"aN.

wa-yata.harrak al-falak al-mA'il .harakaT basI.taT .hawla markazihi
alla_dI hwa markaz al-`Alam 'il_A al-tawAlI 'ay.d"aN
bimiqdAr \textbf{.harakaT markaz z.hl} wa-hwa fa.dl ws.th `l_A
.harakaT al-'awj: wa-hwa fI al-yawm bilaylatihi \aemph{0 b 0 kw _Ar}.

wa-yata.harrak al-.hAmil 'il_A _hilAf al-tawAlI fI 'a`lAh biqdr
.harakaT markaz z.hl alla_dI \VAR{hwa fI}{fawqa al-s.tr [\ma],
nAqi.saT [\md]} al-yawm bilaylatihi \aemph{0 b 0 kw _Ar}.

wa-yata.harrak al-mudIr fI 'a`lAh 'il_A al-tawAlI, qdr .d`f .harakaT
markaz z.hl, wa-hwa fI al-yawm bilaylatihi \aemph{0 d 0 nb ld}.
fa-tkamml al-dawraT minh ma`a ni.sf dawraT min al-.hAmil.

\VAR{wa-tata.harrak}{wa-yata.harrak [\mc]} falak al-tadwIr .harakaT
basI.taT .hawla markazh fI 'a`lAh 'il_A al-tawAlI bimqdAr f.dl
\textbf{.harakaT _hA.saT} z.hl `l_A .harakaT markazh.

\clearpage
\noindent wa-h_dihi al-.harakaT
basI.taT mrkkabaT, li-'annA 'i_dA fara.dnA al-tadwIr sAkin"aN wa-t.hrk
al-mA'il rb` dA'iraT, wa-t.hrk al-.hAmil rb` dA'iraT, wa-t.hrk
al-mudIr ni.sf dA'iraT, 'a`nI intaqala al-q.tr al-mArr bi-al-_dirwaT
wa-al-.h.dI.d rb` dA'iraT, fa-yjb 'an nfr.d lahu .harakaT 'il_A _hilAf
al-tawAlI bimiqdAr .harakaT al-.hAmil allatI\fol{.z 19 \ma} hiya
.harakaT markaz z.hl, fa-_Antql al-q.tr al-mArr bi-al-_dirwaT
wa-al-.ha.dI.d 'il_A mw.d`h.

_tmm wjdnA bi-al-ra.sad 'anna al-tadwIr yata.harrak biqdr _hA.saT z.hl
wa-hiya \VAR{fI}{fawqa al-s.tr [\ma]} al-yawm bilaylatihi \aemph{0 nr
r mj ld kb}, faqad .zahara 'annahu yta.harrak 'il_A _hilAf al-tawAlI
.harakaT basI.taT .hawla markazh. wa-.zahara 'annahu\fol{.z 21 \mc}
yata.harrak \VAR{'il_A al-tawAlI .harakaT basI.taT .hawla markazh}{.harakaT
basI.taT .hawla markazh 'il_A al-tawAlI [\mc]}, fa-ynq.s aqall
al-.harakatayn min al-ak_tar, wa-hiya .harakaT al-markaz min .harakaT
al-_hA.s.saT. fa-tabq_A .harakaT falak al-tadwIr 'il_A al-tawAlI
bi-qadr \VAR{fa.dl}{fI al-hAmi^s [\ma]} .harakaT _hA.s.saT z.hl `l_A
.harakaT markazh: wa-hiya fI al-yawm \VAR{bilaylatihi}{nAqi.saT [\ma]}
\aemph{0 nh r _Ar _Ar kb}. wa-h_dihi hiya al-.harakaT al-basI.taT
al-.haqIqaT, .gayr 'anna al-_dirwaT tat.harrak 'il_A al-tawAlI
'abad"aN bi-qadr .harakaT _hA.s.saT z.hl, wa-hiya mjmU` ha_dihi
al-.harakaT wa-.harakaT markazh. wa-ha_dA ma`n_A la.tIf yjb t.swrh.
\VAR{wa-`l_A}{`l_A [\mc]} _dalika bAq_A al-kawAkib, fa-lA .hAjaT 'il_A
'i`AdaT ha_dA al-^sr.h. wa-\VAR{lammA}{lamnA [\ma]} i.htajnA 'il_A
ba`d al-kawkab min al-_dirwaT, i.htajnA \VAR{tajammu`}{bijam` [\mc]}
.harakaT ha_dA al-tadwIr wa-.harakaT markaz z.hl:
\VAR{fa_A.h.sl}{fa.h.sl [\md,\mc]} min _dalika mi_tl .harakaT _hA.s.saT
z.hl, wa-hwa ba`d al-kawkab min al-_dirwaT.
faqad 'aw.da.htu laka ha_dA al-ma`n_A, wa-fIhi diqqaT fa-ta'ammlhu.

fa-'i_dA fara.dnA marAkiz \VAR{al-.hAmil wa-al-mudIr
wa-al-tadwIr}{al-tadwIr wa-al-mudIr wa-al-.hAmil [\mc]} `l_A
al-_ha.t.t al-mustaqIm al-mArr bi-markaz al-`Alam wa-al-'awj, kAn
markaz al-tadwIr fI ba`dihi al-'ab`ad min al-'ar.d, wa-_dalika
\aemph{sj kh}. fa-'i_dA t.hrk al-mA'il rb` dA'iraT, wa-t.hrk fI _dalika
al-zamAn al-.hAmil rb` dA'iraT 'ay.d"aN, wa-t.hrk al-mudIr fI _dalika
al-zamAn\fol{.z 34 \md} ni.sf dA'iraT, .sAr b`d markaz al-tadwIr min
markaz al-.hAmil sittaT 'ajzA' wa-ni.sf wa-_tl_t.

\clearpage

fa-'i_dA 'a_hrjnA \VAR{_ha.t.t"aN mustaqIm"aN}{_ha.t.t mustaqIm [\ma]}
min markaz al-`Alam 'il_A markaz al-tadwIr, wa-'a_hrjnA
\VAR{_ha.t.t"aN}{_ha.t.t [\ma]} 'A_har min markaz al-`Alam 'il_A markaz
al-.hAmil, kAnat \VAR{al-zAwiyaT}{al-zAwAyaT [\mc]} allatI bayna
ha_dayna al-_ha.t.tayn hiya zAwiyaT \textbf{ta`dIl z.hl al-'awwal}
wa-biha_dA al-miqdAr yakUn \textbf{ta`dIl al-_hA.s.saT}.

wa-ytt.d.h _dalika bi-al-mi_tAl. fa-'i_dA t.hrk al-mA'il ni.sf dA'iraT,
wa-t.hrk al-.hAmil ni.sf dA'iraT 'ay.daN, wa-t.hrk al-mudIr fI _dalika
al-zamAn dA'iraT tAmmaT, .sAr markaz al-tadwIr fI ba`dh al-'aqrab min
markaz al-`Alam, wa-_dalika \aemph{nw lh}, wa-.tAbq al-_ha.t.t al-_hArij
min markaz al-`Alam 'il_A markaz al-tadwIr lil-_ha.t.t al-_hArij minh
'il_A markaz al-.hAmil; fa-in`dama al-ta`dIl al-'awwal alla_dI hwa
ta`dIl al-markaz wa-ta`dIl al-_hA.s.saT.

wa-lammA wajadtu al-^sams tqArn z.hl fI wasa.t istiqAmatihi wa-tqAblh
fI wasa.t rujU`h, `lm 'anna .harakaT falak al-tadwIr biqdr fa.dl
.harakaT wasa.t al-^sams `l_A wasa.t z.hl. famin hunA `lmnA 'annA 'i_dA
'asq.tnA wasa.t z.hl min wasa.t al-^sams\fol{w 22 \mc\\w 20 \ma}
baq_A .harakaT _hA.saT z.hl. wa-`al_A _dalika al-ma^starI wa-al-mrrI_h.

wa-'i_d tqdm _dalika, fa-i`lam 'annahu ylzm `n ha_dihi al-'aflAk
wa-ha_dihi al-.harakAt i_htilAfAt
wa-tasmm_A \textbf{\VAR{al-ta`AdIl}{al-ta`dIl [\md]}}. fa-al-ta`dIl
al-'awwal ysmm_A ta`dIl al-markaz wa-al-_hA.s.saT. wa-hwa zAwiyaT `nd
markaz al-`Alam (alla_dI hwa markaz al-mA'il) bayna _ha.t.tayn
ya_hrujAni minh, fa-yamurru 'a.haduhumA bi-markaz al-.hAmil wa-yamurru
al-'A_har bi-markaz al-tadwIr. wa-ha_dihi al-zAwiyaT musAwiyaT
lil-zAwiyaT allatI `nda markaz al-tadwIr bayna _ha.t.tayn ya_hrujAni
minhi, yamurru 'a.haduhumA bimarkaz al-`Alam,
wa-al-'A_har \VAR{mwAziy}{mwAz"iN [\md,\mc]} lil-_ha.t.t al-_hArij min
markaz al-`Alam al-mArr bi-markaz al-.hAmil. wa-mA bayna .trfay
ha_dayna al-_ha.t.tayn min al-tadwIr, hwa mA bayna \VAR{al-_dirwatayn
al-.haqIqiyyaT}{al-zAwiyatayn al-.haqIqaT [\md,\mc]} wa-al-mar'iyyaT.
fa-tubayinu 'anna ta`dIl al-_hA.s.saT
musAw"iN li-ta`dIl al-markaz li-tasAwiy al-zAwiyatayn. wa-hwa y.zhr min
al-mi_tAl wA.di.h"aN. wa-yn`dm h_dA al-ta`dIl fI al-'awj
wa-al-.ha.dI.d. wa-hwa yazAdu `l_A al-markaz wa-ynq.s min al-_hA.s.saT
'i_dA kAna al-markaz 'ak_tar min sitt burUj; wa-ynq.s min al-markaz
wa-yazAdu `l_A al-_hA.s.saT 'i_dA kAna al-markaz 'aqall min sitt burUj.
wa-nihAyatuhu li-z.hl sittaT 'ajzA' wa-_tl_t wa-_hms, wa-_dlika `nda
kawn ba`d markaz al-.hAmil min al-'awj fI al-jihatayn _talA_t burUj
wa-'arba` drj.

\textbf{\VAR{wa-al-ta`dIl}{wa-'ammA al-ta`dIl [\mc]} al-_tAniy} wa-hwa
alla_dI bi-sabab falak al-tadwIr.

\clearpage
\noindent wa-hwa zAwiyaT `inda markaz al-`Alam bayna _ha.t.tayn ya_hrujAni
minh: yamurru 'a.haduhumA bi-markaz al-tadwIr wa-al-'A_har bi-al-kawkab.
wa-nihAyatuhu \VAR{`inda}{nAqi.saT [\ma]} mumAssaT al-_ha.t.t lil-tadwIr.
wa-yn`adimu fI al-_dirwaT wa-al-.ha.dI.d min al-tadwIr al-mar'iyyatayn.
wa-nihAyatuhu fI z.hl sittaT 'ajzA' wa-_tl_t `a^saraT daqIqaT.
wa-yazAdu `l_A al-wasa.t 'i_dA kAnat al-_hA.s.saT al-mu`addlaT 'aqall
min sitt burUj, wa-yanq.s minh 'i_dA kAnat \VAR{'ak_tarh}{'ak_tar [\md,\mc]}.

\textbf{wa-al-ta`dIl al-_tAli_t} hwa i_htilAf \VAR{al-_tAniy}{_tAniy [\mc]}.
fa-'inna al-_tAniy ya_htalifu bi-.husb qrb markaz al-tadwIr min markaz
al-`Alam wa-ba`dh minh. wa-hwa lAzim lil-_tAniy fI al-ziyAdaT
wa-al-nq.sAn.

\textbf{\VAR{wa-daqA'iq}{wa-'ammA daqA'iq [\mc]} al-nisb} \VAR{hwa}{fa-hwa [\mc]}
`adad nisbath 'il_A sittIn kanisbaT mA yalzimu min al-i_htilAf
al-_tAli_t 'il_A jumlaT _dalika al-i_htilAf. wa-yatt.d.h _dalika fI
.hisAb ha_dihi al-ta`AdIl.

\begin{center}
\large fa.sl\fol{.z 22 \mc}
\end{center}
wa-'i_d tqdm _dalika, fa-i`lam 'anna \textbf{\VAR{'awj
al-kawkab}{al-'awj [\mc]}} qaws min \VAR{dA'iraT al-falak}{nAqi.saT
[\ma,\md]} al-mA'il bayna _ha.t.tayn ya_hrujAni min markazihi: yamurru
'a.haduhumA bi-al-i`tidAl al-rabI`iyy, wa-yamurru al-'A_har bi-markaz
al-.hAmil wa-markaz al-mudIr wa-markaz al-tadwIr\fol{w 23 \mc} 'i_dA
kAna markaz al-tadwIr fI al-ba`d al-'ab`ad min markaz
al-mA'il. fa-'inna ha_dihi al-marAkiz al-_tlA_taT \VAR{yjtm`}{tjtm`
[\md]} `l_A _ha.t.t"iN wA.hid fI al-'awj wa-al-.ha.dI.d; wa-'anA\fol{w
35 \md} 'asm_A al-'awj al-ba`d al-'ab`ad.

\textbf{wa-markaz al-kawkab}\fol{.z 20 \ma} qaws min al-mA'il bayna
_ha.t.tayn ya_hrujAni min markazihi fa-yamurru: 'a.haduhumA bi-al-'awj
wa-al-'A_har bi-markaz al-.hAmil.

\textbf{wa-wasa.t al-kawkab} hwa majmU` al-'awj wa-al-markaz wa-hwa qaws
min al-mA'il bayna _ha.t.tayn ya_hrujAni min markazihi: fa-yamurru
'a.haduhumA bi-'awwal al-.haml, wa-yamurru al-'A_har bi-markaz
al-.hAmil.

\textbf{\VAR{wa-_hA.s.saT al-kawkab}{wa-al-_hA.s.saT [\mc]}} qaws min
falak al-tadwIr bayna al-kawkab wa-al-_dirwaT al-.haqIqiyyaT `l_A
al-tawAlI.

\textbf{wa-al-mu`addlaT} qaws minhi bayna al-kawkab wa-al-_dirwaT
al-mar'iyyaT `l_A al-tawAlI.

\textbf{wa-al-_dirwaT al-mar'iyyaT} minhi, hiya al-nuq.taT allatI yf.slhA
al-_ha.t.t al-mArr bi-markaz al-tadwIr wa-markaz al-mA'il min
\VAR{'a`l_A}{'a`lA [\md,\mc]} al-tadwIr (wa-y.hA_diyhA al-.ha.dI.d
al-mar'iyy).

wa-'i_dA 'a_hrajnA min markaz al-`Alam (alla_dI hwa markaz
\VAR{falak}{fawqa al-s.tr [\ma]} al-burUj) wa-min markaz al-mA'il
_ha.t.t\fol{w 21 \ma\\.z 35 \md} mustaqIm yamurru bi-al-kawkab
wa-ynth_A 'il_A falak al-burUj.

\clearpage
\noindent wa-fara.dnA dA'iraT min
dawA'ir al-`rU.d \VAR{mArr}{mArraT [\md,\mc]} bi.trf
ha_dA al-_ha.t.t, q.t` \VAR{falak}{_dalika [\mc]} al-burUj `l_A
\textbf{mqwm _dalika al-kawkab}; wa-ba`d ha_dA al-taqA.tu` min
'awwal al-.haml \VAR{hwa}{wa-hwa [\md]} mqwm al-kawkab.

wa-ba`d h_dA al-taqA.tu` 'ay.d"aN min al-kawkab min ha_dihi al-dA'iraT
hwa `ar.d al-kawkab. wa-qad 'afradnA `urU.d al-kawAkib fI bAb mfrd
li-yashl ta.sawwurhA.

\VAR{wa-'i_d tqdm _dalika}{nAqi.saT [\mc]}, fa-i`lam 'anna al-wa.d`
al-'awwal fa-hwa madArAt marAkiz al-'ukar al-mujassmaT li-z.hl
li-'ajl al-barAhIn al-hndsyyaT.

wa-'ammA ta.sawwurAthA `l_A 'annahA kurAt, fa-`l_A ha_dihi
\VAR{al-.sUraT}{al-.sUr [\md,\mc]}; \VAR{natawahhamu}{yatawahhamu [\md,\mc]}
falak mu.hI.t \VAR{bi-jumlaT}{t.hmlh [\mc]} 'aflAk z.hl, fI sa.t.h falak
al-burUj wa-`al_A qu.tbayhi, wa-hwa al-muma_t_tal. wa-m.hdbh mumAss
li-mq`r \VAR{al-falak}{nAqi.saT [\md,\mc]} al-_tAmin, wa-mq`r
ha_dA al-falak mumAss li-m.hdb falak z.hl al-mA'il.

wa-mq`r falak z.hl al-mA'il mumAss li-m.hdb falak muma_t_tal al-m^strI,
wa-samk al-falak al-mA'il sittaT wa-`^srUn darjaT wa-_talA_tUn daqIqaT.
wa-s.t.hhu mA'il `n s.t.h falak al-burUj juz'ayn wa-ni.sf.

wa-yatawahhamu kuraT .sa.hI.haTu al-istidAraT ni.sf q.truhA _tal_t
`a^saraT darjaT wa-_tl_t, wa-tusm_A kuraT al-.hAmil.

wa-natawahhamu kuraT _tAniyaT, ni.sf qi.truhA _tamAniyaT 'ajzA'
wa-i_tnA `a^sar daqIqaT wa-ni.sf daqIqaT, .gA'i.saT fI al-falak
al-.hAmil tumAssuhu `l_A nuq.taT"iN. wa-tusm_A falak
\VAR{al-mudIr}{al-tadwIr [\ma,\md,\mc]}.

wa-natawahhamu kuraT _tAli_taT, ni.sf qi.truhA sittaT 'ajzA' wa-ni.sf,
wa-hiya .gA'i.saT fI al-falak al-mudIr mumAssaT lahu `al_A nuq.taT
qibAlahu al-nuq.taT allatI yumAssu `alayhA al-mudIr lil-.hAmil.
wa-yusm_A falak al-tadwIr.

wa-al-kawkab markUz .gA'i.s\fol{.z 23 \mc} fI al-tadwIr tumAssuhu `l_A
al-nuq.taT allatI tuqAbilu al-mumAssaT minhu
lil-mudIr -- \VAR{.hayna}{.hat_A [\md,\mc]} yakUn fI al-'awj.

wa-nufri.du al-.hAmil .gA'i.s fI _ti_han al-falak al-mA'il yumAssuhu
`l_A nuq.taT al-'awj, wa-_Ata.harrak kull falak bi-miqdAr mA fara.dnA
lahu min al-.harakaT wa-al-jihaT. fa-yata.harraku al-muma_t_tal `l_A
qu.tbay al-burUj 'il_A al-tawAlI, mi_tl .harakaT al-'awjAt.
wa-tata.harraku al-mA'il 'il_A al-tawAlI, .harakaT"aN basI.taT .hawla
markazihi, bimiqdAr .harakaT markaz z.hl, wa-hiya fI al-yawm \aemph{0 b
  0 kw _Ar}. 

\clearpage
\noindent wa-_Ata.harraka al-falak al-.hAmil 'il_A _hilAf al-tawAlI
fI 'a`lAh bi-qadr .harakaT markaz z.hl. wa-yata.harraku al-mudIr fI
'a`lAh 'il_A al-tawAlI qadr .da`f .harakaT al-markaz li-z.hl.
wa-tata.harraku falak al-tadwIr .harakaT basI.taT .hawla markazh fI
'a`lAh 'il_A al-tawAlI, bi-miqdAr fa.dl .harakaT _hA.s.saT z.hl `l_A
.harakaT markazihi -- wa-hya al-.harakaT al-basI.taT al-murakkbaT
al-mqddm \VAR{^sr.hhA}{_dkrhA [\mc]}. fa-ta_htalifu 'aw.dA` al-'aflAk,
fa-yr_A lahu .harakaT mu_htalifaT murakkabaT\fol{.z 21 \ma}
min .harakAt basI.taT.

wa-yakUn al-kawkab fI 'ab`ad ba`dh min al-'awj 'i_dA kAna fI _dirwaT
al-tadwIr. wa-yakUn fI 'aqrab qurbihi 'i_dA kAna fI al-.ha.dI.d min
al-tadwIr wa-al-tadwIr fI al-.ha.dI.d min al-.hAmil.
\VAR{wa-yakUn fI ba`dh}{fa-yakUn ba`dh [\md,\mc]}
al-'aws.t fImA bayna al-'awj wa-al-.ha.dI.d.

wa-i`lam 'anna kawkab z.hl lA yantahy 'il_A 'ab`ad b`d 'aflAkihi wa-lA
'il_A 'aqrab qurbihA. fa-'inna 'ab`ad b`d z.hl ts`aT wa-sittUn juz'"aN
wa-_tl_tay juz' wa-rub` juz'; wa-'aqrab qurbh _hamsUn juz'"aN wa-ni.sf
sds juz'; lakin\fol{w 22 \ma} li-'ajl \VAR{tatamAt}{.gayr maqrU' [\ma]}
al-'aflAk .hatt_A ta.sIr kurAt y.hI.t ba`.dhA bi-ba`.d, yakUn 'ab`ad ba`d
mA'il z.hl bi-qadr ni.sf q.tr al-mA'il wa-ni.sf q.tr al-.hAmil, wa-_dlika
_talA_taT wa-sb`Un juz'"aN wa-_tl_t juz'. ykUn fawqa _dlika sumk kuraT
al-muma_t_tal; wl-yafra.du _tl_tay juz', yabla.gu 'arba`aT wa-sab`In
juz'"aN. wa-yakUn 'aqrab qurb mq`r mA'il z.hl sittaT wa-'arba`In
juz'"aN wa-_tl_tay juz'; wa-y.htAj\fol{w 36 \md} 'il_A ni.sf q.tr
al-kawkab ma`a 'a_hlA.t al-falak fa-yakUn sittaT wa-'arba`In
juz'"aN.

fa-i`raf _dalika, wa-qs `layhi .gayrihi min al-kawAkib. wa-h_dA min
al-tawahhumAt al-.sa.hI.haT al-sAlimaT min al-^sukUk; fa-'innahA kurAt
.sa.hI.haT, wa-.harakAthA basI.taT kull minhA mustawiyaT `inda markaz
_dalika al-falak al-mt.hrk yq.t` fI al-'azmAn al-mutasAwiyaT qs_A
mtsAwiyaT. fa-al-.hmd lillah alla_dI hdAnA li-h_dA wa-`lmnAh.
\end{arab}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\footnotesize\input{saturne.pdf_tex}
\end{minipage}
\textarab{.sUraT 'aflAk z.hl `l_A mA _Ar_A fI al-basI.t w hya mnA.tq
  madArAt marAkiz al-'aflAk al-mujassmaT 'aw s.t.h tilka al-mnA.tq
  lishUlaT al-ta.sawwur w 'iqAmaT al-barAhIn}
\end{figure}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\footnotesize\input{saturne_orbes.pdf_tex}
\end{minipage}
\textarab{.sUraT 'aflAk z.hl `l_A 'annahA kurAt tAmmaT `l_A .hsb mA
  yata.swwar `l_A al-basI.t fI al-'awj w al-.ha.dI.d w fI al-b`dayn
  al-'awsa.tayn}
\end{figure}

\begin{arab}
\resetlinenumber\pagewiselinenumbers
\clearpage
\begin{center}
\Large al-bAb al-_tAli_t `a^sar\fol{w 24 \mc}

\large fI .dab.t .harakAt z.hl wa-taqyIdhA lil-ta'rI_h al-mutaqaddm
\end{center}
.hararnA bi-al-ra.sad 'anna wsa.t z.hl, li-ni.sf nahAr yawm al-_tl_tA
'awwal sanaT 'i.hd_A wa-sab`mi'aT li-yzdjrd, \aemph{h r n.h k},
wa-'awjuhu fI _dalika al-waqt
\VAR{\aemph{.h _Ad _Ab}}{\aemph{.h _Ad nb} [\md]}.\fol{.z 24 \mc}
wa-.harakaT al-wsa.t fI `i^srIn sanaT fArisiyyaT \aemph{.h d lj k};
wa-.harakatuhu fI sanaT fArisiyyaT \aemph{0 _Ab _Aj m},
wa-fI _tala_tIn yawm"aN
\VAR{\aemph{0 A 0 _A.h .t _Ah _Aj kw}}{\aemph{0 A 0 _A.h d lh n.h l} [\mc]},
wa-.harakaT wsa.th fI yawm
\VAR{\aemph{0 0 b 0 lw .t _AA mw n nr lb}}{\aemph{0 0 b 0 lw .t _AA mw} [\mc]},
wa-fI sA`aT \aemph{0 0 0 h A l kh}.

wa-.harakaT _hA.s.saT kull kawkab"iN hya fa.dl .harakaT wasa.t
al-^sams\fol{.z 36 \md} `l_A .harakaT \VAR{wasa.t}{nAqi.saT [\md,\mc]}
_dalika al-kawkab, wa-.harakaT markazihi hya fa.dl .harakaT
wasa.tihi `l_A .harakAt al-'awjAt (wa-miqdArhA fI kull sittIn sanaT
darjaT); fa-takUn .harakaT _hA.s.saT \VAR{fI}{nAqi.saT [\ma,\md]} yawm
\VAR{\aemph{0 nz z _Aj ld kA _Ah h}}{\aemph{0 nz _A.h lr kA _Ah h} [\md],
\aemph{0 nz z m.h ld kA nh} [\mc]}, wa-.harakaT markazihi fI yawm
\aemph{0 b 0 kw _Ar}. wa-al-ll_ah 'a`lam.

\clearpage
\begin{center}
\Large al-bAb al-rAbi` `a^sar

\large fI m`rfaT taqwIm z.hl
\end{center}
a.hsab wasa.tahu wa-'awjahu wa-wasa.t al-^sams lil-ta'rI_h \VAR{alla_dI
turId}{al-m.tlUb [\mc]}, _tumma usqu.t wasa.tahu min wasa.t al-^sams,
tabqiy _hA.s.satuhu, _tumma usqu.t \VAR{al-'awj}{'awjh [\mc]} min
wasa.tihi, ybqiy markazh. _tumma ud_hul bimarkaz z.hl 'il_A jadwal
ta`AdIl z.hl, wa-_hu_d bihi al-ta`dIl al-'awwal. fa-'in kAna markaz
z.hl 'aqall min sitt burUj, fa-nqu.s al-ta`dIl min al-wasa.t wa-al-markaz,
wa-zdh `l_A al-_hA.s.saT, \VARX{wa-'in kAna al-markaz 'ak_tar}{min sitt brUj
fa-zad al-ta`dIl `al_A al-wasa.t wa-al-markaz wa-nq.sh}{min
al-_hA.s.saT}{nAqi.saT [\ma,\mc]} \VARX{wa-yabqiy}{al-wasa.t al-m`ddal
wa-al-markaz al-m`ddal wa-al-_hA.s.saT}{al-m`ddalaT}{nAqi.saT [\ma]}.
_tumma ud_hul bi-al-markaz al-m`ddl fI jadwl ta`AdIl z.hl, wa-_hu_d bihi
daqA'iq al-nsb, wa-i`raf 'a hya zA'idaT \VAR{'aw}{'am [\mc]} nAqi.saT,
wa-a.hf.zhA. _tumma ud_hul bi-al-_hA.s.saT al-mu`addlaT
'il_A\fol{.z 22 \ma} jadwal ta`dIl z.hl, wa-_hu_d
bihA al-ta`dIl al-_tAli_t wa-al-rAbi` 'in kAnat daqA'iq al-nisb
zA'idaT -- wa-'in kAnat nAqi.saT fa-_hu_d al-_tAniy wa-al-_tAli_t.
_tumma u.drub al-_tAniy 'aw al-rAbi` fI daqA'iq al-nisb, fa-mA
.h.sala zdh `al_A al-ta`dIl al-_tAli_t 'in kAnat daqA'iq al-nisb
zA'idaT -- wa-unqu.shu min al-_tAli_t 'in kAnat daqA'iq al-nisb
nAqi.saT. yabqiy al-_tAli_t al-mu.hakkm; fa-zdh `al_A al-wasa.t
al-mu`addl 'in kAnat al-_hA.s.saT al-mu`addlaT 'ak_tar min sitt burUj,
\VARX{wa-'in kAnat}{al-_hA.s.saT al-m`ddalaT 'aqall min sitt burUj
fa-nq.sh min al-wasa.t al-m`ddal fa-mA bala.ga 'aw baq_A
fa-hwa}{mqwm z.hl}{y.h.sl mqwm al-kawkab [\ma], wa-'in kAnat al-_hA.s.saT
al-m`ddalaT 'aqall min sitt burUj fa-nq.sh y.h.sl mqwm al-kawkab [\md]}
min falak al-burUj fI al-ta'rI_h alla_dI .hasabta lahu.
fa-i`raf _dalika.

\clearpage
\begin{center}
\Large al-bAb al-_hAmis `a^sar

\large fI hI'aT 'aflAk al-mu^stariy al-mubtakaraT
\end{center}
\VAR{hI'aT}{a`lam anna hI'aT [\mc]} 'aflAk al-mu^stariy `l_A
\VAR{wa.d`i hI'aT}{hI'aT wa.d`i [\mc]} 'aflAk zu.hal
al-mutaqaddamaT, \VAR{siw_A}{siwA [\ma,\md,\mc]} wa-'innamA
\VAR{tu_hAlifuhA fI}{yu_hAlifuhA min [\md,\mc]}
maqAdIr al-'aflAk wa-al-.harakAt.

\VAR{natawahhamu}{yatawahham [\md,\mc]} min 'aflAk al-mu^stariy:

-- falak fI sa.t.h falak al-burUj
wa-`al_A qu.tbayhi wa-markazihi, wa-yusamm_A al-muma_t_tal,

-- wa-natawahhamu falak _tAn"iN, sa.t.huhu mA'il `an sa.t.h al-muma_t_tal
mIl\fol{w 25 \mc} _tAbit, wa-miqdAr ha_dA al-mIl juz' wa-ni.sf, wa-tuqA.ti`u
al-muma_t_tal `al_A nuq.tatayn mutaqAbilatayn tusamm_A 'i.hdAhumA
al-ra's wa-al-'u_hr_A al-_danb,

-- wa-natawahhamu falak _tAli_t markazhu `al_A mu.hI.t al-mA'il wa-ni.sf
qi.trhu 'arba`aT 'ajzA' wa-_tumn juz' (bi-al-'ajzA' allatI bihA ni.sf
qi.tr \VAR{al-mA'il}{al-muma_t_tal [\mc]} sittUn juz'"aN),
wa-yusamm_A al-.hAmil,

-- wa-natawahhamu falak rAbi` markazhu `al_A mu.hI.t al-.hAmil wa-ni.sf
qi.trhu juz'"aN wa-'i_tnayn wa-`i^srIn daqIqaT
\VAR{wa-ni.sf daqIqaT}{nAqi.saT [\mc]}, wa-yusamm_A al-mudIr,

-- wa-natawahhamu falak _hAmis markazhu `al_A mu.hI.t al-mudIr wa-ni.sf
qi.trhu \VAR{'a.hada `a^sar}{i.hd_A `a^sar [\ma]} juz'"aN wa-ni.sf
juz' (bi-tilka al-'ajzA'), wa-yusamm_A falak al-tadwIr,

-- \VAR{wa-natawahhamu}{wa-yfr.d [\mc]} markaz jarim al-mu^stariy
markUz `al_A min.taqaT al-tadwIr.

wa-nufri.du marAkiz al-.hAmil wa-al-mudIr wa-al-tadwIr wa-al-kawkab
`al_A al-_ha.t.t al-mustaqIm al-_hArij min markaz al-muma_t_tal 'il_A
al-'awj. wa-nufri.du al-muma_t_tal muta.harrak .harakaT basI.taT `al_A
qu.tbayhi, 'il_A al-tawAlI, mi_tl .harakaT al-'awjAt: wa-hiya fI al-yawm
bi-laylatihi \aemph{0 0 0 .t nb}. wa-yantaqilu bi-ha_dihi al-.harakaT
al-ra's wa-al-_danb wa-.gAyatA al-mIl. wa-yata.harrak al-falak al-mA'il
.harakaT basI.taT .hawla markazihi (alla_dI hwa markaz al-muma_t_tal),
'il_A al-tawAlI, mi_tl .harakaT markaz al-mu^stariy, wa-hwa fa.dl
wasa.tihi `al_A .harakaT al-'awj: wa-hwa fI
\VAR{al-yawm}{al-yawm bi-laylatihi [\mc]} \aemph{0 d n.t w _Ad lh}
wa-yata.harrak al-.hAmil, 'il_A _hilAf al-tawAlI fI 'a`lAh,
bi-qadr .harakaT markaz al-mu^stariy 'ay.d"aN allatI hiya fI al-yawm
bi-laylatihi \aemph{0 d n.t w _Ad lh}. wa-yata.harrak\fol{w 23 \ma}
al-mudIr, fI 'a`lAh 'il_A al-tawAlI, qadr .da`f .harakaT markaz
al-mu^stariy: wa-hwa fI al-yawm bi-laylatihi \aemph{0 .t n.h _Ab k.t y}.

\clearpage
\noindent wa-yata.harrak falak al-tadwIr .hawla markazihi, fI 'a`lAh
'il_A al-tawAlI, bi-miqdAr
fa.dl .harakaT _hA.s.saT al-mu^stariy `al_A .harakaT markazihi:
wa-miqdArh fI al-yawm bilaylatihi \aemph{0 m.t .t nr kb kd y}. wa-hiya
al-.harakaT al-basI.taT al-murakkabaT, fa-yufAriqu al-kawkab al-_dirwaT
al-wus.t_A kull yawm bi-qadr .harakaT _hA.s.saT al-mu^stariy
\VAR{alla_dI}{allatI [\md,\mc]}
hiya \aemph{0 nd .t j lw n.t y}, `l_A mA ^sara.hnA fI 'aflAk zu.hal.

fa-'i_dA istamarrat al-'aflAk tata.harraka bi-ha_dihi al-.harakAt
'il_A tilka al-jihAt, \VAR{tuwakkadu}{twld [\md,\mc]} lil-kawkab
.harakaT"uN mu_htalifaT murakkabaT\fol{w 37 \md} min basA'i.t.

wa-'ammA\fol{.z 25 \mc} al-i.s.tlA.hAt wa-al-natA'ij fa-`al_A mA
'aw.da.hnA fI hI'aT 'aflAk zu.hal.

wa-n.swr hI'aT 'aflAk al-mu^stariy muqta.srIn `al_A al-dawA'ir `al_A
.husb mA yaqa` `al_A al-basI.t \VAR{`al_A mA .sawarnA bi-'aflAk}{`al_A mA
.sawarnA bi-al-'aflAk [\ma], `al_A .swrnA 'aflAk [\md,\mc]} zu.hal;
_tumma na.swrhA `al_A 'annahA akr mujassamaT `al_A mA tUhimuhu fI
al-falak.

wa-na_dkuru maqAdIrhA wa-'ab`AdhA. wa-i`lam 'anna al-_ha.t.t al-_hArij
min markaz al-`Alam 'il_A markaz al-.hAmil yamurru bi-wasa.t al-kawkab.
wa-al-_hArij minh al-mArr bi-markaz al-tadwIr \VAR{ymurru min al-burUj
bi-markaz al-kawkab al-mu`addal}{ymurru min al-burUj al-m`addal [\md],
ymurru bi-markaz al-burUj [\mc]}, wa-yf.sl min al-tadwIr
_hA.s.saT\fol{w 26 \mc}
al-kawkab al-mu`addalaT. wa-al-_ha.t.t al-_hArij min markaz al-`Alam
al-mArr bi-al-kawkab yamurru min falak al-burUj bi-muqawwm al-kawkab
'in lam yakun lil-kawkab\fol{.z 37 \md} `ar.d; fa-'in kAna lahu `ar.d
fa-al-dawA'ir
allatI tamurru bi-qu.tbay al-burUj wa-'a.trAf al-_hu.tw.t
\VAR{al-ma_dkUraT}{al-markUzaT [\ma,\md,\mc]} tf.sl min al-burUj al-wasa.t
wa-al-markaz wa-al-muqawwm, `al_A mA tuqarrir.

wa-'i_d\fol{w 24 \ma\\.z 26 \mc} tqdm _dalika, fa-i`lam 'anna 'ab`ad
bu`d kawkab al-mu^stariy
`an markaz al-`Alam 'arba`aT wa-sab`In juz'"aN wa-rub` juz', wa-'aqrab
qurbh _hamsaT wa-'arba`Un juz'"aN wa-ni.sf wa-rub` juz'; wa-'ab`ad bu`d
markaz al-tadwIr min markaz al-`Alam \aemph{sb mh}, wa-'aqrab qurbh
\aemph{nr _Ah}; 'illA 'anna al-mu^stariy lA ya.silu 'il_A 'ab`ad bu`d
'aflAkihi al-mujassamaT, wa-lA 'aqrab qurbhA.

\clearpage

`al_A ha_dihi, wa-'ammA 'aqdAr ha_dihi al-'aflAk al-mujassamaT, fa-`al_A
mA 'a.sf, \VAR{ni.sf}{fa-ni.sf [\mc]} q.tr kuraT al-.hAmil sab`aT
`a^sar juz'"aN, wa-ni.sf
qi.tr kuraT al-mudIr 'i_tnay `a^sar wa-'i_tnayn wa-_hamsIn daqIqaT
wa-ni.sf daqIqaT, wa-ni.sf qi.tr kuraT al-tadwIr
\VAR{'i.hd_A `a^sar}{i_tnA `a^sar [\md]}\fol{w 38 \md}
juz'"aN wa-ni.sf juz', wa-ni.sf qi.tr al-mA'il sab`aT wa-sab`In,
wa-m.hdbh yamAssu mq`r al-muma_t_tal min 'aflAkihi, wa-sumk
al-muma_t_tal yumkin 'an nufri.d mA ^si'nA wa-nufri.duhu darjaT.
wa-'aqrab qurb al-mA'il _talA_taT wa-'arba`Un, wa-'aqall min _dalika
bi-miqdAr ni.sf qi.tr kuraT al-kawkab ma`a itti.sAl al-falak, kamA
qulnA, wa-nufri.duhu \VAR{darjaT}{darjaT wA.hidaT [\mc]}.
\end{arab}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\footnotesize\input{jupiter.pdf_tex}
\end{minipage}
\textarab{.sUraT 'aflAk al-mu^stariy wa-hiya madArAt marAkiz al-'akrr
  al-mujassmaT `al_A .husba mA yata.sawwaru `al_A al-basI.t fI al-'awj
  wa-al-.ha.dI.d wa-al-ba`dayn al-'awsa.tayn}
\end{figure}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\footnotesize\input{jupiter_orbes.pdf_tex}
\end{minipage}
\textarab{hI'aT 'aflAk al-mu^stariy al-mujassamaT `l_A 'annahA kurAt
  tAmmaT `al_A .husba mA t^skl `al_A al-basI.t fI al-'awj
  wa-al-.ha.dI.d wa-al-bu`dayn al-'awsa.tayn}
\end{figure}

\begin{arab}
\resetlinenumber\pagewiselinenumbers
\clearpage
\begin{center}
\Large al-bAb al-sAdis `a^sar

\large fI .dabt .harakAt al-mu^stariy 
\end{center}
wa-taqyIdhA, lil-ta'rI_h al-ma_dkUr alla_dI hwa
\VAR{ni.sf nahAr yawm}{nahAr [\mc]}
al-_tl_tA 'awwal sanaT 'a.had wa-sab`a-mi'aT li-yazdajard,
'ammA wasa.th \aemph{.t b w y} wa-'ammA 'awjh \aemph{w 0 nb}.
wa-.harakaT wasa.tihi fI `i^srIn sanaT fArisiyyaT \aemph{.h w nA 0},
wa-fI sanaT \aemph{A 0 k lj}, wa-fI ^sahr fArisiyy
\aemph{0 b k.t l.h j _Ar _Aw}, wa-fI yawm \aemph{0 d n.t _Aw w ld lb},
wa-fI sA`aT
\VAR{\aemph{0 0 yb k.h y yw kw k}}{\aemph{0 0 0 b l.h y _Aw lw k}
  [\ma,\md], .gayr maqrU' [\mc]}.

wa-.harakaT al-'awjAt fI kull sittIn sanaT darjaT wa-.harakaT
al-markaz hiya fa.dl .harakaT al-wasa.t `al_A al-'awj. wa-.harakaT
al-_hA.s.saT hiya, lil-`alwiyaT, fa.dl .harakaT wasa.t al-^sams `al_A
wasa.t _dalika al-kawkab; wa-hiya lil-mu^stariy, fI al-yawm bi-laylatihi,
\aemph{0 nd .t j lw n.t y}. wa-taqwIm al-mu^stariy `al_A .tarIq taqwIm
zu.hal.

\clearpage
\begin{center}
\Large al-bAb al-sAbi` `a^sar

\large fI hI'aT 'aflAk al-mirrI_h `al_A \VAR{w.sfnA}{w.d`nA [\md,\mc]}
wa-nub_d"aN bi-al-dawA'ir allatI hiya madArAt marAkiz al-'ukr
al-mujassamaT
\end{center}
-- fa-natawahhamu falak"aN muma_t_tal"aN li-falak al-burUj `al_A
qu.tbayhi wa-fI sa.t.hihi.

-- wa-natawahhamu falak"aN _tAniy"aN sa.t.huhu
mA'il `an sa.t.h al-muma_t_tal juz'"aN wA.hid"aN muqA.ti` lahu `al_A
nuq.tatayn mutaqAbilatayn tusamm_A 'i.hdAhumA al-ra's wa-al-'u_hr_A
al-_danb.

-- wa-natawahhamu falak"aN _tAli_t"aN markazuhu `al_A mu.hI.t al-mA'il
wa-ni.sf qi.trihi tis`aT\fol{.z 24 \ma} 'ajzA' (bi-al-'ajzA' allatI
bihA ni.sf q.tr \VAR{al-mA'il}{al-muma_t_tal [\mc]} sittIn juz'"aN);
wa-yusamm_A al-.hAmil.

-- wa-natawahhamu falak"aN rAbi`"aN markazuhu `al_A mu.hI.t al-.hAmil
wa-ni.sf qi.trihi _talA_taT 'ajzA'; wa-yusamm_A al-mudIr.

-- wa-natawahhamu falak"aN _hAmis"aN markazuhu\fol{w 27 \mc} `al_A
mu.hI.t al-mudIr wa-ni.sf qi.trihi tis`aT wa-_talA_tUna juz'"aN
wa-ni.sf juz' (bi-tilka al-'ajzA'); wa-\VAR{yusamm_A}{yusamA [\ma]}
falak al-tadwIr.

-- wa-markaz al-kawkab `al_A mu.hI.t \VAR{falak}{nAqi.saT [\mc]} al-tadwIr.

wa-nufri.du markaz al-.hAmil wa-al-mudIr wa-al-tadwIr fI al-'awj, 'a`nI
`al_A al-_ha.t.t al-_hArij min markaz al-`Alam 'il_A al-'awj.
wa-nufri.du al-muma_t_tal muta.harrak .harakaT basI.taT .hawla
markazihi wa-`l_A qu.tbay al-burUj, 'il_A al-tawAlI, mi_tl .harakaT
al-'awjAt: wa-hiya fI al-yawm bilaylatihi \aemph{0 0 0 .t nb}.
fa-yantaqilu bi-ha_dihi al-.harakaT al-ra's wa-al-_danb wa-.gAyatA
al-mIl. wa-yata.harrak \VAR{al-falak}{al-falak al-falak [\ma]}
al-mA'il 'il_A al-tawAlI, .harakaT basI.taT .hawla markazihi, mi_tl
.harakaT markaz al-mirrI_h: wa-hiya fI al-yawm bi-laylatihi \aemph{0 0
  lA kw k.t mh}. wa-yata.harrak al-.hAmil, 'il_A _hilAf al-tawAlI,
bi-qadr .harakaT markaz al-mirrI_h. wa-yata.harrak al-mudIr, fI 'a`lAhi
'il_A al-tawAlI, bi-qadr \VAR{.da`f}{fa.dl .da`f [\ma]} .harakaT markaz
al-mirrI_h: wa-hiya fI al-yawm bi-laylatihi \aemph{0 A b nb n.t
  l}. wa-yata.harrak falak al-tadwIr .hawla markazihi .harakaT
basI.taT, fI 'a`lAh 'il_A _hilAf al-tawAlI, biqadr fa.dl .harakaT markaz
al-mirrI_h `al_A .harakaT _hA.s.satihi.

\clearpage
\noindent fa-y.zhr 'anna falak al-tadwIr
muta.harrak"aN 'il_A al-tawAlI fI 'a`lAhi bi-qadr .harakaT _hA.s.saT
al-mirrI_h, allatI hiya fI \VAR{al-yawm}{al-yawm bi-laylatihi [\mc]}
\aemph{0 kz mA n}; li-'annahu yadUru bi.harakaT al-mudIr wa-bi-.harakatihi,
hwa .hawla \VAR{markazihi}{markaz al-`Alam [\mc]} fI al-yawm
bi-laylatihi \aemph{0 j md m}, fa-yabqiy ha_dA al-miqdAr nAqi.s"aN min
.harakaT markazihi fI yawm (wa-hwa \aemph{0 lA kw k.t mh}); fa-yabqI
\aemph{0 kz mA n} wa-hiya .harakaT al-kawkab al-mar'iyy bi-al-tadwIr,
'il_A al-tawAlI, wa-hiya mi_tl .harakaT _hA.s.saT al-mirrI_h, 'a`nI
fa.dl .harakaT wasa.t al-^sams `al_A .harakaT wasa.tihi. wa-hiya
al-.harkaT al-basI.taT al-murakkabaT
\VAR{al-mutaqaddam}{al-mqdm [\mc]} _dikrhA.

wa-y.zhr fI al-mi_tAl; fa-'i_dA fara.dnA marAkiz al-.hAmil wa-al-mudIr
wa-al-tadwIr `al_A al-_ha.t.t al-_hArij min markaz
al-burUj \VAR{'il_A}{nAqi.saT [\mc]} al-'awj,
wa-ta.harrak kull falak .harakaT basI.taT .hawla markazihi
bi-miqdAr mA fara.dnA lahu\fol{.z 38 \md} min al-.harakaT wa-al-jihaT.
twld lil-kawkab .harakaT mu_htalifaT,
\VAR{wa-jarrat lahu}{wa-.hd_t lahu [\mc]\iscomplet{, wjd lh [\me]}{}} rujU`
'il_A .gayr (_dalika \VAR{min mA}{mimmA [\md,\mc]} wjd lahu bi-al-ra.sad).
wa-hiya al-mu_htalifaT al-murakkabaT min basA'i.t `al_A
mA 'aw.d.hnA fI \VAR{.gayr maw.du`"iN}{.gayr h_dA al-mw.d` [\mc]}.

wa-ha_dihi .sUraT 'aflAk al-mirrI_h, `al_A 'annahA madArAt marAkiz
al-'ukar al-mujassamaT \VAR{`al_A}{`al_A .hsb [\mc]} mA yata.sawwaru
`al_A al-basI.t \VAR{wa-yashalu tawahhumahA}{fI al-.ha.dI.d wa-al-'awj
wa-al-bu`dayn al-'aws.tayn wa-qad tqdm in.sAf iq.tArihA wa-aw.dA`hA
`al_A mA tqdm fI z.hl wa-.gayrhi ma^srU.h"aN fa-lA .hAjaT il_A i`AdaT
_dalika wa-al-lahu a`lam [\mc]}.

wa-'i_d\fol{.z 27 \mc\\w 25 \ma} tqdm _dalika, fa-i`lam 'anna 'ab`ad bu`d
\VAR{markaz tadwIr al-mirrI_h}{al-mirrI_h ay markaz tadwIrhi [\mc]}
min markaz al-`Alam sittaT wa-sittUn juz'"aN, wa-'aqrab qurb
markaz al-tadwIr min markaz al-`Alam 'arba`aT wa-_hamsUn juz'"aN.
wa-'ab`ad bu`d kawkab al-mirrI_h min markaz al-`Alam mi'aT juz'
wa-_hamsaT 'ajzA' wa-ni.sf juz', wa-'aqrab qurbihi 'arba`aT `a^sar
juz'"aN wa-ni.sf juz' (al-jamI` bi-al-'ajzA' allatI bihA\fol{.z 25 \ma}
ni.sf qi.tr al-mA'il\fol{w 28 \mc} sittUn juz'"aN).

\clearpage
\noindent wa-'inna kawkab al-mirrI_h lA ya.silu 'il_A
'ab`ad bu`d 'aflAkh, wa-lA 'il_A 'aqrab qurbhA; li-'anna ni.sf qi.tr
kuraT al-.hAmil 'a.had wa-_hamsUn juz'"aN
\VAR{wa-ni.sf}{nAqi.saT [\md,\mc]}, wa-ni.sf qi.tr
kuraT al-mudIr 'i_tnayn wa-'arba`Un juz' wa-ni.sf, wa-ni.sf qi.tr
kuraT al-tadwIr tis`aT wa-_talA_tUn juz'"aN wa-ni.sf juz', fa-yakUn
'ab`ad bu`d al-mA'il (wa-hwa ni.sf qi.trh) mi'aT wa-'a.had `a^sar darjaT
wa-ni.sf, wa-sumk al-muma_t_tal fawqa _dalika, wa-nufri.duhu _talA_tIn
daqIqaT, fa-yabqiy 'ab`ad al-bu`d mi'aT juz'-"aN wa-'i_tnA `a^sar
juz'"aN, wa-'aqrab qurbh _tamAniyaT 'ajzA' wa-_talA_tUn daqIqaT,
ma`a itti.sAl al-falak, wa-nufri.duhu _talA_tIn daqIqaT,
fa-tabqiy al-_tamAniyaT. fa-yakUn 'aqrab qurb 'aflAk al-mirrI_h
_tamAniyaT, wa-'ab`ad bu`dhA mi'aT wa-'i_tnA `a^sar juz'"aN. wa-`al_A
_dalika i`tamdnA.

wa-ha_dihi\fol{w 26 \ma\\w 39 \md} .sUraT 'aflAk al-mirrI_h
al-mujassamaT `al_A mA yatawahhamu fI al-falak; wa-hiya kurAt tAmmaT
wa-taqaddm in.sAf iq.tArhA wa-'aw.dA`hA `al_A mA taqaddam ma^srU.h"aN
fI zu.hal wa-.gayrihi, fa-lA .hAjaT 'il_A 'i`AdaT _dalika.
\end{arab}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\footnotesize\input{mars.pdf_tex}
\end{minipage}
\textarab{hI'aT 'aflAk al-mirrI_h wa-hiya madArAt marAkiz al-'akar
  al-mujassamaT `al_A mA yata.sawwaru fI al-basI.t fI al-'awj
  wa-al-.ha.dI.d wa-al-bu`dayn al-'aws.tayn}
\end{figure}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\footnotesize\input{mars_orbes.pdf_tex}
\end{minipage}
\textarab{hI'aT 'aflAk al-mirrI_h al-mujassamaT wa-hiya kurAt tAmmaT
  `al_A mA yata.sawwaru `al_A al-basI.t fI al-'awj wa-al-.ha.dI.d
  wa-al-bu`dayn al-'aws.tayn}
\end{figure}

\begin{arab}
\resetlinenumber\pagewiselinenumbers
\clearpage
\begin{center}
\Large al-bAb al-_tAmina `a^sar

\large fI .dabt .harakAt al-mirrI_h
\end{center}
wa-\VAR{taqyIdhA}{.gayr maqrU' [\ma], bu`dhA [\mc]} li-ni.sf nahAr
\VAR{yawm}{nAqi.saT [\mc]} al-_tl_tA \VAR{'awwal}{nAqi.saT [\md]}
sanaT 'i.hd_A wa-sab`a mi'aT li-yazdjard li-dami^sq, 'ammA
\VAR{wasa.t al-mirrI_h}{wasa.th [\mc]} \aemph{.t kb 0 0},
wa-'awjuhu \aemph{d _Ar _Ab 0}.
wa-.harakaT wasa.tihi fI `i^srIn sanaT fArisiyyaT \aemph{r _Ah mj m};
wa-fI sanaT fArisiyyaT, \aemph{w _AA _Ar _AA 0}; wa-fI _talA_tIn yawm"aN,
\VAR{\aemph{0 _Ah mj _A.t m.h k.t l.t}}{\aemph{0 _Ah mj _A.t m.h .t l.t} [\md]};
wa-fI yawm bi-laylatihi
\VAR{\aemph{0 0 lA kw l.t lw n.t _A.h}}{\aemph{0 0 lA kw l.t lw} [\mc]};
wa-fI sA`aT \aemph{0 0 A _A.h lw l.t}.
wa-.harakaT al-'awjAt fI kull sittIn sanaT darjaT,  wa-hiya fI al-sanaT
daqIqaT wA.hidaT, wa-fI al-yawm \aemph{0 0 0 .t nb}.
wa-.harakaT _hA.s.saT al-mirrI_h
bi-qadr fa.dl .harakaT wasa.t al-^sams `al_A wasa.tihi, wa-hiya fI
\VAR{al-yawm}{al-yawm bi-laylatihi [\mc]}
\VAR{\aemph{0 0 kr mA m r}}{\aemph{0 0 kr mA n r} [\ma,\md]}.
wa-taqwIm al-mirrI_h `al_A na.hw taqwIm zu.hal.

\clearpage
\begin{center}
\Large al-bAb al-tAsi`a `a^sar

\large fI hI'aT 'aflAk al-zuhraT `al_A wa.d`nA \VAR{wa-nub_d}{wa-nub_d"aN
[\md,\md]} bi-al-dawA'ir allatI hiya madArAt al-'ukar al-mujassamaT
\end{center}
fa-natawahhamu:

-- falak"aN muma_t_tal"aN bi-falak al-burUj, fI sa.t.hihi
wa-`al_A qu.tbayhi.

-- wa-natawahhamu falak"aN _tAniy"aN, `al_A markaz al-burUj, wa-sa.t.huhu
mA'il `an sa.t.h al-muma_t_tal suds juz'
\VAR{_tAbit al-mIl}{wa-_tAbit al-mIl [\md], wa-_tAbit al-muma_t_tal [\mc]}
(`al_A 'a.sa.h.h al-qUlIn), \VAR{wa-muqA.ti`}{wa-yuqA.ti` [\md,\mc]}
lahu `al_A nuq.tatayn mutaqAbilatayn tsmm_A
'i.hdAhumA al-ra's wa-al-'u_hr_A al-_danb.

-- wa-natawahhamu falak"aN _tAli_t"aN markazuhu `al_A mu.hI.t al-mA'il,
wa-ni.sf qi.trihi juz'"aN wa-'i.hd_A wa-'arba`In daqIqaT (bi-al-'ajzA'
allatI bihA ni.sf qi.tr al-mA'il sittUn juz'"aN); wa-ysmm_A al-.hAmil.

-- wa-natawahhamu falak"aN rAbi`"aN markazuhu `al_A mu.hI.t al-.hAmil
wa-ni.sf qi.trihi sittaT wa-`i^srUn daqIqaT; wa-ysmm_A al-mudIr.

-- wa-natawahhamu falak"aN _hAmis"aN markazuhu `al_A mu.hI.t al-mudIr
wa-ni.sf qi.trihi, `al_A ra.sadnA, _talA_taT wa-'arba`Un juz'"aN
wa-_talA_taT wa-_talA_tUn daqIqaT (bi-al-'ajzA' al-ma_dkUraT); wa-ysmm_A
falak al-tadwIr.

-- wa-markaz al-kawkab, `al_A mu.hI.t ha_dA al-falak\fol{.z 28 \mc}, lAzim
li-nuq.taT minhi.

wa-nufri.d \VAR{marAkiz}{markaz [\md]} al-.hAmil wa-al-mudIr wa-al-tadwIr
`al_A al-_ha.t.t al-_hArij min markaz al-mA'il 'il_A al-'awj.
wa-nufri.du al-muma_t_tal
muta.harrak `al_A qu.tbayhi 'il_A al-tawAlI mi_tl .harakaT al-'awjAt:
wa-hiya fI al-yawm bi-laylatihi \aemph{0 0 0 .t nb}. fa-yantaqilu
bi-ha_dihi al-.harakaT al-ra's wa-al-_danb wa-.gAyatA al-mIl.
wa-yata.harrak\fol{.z 26 \ma} al-mA'il 'il_A al-tawAlI, mi_tl .harakaT
markaz al-zuhraT allatI hiya mi_tl .harakaT markaz al-^sams: wa-hwa
fI al-yawm bi-laylatihi \aemph{0 n.t .h .t}. wa-yata.harrak al-.hAmil
'il_A _hilAf al-tawAlI, \VAR{bi-miqdAr}{bi-qdr [\md,\mc]} \VARX{.harakaT
markaz}{al-zuhraT; wa-yata.harrak al-mudIr 'il_A
al-tawAlI,}{bi-mqdAr}{nAqi.saT [\ma,\md,\mc]} .da`f .harakaT
markaz al-zuhraT: wa-hwa fI al-yawm
bi-laylatihi \aemph{a n.h _Aw _A.h}.

\clearpage
\noindent wa-yata.harrak falak al-tadwIr
.harakaT basI.taT .hawla markazihi, fI 'a`lAh 'il_A _hilAf al-tawAlI,
bi-qdr fa.dl .harakaT markaz al-zuhraT `al_A _hA.s.satihA: wa-hwa fI
al-yawm bilaylatihi \VAR{\aemph{0 kb .h mA kh lj nj}}{\aemph{kh lj nj}
  fI hAmi^s [\ma]}. fa-y.zhuru \VAR{lahu}{nAqi.saT [\md]}
  \VAR{ta.sIru}{taq.sIrA [\md,\mc]} 'il_A al-tawAlI bi-qadr
\VAR{.harakaT}{fI al-hAmi^s [\ma]} _hA.s.saT al-zuhraT allatI hiya fI
al-yawm bi-laylatihi
\VAR{\aemph{0 lw n.t k.h kw 0} li-'annanA}{\aemph{0 lw n.t l.h kw _Aj d _Aw}
li-'anna [\ma,\md]}, 'i_dA fara.dnA al-tadwIr _tAbit, wa-ta.harrak
al-mA'il wa-al-.hAmil wa-al-mudIr: intaqalat al-_dirwaT 'il_A al-tawAlI,
bi-qadr .harakaT al-markaz. fa-yfri.du lahu .harakaT 'u_hr_A, 'il_A
_hilAf al-tawAlI, bi-qadr .harakaT al-markaz, fa-taradd al-_dirwaT
makAnahA; _tumma 'innah
wujid bi-al-ra.sad muta.harrak, `an al-_dirwaT, 'il_A al-tawAlI, bi-qadr
.harakaT al-_hA.saT. fa-qad tubayyinu 'annA, 'i_dA fara.dnA al-tadwIr
muta.harrak"aN _hilAf al-tawAlI, bi-qadr fa.dl .harakaT al-markaz `l_A
.harakaT al-_hA.saT, baqiyat al-_dirwaT\fol{.z 39 \md} muqa.s.saraT
bi-qadr .harakaT al-_hA.s.saT: wa-ha_dihi hya al-.harakaT al-basI.taT
al-murakkabaT wa-qad taqaddama bayAnuhA.

wa-'i_dA fara.dnA marAkiz al-.hAmil wa-al-mudIr wa-al-tadwIr `al_A
al-_ha.t.t al-_hArij min markaz al-burUj 'il_A al-'awj, wa-ta.harrakat
al-'aflAk bi-miqdAr mA fara.dnA lahA min al-.harakAt 'il_A tilka
al-jihAt, .zahara lil-kawkab .harakaT mu_htalifaT murakkabaT min
basA'i.t, wa-hya al-mawujUdaT bi-al-ra.sad.

\VAR{wa-'i_d}{wa-'i_dA [\mc]} tqdm _dalika, fa-i`lam 'anna 'ab`ad
bu`d markaz tadwIr
al-zuhraT min markaz al-`Alam 'a.had wa-sittUn juz'"aN wa-rub` juz',
wa-'aqrab qurbihi
\VAR{_tamAniyaT wa-_hamsUn juz'"aN wa-ni.sf wa-rub` juz'}{\aemph{n.h
l _Ah} [\mc]}.
wa-'ab`ad bu`d al-zuhraT min markaz al-`Alam mi'aT juz' wa-'arba`aT
'ajzA' \VARX{wa-_tamAniyaT wa-'arba`Un}{daqIqaT, wa-'aqrab qurbh}
{_hamsaT `a^sar juz'"aN}{nAqi.saT [\ma,\md,\mc]}
wa-_hums juz' (wa-al-jamI` bi-al-'ajzA' allatI bihA ni.sf qi.tr
al-mA'il sittUn juz'"aN). 'illA 'anna \VAR{kawkab}{nAqi.saT [\mc]}
al-zuhraT lA \VAR{ya.silu}{ta.silu [\md,\mc]} 'il_A
\VAR{'aqrab qurb}{'aqrab [\ma]} 'aflAkihA, wa-lA 'il_A 'ab`ad bu`d
'aflAkihA, li-'anna ni.sf
qi.tr kuraT al-.hAmil _hamsaT wa-'arba`Una juz'"aN wa-_tul_tA juz'
(wa-ni.sf qi.tr al-mudIr _talA_taT wa-'arba`Un juz'"aN wa-tis`aT
wa-_hamsUn daqIqaT), fa-yakUn\fol{w 29 \mc} 'ab`ad bu`d al-falak al-mA'il,
lil-zuhraT,
mi'aT juz' wa-_hamsaT 'ajzA' wa-_tul_tA juz' wa-fawqahu sumk
al-muma_t_tal wa-nufri.dhu _tul_t juz', wa-'aqrab qurb al-muma_t_tal
'arba`aT `a^sar juz'"aN wa-_tul_t juz' wa-yujib 'an yanqu.su bi-qadr
itti.sAl al-falak wa-layakun _dalika bi-al-far.d _tul_t juz':
fa-.zahara 'anna 'aqrab qurb\fol{w 27 \ma} 'aflAk al-zuhraT 'arba`aT
`a^sar juz'"aN,
wa-'ab`ad bu`d 'aflAkihA mi'aT wa-sittaT 'ajzA' (wa-yumkin 'an yakUn
'ak_tar min _dalik wa-lA yumkin 'an yakUn 'aqall).

\clearpage

\begin{center}
\large tanbIh
\end{center}
'i_dA kAna al-mar.sUd 'an.sAf 'aq.tAr al-madArAt marAkiz
\VAR{al-'ukar}{al-'ukar al-tAmaT [\mc]} (wa-hiya al-dawA'ir
al-mutawahhamaT `al_A al-basI.t), \VAR{wa-'aradta}{wa-'aradnA [\mc]}
.hisAb 'an.sAf 'aq.tAr al-'ukar al-mujassamaT li-_dalik al-kawkab.
fa-.tarIqh: 'an tajma`u ni.sf qi.tr falak al-tadwIr wa-ni.sf
\VAR{qi.tr}{qi.tr falak [\mc]}
al-mudIr fa-mA .ha.sala fa-hwa ni.sf qi.tr kuraT \VARX{al-mudIr, wa-ni.sf
qi.tr}{al-.hAmil famA .ha.sala fa-hwa ni.sf}{qi.tr kuraT}{nAqi.saT [\mc]}
al-.hAmil.
wa-'i_dA zadnA ni.sf qi.tr kuraT al-.hAmil `al_A sittIn, .ha.sala ni.sf
qi.tr m.hdb \VAR{al-mA'il}{al-falak al-mA'il [\mc]} wa-fawqahu
sumk al-muma_t_tal; wa-'i_dA nq.snAhu
min sittIn, wa-nq.snA mimmA yabqI itti.sAl al-falak, .ha.sala ni.sf
qi.tr \VAR{al-mA'il}{al-falak al-mA'il fa-i`lam _dalika [\mc]}.

\VARX{wa-ha_dihi .sifaT}{'aflAk al-zuhraT `al_A 'annahA
madArAt marAkiz al-'ukar}{wa-'aflAk}{wa-ha_dihi 'aflAk [\mc],
'aflAk [\md]} al-zuhraT al-mujassamaT
`al_A .hsb mA yaqa` `al_A al-basI.t wa-hiya manA.tiq al-kurAt
al-tAmmAt.
\end{arab}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\footnotesize\input{venus.pdf_tex}
\end{minipage}
\textarab{hI'aT 'aflAk al-zuhraT `al_A 'annahA madArAt marAkiz
  al-'aflAk al-mujassamaT `al_A mA yata.sawwaru `al_A al-basI.t fI
  al-'awj wa-al-.ha.dI.d wa-al-bu`dayn al-'aws.tayn}
\end{figure}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\footnotesize\input{venus_orbes.pdf_tex}
\end{minipage}
\textarab{hI'aT 'aflAk al-zuhraT al-mujassamaT `al_A mA yatawahhamu fI
  al-falak 'innahA kurAt tAmmaAt `al_A mA yata.sawwaru `al_A al-basI.t
  fI al-'awj wa-al-.ha.dI.d wa-al-bu`dayn al-'aws.tayn}
\end{figure}

\begin{arab}
\resetlinenumber\pagewiselinenumbers
\clearpage
\begin{center}
\Large al-bAb\fol{w 30 \mc\\.z 40 \md\\.z 27 \ma} al-`i^srUn

\large fI .dab.t .harakAt al-zuhraT
\end{center}
wa-taqyIdhA li-ni.sf nahAr yawm al-_tl_tA 'awwal sanaT 'i.hd_A
wa-sab`a-mi'aT \VAR{li-yazdjard}{min ta'rI_h yazdjard [\mc]}
'ammA wasa.t al-zuhraT fa-mi_tl wasa.t al-^sams, wa-hwa lil-ta'rI_h al-ma_dkUr
\aemph{.t y .t 0}, wa-al-'awj lil-ta'rI_h al-ma_dkUr \aemph{b _Ar nb 0}.
wa-.harakaT wasa.tihA mi_tl .harakaT wasa.t al-^sams, wa-hiya fI
`i^srIn sanaT fArisiyaT \aemph{_AA kh _Aj k}, wa-fI sanaT fArisiyaT
\aemph{_AA k.t mh m 0}, wa-fI ^sahr fArisiy
\aemph{0 k.t ld .t nA mw n nr lb}, wa-fI\fol{.z 30 \mc} yawm \aemph{0
  n.t .h _A.t mj lj mA nh d w}, wa-fI sA`aT \aemph{0 b kr n n}.
wa-.hA.sala _hA.saT al-zuhraT, lil-ta'rI_h al-ma_dkUr, \aemph{y k n y.t};
wa-.harakaT al-_hA.saT fI `i^srIn sanaT fArisiyaT \aemph{w 0 lw 0},
wa-fI sanaT fArisiyaT\fol{w 28 \ma} \aemph{r _Ah A m.h mA}, wa-fI
^sahr \aemph{0 _A.h k.t md nj .t}, wa-fI yawm \aemph{0 lw n.t k.h
kw _Aj d _Aw}, wa-fI sA`aT \aemph{0 0 A lb k.h mA w}.
wa-taqwImuhA `al_A \VAR{.tarIq}{nAqi.saT [\mc]} taqwIm
zu.hal wa-.gayrihi min al-sayAraT.

\clearpage
\begin{center}
\Large al-bAb al-.hAdI wa-al-`i^srUn

\large fI hI'aT 'aflAk `.tArd `al_A m_dhbnA al-muwAfiq lil-ra.sad
\end{center}
-- natawahhamu falak"aN fI sa.t.h falak al-burUj wa-`al_A qu.tbayhi
wa-markazihi,\fol{w 41 \md} wa-ysmm_A al-muma_t_tal.

-- wa-natawahhamu falak"aN _tAniy"aN sa.t.huhu mA'il `an sa.t.h
al-muma_t_tal ni.sf wa-rub` darjaT `inda al-'awj 'il_A jihaT al-junUb,
wa-ha_dA al-mIl .gayr _tAbit"iN. wa-`al_A qawl
\VAR{annahu}{nAqi.saT [\ma,\md]} mA'il
\VAR{suds}{\aemph{_Ab} [\mc], wa-kutiba fI hAmi^s [\mc] >>suds<<} juz'
wa-hwa _tAbit al-mIl: wa-hwa al-'a.sa.h.h. wa-sa.t.h al-mA'il yuqA.ti`u sa.t.h
al-muma_t_tal `al_A nuq.tatayn mutaqAbilatayn tsmm_A 'i.hdahumA
al-ra's wa-al-'u_hr_A al-_danb.

-- wa-natawahhamu falak"aN _tAli_t"aN markazuhu `al_A min.taqaT al-mA'il,
wa-ni.sf qi.trihi
\VAR{'arba`aT 'ajzA' wa-_hums daqA'iq}{\aemph{d h} [\mc]}
(bi-al-'ajzA' allatI bihA ni.sf qi.tr al-mA'il sittUn juz'"aN),
wa-tsmm_A al-.hAmil.

-- wa-natawahhamu falak"aN rAbi`"aN markazuhu `al_A min.taqaT al-.hAmil,
wa-ni.sf qi.trihi ni.sf wa-_tul_t darjaT, wa-ysmm_A al-mudIr.

-- wa-natawahhamu falak"aN _hAmis"aN markazuhu `al_A min.taqaT al-mudIr,
wa-ni.sf qi.trihi 'i_tnAn wa-`i^srUn juz'"aN wa-sitt wa-'arba`Un
daqIqaT (min tilka al-'ajzA'), wa-tsmm_A falak al-tadwIr.

-- wa-natawahhamu falak"aN sAdis"aN markazuhu `al_A min.taqaT al-tadwIr,
wa-ni.sf qi.trihi _talA_t wa-_talA_tUn daqIqaT, wa-ysmm_A al-mu.hI.t.

-- wa-natawahhamu falak"aN sAbi`"aN markazuhu `al_A al-mu.hI.t, wa-ni.sf
qi.trihi mi_tl ni.sf qi.tr al-mu.hI.t (wa-hwa _talA_t wa-_talA_tUn
daqIqaT), wa-ysmm_A al-.hAfi.z.

-- wa-`.tArd markUz `al_A min.taqaT ha_dA al-falak.

wa-'ammA al-.harakAt fa-'inna al-muma_t_tal yata.harrak `al_A qu.tbay
al-burUj, 'il_A al-tawAlI, fI kull sittIn sanaT darjaT, wa-_dalika mi_tl
.harakaT al-'awjAt.

wa-'ammA al-mA'il fa-'innahu yata.harrak 'il_A al-tawAlI, mi_tl
.harakaT markaz `.tArd, wa-hwa mi_tl markaz al-^sams: wa-hwa fI al-yawm
bi-laylatihi \aemph{0 n.t .h y}.

wa-'ammA al-.hAmil fa-'innahu yata.harrak fI 'a`lAh 'il_A _hilAf
al-tawAlI, mi_tl .harakaT markaz `.tArd 'ay.d"aN.

wa-'ammA falak al-tadwIr fa-'innahu yata.harrak fI 'a`lAh 'il_A
al-tawAlI bi-qadr fa.dl .harakaT _hA.saT `.tArd `al_A .harakaT
markazihi: wa-hwa fI al-yawm bi-laylatihi
\VAR{\aemph{0 b r yw 0 .t nA l.t nw l.t}}{\aemph{0 b _A.h _Ad b} [\ma,\md,\mc],
wa-kutiba fI hAmi^s [\ma] >>\aemph{0 b r yw 0 .t nA l.t nw l.t}<<}.

\clearpage
\noindent\fol{w 31 \mc} \VAR{wa-ha_dihi}{wa-hwa [\md,\mc]}
.harakaT basI.taT. wa-'ammA .harakaT _hA.s.saT `.tArd,
fa-'innahA basI.taT murakkabaT, li-'annahA bi-qadr .harakaT ha_dA
al-tadwIr allatI hiya
\VAR{\aemph{0 b r yw 0 .t nA l.t nw l.t}}{\aemph{0 b _A.h _Ad b} [\ma,\md,\mc]}
ma`a .harakaT markaz
`.tArd allatI hiya \aemph{0 n.t .h y}; wa-_dalika li-kawn
al-.harakatayn 'il_A \fol{.z 28 \ma} jihaT wA.hidaT.
fa-y.h.sl mufArqaT al-kawkab
lil-_dirwaT, bi-qadr majmU` al-.harakatayn, \VAR{hiya}{wa-hiya [\md]}
\aemph{0 j w kd y A l.h lr k.h mb}; wa-hiya .harakaT _hA.s.saT `.tArd
al-murakkabaT, wa-hiya mustawiyaT `inda markaz al-tadwIr.

wa-mimmA yzId _dalika 'iy.dA.h"aN: annah 'i_dA ta.harrak al-mA'il rub`
dA'iraT, wa-ta.harrak al-.hAmil rub` dA'iraT, wa-ta.harrak al-mudIr
ni.sf dA'iraT, intaqalat al-_dirwaT (allatI hiya
\VAR{mubtada'}{mbdA [\mc]} .harakaT
al-_hA.s.saT) rub` dA'iraT 'il_A al-tawAlI. wa-'innamA
\VAR{wujida}{wjdt [\md,\mc]}
bi-al-ra.sad 'annahA muntaqalaT, 'il_A al-tawAlI, mi_tl .harakaT
_hA.s.saT `.tArd (allatI hiya \aemph{0 j w kd y}), fa-yakUn .harakaT
al-tadwIr .hawla markazihi, 'il_A al-tawAlI, \VAR{bu`d}{bi-qdr [\md,\mc]}
fa.dl ha_dihi
al-_hA.s.saT \VAR{`al_A}{`nd [\mc]} .harakaT al-markaz (li-kawnihA
'il_A jihaT wA.hidaT). fa-qad att.d.h _dalika.

wa-'ammA al-^sAmil fa-'innahu yata.harrak fI 'a`lAh 'il_A al-tawAlI,
mi_tl .da`f .harakaT markaz `.tArd: wa-hwa fI al-yawm \VAR{\aemph{A n.h
    yw k}}{.gayr maqrU' [\ma], \aemph{A _A.h 0 _A.h k} [\md,\mc]}.

\VAR{wa-'ammA al-.hAfi.zaT fa-'innahA tata.harrak}{wa-'ammA al-.hAfi.z
fa-'innahu yata.harrak [\md]} fI 'a`lAh 'il_A _hilAf
al-tawAlI, 'arba`aT am_tAl .harakaT markaz `.tArd: wa-hiya fI al-yawm
\VAR{\aemph{j nw lw m}}{\aemph{j nw lw l.t} [\ma,\md,\mc]}.

fa-lA yazAlu `.tArd `al_A al-_ha.t.t al-_hArij min markaz al-tadwIr
'il_A markaz al-^sAmil yqrb min markaz al-tadwIr wa-yb`d; wa-hwa `al_A
al-_ha.t.t .gayr _hArij `anhu. wa-'i_dA kAna markaz al-tadwIr fI
al-'awj \VAR{'aw al-.ha.dI.d}{wa-al-.ha.dI.d [\md,\mc]}, kAna `.tArd
fI 'aqrab qurbh min markaz tadwIrh,
wa-ysmm_A ha_dA al-qurb ni.sf qi.tr al-tadwIr al-mar'iyy wa-hwa i.hda
wa-`i^srUn juz'"aN wa-\VAR{_tul_t_A}{_tul_t [\ma,\md], \aemph{kA k} [\mc]}
juz'. wa-'i_dA kAna
al-markaz _talA_t burUj, kAna `.tArd fI 'ab`ad bu`dh min markaz
al-tadwIr, wa-hwa _talA_t wa-`i^srUn darjaT wa-'i_tnAn wa-_hamsUn
daqIqaT.

fa-yakUn 'ab`ad bu`d `.tArd min markaz al-`Alam sittaT wa-_tamAnUn
wa-_tul_t_A. wa-'aqrab qurbh _talA_taT wa-_talA_tIna wa-_tul_t"aN. 'illA
'anna `.tArd \VAR{lA}{ilA [\md]} yqrb 'il_A 'aqrab qurb 'aflAkihi
al-mujassamaT, `l_A mA 'aw.da.hnA qabl fI .gayr
\VAR{maw.da`}{h_dA al-mw.d` [\md,\mc]}.

\clearpage

wa-'ammA aqdAr al-'aflAk al-mujassamaT: fa-'inna ni.sf
\VAR{qi.tr kuraT}{qi.trh [\md]}
al-.hAmil \aemph{k.h nb},
\VAR{wa-ni.sf qi.tr kuraT al-mudIr \aemph{kd mr}
wa-ni.sf qi.tr kuraT al-tadwIr \aemph{kj nb}}{wa-ni.sf qi.tr kuraT
al-tadwIr \aemph{kj nb} wa-ni.sf qi.tr kuraT al-mudIr \aemph{kd mr} [\mc]},
wa-ni.sf qi.tr kuraT
al-^sAmil \aemph{A w}, wa-ni.sf qi.tr kuraT \fol{.z 41 \md} al-.hAfi.z
\aemph{0 lj} (al-jamI` bi-al-'ajzA' allatI bihA ni.sf qi.tr
al-muma_t_tal sittUn juz'"aN).

fa-yakUn 'ab`ad bu`d al-muma_t_tal _tamAniyaT wa-_tamAnIn
wa-'i_tnatayn wa-_hamsIn daqIqaT, wa-fawqa _dalika sumk al-muma_t_tal;
\VAR{wa-lnufri.dh tatamh \aemph{f.t}}{wa-lnufri.d tatamaT \aemph{n.t l} [\md],
wa-lnufri.dh \aemph{n.t l} [\mc]}. wa-'aqrab qurb 'aflAkihi \aemph{lA .h},
wa-'aqall min _dalika bi-itti.sAl al-falak; fa-nufri.dh \aemph{lA 0}.
wa-al-ll_ah 'a`lam.
\end{arab}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\footnotesize\input{mercure.pdf_tex}
\end{minipage}
\textarab{hI'aT 'aflAk `.tArd `al_A 'annahA marAkiz al-akr al-tAmmaT
  `al_A .husb mA yata.sawwaru `al_A al-basI.t}
\end{figure}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\footnotesize\input{mercure_orbes.pdf_tex}
\end{minipage}
\textarab{hI'aT 'aflAk `.tArd al-mujassamaT wa-hya kurAt tAmmaT `al_A
  .hsb mA yata.sawwaru `al_A al-basI.t fI al-'awj wa-al-.ha.dI.d
  wa-al-bu`dayn al-'aws.tayn}
\end{figure}

\begin{arab}
\resetlinenumber\pagewiselinenumbers
\clearpage
\begin{center}
\Large al-bAb \fol{.z 31 \mc} al-_tAniy wa-al-`i^srUn

\large fI \fol{w 29 \ma} .dab.t .harakAt `.tArd
\end{center}
wa-taqyIdhA li-ni.sf nahAr al-_tl_tA 'awwal sanaT 'i.hd_A wa-sab`
mi'aT li-yazdjard, 'ammA al-wasa.t fa-'a.slh \aemph{.t y .t 0} (wa-hwa
mi_tl 'a.sl wasa.t al-^sams wa-al-zuhraT), wa-al-'awj \aemph{r b nb 0}.
wa-'a.sl al-_hA.s.saT lil-ta'rI_h al-ma_dkUr \aemph{h d b 0}.

wa-.harakaT al-wasa.t mi_tl .harakaT wasa.t al-^sams (wa-hiya fI
al-sanaT \aemph{yA k.t mh m}). wa-.harakaT _hA.s.saT `.tArd: \fol{w 32 \mc}
fI `i^srIn sanaT fArisiyaT \aemph{yA k.t 0 k 0}, wa-fI sanaT
\aemph{A kj nr A}, wa-fI ^sahr \aemph{j j _Ab h A}, wa-fI yawm
\aemph{0 j w kd y A l.h lr k.t}, wa-fI sA`aT
\VAR{\aemph{0 0 r mw 0 kh}}{\aemph{0 0 r mw j kh} [\md]}.
wa-'i_dA asqa.tnA .harakaT al-'awj min .harakaT al-wasa.t, .ha.sal
.harakaT al-markaz.

wa-.tarIq taqwIm h_dA al-kawkab \VAR{ka-.tarIq taqwIm}{mi_tl taqwIm [\mc]}
zu.hal.

\clearpage
\begin{center}
\Large al-bAb\fol{.z 29 \ma\\w 42 \md\\.z 32 \mc} al-_tAli_t wa-al-`i^srUn

\large fI .hisAb ta`dIl al-kawAkib
\end{center}
'ammA \textbf{al-ta`dIl al-'awwal} li-zu.hal wa-al-mu^stariy wa-al-mirrI_h
wa-al-zuhraT, fa-.hisAbh 'an ta'_hu_d jIb al-markaz wa-jIb tamAmihi,
wa-ta.drub kull wA.hid min al-jIbayn fI ni.sf qi.tr al-.hAmil
li-_dalika al-kawkab mun.hi.t"aN. fa-mA _haraja min jIb al-markaz, fasmh
al-'a.sl; wa-mA _haraja min jIb al-tamAm, fasmh al-miqdAr. _tumma 'u.drub
kull wA.hid min jIb al-markaz wa-jIb tamAmihi fI ni.sf qi.tr falak
al-mudIr. fa-mA .ha.sala min jIb al-markaz,
\VAR{fa-zidh}{zidh [\mc]} `al_A al-'a.sl 'in
kAna al-markaz 'aqall min _talA_t burUj, wa-'in kAn al-markaz 'ak_tar
min _talA_t burUj fa-nqu.shu minh. fa-mA bala.ga 'aw baq_A fa-hwa
\VAR{al-maqsUm}{al-mqwm [\md,\mc], wa-kutiba >>s<< fawqa al-s.tr fI
[\mc]}. wa-mA .ha.sala min jIb al-tamAm, nq.sh min \fol{w 30 \ma} al-miqdAr;
fa-mA baq_A zidh `al_A sittIn 'in kAn al-markaz 'aqall min _talA_t burUj,
wa-'unqu.sh min sittIn 'in kAn al-markaz 'ak_tar min _talA_t burUj.
fa-mA \VAR{baq_A}{bala.ga [\mc]} 'u.drubhu fI nafsihi,
wa-mA \VAR{bala.ga}{baq_A [\mc]} zid `alayhi ma.drUb
al-maqsUm fI nafsihi. wa-_hu_d ja_dr al-jumlaT: fa-hwa bu`d markaz
al-tadwIr min markaz al-`Alam. fa-aqsm `alayhi al-maqsUm al-ma.hfU.z,
y_hruju jIb \fol{.z 42 \md} al-ta`dIl al-'awwal. qawsh fI jadwal al-jIb,
y_hruju al-ta`dIl al-'awwal. \VAR{fa-a_tbatathu}{fa-a_tbathu [\mc]}
bi-'izA'i al-juz' alla_dI .hsabta lahu, wa-hwa
ta`dIl al-markaz wa-al-_hA.s.saT.

wa-.hisAb \textbf{al-ta`dIl al-_tAniy}, 'an ta.drub jIb al-_hA.s.saT
al-mu`addalaT (wa-jIb tamAmihA) fI ni.sf qi.tr falak al-tadwIr
li-_dalika al-kawkab. fa-mA .ha.sala min jIb al-tamAm, zidh `al_A bu`d
markaz al-tadwIr min markaz al-`Alam li-_dalika al-kawkab (wa-hwa
li-zu.hal \aemph{sj kh}, wa-lil-mu^stariy \aemph{sb mh}, wa-lil-mirrI_h
\aemph{sw}, wa-lil-zuhraT \aemph{sA yh}, wa-li-`.tArd \aemph{sh}) 'in
kAnat al-_hA.s.saT al-mu`addalaT fI al-ni.sf al-'a`l_A min falak
al-tadwIr, \VAR{wa-unqu.s}{wa-unqu.sh [\mc]} 'in kAnat al-_hA.s.saT
\VAR{al-mu`addalaT}{nAqi.saT [\mc]} fI al-ni.sf
al-'asfal minh. fa-mA .ha.sal, \VAR{fa-zid}{zid [\md,\mc]} murabba`h
`al_A murabba`
al-muta.ha.s.sl min .darb jIb al-_hA.s.saT fI ni.sf qi.tr al-tadwIr
(wa-hwa al-maqsUm); wa-_hu_d ja_dr al-murabba`ayn, aqsm `alayhi al-maqsUm,
y.h.sl jIb al-ta`dIl al-_tAniy li-_dalika al-kawkab. qawsh fI jadwal
al-jIb; \VAR{wa-_h_d qwsh}{nAqi.saT [\ma]} wa-a_tbatath bi-.hiyAl
al-_hA.s.saT al-mu`addalaT allatI .hasabta lahA.

\clearpage

\textbf{tanbIh}. ja_dr al-murabba`ayn hwa bu`d al-kawkab fI _dalika al-waqt
min markaz al-`Alam, bi-al-'ajzA' allatI bi-hA ni.sf qi.tr al-mA'il sittIn
juz'"aN, wa-ni.sf qi.tr al-tadwIr, li-zu.hal \aemph{w l},
wa-lil-mu^stariy \aemph{yA l}, wa-lil-mirrI_h
\VAR{\aemph{l.t l}}{\aemph{ld l} [\md,\mc]},
wa-lil-zuhraT \aemph{mj lj}, wa-li-`.tArd \fol{w 33 \mc}
\VAR{\aemph{kA m}}{\aemph{.t m} [\md,\mc], wa-kutiba >>\aemph{kA m}<< fI
hAmi^s [\md]}
(wa-hwa ni.sf qi.tr tadwIrihi al-mar'iy fI al-bu`d al-'ab`ad wa-al-'aqrab).

wa-.hisAb 'i_htilAf al-bu`d al-'aqrab, wa-hwa \textbf{al-ta`dIl al-_tAli_t},
mi_tl .hisAb al-ta`dIl al-_tAniy, sawA' 'illA 'annaka tufri.du markaz
al-tadwIr fI al-bu`d al-'aqrab, wa-hwa li-zu.hal \aemph{nw lh},
wa-lil-mu^stariy \aemph{nz yh}, wa-lil-mirrI_h \aemph{nd}, wa-lil-zuhraT
\aemph{n.h mh}, wa-li-`.tArd \aemph{nh 0}. wa-ta.hsabu `al_A .tarIq
al-ta`dIl al-_tAniy. fa-mA .ha.sala 'unqu.s minhu al-ta`dIl al-_tAniy
li-_dalika al-juz', fa-mA baq_A
\VAR{fa-a_tbath bi-'izA' al-juz'}{qAbilath bi-al-juz' [\mc]} alla_dI
.hasabta lahu: wa-hwa 'i_htilAf al-bu`d al-'aqrab, wa-hwa yazAd `al_A
al-ta`dIl al-_tAniy 'abad"aN \fol{.z 30 \ma} (kamA fI al-qamar,
wa-qad nabahtu `al_A _dalika).

\VAR{wa-.tarIq}{wa-'amma .tarIq [\mc]} .hisAb \textbf{daqA'iq al-nisb}
`al_A mA `araftuka fI .hisAb daqA'iq
al-nisb lil-qamar. fa-'innI \VAR{ra'aytu}{.gayr maqrU' [\ma]}
al-ta`AdIl 'in yazAd al-i_htilAf `al_A al-ta`dIl al-_tAniy (fa-'innahu
'ashal). wa-.tarIq \VAR{.hisAb daqA'iq al-nisb}{.hisAbhA [\mc]}
'an t.hsb bu`d markaz
al-tadwIr min markaz al-`Alam kamA `araftuka, wa-t.hsab
\VAR{ni.sf}{nAqi.saT [\md,\mc]} qi.tr
al-tadwIr al-mar'iy. wa-aqsmh `al_A bu`d markaz al-tadwIr
\VAR{alla_dI}{wa-hwa alla_dI [\md,\mc]} .hasabth.
fa-mA _haraja qawsh fI jadwal al-jIb: fa-mA .ha.sala fa-hwa
.gAyaT al-ta`dIl al-mu.hakkam fI tilka al-darjaT. fa-unqu.s minh .gAyaT
al-ta`dIl fI al-bu`d al-'ab`ad li-_dalika al-kawkab. famA baq_A
fa-aqsmh `al_A fa.dl mA bayna al-ta`dIl fI al-bu`d al-'ab`ad
wa-al-bu`d al-'aqrab. famA _haraja fa-hwa daqA'iq al-nisb.

\clearpage

wa-yu.htAju 'il_A \VAR{.husn}{jns [\mc]} al-ta.sarruf 'il_A
.hisAbh, fa-'inna fIhi diqqaT.
wa-'in i_htarta .hisAb \VAR{al-ta`AdIl}{al-ta`dIl [\mc]}
`al_A al-ma^shUr, fa-innahu
y.hsb `al_A kawn al-tadwIr fI al-bu`d al-'awsa.t, wa-yazAdu `alayhi
i_htilAf al-bu`d al-'aqrab, wa-ynqu.s minh i_htilAf al-bu`d al-'ab`ad.
wa-qad `araftuka fI bAb .hisAb ta`AdIl al-qamar 'annahu yumkin 'an
y.hsb jadwal wA.hid yqUm minh al-qamar. wa-`al_A tilka al-jihaT yumkin
'an y`ml likull kawkab"iN ta`dIl wA.hid yqwm bihi min .gayr ta`dIl
markaz wa-lA _hA.s.saT \VAR{fa-tafhamuhu}{.gayr maqrU' [\ma]} min
hunAk.

\clearpage
\begin{center}
  \Large al-bAb al-rAbi` wa-al-`i^srUn

  \large fI `urU.d al-kawAkib al-_talA_taT al-`alwiyyaT zu.hal
  wa-al-mu^stariy wa-al-mirrI_h
\end{center}
qad tqddm fI hI'aT 'aflAk kull wA.hid minhum 'an .gAyaT mIl al-falak
al-mA'il `an sa.t.h al-muma_t_tal: li-zu.hal juz'An wa-ni.sf,
wa-lil-mu^stariy juz' wa-ni.sf, wa-lil-mirrI_h juz'"uN wA.hid.

wa-'aqUl 'annahu wujida bi-al-ra.sad 'ay.d"aN 'anna .gAyaT mIl sa.t.h
al-tadwIr `an al-mA'il, wa-_dalika 'i_dA kAna markaz al-tadwIr fI
munta.saf mA \fol{.z 33 \mc} bayna al-`uqdatayn, wa-_dalika `inda
nihAyaT mIl al-mA'il
`an al-muma_t_tal fI al-^simAl: li-zu.hal 'arba`aT 'ajzA' wa-ni.sf,
wa-lil-mu^stariy juz'An wa-ni.sf, wa-lil-mirrI_h juz'An wa-rub`.
wa-\VAR{ra.sadtu}{.gayr maqrU' [\ma]} hunAk
fa-\VAR{wujida}{wajadtu \iscomplet{[\mb,\mc,\md,\me]}{[\md,\mc]}}
al-qi.tr al-mArr bi-'awj al-tadwIr
wa-.ha.dI.dh .tarfh al-'awjiy bayna al-mA'il wa-al-muma_t_tal,
wa-.tarfh al-.ha.dI.diy mA'il 'il_A al-jihaT allatI fIhA mIl al-mA'il,
wa-al-qi.tr al-qA'im `al_A \fol{w 43 \md} al-qi.tr al-ma_dkUr
muwAziy"aN li-sa.t.h al-burUj.

_tumma ra.sadtu 'i_dA kAna markaz al-tadwIr fI al-`uqdatayn, fa-wajadtu
su.tU.h al-dawA'ir al-_talA_taT fI sa.t.h al-falak al-muma_t_tal,
'a`niy sa.t.h \fol{w 31 \ma} falak al-burUj.
fa-'innahA wujidat `adImaT al-`ar.d 'i_dA
kAna markaz al-tadwIr fI al-ra's
\VAR{'aw}{wa \iscomplet{[\md,\me]}{[\md]}} al-_danb
wa-al-kawkab fI \VAR{'ayy}{nAqi.saT [\mc]} nuq.taT fara.dta min falak
al-tadwIr.

fa-\VAR{'ujmu`}{ajtm` \iscomplet{[\mb,\mc]}{[\mc]}}
min _dalika 'anna al-iq.tAr al-mArraT
bi-al-_drI lA
\VAR{t_tbt}{t_ttbt [\mc?]\iscomplet{, y_tbt [\me]}{}} fI su.tU.h
al-'aflAk al-mA'ilaT, wa-lA fI su.tU.h al-muma_t_talaT, 'illA 'i_dA kAna
\VAR{marAkiz tadAwIrhA}{>> marAkizhA <<, wa-kutiba >> tadAwIr << fI
  al-hAmi^s [\mc,\md]} fI 'i.hd_A al-`uqdatayn. wa-bu`d _dalika
\VAR{tamIl}{yamIl [\mc]\iscomplet{, nAqi.saT [\me]}{}}
_drI al-`alwiyyaT 'abad"aN
'il_A jihaT sa.t.h al-burUj wa-.ha.dI.dhA 'il_A _hilAfihA.
wa-\VARC{tzdAd}{yzdAd [\me]} muyUlhA,
wa-\VAR{tantah_A}{yantah_A \iscomplet{[\mb,\mc,\me]}{[\mc]}}
'il_A .gAyatihA fI munta.saf mA bayna al-`uqdatayn,
_tumma ya'_hu_d al-mIl fI al-tarAju` 'il_A 'an yan`adimu
\VAR{`inda}{fI [\mc]} al-`uqdaT al-_tAniyaT. _tumma yabtadiy mIl
al-_dirwaT `an al-muma_t_tal 'il_A jihaT sa.t.h al-burUj,
wa-al-.ha.dI.d 'il_A _hilAfihi; wa-ya'_hu_d al-mIl fI al-tazAyud 'il_A
'an yabla.gu .gAyatihi `inda munta.saf mA bayna al-`uqdatayn, _tumma
yatanAqi.s 'il_A 'an yan`adimu `inda al-ra's; wa-ya`Ud al-'amr min
al-'awwal.

\clearpage

wa-\VARC{kawn}{takUn [\mb], yakUn [\me]} al-_dirwaT ba`d mufAriqaT
al-`uqdatayn fImA bayna al-min.taqatayn 'abad"aN, dUna al-.ha.dI.d.
\VAR{yqll}{tqll [\mc]\iscomplet{, wa-tqll [\mb], wa-yqll [\me]}{}}
`urU.d al-_drI,
wa-\VAR{yk_tr}{tk_tr \iscomplet{[\mb,\mc,\md]}{[\md,\mc]}}
`urU.d al-.ha.dI.dAti. wa-'i_dA
i_htalaf bu`d markaz al-tadwIr min markaz al-burUj, i_htalafa mIl
al-_dirwaT wa-al-.ha.dI.d `inda markaz al-burUj: wa-'i_dA zAda bu`d
markaz al-tadwIr, nq.s mIl al-_dirwaT, wa-`aksahu.

wa-ra's zu.hal fI 'awwal \VARC{sanaT}{nAqi.saT [\me]} tis`a
wa-sab`a-mi'aT fArisiyyaT fI _hamsaT 'ajzA' min al-'asad, wa-ra's
al-mu^stariy fI al-juz' al-.hAdI wa-al-`i^srIn min al-sr.tAn, wa-ra's
al-mirrI_h fI al-juz' al-_tAmin `a^sar min al-_tawr, wa-_danb kull
\VAR{wA.hid}{nAqi.saT \iscomplet{[\mb,\mc,\md,\me]}{[\md,\mc]}}
kawkab muqAbilaT ra'sahu.
wa-ba`d al-ra's bi-rub` dawr yakUn nihAyaT al-`ar.d al-^simAlI, wa-hwa
li-zu.hal \VAR{'in}{'i_dA [\mc]} kAna fI al-_dirwaT min al-tadwIr
\aemph{b d} wa-'in kAna fI al-.ha.dI.d minhi \aemph{j j},
wa-\VAR{lil-mu^stariy}{al-mu^stariy \iscomplet{[\mb,\mc,\md,\me]}{[\md,\mc]}}
'i_dA kAna
fI al-_dirwaT \aemph{A w} \VAR{wa-fI}{wa-'i_dA kAna fI [\mc]} \fol{w 34 \mc}
al-.ha.dI.d \aemph{b d}, wa-lil-mirrI_h 'i_dA kAna fI al-_dirwaT
\aemph{0 r} wa-'i_dA kAna fI al-.ha.dI.d \aemph{d kA}. wa-b`d al-_danb
bi-rub` \VAR{dA'iraT}{dawr [\mc]} yakUn nihAyaT al-`ar.d al-junUbiy;
wa-hwa li-zu.hal 'i_dA kAna fI _dirwaT al-tadwIr \aemph{b b}
wa-\VAR{'in}{'i_dA [?,\md]} kAna fI .ha.dI.dh \aemph{j h}, wa-hwa
lil-mu^stariy 'i_dA kAna fI al-_dirwaT min al-tadwIr \VAR{\aemph{a
    h}}{nAqi.saT [\ma]} wa-'in kAna fI al-.hA.dI.d \aemph{b .h}, wa-hwa
lil-mirrI_h 'i_dA kAna fI _dirwaT al-tadwIr \VARC{\aemph{0 j}}{\aemph{0
    .h} [\me]} wa-'i_dA kAna fI al-.ha.dI.d \VAR{minhi \aemph{r
    r}}{fI hAmi^s [\ma]},
\VAR{wa-al-ll_ah 'a`lam}{nAqi.saT \iscomplet{[\ma,\mb,\me]}{[\ma]}}.

\begin{center}
\large fa.sl
\end{center}
i`lam 'anna ha_dihi al-'u.sUl allatI _dakrtuhA fI 'amr `urU.d
ha_dihi al-kawAkib .durUriyaT wujidat bi-al-ra.sad wa-dall `al_A
ba`.dhA
\VAR{al-.hisAb}{bi-al-.hisAb \iscomplet{[\mc,\me]}{[\mc]}}; \fol{.z 31 \ma}
fa-lA yajUz al-_hurUj `an kulliyatihA. wa-lam yumkin
\VAR{b.tulamiyUs wa-'ibar_hus}{'ibar_hus
  wa-b.tulamiyUs \iscomplet{[\mb,\mc,\me]}{[\mc]}, 'ibar_hus
  wa-lA b.tulamiyUs [\md]} wa-lA
\VAR{.gayrhum}{.gayrhumA \iscomplet{[\mb,\md,\me]}{[\md]}}
min al-mutaqaddimIn wa-al-muta'a_h_hirIn
qA.tibaT"aN 'il_A yawminA ha_dA wa.d` hI'aT"aN `al_A 'u.sUl"iN
\VARC{basI.taT"iN .sa.hI.haT"iN}{.sa.hI.haT"iN basI.taT"iN
  [\mb,\me]} tfI bi-al-.harakAt al-.tUliyyaT wa-al-`ar.diyyaT.
wa-lam yumkin b.tulamiyUs twhhum 'u.sUl tf_A bi-al-.harakAt
al-`ar.diyaT. \VAR{min .gayr tasAhul"iN}{.gayr maqrU' [\md]}
\VAR{wa-min tasAhul}{nAqi.saT [\mc]}
wa-\VARC{ma^s_A}{ma^s^s_A [\me?]}
al-.harakAt al-.tUliyyaT `al_A al-hI'aT al-ma^shUraT, lam
\VARC{yumkin}{yumkinh [\me]} al-tasAhul fI al-.harakAt al-`ar.diyyaT.

\clearpage

fa-'innahu 'in furi.da markaz al-tadwIr fI munt.saf mA bayna
al-`uqdatayn wa-furi.da sa.t.h al-tadwIr
\VAR{mA'il}{mA'il"aN \iscomplet{[\mc,\md,\me]}{[\md,\mc]}}
`an sa.t.h al-mA'il (`al_A mA qultuhu wa-hwa
al-mawjUd bi-al-ra.sad) wa-dAr al-mA'il 'il_A al-`uqdaT, fa-yalzimu 'an
lA yazAlu sa.t.h al-tadwIr mA'il"aN `an al-mA'il, wa-fI al-`uqdaT
'ay.d"aN. wa-qad wajadnA bi-al-ra.sad sa.t.h al-tadwIr .gayr mA'il `an
sa.t.h al-burUj, wa-\VARC{`adm}{`adIm [\mb]} al-`ar.d fIhumA. wa-ka-_dA
`aksahu, 'a`nI 'in fr.d al-tadwIr fI sa.t.h al-burUj wa-dAr 'il_A mA
bayna al-`uqdatayn, \VAR{wujida}{wa-wujida [\mc,\md]} lahu mIl laysa
bi-al-qalIl.

wa-tuqArib min.taqaT al-tadwIr min min.taqaT al-mA'il min .gayr m.hrk
lA \VAR{y_hll}{_A.hl [\ma]} bi-al-.harakAt al-.tUliyaT `al_A al-hI'aT
al-ma^shUraT fI \textbf{al-majis.tI} wa-\textbf{al-iqti.sA.s} fI 'amr
al-'ajsAm al-mu.harrkaT fI al-`ar.d mu.hAl. wa-mA tklfh b.tulamiyUs
wa-man ba`dahu ka-'ibn al-hay_tam fI \textbf{risAlatihi}, wa-al-na.sIr
\VARC{al-.tUsI}{nAqi.saT [\me]} fI \textbf{\VARC{ta_dkiratihi}{ta_dkIratihi
  [\mb]}}, al-mu'ayyid al-`ur.diyy fI \textbf{hI'atihi},
  wa-al-qu.tb al-^sIrAzI \fol{.z 43 \md} fI \textbf{muntah_A 'adwArihi}
  wa-mA naqalahu man nqlh min 'aqAwIl min _dikrhum
fI kitAbihi (wa-lA mA 'a.tnb
\VARC{mA}{fI [\me] faqa.t} fIhi \VARC{wa-afta_hara}{.gayr maqrU'
  [\me]} bihi min al-'a.sl al-abdA`I)
\VAR{lA}{nAqi.saT [\ma,\mc,\md]\iscomplet{, fawqa al-sa.tr [\mb,\me]}{}}
\VAR{tfI}{yfI [\mc,\md]}
bi-al-maq.sUd fI al-.tUl wa-al-`ar.d, fa-'innahu 'in
wAfaqa fI \VAR{'i.hdahumA}{\iscomplet{'i.hdIhumA [\mb,\me], }{}'i.hdAhumA
  [\md]}, _hall fI al-'u_hr_A; `al_A 'annahum \fol{.z 34 \mc}
  ra.hmahum al-ll_ah i`tarafUA bi-al-`ajz `an _dalika.

fa-'inna qu.tb al-dIn qAl 'A_hr mA qAlahu (\VARC{wa-la-`all}{la-`all
  [\mb,\me]} al-ll_ah 'an ywfq al-nA.zir fI ha_dA al-kitAb) 'an
\VAR{yastabna.t}{yastanba.t [\md]} wajh"aN tAmm"aN
\VAR{y.hdd}{\iscomplet{y.hll [\mb,\me], }{}_Ajd [\mc], yjd [\md]}
jamI`hA 'aw yzIl
\VAR{al-_hAl al-_AAf_A}{al-bAq_A [\mc], al-_halal al-bAqI [\md]
  \iscomplet{, al-_hlal al-tAf_A [\mb], al-_halal al-baq_A [\me]}{}}
fI mA _dakarnAhu ('annahu \VARC{ylhm}{fa-lahum [\me]} al-.swAb
wa-al-hAdI 'il_A
sawA'i \VAR{al-.sirA.ti}{al-.tarIq [\mc,\md]}); wa-qad qAl b.tulamiyUs
fI .gayr makAn \VAR{mA ha_dA yqrb}{.gayr maqrU' [\ma]} min m`nAh; `al_A
'anna al-ma_dkUrIn intah_A 'ilayhim ha_dA al-`ilm wa-'ilayhim
ynsb.

wa-i`lam 'anna sabab imtinA` izAlaT mA fI al-hI'aT al-ma^shUraT min
al-^sukUk, hwa 'an mbdAhA `al_A .gayr wa.d`"iN .sa.hI.h .tabI`iyy, fa-lA
budda min \VAR{ta.gayyur}{ta.gyIr [\mc]} jumlaT tilka al-'u.sUl
'il_A wa.d` .sa.hI.h lA yd_hl `alayhi ^sukk wa-y.h.sl bihi al-ma.tlUb,
an umkinu, ka-mA fa`alnA.

fa-'innA lamA twhmnA hI'aT al-'aflAk `al_A al-wajh alla_dI
\VAR{_dakarnAhu}{ibtakarnAh [\mc]}, wa-intahaynA 'il_A `urU.d
ha_dihi al-kawAkib, wa-naqalnA mA wajadnA bi-al-ra.sad min `urU.dihA
wa-mIl \fol{w 32 \ma} 'aflAkihA, wajadnA _dalika muwAfiq"aN `al_A mA
twhmnAhu min al-'aflAk wa-al-.harakAt.
wa-_dalika ytbyn bi-mA 'aw.da.huhu \VAR{hAhunA}{hahunA [\md,\mc]}.

\clearpage

fa-'aqUlu nufri.du, 'i_dA kAn markaz al-.hAmil wa-al-mudIr fI munta.saf
mA bayna al-`uqdatayn, wa-qi.tr al-.hAmil mA'il `an al-mA'il 'il_A
al-jihaT allatI wujida mIl .ha.dI.d al-tadwIr fIhA, 'ammA li-zu.hal
fa-_talA_taT 'ajzA' wa-ni.sf; wa-al-mudIr li-zu.hal mA'il `an sa.t.h
al-.hAmil lahu \VAR{juz' wA.hid}{juz'-"aN wA.hid"aN [\mc]}.
wa-al-falak al-.hAmil lil-mirrI_h mA'il `an
sa.t.h al-mA'il darjaT wa-ni.sf wa-_tumn, wa-\VAR{tadwIr}{mudIr?}
al-mirrI_h mA'il `an sa.t.h al-falak al-.hAmil ni.sf wa-_tumn juz'.
wa-qi.tr al-falak al-.hAmil lil-mu_stariy mA'il `an sa.t.h al-falak
al-mA'il juz'ayn, wa-qi.tr \VAR{tadwIr}{mudIr?} al-mu^stariy mA'il `an
sa.t.h al-.hAmil lil-mu^stariy ni.sf juz'. _tumma
\VAR{nata.harraku}{tata.harrak [\md,\mc]}
al-'aflAk bimA lahA min al-.harakAt al-basI.taT .hawla marAkizhA
bi-al-miqdAr alla_dI furi.da lahA 'il_A al-jihAt allatI furi.dat.
fa-'i_dA ta.harrak al-mA'il rub` \VAR{dawr}{dawraT [\md,\mc]},
wa-ta.harrak al-.hAmil rub` dawr
'ay.d"aN, wa-ta.harrak al-mudIr ni.sf dawr, 'inqalaba al-mIl 'il_A
al-jihaT al-'u_hr_A: fa-.sAr jihaT mIl al-tadwIr fI _hilAf jihaT mIl
al-.hAmil wa-.sAra sa.t.h al-tadwIr fI sa.t.h al-burUj. li-'anna mIl
al-.hAmil ja`alnAhu mi_tl mIl al-mA'il wa-mi_tl mIl al-tadwIr. fa-'i_dA
in`akasa mIl al-tadwIr .sAra mIl al-tadwIr nAqi.s"aN `an mIl al-.hAmil,
\VAR{fa-tabqI}{fa-yabqI [\md,\mc]} fa.dl mIl al-.hAmil `an mIl al-tadwIr,
wa-_dalika al-fa.dl bi-qadr \fol{w 35 \mc} mIl al-mA'il;
wa-markaz al-.hAmil wa-qad wa.sala 'il_A al-`uqdaT,
fa-qad mAss sa.t.h al-burUj fa-yakUn li-_dalika sa.t.h al-tadwIr
fI sa.t.h al-burUj. wa-_dalika .zAhir.

fa-ta'amlh wa-i`lam 'anna majmU` mIl al-.hAmil wa-mIl al-tadwIr
ja`alnAhu mi_tl mIl al-tadwIr `an sa.t.h al-mA'il al-mar.sUd, wa-fa.dl
mIl al-.hAmil `an mIl al-tadwIr bi-qadr mIl al-mA'il. fa-min hunA
\VAR{ta`lm}{ya`lm [\md,\mc]} 'ay.d"aN 'annahu,
'i_dA ijtama`a al-mIlAn kAna al-mIlAn, fI al-.gAyaT
wa-_dalika fI munta.saf mA bayna al-`uqdatayn; wa-'i_dA i_htalafa
al-mIlAn, kAna al-bAqI bi-qadr mIl al-mA'il, wa-_dalika `nda
al-`uqdatayn, fa-yakUn al-tadwIr fI sa.t.h al-burUj. wa-haka_dA fr.d
al-tadwIr fI sa.t.h al-burUj bi-al-ra.sad, haka_dA yakUn al-ta.sawwur
al-.sa.hI.h.

\clearpage

\noindent \VAR{wa-n_h.t.t}{wa-y_h.t.t [\md,\mc]} li-biyAn _dalika
_ha.t.t \aemph{a b} fI sa.t.h al-burUj, wa-nufri.du \aemph{b} markaz
al-burUj. \VAR{wa-n_hrj}{wa-y_hrj [\md,\mc]} minhu _ha.t.t
\VAR{\aemph{b h}}{\aemph{A d} [\ma,\mc]} mA'il `an \aemph{a b} biqadr mIl
al-mA'il `an sa.t.h al-burUj. wa-n_hrj _h.t.t \aemph{j h d}
wa-nufri.dhu qi.tr al-falak al-.hAmil; wa-n_hrj min nuq.taT \aemph{h}
_ha.t.t \aemph{z .t} wa-nfr.dh qi.tr al-tadwIr \fol{.z 32 \ma}
li-zAwiyaT \aemph{s h z} majmU` al-mIlayn wa-al-mIlAn fI jihaT wA.hidaT
(`inda munta.saf mA bayna al-`uqdatayn).
fa-'i_dA intaqala markaz al-.hAmil alla_dI hwa
nuq.taT \aemph{b}, kAna qi.tr al-.hAmil \VAR{wa-hwa}{hwa [\md]}
_ha.t.t \aemph{j d} bAq"iN `al_A mIlh wa-ya.sIr ka-'annahu
_ha.t.t \aemph{q .s}. fa-'i_dA \fol{w 44 \md}
fr.dnA \VAR{baqI}{\aemph{bq_A A} [\md,\mc]} qi.tr al-tadwIr `al_A mIlh,
\VAR{fa-ya.sIr}{fa-ni.sf [\ma,\md,\mc]}
_ha.t.t \aemph{z .t} ka-'annahu _ha.t.t \aemph{` k}; fa-'i_dA dAra
al-mudIr ni.sf dA'iraT, .sAra \VAR{mIl}{mi_tl [\md,\mc]} qi.tr
\aemph{` k} `an qi.tr \aemph{.s q} fI al-jihaT al-'u_hr_A,
wa-.sArat zAwiyaT \aemph{q b k} mi_tl
zAwiyaT \aemph{lA b q} fa-.tAbaqa qi.tr al-tadwIr (alla_dI huwa _ha.t.t
\aemph{` k}) li-sa.t.h al-burUj. wa-_dalika li-kawn majmU` mIl al-.hAmil
wa-al-mA'il mi_tl mIl al-tadwIr \VAR{wa-fa.dl}{wa-fa.dl mIl 
 al-tadwIr wa-fa.dl [\ma,\md,\mc]} mIl al-.hAmil `al_A mIl al-tadwIr
 bi-qadr mIl al-mA'il. wa-qad tkrrar _dalika. wa-_Ajb 'an yst`ml al-markaz
al-mu`addal lA al-mu.tlaq, wa-_dalika .hayna wu.sUl markaz al-tadwIr
'il_A al-`uqdatayn; fa-afham _dalika.

\begin{center}
\large tanbIh
\end{center}
law ja`alnA mIl al-.hAmil bi-qadr mIl al-tadwIr, wa-majmU`
al-mIlayn biqadr mIl al-tadwIr al-mawjUd bi-al-ra.sad, kAn, 'i_dA
t.harrak al-.hAmil rub` dawr wa-al-mudIr ni.sf dawr 'ay.d"aN, .sAr
sa.t.h al-tadwIr fI sa.t.h al-mA'il; \VAR{wa-ha_dA}{wa-hwa [\mc]} .zAhir.
wa-'innamA ^shd
al-ra.sad bi-'annahu ya.sIru fI sa.t.h al-burUj lA \fol{.z 35 \mc} fI
sa.t.h al-mA'il.
wa-.gAlib al-muta'a_h_hirIn ka-al-n.sIr al-.tUsI wa-al-mu'ayyad
al-`ur.dI wa-al-qu.tb al-^sIrAzI tawahhamUA 'annahu, 'i_dA .sAra fI
sa.t.h al-mA'il, 'in`adama al-`ar.d: wa-_dalika mu.hAl li-baqA mIl
sa.t.h al-tadwIr `an sa.t.h al-burUj. wa-ha_dA .gAyaT al-wu.dU.h; `al_A
'anna al-ra.sAd _dakarUA 'annahu yakUn 'ammA fI sa.t.h al-burUj 'aw
qarIb min _dalika, fa-'innahu lam yata.haqqaq lahum 'annahu fI sa.t.h
al-burUj mu.tlaq"aN.

\clearpage

\begin{center}
\large tanbIh _tAn"iN 
\end{center}
law kAna wjd bi-al-ra.sad 'anna mIl al-tadwIr \textbf{`an al-mA'il}
bi-qadr al-mawjUd bi-al-ra.sad, fa-'i_dA ta.harraka
\VAR{al-.hAmil}{al-mA'il [\mc]} rub` dA'iraT,
wa-ta.harraka fI _dalika al-zamAn al-mudIr ni.sf dA'iraT,
.sAra \VAR{mIl}{mi_tl [\mc]} al-tadwIr fI _hilAf al-jihaT allatI
kAna fIhA al-mIl; fa-.sAra fI sa.t.h al-burUj;
wa-'innamA wjd bi-al-ra.sad mIl al-tadwIr
mu_hAlif li-mIl al-mA'il. fa-min 'ajl _dalika, astnb.tnA muqAdIr muyUl
al-.hawAmil wa-al-tadAwIr bi-.hay_tu kAna majmU` al-mIlayn mi_tl mIl
al-tadwIr fI al-ra.sad, wa-fa.dl al-mIlayn bi-qadr mIl al-mA'il.
fa-.sa.h.ha mA \VAR{qa.daynAhu}{fa.dInAhu [\ma]}.

\begin{center}
\large tanbIh _tAli_t
\end{center}
lammA kAna al-mawjUd bi-al-ra.sad, 'anna nihAyaT mIl
al-tadwIr `an al-mA'il `inda munta.saf mA bayna al-`uqdatayn, wa-hunAka
wujd \fol{w 33 \ma} nihAyaT al-`ar.d al-^simAliy,
wa-kAna ha_dA al-maw.du` \VAR{fI}{min [\md,\mc]}
al-mirrI_h maw.du` 'awjihi, \VAR{kAnat}{kAn [\md,\mc]} qi.tray
al-.hAmil wa-al-tadwIr
mArrayn bi-al-'awj wa-al-.ha.dI.d \VAR{hiya}{hwa [\md,\mc]} mu.tAbqaT
lil-_ha.t.t al-_hArij
min markaz al-burUj al-mArr bi-maw.du` nihAyaT al-`ar.d al-^simAliy
('a`niy munta.saf mA bayna al-`uqdatayn): wa-_dalika li-kawn _dalika
al-maw.du` fI maw.du` 'awj al-mirrI_h.

wa-lammA kAna mawu.du` nihAyaT al-`ar.d al-^simAliy alla_dI hwa
munta.saf mA bayna al-`uqdatayn lil-mu^stariy ba`da mawu.du` 'awjihi
`inda b.tulamyUs bi-`i^srIn juz' wa-bi-ra.sadnA bi-_tamAniyaT
wa-`i^srIn juz'"aN, wa-li-zu.hal qabla maw.du` 'awjihi bi-_hamsIn
juz'"aN, kAna al-qi.tr alla_dI `inda nihAyaT al-`ar.d .gayr al-mArr
bi-'awj al-.hAmil wa-'awj al-mudIr. fa-'innA, 'i_dA fara.dnA al-'aflAk
fI al-'awj, wa-ta.harrakat 'ammA al-.hAmil fa-`i^srIn juz'"aN wa-'ammA
al-mudIr fa-.da`f _dalika, intaqala 'awj al-.hAmil 'il_A al-tawAlI
`i^srIn juz'"aN fa-.sAra `inda nuq.taT \aemph{d}, wa-.sAra qi.tr
\aemph{h .t} hwa alla_dI `indah nihAyaT al-`ar.d;
\VAR{wa-'i_dA}{fa-'i_dA [\mc]} dAra
al-mudIr .da`f _dalika .sAra 'awj al-mudIr 'il_A nuq.taT
\VAR{\aemph{w}}{\aemph{d} [\ma,\md,\mc]}
wa-.sAra qaws \aemph{d h} mi_tl qaws \aemph{h w}, wa-.sAra al-qi.tr
al-mu.tAbiq li-_ha.t.t \aemph{h .t} hwa alla_dI `indah nihAyaT
al-`ar.d. \fol{w 36 \mc}

\clearpage

wa-`al_A _dalika \VAR{aqmnA al-burhAn}{nAqi.saT [\md,\mc]} 
'i_dA tawahhamnA _dalika fI zu.hal: wa-ja`alnA al-'aflAk
\VAR{yata.harrak}{tata.harrak [\md,\mc]}
rAj`aT"aN 'il_A `inda al-maw.du` alla_dI qabla 'awj zu.hal bi-_hamsIn juz',
alla_dI fIhi nihAyaT `ar.dh kAna mA y.tAbq al-_ha.t.t al-_hArij min
markaz al-burUj 'il_A al-maw.du` alla_dI fIhi nihAyaT `ar.dh min
aq.tAr al-.hAmil wa-min aq.tAr al-mudIr,
humA \textbf{al-qi.trAn al-`ar.diyAn}
('a`niy alla_dI `indahumA nihAyaT
\VAR{al-`ar.d al-`ar.d}{al-`ar.d [\md,\mc]}).

\begin{center}
\large tanbIh\fol{.z 44 \md\\.z 33 \ma\\.z 36 \mc}
\end{center}
law fara.dnA al-.hAmil fI sa.t.h al-mA'il wa-fara.dnA al-mudIr
\VAR{mA'il}{mA'il"aN [\md,\mc]} `an sa.t.h al-.hAmil bi-qadr mA fara.dnA
mIl al-.hAmil `an al-mA'il, wa-fara.dnA mIl
al-tadwIr \VAR{`an al-mudIr}{fI hAmi^s [\ma]}
`al_A .hAlh, kAna
\VAR{al-.hA.sil min al-far.dayn}{al-.hAmil min al-`r.dayn [\md,\mc]}
^say"uN wA.hd. fa-a`rf _dalika.
\end{arab}

\begin{figure}[h!]
\centering
\footnotesize\input{lat_inf_profil.pdf_tex}
\end{figure}

\begin{figure}
\centering
\noindent\hspace{-85mm}\hspace{.5\textwidth}\begin{minipage}{17cm}
\footnotesize\input{lat_inf.pdf_tex}
\end{minipage}
\end{figure}


==> fichier2d.tex <==
\begin{arab}
\resetlinenumber\pagewiselinenumbers
  
\clearpage
\begin{center}
\Large al-bAb al-_hAmis wa-al-`i^srUn

\large \VAR{fI .harakAt
   al-zuhraT wa-`u.tArad fI al-`ar.d wa-fIhi fa.slAn}{fI hAmi^s
  [\md], fI .harakAt al-zuhraT wa-`u.tArad wa-fIhi fa.slAn [\mc]}
\end{center}

\begin{center}
\large \VAR{al-fa.sl}{nAqi.saT [\mc]} al-'awwal

\normalsize fI \VAR{`urU.d}{.harakAt [\mc]} al-zuhraT
\end{center}
wa-fIhi ma_dhabAn li-b.tulamiyUs

\textbf{al-'awwal} mA _dakarahu fI \textbf{al-majis.tI} .hay_tu qAla
'anna mA'il
al-zuhraT yaqrab wa-yab`ad `an sa.t.h al-burUj. fa-lA yazAlu markaz
tadwIr al-zuhraT bayna al-`uqdatayn fI sa.t.h falak al-burUj, wa-fI
.gayr al-`uqdatayn ^simAliyy `an sa.t.h al-burUj bi-miqdAr 'ak_taruhu
suds juz' wa-yuqAbilu
\VAR{mIl}{m_tl \iscomplet{[\md,\me,\mc,\mb]}{[\md,\mc]}} mA'il
al-zuhraT al-^simAliyy `inda 'awjihA. wa-'i_dA \fol{w 45 \md} kAna
markaz tadwIrhA fI
al-`uqdatayn, 'a`niy `inda tarbI` al-'awj, kAna al-qi.tr al-qA'im `al_A
al-qi.tr al-mArr bi-'awj al-tadwIr wa-.ha.dI.dh min sa.t.h al-burUj;
fa-'i_dA kAna fI `uqdaT al-_danb, kAna mIl 'awj al-tadwIr 'il_A
al-^simAl wa-.ha.dI.duhu 'il_A al-junUb; wa-'i_dA kAna fI `uqdaT
al-ra's, kAn mIl 'awj al-tadwIr 'il_A al-junUb wa-.ha.dI.dh 'il_A
al-^simAl, wa-miqdAr ha_dA\fol{w 34 \ma} al-mIl fI \textbf{al-majis.tI}
juz'ayn wa-ni.sf wa-y`rf \textbf{bi-mIl al-tadwIr}.
wa-'i_dA kAna markaz al-tadwIr fI al-'awj,
kAna \VARC{al-qi.tr}{qi.tr [\mb]} al-mArr bi-'awj al-tadwIr
wa-.ha.dI.dh fI sa.t.h \VARC{al-mA'il}{nAqi.saT [\me]} wa-al-qi.tr
al-qA'im `alayhi mA'il `an sa.t.h al-burUj bi-.hay_tu yakUn al-ni.sf
alla_dI min al-'awj 'il_A al-.ha.dI.d min al-tadwIr
\VAR{^simAliy"aN}{^simAliyy \iscomplet{[\ma,\mb,\mc,\me]}{[\ma,\mc]}}
`an al-mA'il wa-al-'A_har
\VAR{junUbiy"aN}{junUbiyy \iscomplet{[\ma,\mb,\mc,\me]}{[\ma,\mc]}}
`anhu, wa-miqdAr ha_dA
al-mIl `an sa.t.h al-burUj _talA_taT 'ajzA' wa-ni.sf
\VAR{juz'}{nAqi.saT \iscomplet{[\ma,\md,\mb]}{[\ma,\md]}}
wa-y`rf \textbf{bi-mIl al-wrAb}; \VARC{ha_dA}{wa-ha_dA [\me]}
ma_dhabh fI \textbf{al-majis.tiy}. wa-qad .sa.h.ha.h ba`.d
al-muta'a_h_hirIn \VARC{bi-al-ra.sad}{fI al-ra.sad [\me,\mb]}, fa-wjd
mIl al-tadwIr mi_tl mIl al-wrAb wa-`alayhi .hisAb jadAwil `ar.d
al-zuhraT `inda mu.haqaq_A ha_dA al-fann.

\textbf{wa-ma_dhabh al-_tAniy} mA _dakarhu fI kitAbihi al-ma`rUf
\textbf{bi-al-iqti.sA.s}, wa-hwa ba`d
al-'awwal \VARC{'anna}{'ammA [\mb]} mA'il al-zuhraT _tAbit al-mIl fI
al-jihatayn, wa-nihAyaT mIlh suds \VARC{juz'-"aN}{juz' [\mb]} fI
al-^simAl wa-mi_tlh fI al-junUb, wa-mIl al-tadwIr fIhi fI al-.hAlatayn
_talA_taT 'ajzA' wa-ni.sf juz'.

\clearpage

wa-lam yumkin b.tulamyUs wa-lA .gayrihi 'il_A waqtinA ha_dA wa.d`
\VAR{'u.sUl}{'u.sUl"aN [\md,\mc]} ta.harruk al-tadwIr wa-al-mA'il
bi-al-.sifaT \fol{w 37 \mc} al-ma_dkUraT li-i_htilAf mIl al-tadwIr
fI al-.hAlatayn wa-i_htilAf al-qi.trayn alla_dIna yakUn 'a.hadhumA
\VAR{mA'il"aN}{mA'il \iscomplet{[\ma,\mb]}{[\ma]}} wa-al-'A_har
'immA fI sa.t.h al-burUj 'aw fI sa.t.h al-mA'il. wa-qad tayassara
bi-.hamd al-ll_ah ta`Al_A.

wa-hwa 'an yfr.d nihAyaT mIl al-mA'il fI al-^simAl `inda 'awj
al-zuhraT wa-nihAyath suds juz', wa-hwa mIl _tAbit al-miqdAr fI
al-^simAl wa-mi_tlh fI al-junUb, wa-hwa
\VARC{yata.harrak}{mt.hrrk [\me,\mb]},
fa-yantaqilu ma`a intiqAl al-'awj wa-yantaqilu
\VARC{bi-intiqAlihi}{bi-intiqAl [\me]} al-`uqdatayn al-ra's
wa-al-_danb.
\VAR{wa-nufri.du}{wa-nufri.du wa-nufri.du [\ma],
  wa-yfr.d \iscomplet{[\md,\me,\mc]}{[\md,\mc]}}
markaz al-tadwIr wa-al-mudIr `al_A al-_ha.t.t
al-mArr bi-al-'awj, \VAR{wa-nufri.du}{wa-yfr.d [\mc]} al-.hAmil fI
sa.t.h al-mA'il, wa-nufri.du _dirwaT
\VAR{al-mudIr}{al-tadwIr [\mc,\md,\ma]\iscomplet{, al-mudwIr [\mb]}{}}
al-ws.t_A mA'ilaT 'il_A al-junUb
`an sa.t.h al-mA'il zAwiyaT miqdArhA _hams daqA'iq wa-al-ni.sf min
al-mudIr alla_dI ibtidA'uhu min al-'awj wa-hwa al-'awwal ^simAliyy `an
sa.t.h al-mA'il zAwiyaT \VARC{`an}{`nda [\me,\mb]} markazh miqdArhA
_talA_taT 'ajzA'. wa-nufri.du _dirwaT al-tadwIr mA'ilaT `an _dirwaT
al-mudIr 'il_A al-^simAl _hams daqA'iq, fa-yabq_A qi.tr al-tadwIr
\VAR{al-'awj}{al-'awjiy [\md]\iscomplet{, nAqi.saT [\me]}{}}
fI sa.t.h al-mA'il.
\VARC{wa-nufri.du}{wa-yfr.d [\me,\mb]} ni.sf al-tadwIr al-'awwal,
wa-hwa \VAR{alla_dI}{nAqi.saT [\mc]} ibtidA'uhu min al-'awj,
\VAR{mA'il"aN}{mA'il \iscomplet{[\ma,\mb,\mc,\me]}{[\ma,\mc]}}
`an ni.sf al-mudIr al-mA'il
'il_A al-^simAl ni.sf juz' 'il_A jihaT al-^simAl 'ay.d"aN.

wa-'i_dA tqarrar _dalika wa-dArat al-'aflAk, fa-dAra al-mA'il rub`
dA'iraT wa-dAra al-.hAmil rub` dA'iraT 'ay.d"aN wa-dAra al-mudIr fI
_dalika al-zamAn ni.sf dA'iraT, fa-inqalaba mIl al-tadwIr, fa-.sAra
al-qi.tr al-qA'im `al_A \VAR{al-'awjiy}{al-'awj [\mc]} fI sa.t.h
al-burUj wa-al-qi.tr al-'A_har
\VAR{mA'il"aN}{mA'il \iscomplet{[\ma,\mb,\mc,\me]}{[\ma,\mc]}}
`an sa.t.h al-burUj zAwiyaT
\VARC{miqdArhA}{miqdAr [\me]} juz'ayn \fol{.z 34 \ma}
wa-ni.sf; ha_dA `al_A \VARC{'anna}{nAqi.saT [\me]} i_htilAf mIl
al-tadwIr mi_tl mA \VAR{_dkr}{_dakarah [\mc]} fI \textbf{al-majis.tI}.

wa-'ammA mA .sa.h.ha.hh al-muta'a_h_hirUn min kawn mIl al-tadwIr fI
al-`uqdatayn wa-fI al-'awj wa-al-.ha.dI.d _talA_taT 'ajzA' wa-ni.sf
juz', wa-ta.sawwur ma_dhabh al-ma_dkUr fI
\textbf{al-iqti.sA.s} 'an
\VAR{nufri.du}{yfr.d \iscomplet{[\md,\me,\mc]}{[\md,\mc]}}
al-mA'il `al_A mA \VARC{_dakara}{_dakarahu [\me]}
fI al-ma_dhab al-'awwal wa-fI \VARC{sa.t.hihi}{sa.t.h [\me]}
al-.hAmil.

\clearpage
\noindent fI al-'awj, wa-_dirwaT al-mudIr mA'ilaT
\VAR{`al_A}{`an [\md,\mc]} al-mA'il 'il_A al-junUb _hams daqA'iq
\VARX{wa-_dirwaT al-tadwIr}{mA'ilaT `an _dirwaT al-mudIr}{_hams
  daqA'iq}{fI al-hAmi^s [\md,\mc]} 'il_A al-^simAl wa-ni.sf
al-tadwIr alla_dI ibtidA'uhu min al-'awj mA'il 'il_A al-^simAl
_talA_taT 'ajzA' wa-ni.sf.

qultu: wa-ha_dA al-wajh hwa al-mu`tamad `alayhi wa-hwa mA .sa.h.ha.hah
al-mu.haqaqUn.

wa-nihAyaT mIl al-tadwIr fI al-junUb \aemph{.h m} wa-fI al-^simAl
\VAR{\aemph{A j}}{\aemph{A .h} \iscomplet{[\md,\mb]}{[\md]}} \fol{.z 37 \mc}
wa-'ak_tar mIl al-wrAb \aemph{b l}. wa-nihAyaT al-`ar.d
\VARC{lil-mA'il}{al-mA'il [\me,\mb]}
fI al-^simAl 'abad"aN suds juz'. wa-al-ra's lil-zuhraT
qabla al-'awj bi-rub` dawr
\VARC{wa-al-_danb ba`da al-'awj bi-rub` dawr}{nAqi.saT [\me]}.
wa-nihAyaT al-`ar.d fI al-^simAl
\VAR{wa-al-junUb}{fI hAmi^s [\ma]} lil-mA'il fI al-'awj wa-al-.ha.dI.d.

\textbf{tanbIh}. jamI` mA takallafUhu al-mutaqaddimUn \fol{.z 45 \md}
wa-al-muta'a_h_hirUn fI
'amr `ar.d al-zuhraT min taqArub al-min.taqatIn wa-'i_htilAf mIl falak
al-tadwIr mu.hAl
\VAR{wa-laysa}{laysa \iscomplet{[\md,\me,\mc,\mb]}{[\md,\mc]}}
\VAR{y_hf_A}{mu_hfiyy \iscomplet{[\mb,\md]}{[\md]}}
`al_A man lahu i.tlA` `al_A kutub m.hqqaq_A ha_dA al-fann.

\begin{center}
\large al-fa.sl al-_tAniy

\normalsize fI `urU.d `u.tArad
\end{center}
wa-fIhA ma_dhabAn li-b.tulamiyUs: al-'awwal alla_dI _dakarahu fI
\textbf{al-majis.tI}, \VAR{wa-al-_tAniy}{al-_tAniy [\mc]} alla_dI _dakarahu
fI \textbf{al-iqti.sA.s}.

'ammA \textbf{ma_dhabuhu al-'awwal} 'an nufri.du falak"aN mA'il"aN `an
al-muma_t_tal nihAyaT mIlihi `inda al-'awj 'il_A al-junUb ni.sf
wa-rub` juz', fa-yqA.t` ha_dA al-mA'il `al_A al-`uqdatayn,
\VAR{wa-y.sIr}{.gayr maqrU' [\ma]} n.zIr al-juz'
alla_dI `inda al-'awj `inda al-.ha.dI.d mA'il"aN `anhu 'il_A al-^simAl
bi-mA `alamta. wa-'inna min.taqaT al-mA'il \VARC{tuqArib}{yqArb [\mb]}
li-min.taqaT al-burUj .hatt_A \VARC{tan.tabiqu}{yan.tabiqu [\me]}
`alayhA, _tumma \VAR{ymIlu}{tmIlu [\md,\mc]} 'il_A al-jihaT
al-'u_hr_A bi-_dalika al-miqdAr \VARC{wa-ka-_dalika}{wa-li-_dalika
  [\me,\mb]} al-juz' al-muqAbal lahu; wa-ha_dA mu.hAl: lA yumkin 'an
yata.sawwur \VAR{`al_A}{`al_A `al_A [\ma]} hI'aT b.tulamiyUs wa-lam
yata`arra.d hwa wa-lA .gayrh li-m.harrik ha_dihi al-.harakaT.
 
\clearpage

_tumma fr.d 'i_dA kAna markaz al-tadwIr fI munta.saf mA bayna
al-`uqdatayn fI al-'awj
\VAR{`inda}{nAqi.saT \iscomplet{[\md,\me,\mc,\mb]}{[\md,\mc]}}
nihAyaT al-`ar.d al-junUbiy 'anna al-qi.tr al-mArr bi-'awj al-tadwIr
wa-.ha.dI.dh fI sa.t.h al-mA'il wa-al-qi.tr al-'A_har mA'il bi-.hay_tu
ykUn al-ni.sf al-'awwal min al-tadwIr
\VAR{junUbiy"aN}{junUbiy \iscomplet{[\ma,\mb,\mc,\md]}{[\ma,\md,\mc]}}
\VAR{wa-al-ni.sf al-'A_har}{wa-al-'A_har [\md,\mc]}
\VAR{^simAliy"aN}{^simAliyy \iscomplet{[\ma,\mb,\mc,\md]}{[\ma,\md,\mc]}}
wa-zAwiyaT ha_dA al-mIl sab`aT
'ajzA', wa-ysmm_A \textbf{al-wrAb}. wa-'i_dA kAna markaz al-tadwIr fI
al-`uqdatayn, kAna al-qi.tr al-qA'im `al_A al-'awj fI sa.t.h al-burUj
wa-al-qi.tr al-'awjiy mA'il `an sa.t.h al-burUj, 'ammA .ha.dI.dh
fa-'il_A jihaT al-^simAl \VAR{wa-'awjh 'il_A}{wa-'ammA 'awjh fa-'il_A
  [\md], wa-'ammA 'awjh 'il_A [\mc]} \fol{w 35 \ma} jihaT al-junUb;
  wa-zAwiyaT ha_dA al-mIl sittaT 'ajzA' wa-rub` juz',
  wa-y`rf \textbf{bi-mIl al-tadwIr}; fa-lA
yazAlu markaz al-tadwIr 'immA junUbiy `an sa.t.h al-burUj wa-'immA
fIhi `inda al-`uqdatayn. ha_dA ma_dhabahu fI \textbf{al-majis.tI}.

\textbf{wa-ma_dhabuhu al-_tAniy} alla_dI _dakarahu fI \fol{w 38 \mc}
\textbf{al-iqti.sA.s} 'an mA'il `.tArd _tAbit
al-mIl fI al-jihaT al-junUbiyaT `an al-'awj wa-miqdAruhu suds juz'
wa-al-.tarf al-'A_har mA'il 'il_A al-^simAl `inda al-.ha.dI.d suds
juz'. wa-'i_dA kAn markaz al-tadwIr fImA bayna al-`uqdatayn, kAna
al-qi.tr al-mArr bi-al-'awj
\VAR{mu.tAbaq"aN}{mu.tAbaq \iscomplet{[\ma,\mb,\md,\me]}{[\ma,\md]}}
lil-mA'il wa-al-qi.tr al-'A_har mA'il bi-al-ni.sf al-_tAniy
\VARC{min al-tadwIr}{bi-al-tadwIr [\me,\mb]} 'il_A al-^simAl, wa-miqdAr
zAwiyaT al-mIl sittaT 'ajzA' wa-ni.sf juz',
wa-y`rf bi-mIl al-wrAb.
wa-'i_dA kAna markaz al-tadwIr bayna al-`uqdatayn, kAna al-qi.tr
al-qA'im `al_A
\VAR{al-'awjiy}{al-'awj \iscomplet{[\md,\me,\mc,\mb]}{[\md,\mc]}}
fI sa.t.h al-burUj wa-al-qi.tr al-'awjiy mA'il, .h.dI.dh 'il_A al-^simAl
wa-'awjuhu 'il_A al-junUb, wa-zAwiyaT ha_dA al-mIl
\VARC{mi_tl mIl}{m_Al [\me]} al-wrAb; wa-_dalika sittaT
\VAR{'ajzA'}{nAqi.saT \iscomplet{[\ma,\md,\mb]}{[\ma,\md]}}
wa-ni.sf. ha_dA ma_dhabahu al-_tAniy, wa-lam yumkin
b.tulamiyUs wa-lA .gayrh w.d` 'u.sUl yumkin ta.sawwur ha_dihi
\VARC{al-muyUl}{.gayr maqrU' [\me], al-mdl [\mb]} fIhA wa-lA
tu_hillu bi-al-.harakAt
\VAR{al-.tUliyaT}{al-.tUyilaT \iscomplet{[\md,\mb,\me]}{[\md]}}.

wa-qad \VAR{'amkananA}{'amkanA \iscomplet{[\me,\mc]}{[\mc]}}
\VAR{nu.sawwiru}{t.swwr \iscomplet{[\md,\mc,\mb]}{[\md,\mc]}}
\VAR{ha_dayna}{ha_dA \iscomplet{[\ma,\mb,\md,\me]}{[\ma,\md]}}
al-ma_dhabayn wa-lillah al-.hamd.

'ammA \textbf{al-ma_dhab al-mu`tamad `alayhi} wa-hwa 'an nufri.du nihAyaT
mIl al-mA'il al-junUbiy `inda al-'awj \VAR{wa-al-^simAliyy}{al-^simAliyy
  [\mc]} `inda al-.ha.dI.d, \VAR{wa-nihAyaT}{wa-nihAyath [\mc]} ha_dA
al-mIl fI \textbf{al-iqti.sA.s} suds juz'.

\clearpage
\noindent wa-nufri.du _dirwaT al-mudIr
mA'ilaT 'il_A al-^simAl _hams daqA'iq wa-ni.sf al-mudIr
\VAR{al-_tAniy}{al-'awwal [\md]} mA'il 'il_A
\VARC{al-junUb}{al-junUbiy [\mb]} wa-zAwiyaT al-mIl `an sa.t.h al-mA'il
sittaT 'ajzA' wa-ni.sf wa-_tumn wa-_dirwaT al-tadwIr mA'ilaT `an
_dirwaT al-mudIr 'il_A al-junUb _hams daqA'iq wa-ni.sfh al-_tAniy
mA'il 'il_A al-^simAl `an sa.t.h al-mA'il sab`aT 'ajzA', fa-yakUn
mA'il"aN `an sa.t.h al-mudIr rub` wa-_tumn juz'. fa-'i_dA ta.harrakat
al-'aflAk 'ammA al-mA'il fa-rub` dawr wa-ka-_dalika al-.hAmil wa-'ammA
al-tadwIr fa-ni.sf dA'iraT, fa-ya.sIru mIl \VARC{al-qi.tr sittaT wa-rub`
  fa-ya.sIru}{nAqi.saT [\me,\mb]} al-qi.tr al-'awjiy mA'il"aN
sittaT wa-rub` wa-al-qi.tr al-qA'im `alayhi fI sa.t.h al-burUj.
wa-haka_dA kAn fI al-ra.sad, wa-ha_dA al-wajh hwa al-mu`tamad `alayhi
wa-lA
\VAR{yaltafitu}{taktrt [\md], taktara_tu [\mc], wa-kutiba fI
  hAmi^s [\mc] >>yaltafitu<< 'ay.d"aN\iscomplet{, .gayr maqrU' [\mb]}{}}
'il_A mA
qAlahu b.tulamiyUs bi-'an markaz al-tadwIr yakUn junUbiy"aN 'abad"aN,
fa-'innahu raja`a `an _dalika fI \textbf{al-iqti.sA.s},
fa-a`rf \fol{w 46 \md} _dalika.

wa-'ammA ta.sawwur al-ma_dhab al-_tAniy 'an \VAR{nufri.du}{tfr.d
  [\mc]} al-mA'il `al_A al-.sifaT al-ma_dkUraT al-mutaqaddamaT
bi-.hay_tu yuqA.ti` \VAR{al-muma_t_tal}{lil-muma_t_tal [\md,\mc]}
`al_A al-`uqdatayn wa-yakUn nihAyaT al-mIl al-junUbiy `inda al-'awj
\VARC{wa-al-^simAliyy}{wa-al-^simAl [\mb]} `inda \fol{.z 35 \ma}
al-.ha.dI.d; \fol{.z 38 \mc}
wa-nufri.du markaz al-tadwIr fI al-'awj fI munta.saf mA bayna
al-`uqdatayn; wa-nufri.du 'awj al-mudIr
\VAR{mA'il"aN}{mA'il \iscomplet{[\ma,\mb,\me]}{[\ma]}}
'il_A al-^simAl _hams daqA'iq wa-ni.sf al-mudIr
\VAR{al-_tAniy}{al-'awwal [\md]}
\VAR{mA'il"aN}{mA'il \iscomplet{[\ma,\mb,\mc,\me]}{[\ma,\mc]}}
'il_A al-^simAl wa-ni.sfh al-'A_har mA'il"aN 'il_A al-junUb wa-miqdAr zAwiyaT
ha_dA al-mIl sittaT 'ajzA' wa-ni.sf juz', wa-y`rf \textbf{bi-mIl al-wrAb};
\VARC{wa-nufri.du}{wa-y`rf [\me]} _dirwaT al-tadwIr mA'ilaT `an
_dirwaT al-mudIr 'il_A al-junUb _hams daqA'iq, fa-yakUn al-qi.tr
al-'awjiy fI sa.t.h al-mA'il; wa-nufri.du ni.sf al-tadwIr al-_tAniy
\VAR{mA'il"aN}{mA'il \iscomplet{[\ma,\mb,\me]}{[\ma]}}
`an sa.t.h al-mA'il sittaT 'ajzA'
wa-ni.sf. wa-'i_dA ta.sawwarta _dalika, _tumma ta.harrakta al-'aflAk
'il_A 'an .sAra markaz al-tadwIr fI al-`uqdaT, .tAbaq al-qi.tr al-qA'im
`al_A al-'awjiy li-sa.t.h al-burUj, wa-baq_A al-qi.tr
\VARC{al-'awjiy}{al-qA'im `l_A al-'awjiy [\me]}
\VAR{mA'il"aN}{mA'il \iscomplet{[\ma,\mb,\me]}{[\ma]}}
`an sa.t.h al-burUj sittaT 'ajzA' wa-ni.sf juz'
wa-yakUn al-ni.sf alla_dI fIhi \VARC{'awjh}{al-'awj 'awjh [\me]}
\VAR{junUbiy"aN}{junUbiy \iscomplet{[\ma,\mb,\mc,\me]}{[\ma,\mc]}}
wa-al-'A_har
\VAR{^simAliyy"aN}{^simAliyy \iscomplet{[\ma,\mb,\mc,\me]}{[\ma,\mc]}}.
haka_dA yjb ta.sawwur .harakAt
al-kawAkib fI al-`r.d bi.hay_tu lA t_hll bi-al-.harakAt
\VAR{al-.tUliyaT}{al-.tUylaT \iscomplet{[\md,\me,\mb]}{[\md]}}.

\clearpage

\begin{center}
\large tanbIh
\end{center}
muqta.d_A \VARC{far.d}{frU.d [\me]} al-'aflAk fI su.tU.h
al-.hawAmil fI \VARC{al-'a.sl}{al-'u.sUl [\mb]} lA
\VAR{y_hillu}{t_hll [\mc]} bi-al-.harakAt
al-.tUliyaT bi-mA lahu
\VAR{ka_tIr}{kabIr \iscomplet{[\md,\me,\mb]}{[\md]}}
qadr wa-'ant ta`lm 'anna _dalika \VAR{bim_tl}{mum_tl bi-mi_tl [\mc]} nql
\VAR{mqwm}{fI hAmi^s [\ma]\iscomplet{, muqaddam [\me]}{}}
al-qamar min al-mA'il 'il_A al-muma_t_tal. wa-lamA kAna nihAyaT `ar.d
al-qamar _hamsaT 'ajzA' wa-kAna nihAyaT al-i_htilAf lil-naql sitt
daqA'iq wa-_tul_tay, kAna 'ak_tar mA y_hll bi-'ihmAl al-naql min
\VAR{al-mudA'ir}{al-mdAr \iscomplet{[\md,\me,\mc,\mb]}{[\md,\mc]}}
\VARC{al-`r.diy}{al-`r.d [\mb]} 'il_A min.taqaT al-burUj 'ak_tarh
likull darjaT min al-`ar.d daqIqaT wa-_tul_t wa-ha_dA miqdAr ysIr.

wa-'in ^si't fa-anql, wa-.tarIq _dalika 'an ta'_hu_du bu`d muqawwam
al-kawkab min ra's _dalika al-kawkab, wa-hwa al-`uqdaT al-^simAliyaT;
fa-mA .ha.sala \VAR{fa-_hu_d}{_hu_d [\md,\mc]} mA yuqAbiluhu min
jadwal ta`dIl \VARC{naql}{nAqi.saT [\me,\mb]} al-qamar min al-ta`dIl,
fa-mA kAna \VAR{fa-u.drubhu}{u.drubhu [\mc]} fI `ar.d _dalika
al-kawkab, fa-mA bala.ga \VAR{fa-aqsamhu}{aqsamhu [\mc]} `al_A nihAyaT
`ar.d al-qamar, wa-hwa _hamsaT 'ajzA'; famA _haraja fa-hwa al-ta`dIl
fa-zadh `al_A taqwIm al-kawkab, 'in kAna al-`adad alla_dI da_halta bihi
'il_A al-jadwal 'ak_tar min tis`In juz'"aN 'il_A mi'aT wa-_tamAnIn 'aw
'ak_tar min mi'atayn wa-sab`In \VARC{'il_A _talA_ta-mi'aT
  wa-sittIn}{nAqi.saT [\me]}; wa-'in \VARC{kAna}{nAqi.saT
  [\me,\mb]} .gayr _dalika, fa-nq.sh min taqwIm al-kawkab, ybq_A
al-muqawwam al-mu.haqqaq min falak al-burUj wa-'ak_tarh fI an.sAf
al-arbA` wa-yan`adimu fI al-`uqdatayn \VARC{wa-`inda}{'aw `inda
  [\me,\mb]} nihAyaT al-`ar.d \fol{w 39 \mc} fI
  al-jihatayn -- wa-al-ll_ah ta`Al_A 'a`lam.

\clearpage
\begin{center}
\Large al-bAb al-sAdis wa-al-`i^srUn

\large fI sabab sur`aT al-kawAkib wa-bu.tu'i-hA wa-wuqUfihA wa-rujU`ihA
\end{center}
qad tqaddam 'anna markaz al-tadwIr `al_A mu.hI.t al-mA'il, wa-.harakaT
al-mA'il 'il_A al-tawAlI, wa-.harakaT al-tadwIr fI 'a`lAhi 'il_A
al-tawAlI 'ay.d"aN. \fol{w 36 \ma}
fa-'i_dA kAna al-kawkab fI al-ni.sf al-'a`l_A min
al-tadwIr, kAnat .harakaT al-tadwIr wa-al-mA'il 'il_A al-tawAlI,
fa-ya.h.sulu lil-kawkab sur`aT li-ijtimA` al-.harakatayn 'il_A jihaTiN
wA.hidaTiN. wa-'i_dA kAna fI al-ni.sf al-'asfal min al-tadwIr, kAnat
.harakaT al-tadwIr 'il_A _hilAf jihaT .harakaT al-mA'il. fa-'i_dA sAwat
zAwiyaT .harakaT al-mA'il li-zAwiyaT .harakaT al-tadwIr fI al-yawm,
r"u'iya al-kawkab \VAR{wAqif}{wAqif"aN [\md,\mc]};
fa-'in zAdat zAwiyaT al-tadwIr `al_A zAwiyaT
al-mA'il, r"u'iya al-kawkab \VAR{rAji`}{rAji`"aN [\md,\mc]} bi-qadr
al-ziyAdaT; wa-'in naqa.sat
zAwiyaT al-tadwIr `an zAwiyaT al-mA'il fI .harakaT yawm, r"u'iya
al-kawkab \VAR{mustaqIm}{mustaqIm"aN [\md,\mc]} bi-qadr fa.dl al-zAwiyatayn.

wa-'i_dA .sawarnA falak tadwIr, wa-'a_hrajnA 'il_A markazihi _ha.t.t"aN
mustaqIm"aN min markaz falak al-burUj `al_A ha_dihi al-.sUraT, fa-lA
\VAR{ta_hlU}{ta_hlUA [\ma]} 'an takUn nisbaT .harakaT al-tadwIr 'il_A
.harakaT al-mA'il 'ammA 'a.s.gar min nisbaT al-_ha.t.t al-wA.sil bayna
markaz al-mA'il wa-bayna .ha.dI.d al-tadwIr 'il_A ni.sf qi.tr\fol{.z 46 \md}
al-tadwIr, wa-'ammA musAwiyaT la-hA, wa-'ammA 'ak_tar min-hA.

\textbf{fa-'in kAnat 'a.s.gar} fa-lA y.hd_t lil-kawkab bi-sabab
al-.harakatayn 'illA
al-sur`aT fI al-qi.t`aT al-ba`IdaT wa-al-bu.tu'u fI al-qi.t`aT
al-qarIbaT, li-'anna al-.harakaT fI al-qi.t`aT al-ba`IdaT majmU`
al-.harakatayn, wa-fI al-qarIbaT fa.dl .harakaT al-mA'il `al_A .harakaT
al-tadwIr. wa-'innamA lA y.hd_t lil-kawkab
\VAR{al-wuqUf wa-al-rujU`}{al-rujU` wa-al-wuqUf [\mc]},
li-tawaqquf \VAR{al-wuqUf}{al-wqf [\mc]} `al_A wujUd
\VAR{nisbaT}{nisbath [\md,\mc]} fI al-_hu.tU.t al-ma_dkUraT
musAwiyaT ka-nisbaT al-.harakatayn, wa-al-rujU` mawuqUf `al_A wujUd
nisbaT 'a.s.gar ma`a 'an wjdAn mi_tlhA mu.hAl li-'annahA 'a.s.gar min
'a.s.gar tilka al-nsb falA yUjid mi_tluhA wa-lA 'a.s.gar minhA.

\textbf{wa-'in kAnat al-nisbaT musAwiyaT} .hd_t lil-kawkab fI munta.saf zamAn
al-bu.tu'i wuqUf, wa-hwa `inda kawnihi fI al-ba`d al-'aqrab `al_A
al-_ha.t.t al-ma_dkUr.

\clearpage
\noindent fa-lA\fol{.z 39 \mc} yakUn la-hu rujU`,
\VAR{li-tawaqquf}{li-tawaffuq [\ma]} al-rujU` `al_A wujUd
\VAR{nisbaT}{nisbath [\mc]} min al-_hu.tU.t 'a.s.gar\fol{.z 36 \ma}
min nisbaT al-.harakatayn, la-kin ha_dihi al-nisbaT,
\VAR{li-musAwAtihA}{li-musAw_AhA [\md]} li-'a.s.gar tilka al-nsb, takUn
'a.s.gar min-hA mumtan`: li-'anna 'a.s.gar al-nsb fI al-tadwIr `inda
murUr al-_ha.t.t \VAR{bi-markazihi}{markazihi [\md,\mc]}.
fa-lA yakUn lil-kawkab rujU`.

\textbf{wa-'in kAnat al-nisbaT 'ak_tar} .hd_t lil-kawkab rujU` fI al-qi.t`aT
al-qarIbaT, bayna wuqUfayn. wa-yakUn \VAR{maw.dU`}{maw.d` [\md]} al-wuqUfayn
`inda al-_ha.t.tayn al-_hArijayn min markaz al-burUj 'il_A janbatay
al-tadwIr, bi-.hay_tu yakUn nisbaT .harakaT al-tadwIr 'il_A .harakaT
al-mA'il musAwiyaT li-nisbaT mA waqa`a min kull wA.hid min
\VAR{tilka}{ha_dayna [\md,\mc]}
al-_ha.t.tayn bayna markaz al-mA'il wa-mu.hI.t al-tadwir min jihaT
al-.ha.dI.d 'il_A ni.sf al-watar al-wAqi` min tilka al-_ha.t.tayn fI
al-tadwIr. fa-yakUn lil-kawkab, `inda wu.sUlihi fI al-qi.t`aT al-qarIbaT
'il_A 'awwal al-_ha.t.tayn (wa-yuqAlu lahu al-maqAm al-'awwal), wa-yqAl
'anna al-kawkab \textbf{muqIm lil-rujU`}: wAqif ba`da bu.tu'i
\VAR{mutdrj}{mundaraj [\mc]} wa-min-hi,
'il_A wu.sUlihi 'il_A al-_ha.t.t al-_tAniy, rAji`"aN rujU`"aN
\VAR{mutadarrj"aN}{mundaraj"aN [\md,\mc]}
min bu.tu'i 'il_A sur`aT sIr .gAyatihi fI al-bu`d al-'aqrab,
_tumma min-hA 'il_A bu.tu' yntahI `inda al-_ha.t.t al-_tAniy,
wa-`indahu al-maqAm al-_tAniy, wa-hunAk yuqAlu 'anna al-kawkab
\textbf{muqIm lil-istiqAmaT} \VAR{wAqif"aN}{wAqif [\md]} wuqUf"aN _tAniy"aN.
wa-mA bayna al-_ha.t.tayn min jihaT al-.ha.dI.d yqAlu lahu
\textbf{qaws al-rujU`}, wa-mA bayna al-_ha.t.tayn min jihaT 'awj al-tadwIr
al-mar'iy yuqAlu lahu \textbf{qaws al-'istiqAmaT}.
wa-ba`da al-wuqUf al-_tAniy, yastaqImu \VAR{mutadarrj"aN}{mundaraj"aN [\mc]}
min wuqUf 'il_A bu.tu'i sIr, _tumma 'il_A tws.t sIr, _tumma 'il_A sur`aT sIr.
wa-yakUn al-sIrAn al-mutawass.tAn bayna al-bu.tu'i wa-al-sur`aT, `inda
al-bu`dayn al-'aws.tayn min al-tadwIr. wa-'asra` al-istiqAmaT `inda
al-_dirwaT al-mar'iyyaT \VAR{fI}{nAqi.saT [\ma]} munta.sf qaws al-istiqAmaT.
wa-'asra` al-rujU` `inda al-.ha.dI.d al-mar'iyy, fI munta.sf qaws al-rujU`.

\clearpage

wa-kawn nisbaT mA bayna markaz al-burUj wa-.ha.dI.d tadwIr al-qamar
'aw al-^sams 'il_A ni.sf qi.tr al-tadwIr \VAR{'ak_tar}{'a.s.gar [\ma,\md,\mc]}
min nisbaT .harakaT al-tadwIr 'il_A .harakaT al-mA'il,
lA yakUn li-'i.hdAhunna rujU` wa-lA
wuqUf, bal bu.tu'u wa-sur`aT, `al_A mA
\VAR{'aw.da.htu}{'aw.da.hnA [\mc]}\fol{w 40 \mc} laka. wa-al-.dAb.t hiya
al-nisbaT al-mutaqaddmaT. wa-i`lam 'anna al-rujU` wa-al-istiqAmaT
murakkbaT min al-zawAyA al-munfa`alaT `an al-.harakAt al-mustawiyaT.
fa-tasqu.tu al-'aqall min al-'ak_tar: fa-'in zAda mA 'il_A al-tawAlI,
fa-'inna al-kawkab mustaqIm,\fol{w 57 \md} wa-'in nq.s, kAna rAji`"aN.
wa-'in \VAR{takifAni}{takifA [\md,\mc]} al-zA'id bi-al-nAqi.s,
r"u'iya al-kawkab wAqif"aN.

\textbf{tanbIh}. al-_talA_taT al-`alwiyaT tqArn al-^sams fI _drI al-tadAwIr
(wa-tsmm_A .harIq"aN), wa-tqAbilhA fI .ha.dI.dAt al-tadAwIr.
wa-al-safliyaT tqArn al-^sams fI\fol{w 37 \ma} _drI al-tadAwIr wa-.ha.dA'i.dhA
(wa-tsamm_A .harIq"aN 'ay.d"aN). wa-al-ll_ah t`Al_A 'a`lam.

\clearpage
\begin{center}
\Large al-bAb al-sAbi` wa-al-`i^srUn

\large fi .zuhUrAt al-kawAkib al-_hamsaT al-muta.hayyiraT wa-i_htifA'ihA
\end{center}
'ammA \textbf{al-_talA_taT al-`alwiyyaT} \VAR{fa-'inna}{fa-inh [\md,\mc]},
'i_dA kAna in.hi.tA.t
al-^sams ta.hta al-'ufuq `inda al-.tulU` li-zu.hal \aemph{_AA 0}
wa-lil-mu^stariy \aemph{y 0} wa-lil-mirrI_h \aemph{yA l}, kAnat
\VAR{fI}{nAqi.saT [\md,\mc]} .hudUd .zuhUrihA.

wa-.zuhUr ha_dihi al-kawAkib 'i_dA kAnat fI muqAbilaT al-^sams,
fa-'inna qaws al-ru'yaT yakUn qadr al-ni.sf min al-qs_A al-ma_dkUraT.

wa-'ammA \textbf{al-zuhraT wa-`.tArad} fa-qaws ru'yatihimA, li-'awwal
.zuhUrihimA bi-al-`a^siyyAt (wa-'A_hir ru'yatihimA bi-al-.gdwAt), sab`aT
'ajzA' lil-zuhraT wa-'i_tnA `a^sar juz'"aN li-`.tArad. wa-qaws ru'yaT
al-zuhraT wa-`.tArad li-.zuhUrihimA \VAR{bi-.gdwAt}{bi-al-.gdwAt [\md,\mc]}
(wa-'A_hir ru'yatihimA bi-al-`a^siyyAt) lil-zuhraT _hamsaT 'ajzA'
wa-li-`.tArad sab`aT 'ajzA'.
wa-'ammA sabab nuqu.s al-qawsayn, fa-li-kawn ha_dayni al-kawkabayn
.hayna'i_d"iN qarIbayna min .ha.dI.d al-tadwIr al-mwjb `.zm
\VAR{jarimayhimA}{juz' minhmA [\md,\mc], wa-kutiba >>jrmhmA<< fI hAmi^s
[\md]}.

wa-ha_dihi al-.hudUd 'i_dA kAna markaz al-tadwIr fI al-bu`d al-aws.t;
wa-y_htalifu bi-i_htilAf _dalika wa-i_htilAf `urU.d al-kawAkib wa-min
asbAb 'u_har. 'aw.da.hnA _dalika ma`a tafrI`At ha_dA al-kitAb fI
kitAbiy al-msm_A \textbf{bi-ta`lIq al-'ar.sAd}.

\clearpage
\begin{center}
\Large al-bAb al-_tAmin wa-al-`i^srUn

\large \VAR{fI sabab _husUf al-qamar
  wa-kusUf al-^sams wa-fIhi fa.slAni}{fI al-hAmi^s [\ma]}
\end{center}

\begin{center}
\large \VAR{al-fa.sl al-'awwal}{fI al-hAmi^s [\ma]}

\normalsize fI sabab _husUf al-qamar
\end{center}
qad _tabata 'anna al-qamar jism kuriyy"uN ka_tIf mu.zlim, ta.hta nUr
al-^sams. wa-lA \VAR{yanqulu}{ynfd [\md,\mc]} ^si`A`ahA minhu;
wa-hwa ma`a ki_tAfatihi .saqIl yn`ks `anhu ^si`A` al-^sams.
wa-yunsab al-.daw' 'ilayhi, wa-hwa fI
al-.haqIq ^si`A` al-^sams al-mun`akas min jarim al-qamar. fa-yakUn
al-wajh al-muqAbil lil-^sams nIr"aN 'abad"aN wa-al-'A_har mu.zlim"aN
'abad"aN.

fa-fI 'ihlAlihi yakUn al-mar'iy minh\fol{.z 40 \mc} miqdAr mA in.hrafahu
al-ni.sf al-mu.diy al-muqAbil lil-^sams. wa-fI kull laylaT"iN yazdAdu
al-in.hirAf 'il_A al-muqAbilaT; fa-yakUn al-wajh al-muqAbil lil-^sams
\VAR{mar'iy"uN}{mariy"aN [\mc]} bi-'asrh li-tawassu.t al-ba.sir bayna
al-nIrayn. _tumma ya`Udu al-'amr: fa-yanqu.s al-mar'iy min al-nIr 'il_A
ijtimA` al-nIrayn. _tumma ya`Udu al-'amr min al-'awwal.

wa-'ammA sabab al-_husUf fI al-qamar fa-hwa du_hUlihi fI ma_hrU.t
\VAR{.zll al-'ar.d}{al-.zll [\mc]}.
wa-lA yakUn _dalika 'illA fI muqAbilaT al-nIrayn.

\VAR{^sr.t}{bi-^sr.t [\mc]} 'A_har wa-hwa 'an yakUn `ar.dahu 'aqall min
_talA_taT wa-sittIn daqIqaT. fa-'in kAna `ar.dahu mi_tl _dalika,
mAss li-ma_hrU.t .zill al-'ar.d wa-lA yaqa` fIhi.
wa-'in nq.s `n _dalika,\fol{.z 37 \ma} da_hala fI ma_hrU.t
.zill al-'ar.d: \VAR{wa-in_hasafa minhi miqdAr mA yad_hul minhi fI
  ma_hrU.t .zill al-'ar.d}{fI al-hAmi^s [\ma], wa-in_fasafa minhi miqdAr mA
  yad_hul fI ma_hrU.t .zill al-'ar.d [\md,\mc]}. wa-'in zAda al-`ar.d
`an darjaT wa-_talA_taT daqA'iq, lam yata_hassaf wa-nafa_da .dU
al-^sams 'il_A sa.t.hihi fa-ru'y `al_A `Adatihi \VAR{nIr}{nIrA [\mc]}.

wa-al-.dAbi.t 'anna `ar.d al-qamar `inda muqAbilaT al-^sams: 'ammA 'in
yakUn 'ak_tar min ni.sfay qi.tray al-qamar wa-.zill al-'ar.d fa-lA
taqa` lil-qamar _husUf. wa-'ammA 'in yakUn musAwiy"aN li-ni.sf
al-qi.trayn \VAR{fa-yamAs}{fI-mA bayna [\mc]} al-qamar mu.hI.t dA'iraT
al-.zill, min _hArij, min jihaT `ar.d al-qamar, wa-lA yan_hasafu
\VAR{'ay.d"aN}{abad"aN [\mc]}. wa-'ammA 'in yakUn
al-`ar.d 'aqall min ni.sf al-qi.trayn wa-.hayna'i_d"iN yan_hasafu.

\clearpage
\noindent lakin 'in kAna al-`ar.d
\VAR{'ak_tar}{'aqall [\ma,\md,\mc], wa-kutiba
>>'ak_tar<< fI hAmi^s [\mc]} min ni.sf qi.tr al-.zill,
in_hasafa minh 'aqall min ni.sfh; \VARX{wa-'in kAna musAwiy"aN}{lahu,
marrat dA'iraT al-.zill bi-markaz .saf.haT al-qamar}{wa-in_hasafa
ni.sfh}{nAqi.saT [\md,\mc], wa-kutiba fI hAmi^s [\mc] >>wa-'in kAna al-`ar.d
musAwiy"aN li-ni.sf qi.tr al-.zill in_hasafa ni.sf jarim al-qamar<<};
wa-'in kAna al-`ar.d 'aqall min ni.sf qi.tr al-.zill wa-'ak_tar
min fa.dl ni.sf qi.tr al-.zill `al_A ni.sf qi.tr al-qamar,\fol{.z 47 \md}
in_hasafa minh 'ak_tar min ni.sfh; wa-'in kAna musAwiy"aN li-fa.dl ni.sf qi.tr
al-.zill `al_A ni.sf qi.tr al-qamar mAss al-qamar mu.hI.t dA'iraT
al-.zill, min dA_hil, `al_A nuq.taT min jihaT `ar.dihi, wa-in_hasafa
kullh wa-lam \VAR{yumkin}{ykn [\mc]} lahu mak_t fI al-_husUf;
wa-'in kAna al-`ar.d 'aqall min ha_dA al-fa.dl,
in_hasafa kullh wa-maka_ta bi-.hsb mA yaqa` fI dA'iraT al-.zill.
wa-.gAyath 'in yamurru markaz jarim al-qamar, fI
wasa.t zamAn al-_husUf, `al_A markaz dA'iraT al-.zill -- wa-al-mak_t 'an
yabq_A jarimh zamAn"aN ma_hsUf"aN m.zlm"aN, wa-_dalika bi-qadr mA yq.t`
al-qamar bi-fa.dl sIrh `al_A sIr al-^sams mA waqa`a dA_hila dA'iraT
al-.zill min .tarIq al-^sams.

wa-yakUn bad'u al-.zilAm wa-al-injila' min nA.hiyaT al-ma^sraq
wa-al-junUb 'in kAna `ar.d al-qamar ^simAliy"aN, wa-min nA.hiyaT
al-ma^sraq wa-al-^simAl 'in kAna al-`ar.d junUbiy"aN, wa-'in lam yakun
lahu `ar.d\fol{w 41 \mc} fa-.hA_diy darjaT al-.tAli`.

wa-al-m.zlm min al-qamar 'abad"aN _dU .hdbatayn i.hdhumA (wa-hiya
allatI fI _hilAf jihaT al-`ar.d) min al-qamar, wa-al-.hdbaT al-'u_hr_A
min dA'iraT al-.zill. wa-al-mustanIr minh 'abad"aN hilAliy al-^sakl
ma.hdabh min al-qamar wa-maq`arh min dA'iraT al-.zill.

\begin{center}
\large al-fa.sl al-_tAniy

\normalsize fI sabab kusUf al-^sams
\end{center}
wa-hwa `dm 'i.dA'aT al-^sams `al_A al-`anA.sr mimmA yalaynA, fI al-waqt
alla_dI \VAR{fI}{min [\md,\mc]} ^sa'nihi ta.d_A fIhi.

wa-sababuhu tawassu.t al-qamar \VAR{baynanA ay}{nAqi.saT [\ma]}
bayna al-ba.sir wa-al-^sams: fa-ya.hjubu
nUr al-^sams `an al-ba.sir li-ka_tAfatihi. fa-'i_dA qa.ta`a al-masAfaT
allatI bayna al-ba.sir wa-al-^sams bi-.harakatihi, zAla al-kusUf.
\VAR{wa-yaqa`u}{wa-hwa yaqa`u [\md]}
_dalika fI al-'ijtimA`At al-nahAriyaT allatI yakUn al-qamar
fIhA `al_A mu.hA_dAT al-^sams wa-al-ba.sir. wa-'i_dA lam yad_hul fI
mu.hA_dAT al-ba.sir lil-^sams, lam yankasaf al-^sams fI _dalika
al-'ijtimA`.

\clearpage

wa-al-mu`tabar\fol{w 38 \ma} hwa al-'ijtimA` al-mar'iyy al-mu`addal
bi-'i_htilAf al-mn.zr:
famin hunA y`lm 'annahu \VAR{yumkin 'an}{nAqi.saT [\mc]} yq` kusUf
bi-al-qiyAs 'il_A qawm dUn
'A_harIn ma`a kawn al-^sams fawqa 'ufuq kull minhumA, wa-_dalika
li-'i_htilAf \VAR{wa.d`}{mw.d` [\md,\mc]} al-qamar
\VAR{min al-'ab.sAr}{fI al-am.sAr [\mc]} bi-'i_htilAf al-masAkin.
wa-y_htalifu bi-'i_htilAf al-bilAd: \VAR{Amkn}{nAqi.saT [\md,\mc]}
'an yankasaf fI balad"iN wa-lA yankasf fI al-'A_har, 'aw tankasf
fI al-'A_har lakin y_htalifAni
\VAR{qdr"aN 'aw jihaT 'aw zamAn"aN}{qdr"aN wa-jihaT"aN wa-zamAn"aN [\md,\mc]}.

wa-i`lam 'an qi.tray al-nIrayn 'ammA 'an yatasAwiyA fI al-mn.zr, 'aw
ya_htalifA. fa-'in tasAwiyA, fa-al-`ar.d al-mar'iy alla_dI hwa 'aqall
min ni.sf qi.tray al-nIrayn ykUn musAwiy"aN li-ni.sf qi.tr al-^sams,
fa-ynkasf ni.sfhA; 'aw ak_tar minh, fa-ynksf 'aqall min al-ni.sf; 'aw
'aqall, fa-ynksf 'ak_tar min al-ni.sf; wa-'in lam ybq al-`ar.d al-mar'iy,
inkasafa kullahA wa-lA yakUn lahA mak_t. wa-'in i_htalafa qi.tray
al-nIrayn bi-al-n.zr? wa-kAna qi.tr al-^sams 'a`.zam fI al-ru'yaT min
qi.tr al-qamar \VAR{bi-al-ru'yaT}{nAqi.saT [\md,\mc]}; fa-al-`ar.d
al-mar'iy al-ma_dkUr 'in kAna 'ak_tar min ni.sf qi.tr al-^sams,
inkasafa minhA 'aqall min al-ni.sf; wa-ka_dA 'in kAna musAwiy"aN lahu,
\VAR{inkasafa minh}{nAqi.saT [\mc]} 'aqall min ni.sfhA,
_Aqadr ziyAdaT ni.sf qi.trhA `al_A ni.sf qi.tr al-qamar; wa-'in kAna
'aqall minh wa-musAwiy"aN li-fa.dl \VAR{ni.sf}{nAqi.saT [\md,\mc]} qi.tr
al-^sams `al_A ni.sf qi.tr al-qamar, \VAR{mAss}{mA bayna [\mc]}
al-qamar min dA_hil mu.hI.t dA'iraT al-^sams
wa-baq_A minhA .halaqaT nUrAniyaT hilAliyaT \fol{.z 41 \mc} al-^sakl;
wa-'in lam ybq lil-qamar `ar.d mar'iy 'albattaT, fI wasa.t zamAn
al-kusUf .sArat
al-.halaqaT mustadIraT, .hawla jarim al-qamar, 'istidAraTi mutasAwiyaT;
wa-'in kAna bayna hAtayn al-.hAlatayn; .sArat mu_htalifaT
\VAR{al-na.ht}{al-^sakl lA hilAliyaT wa-lA mustadIraT tAmaT [\md,\mc]}.
wa-yakUn .gal.z al-nUr fIhA wa-fI al-hilAliyaT 'il_A _hilAf jihaT
al-`ar.d al-mar'iy. wa-'in kAna qi.tr al-qamar fI al-ru'yaT 'a`.zam min
qi.tr al-^sams, fa-al-mar'iy al-ma_dkUr 'in kAna musAwiy"aN li-ni.sf
qi.tr al-qamar, inkasafa minhA ni.sfhA li-murUr mu.hI.t al-qamar
bi-markaz al-^sams; wa-'in kAna 'ak_tar minh, inkasafa minhA 'aqall min
al-ni.sf; wa-'in kAna 'aqall minh \VAR{wa-kAna}{kAna [\md]}
musAwiy"aN li-fa.dl ni.sf
qi.tr al-qamar `al_A ni.sf qi.tr al-^sams,
\VAR{inkasafa}{inkasafat [\md,\mc]} kullhA wa-lam yakun
lahA mak_t; wa-'in kAna 'aqall min al-fa.dl 'ay.d"aN, maka_tat bi.hsb
_dalika; wa-.gAyath 'in lA ybq_A lil-qamar fI wasa.t zamAn al-kusUf
`ar.d mar'iy"uN 'albattaT, wa-hwa yqdr mA yq.t` al-qamar bi-sabqihi
fa.dl qi.trh `al_A qi.tr al-^sams. wa-al-ll_ah 'a`lam bi-_dlika.

\clearpage
\begin{center}
\Large al-bAb al-tAsi`a wa-al-`i^srUn

\large fI 'azmAn mA bayna al-_husUfIn wa-al-kusUfIn wa-fIhi fa.slAn
\end{center}

\begin{center}
\large al-fa.sl\fol{w 48 \md} al-'awwal

\normalsize fI 'azmAn mA bayna al-_husUfayn
\end{center}
i`lam 'an .hudUd
al-_husUfAt 'in yakUn `inda 'istiqbAl al-nIrayn `ar.d al-qamar 'aqall
min darjaT wa-'arba`a daqA'iq. \VAR{wa-_Awjab}{wa-mwjb [\md,\mc]}
ha_dA al-`ar.d 'an yakUn
al-bu`d min al-`uqdaT ('ay `uqdaT kAnat
\VAR{sawA' an kAna al-bu`d}{nAqi.saT [\mc], sawA' kAna al-bu`d [\md]} `al_A
al-tawAlI 'aw 'il_A _hilAfihi) 'i_tn_A `a^sara darjaT. li-anna `ar.dh
'i_dA zAda `al_A _dalika, zAda `al_A ni.sfay qi.tray al-qamar
\VAR{wa-.zill al-'ar.d}{wa-qi.tr al-.zill [\mc]}.

wa-'i_dA `arafta _dalika, fa-i`lam 'annahu lA yumkin 'an yakUn _husUfAn
baynahumA ^sahr wA.hid, li-anna .gAyaT .hdd al-_husUf, min al-.tarfayn,
lA yabla.gu _hamsaT wa-`i^srIn juz'"aN, wa-al-^sams fI muddaT ^sahr"iN
qmriy taq.tu`u 'ak_tar min ha_dA al-miqdAr fa-y_hruju `an .hudUd
al-_husUf.

wa-lA yumkin 'an yakUn bayna _husUfayn sab`aT 'a^shar bi-'an yakUn
al-'istiqbAl \VAR{al-_husUfay}{li-al-_husUfIn [\md,\mc]} qabla
al-wu.sUl 'il_A al-`uqdaT al-'Ul_A,
\VAR{`al_A .hadd}{`al_A _hilAf [\md,\mc]} .tarf al-.hadd, wa-al-'istiqbAl
al-'A_har ba`d al-tajAwuz
`an al-`uqdaT al-_tAniyaT, ba`d sab`aT 'a^shar, li-'anna al-'istiqbAl
al-_tAniy lA yaqa` fI .hidd al-_husUf
\VAR{li-tajAwuzh}{li-tajAwuz [\md,\mc]} al-`uqdaT,
'il_A _hilAf al-tawAlI, `an al-miqdAr al-ma.hdUd\fol{w 42 \mc}
lil-_husUf. li-'anna al-^sams
tata.harrak fI sab`aT 'a^shar qamriyaT qarIb"aN min mi'atayn wa-_hams
darjAt wa-limA kAnat fI al-'istiqbAl al-'awwal
\VAR{`al_A}{`an [\md,\mc]} .hidd al-_husUf
(kamA hwa al-mafrU.d), kAnat fI al-_tAniy mujAwizaT .hidd al-_husUf min
al-`uqdaT al-_tAniyaT bi-darjaT: li-annahA ba`d qi.t` 'i_tnA `a^sara
darjaT ta.silu 'il_A al-`uqdaT al-'Ul_A, wa-ba`da mi'aT wa-_tamAnIna
ta.silu 'il_A al-`uqdaT al-_tAniyaT, wa-ba`da _talA_taT `a^sar yawm"aN
tujAwiza `an .hidd al-_husUf bi-darjaT. law kAnat al-`uqdaT sAkinaT,
lakinhA muta.harrakaT"aN fI
\VAR{ha_dA}{ha_dihi [\md,\mc]} al-muddaT 'i.hd_A `a^sar darjaT 'il_A
_hilAf al-tawAlI, fa-ya.sIru al-bu`d bayna al-^sams wa-.hidd
\VAR{al-_husUf}{al-kusUf [\md,\mc]} 'i_tn_A `a^sara darjaT,
fa-min ha_dA imtana`a wuqU` _husUfayn baynahumA sab`aT 'a^shar.

wa-'ammA 'ak_tar al-wuqU`, fa-'an yakUn bayna al-_husUfayn sittaT
'a^shar, li-'intiqAl al-^sams fI ha_dihi al-muddaT min qarIb 'i.hd_A
al-`uqdatayn 'il_A qarIb al-'u_hr_A.

\clearpage

wa-yumkin 'an yaqa` bayna _husUfayn _hamsaT 'a^shar, wa-lakin 'aqall
min al-'awwal wuqU`"aN. wa-_dalika 'i_dA waqa`a 'istiqbAl
\VAR{_husUfy}{_husUfIn [\md,\mc]} ba`da
tajAwuz al-`uqdaT `al_A .tarf al-.hidd, _tumma 'istiqbAl 'A_har
\VAR{ba`da}{ba`dahu ay ba`d [\mc], ba`dahu [\md], wa-kutiba >>ay ba`d<< fI
hAmi^s [\md] ay.d"aN}
_hamsaT 'a^shar qabla al-'intihA 'il_A al-`uqdaT al-'u_hr_A. fa-'innahu
yumkin 'an yaqa`u fI .hidd al-_husUf, wa-_dalika li-.harakaT al-`uqdaT
'il_A _hilAf al-tawAlI wa-'istiqbAlhA li-maw.du` al-_husUf fI
al-muddaT _tamAniyaT 'ajzA', lakin lA yakUn 'a.had al-_husUfayn
tAmm"aN \fol{w 39 \ma} (bi-_hilAf alla_dI baynahumA sittaT 'a^shar li-jiwAz
'an yakUn \VAR{tAmmayn wa-nAqi.sayn}{.gayr maqrU` [\ma]} wa-'an yakUn
'a.hadhumA tAmm"aN wa-al-'A_har nAqi.s"aN).

\begin{center}
\large al-fa.sl al-_tAniy

\normalsize fI 'azmAn mA bayna al-kusUfayn
\end{center}
wa-yu`lam _dalika min .hudUd al-kusUfAt lakinhA laysat mutasAwiyaT min
al-jihatayn limA fI .hudUd
\VAR{al-_husUfAt}{al-kusUfAt [\md,\mc]}, li-'anna al-mu`tabar al-`ar.d
al-mir'iy (wa-fI al-_husUfAt al-`ar.d al-.haqIqiy), li-'anna 'i_htilAf
al-man.zar fI al-`ar.d yujib 'an yazAdu tAraT"aN `al_A
\VAR{`ar.d al-qamar}{al-`ar.d [\mc]},
wa-yanqu.su minh 'u_hr_A, li-ya.sIr mir'iy"aN, fa-lazima 'an yakUn
al-.hidd min al-`uqdaT fI al-jAnibayn mu_htalif bi.husb 'i_htilAf
al-man.zar fI al-baqA`.

fa-fI wasa.t al-maskUn, \VAR{jIb}{.hay_tu [\md], .hsb [\mc]}
al-`ar.d sittaT wa-_talA_tIn juz'"aN, \VAR{yakUn}{layakUn [\md,\mc]}
amkAn al-kusUf `al_A b`d .gAyath ba`d `uqdaT al-ra's 'aw qabla `uqdaT
al-_danb 'il_A _tamAniya `a^saraT darjaT, 'aw `al_A .hdd .gAyath qabla
`uqdaT al-ra's 'aw ba`da `uqdaT al-_danb
\VAR{ts`}{bi-sab` [\md,\mc]}\fol{.z 42 \mc} darjAt. li-'anna .gAyaT
'i_htilAf al-man.zar fI al-`r.d 'arba`aT wa-sittIn daqIqaT; wa-ni.sfay
qi.tray al-nIrayn 'ak_tarh 'arba`aT wa-_talA_tUn daqIqaT;
\VAR{fa-'i_dA}{wa-'i_dA [\md,\mc]} kAna
al-`ar.d \VAR{^simAl}{^simAliy [\md,\mc]} _tamAniyaT wa-tis`In daqIqaT,
wa-nuq.s minh 'i_htilAf al-man.zar, baq_A \fol{.z 48 \md}
al-`ar.d al-mir'iy 'arba`aT wa-_talA_tIn daqIqaT,
musAwiy"aN li-ni.sf al-qi.trayn, fa-yujib 'an yakUn al-'awwal .hidd
al-kusUf fI al-^simAliyaT (.hay_tu `ar.d al-qamar _tamAniyaT wa-tis`Un
daqIqaT wa-hwa ba`d `uqdaT al-ra's wa-qabl `uqdaT al-_danb
bi-_tamAniyaT `a^saraT darjaT \VAR{bi-taqrIb}{bi-al-taqrIb [\md,\mc]}).
wa-'ammA fI `ar.d al-qamar
al-junUbiy, fa-.gAyath 'arba`aT wa-_talA_tUn daqIqaT, wa-_dalika 'in
yakUn ba`da `uqdaT al-_danb wa-qabla al-ra's bi-sitt darjAt wa-ni.sf.

\clearpage

wa-'i_d taqddam _dalika, fa-i`lam \VAR{'an}{'annahu [\md,\mc]}:

-- lA yumkin 'an yakUn kusUfAni
baynahumA ^sahr wA.hid fI buq`aT wA.hidaT,

-- wa-yumkin fI buq`atayn
mu_htalifatayn fI jihaT `ar.d al-bilad.

'ammA al-'awwalu fa-li-'anna
.gAyaT al-.hidd alla_dI yumkinu fIhi al-kusUf, min qabla al-`uqdaT
wa-ba`dahA, _hamsa wa-`i^srUn darjaT, wa-al-^sams fI muddaT"iN ^sahr
qamariy tata.harrak qarIb burj, wa-hwa _talA_tUn darjaT, fa-y_hruju `an
.hidd al-kusUf fa-'imtana`a _dalika. wa-'ammA al-_tAniy, fa-'in .hkm
al-`ar.d al-junUbiy fI al-bilAd al-junUbiyaT al-`ar.d ka-.hkm al-`ar.d
al-^simAliy fI al-bilAd al-^simAliyaT al-`ar.d, fa-yakUn bayna .hidday
al-kusUfayn sittaT wa-_talA_tUn darjaT, wa-al-^sams tq.t` fI al-^sahr
_talA_tUn darjaT, fa-taqa`u fI .hidd al-kusUf.

wa-fI\fol{.z 39 \ma} buq`aT"iN wA.hidaT"iN wuqU` kusUfAn baynahumA
_hamsaT 'a^shar,
'i.hdhumA ba`da al-ra's, wa-al-'A_har qabla al-_danb; 'aw `al_A sab`aT
'a^shar, 'i.hdahumA qabla al-_danb, wa-al-'A_har ba`da al-ra's.
wa-al-'awwal 'ak_tar wuqU`"aN. wa-'ammA wuqU` bayna kusUfAni
\VAR{sittaT}{fI hAmi^s [\ma]} 'a^shar fa-lA 'i^stiba'ahu fIhi: wa-hwa
'ak_tariy"uN. wa-yumkin wuqU` _husUf wa-kusUf baynahumA ni.sf ^sahr.

wa-.hudUd al-_husUf min al-dA'iraT
\VAR{al-mArraT}{fI hAmi^s [\md], nAqi.saT [\mc]} bi-markaz al-.zill,
al-qA'imaT `al_A al-mA'il; wa-.hidd al-kusUf yakUn min al-qaws
al-mArraT bi-markaz al-qamar, al-qA'imaT `al_A al-burUj. wa-al-ll_ah
'a`lam.

\clearpage
\begin{center}
\Large al-bAb \VAR{al-muwafiy _talA_tUn}{al-_talA_tUn [\md,\me]}

\large fI ma`rifaT ^sakl al-'ar.d wa-musA.hatihA
\end{center}
qad _tbt fI `ilm al-hI'aT ba`d 'adillaT"iN 'an jumlaT al-'ar.d ma`a
al-mA' kuriyyaT, wa-'annahA fI wasa.t al-'aflAk, wa-markaz _taqlihA
mu.tAbiq li-markaz al-`Alam, _tAbitaT fI al-wasa.t. laysa lahA mIl 'il_A
jAnib min al-jawAnib siw_A mA yaqta.diyhu al-'i_htilAf bayna markaz
_taqlihA wa-markaz .hajmihA. fa-yakUn 'istidAraT \fol{w 43 \mc} sa.t.h
al-'ar.d ma`a
al-mA' muwAziy"aN li-'istidAraT al-'aflAk; wa-'inna ta.dArIshA allatI
yalzamuhA min jihaT al-jibAl wa-al-'a.gwAr lA ta_hrjhA `an .hidd
al-'istidAraT, li-'anna nisbaT _dalika 'il_A `i.zm al-'ar.d
\VAR{yasIru}{yasIru jidd"aN [\mc]}
.gayr ma.hsUs. fa-'innahu
\VAR{qad tbyn 'anna jabal"aN
  yrtf`}{\iscomplet{qad buyyina 'anna jabal"aN tarbI` [\me], }{}qad
  buyyina 'anna jabal"aN yrtf` [\mc,\md]} ni.sf farsa.h, wa-_dalika
sittaT 'AlAf _dirA`. takUn nisbath `inda jumlaT al-'ar.d
\VAR{bi-_hums sb`}{bi-_hums ts` [\mc],
  .gayr maqrU' \iscomplet{[\ma,\me]}{[\ma]}}
`ar.d ^sa`IraT `inda kuraT"iN qi.trhA _dirA`;
wa-ha_dA al-miqdAr yasIru fI ha_dihi al-kuraT.

wa-i`lam 'anna al-dawA'ir al-`i.zAm allatI fI sa.t.h al-'ar.d
muwAziyaT lil-dawA'ir al-`i.zAm al-falakiyaT. allatI hiya fI sa.t.hihA
wa-tanqsm ka-inqisAmhA `al_A _talA_t-mi'aT wa-sittIn juz'"aN, wa-ysAmat
kull juz' min \VAR{al-dA'iraT}{al-dAwyr [\mc]} al-'ar.diyaT
li-na.zIrihi min al-falakiyaT.

fa-'i_dA sAra sA'ir `al_A _ha.t.t ni.sf al-nahAr fI 'ar.d"iN
mustawiyaT `al_A istiqAmh
% A39v l. 17
.hatt_A yartafi`u lahu al-qu.tb 'aw yan_hfi.du darjaT wA.hidaT,
fa-al-qadr alla_dI sArahu min tilka al-dA'iraT darjaT minhA, wa-yakUn
jumlaT mu.hI.thA _talA_t-mi'aT wa-sittIn mi_tl _dalika al-qadr alla_dI
sArahu.

\clearpage
\noindent wa-qad ru.sida _dalika 'ibar_hus wa-b.tulamiyUs .sA.hib
\textbf{al-majis.tiy} fa-wajadUA .hi.s.saT darjaT wA.hidaT min
\VAR{al-dA'iraT}{al-dawA'ir [\mc]}
al-`a.zImaT al-mutawahhamaT `al_A al-'ar.d sittaT wa-sittIn mIl"aN
wa-_tul_tay mIl, bi-al-mIl alla_dI huwa _talA_taT 'AlAf _dirA`,
bi-al-_dirA` alla_dI huwa 'i_tnAn wa-_talA_tUn
\VAR{a.sb` bi-al-a.sAbi`}{a.sb`"aN
  bi-al-a.sb` [\md,\mc]\iscomplet{, a.sb` bi-al-a.sb` [\me]}{}}
allatI hiya sitt ^sa`IrAt \fol{w 49 \md}
mu`tadilAt ma.dmUm
\VAR{.tUlu ba`.dhA li-ba`.d}{bi-.tUn ba`.dhA li-ba`.d [\md],
  bi-.tUn ba`.dhA li-.zuhUr
  ba`.d [\mc]\iscomplet{, .tUlu ba`.dhA 'il_A ba`.d [\me]}{}}.
_tumma qAma \VAR{bi-ra.sad}{yr.sd [\mc]}
_dalika .tA'ifaT min \fol{w 40 \ma} al-.hukamA fI zaman
\VARC{al-ma'mUn}{al-.hukamA [\me]}
\VAR{wa-bi-amrh fI bryaT snjAr}{.gayr maqrU' [\ma]}.
% A40r l. 1
fa-wajadUA .hi.s.saT al-darjaT
al-wA.hidaT sittaT wa-_hamsIn mIl"aN wa-_tul_tay mIl, bi-al-mIl alla_dI
hwa 'arba`aT 'AlAf _dirA`, bi-al-_dirA` alla_dI hwa 'arba`aT wa-`i^srUn
a.sba`"aN, bi-al-'a.sba` allatI hiya sitt ^sa`IrAt mu`tadalAt. wa-qad
`lmt 'an bayna al-qudamA' 'i_htilAf"aN fI al-'i.s.tilA.h `al_A
al-_dirA` wa-al-mIl wa-al-farasa_h (wa-laysa baynahum 'i_htilAf fI
al-'a.sb`): wa-'inna _dirA` al-aqdimIn _dirA` wa-_tul_t min _dirA`
al-mu.hdi_tIn, wa-al-mIl `inda al-.tA'ifatayn sittaT
\VAR{wa-tis`Un}{wa-sb`Un [\md]} 'alf
'a.sba`, wa-'innamA hwa bi-_dirA` al-'aqdimIn _talA_taT 'AlAf _dirA`,
wa-bi-_dirA` al-mu.hdi_tIn 'arba`aT 'AlAf _dirA`. wa-al-'i_htilAf fI
al-_dirA` .haqIqiy, wa-fI al-mIl laf.ziyy; wa-'ammA al-farasa_h fa-lA
_hilAf fIhi
\VAR{li-annahu}{li-'an al-farsa_h [\md,\mc]} `inda al-qudamA'
wa-al-mu.hdi_tIn _talA_taT
amyAl, fa-al-farasa_h `inda al-mu.hdi_tIn 'i_tnA-`a^sar 'alf _dirA`;
wa-qad `alamtu 'an bayna al-aqdimIn \VAR{wa-al-mu.hdi_tIn}{nAqi.saT [\mc]}
\VARC{'i_htilAf"aN fI}{'i_htilAf [\me]}
.haqIqaT qiyAs al-darjaT wa-'an _dalika
\VAR{min tafAwt al-`aml}{.gayr maqrU' [\ma]}. wa-miqdAr al-'i_htilAf
`a^saraT 'amyAl. wa-'i_d taqdm _dalika, fa-i`lam 'anna firAsa_h darjaT
wA.hidaT `inda al-aqdimIn 'i_tnAn wa-`i^srUn farsa_h"aN wa-t"us`A
farasa_h, wa-firAsa_h darjaT wA.hidaT `inda al-mu.hdi_tIn _tamAniyaT
`a^sar farasa_h"aN wa-_tamAniyaT \VAR{atsA`}{asbA` [\mc]} farasa_h.
wa-al-`amal \VAR{`al_A ma_dhab}{bi-ma_dhab [\mc]} al-qudamA' muwAfiq
lil-jumhUr.

fa-'i_dA .darabnA .hi.s.saT al-darjaT fI _talA_t-mi'aT wa-sittIn
(wa-hiya 'ajzA' dawr al-'ar.d), .ha.sala miqdAr dawr al-'ar.d: `al_A
ma_dhab al-'aqdimIn _tamAniyaT 'AlAf farasa_h, wa-`al_A ma_dhab
al-mu.hdi_tIn sittaT 'AlAf
\VARC{wa-_tamAn-mi'aT}{wa-_tamAniyaT [\me]}
farasa_h (wa-hwa yanqu.s `ammA hwa `inda al-'aqdimIn
'alf"aN wa-mi'atayn farasa_h).

\clearpage
\noindent wa-'i_dA qsm al-mu.hI.t `al_A _talA_taT
wa-sub`, .ha.sala qi.tr jumlaT \VAR{kuraT}{nAqi.saT [\md,\mc]} al-'ar.d
(ma`a al-mA'): wa-hwa `al_A
ma_dhab al-qudamA' 'alfAn wa-_hams-mi'aT wa-_hamsaT wa-'arba`Un
farasa_h"aN wa-_hamsaT 'ajzA' min 'i.hd_A `a^sar juz'"aN min farasa_h,
wa-qi.tr al-'ar.d `al_A ma_dhab al-mu.hdi_tIn 'alfAn wa-mi'aT
wa-_talA_taT wa-sittUn farasa_h"aN wa-sab`aT 'ajzA' min 'i.hd_A `a^sar
juz'"aN min farasa_h.

wa-'i_dA .drbt jumlaT al-qi.tr fI jumlaT al-dawr, .ha.sala musA.haT
kuraT al-'ar.d (ma`a al-mA'): wa-hwa `al_A ma_dhab al-'aqdimIn
\VAR{20363636}{20362636 \iscomplet{[\ma,\md,\mc,\me]}{[\ma,\md,\mc]}}
farasa_h"aN wa-'arba`aT
'ajzA' min 'i.hd_A `a^sar juz'"aN min farasa_h, wa-`al_A ma_dhab
al-mu.hdi_tIn
\VAR{14712727}{153927727 \iscomplet{[\ma,\md,\mc,\me]}{[\ma,\md,\mc]}}
farasa_h"aN wa-_talA_taT 'ajzA' min 'i.hd_A `a^sar juz'"aN min farasa_h.

wa-qad i^stahara 'anna al-maskUn rub` kuraT al-'ar.d,
wa-.tUl \fol{.z 40 \ma} al-rub` ni.sf al-mu.hI.t,
wa-`ar.duhu rub` al-mu.hI.t.

wa-musA.haT \VAR{jarim}{juz' min [\md,\mc]} jumlaT kuraT al-'ar.d
ma`a al-mA', bi-mk`b al-farasa_h \VAR{al-wA.hid}{nAqi.saT [\md,\mc]},
`al_A \VAR{ru'yaT}{ma_dhab [\md,\mc]} al-aqdimIn, 8630116345 wa-'i.hd_A
wa-`i^srIn juz'"aN wa-_tul_tay juz' \VARC{min mi'aT}{nAqi.saT [\me]}
wa-'a.had wa-`i^srIn juz'"aN min mk`b al-farasa_h (wa-hwa suds
taqrIb"aN); wa-`al_A ma_dhab al-mu.hdi_tIn bi-mk`b al-farasa_h 'ay.d"aN,
wa-hwa 5033856498 farasa_h"aN wa-'i_tnAn wa-'arba`Un juz'"aN min mi'aT
wa-'a.had wa-`i^srUn juz'"aN min muka``b al-farasa_h.

fa-'in aradta
`ilm _dalika bi-al-_dirA`, fa-'u.drub muka``ab a_dra` al-farasa_h fI
`adad farAsa_h musA.haT al-jarim. wa-'in aradta musA.haT basI.t
al-'ar.d bi-al-_dirA`, \fol{w 44 \mc} fa-u.drub murabba` `adad
a_dra` al-farasa_h fI
`adad firAsa_h musA.haT basI.t al-'ar.d; `al_A 'ay ma_dhab aradta, fa-mA
.ha.sala fa-hwa musA.haT basI.t al-'ar.d
\VAR{bi-murabba`}{li-murabba` [\md,\mc]} _dirA` wA.hid
`al_A al-ma_dhab alla_dI .hasabta `alayhi. wa-_dalika mA aradnA an
nubayyina.

\clearpage
\begin{center}
\Large al-_hAtimaT

\large  fI \fol{.z 49 \md} al-'ab`Ad wa-al-'ajrAm wa-fIhi fu.sUl 'arba`aT
\end{center}

\begin{center}
\large al-fa.sl al-'awwal

\normalsize fI ta.s.hI.h 'ab`Ad al-nIrayn min markaz al-'ar.d
\end{center}
qad _dakara b.tulamiyUs fI al-majis.tiy 'anna ni.sf qi.tr al-falak
al-mA'il lil-qamar mi_tl ni.sf qi.tr al-'ar.d tis`aT wa-_hamsUn marraT,
wa-hwa 'ab`ad bu`d markaz al-tadwIr. wa-`aml `al_A _dalika _tumma 'anna
mu.haqqaqiy ha_dA al-fann .sa.ha.hUA _dalika fI al-mudad
al-muta.tAwlaT bi-.turuq 'a.dba.t min .tarIq b.tulamiyUs: wa-_dalika
'annahum wajadUA 'i_htilAf al-man.zar al-musta`mal fI al-kusUfAt `al_A
.tarIq b.tulamiyUs \VAR{wa-fIhi}{fIhi [\ma,\md,\mc]} nq.s, fa-.ha_darUA
_dalika al-nq.s, wa-fara.dUA ni.sf qi.tr al-muma_t_tal _tamaniyaT
wa-_hamsIn marraT"aN mi_tl ni.sf qi.tr al-'ar.d. wa-`amalUA `al_A
_dalika fa-wajadUA 'i_htilAf al-man.zar muwAfiq"aN lil-ra.sad.
wa-tkrriru _dalika: fa.sa.h.h `indahum, wa-`alayhi i`tamadnA. wa-qad
baynanA 'anna ni.sf qi.tr al-tadwIr al-mar'iyy fI al-ijtimA`At
wa-al-istiqbAlAt _hamsaT 'ajzA' wa-suds juz', bi-al-'ajzA' allatI bihA
ni.sf qi.tr al-muma_t_tal sittIn juz'"aN. fa-yakUn, bi-al-'ajzA' allatI
bihA ni.sf qi.trih _tamAniyaT wa-_hamsIn, _hamsaT 'ajzA'. wa-'i_dA zyd
_dalika `al_A ni.sf qi.tr al-muma_t_tal, bala.ga _talA_taT wa-sittIn,
wa-hwa 'ab`ad bu`d al-qamar fI al-ijtimA`At wa-al-istiqbAlAt min
markaz al-'ar.d. wa-qad tu.harrir 'anna qi.tr al-qamar fI ha_dA al-bu`d
wa-hwa _talA_taT wa-sittUn juz'"aN mi_tl ni.sf qi.tr al-'ar.d (wa-hwa
al-bu`d al-'ab`ad fI al-ijtimA`At wa-al-istiqbAlAt) \fol{w 41 \ma}
\aemph{0 l _A.h}.

wa-qad tu.harriru bi-'ar.sAd"iN ka_tIraT 'anna qi.tr al-^sams fI
bu`dhA al-'ab`ad \aemph{k.t h}, wa-fI bu`dihA al-'awsa.t \aemph{lb lb},
wa-fI bu`dihA al-'aqrab \aemph{lw nd mA}. wa-qad _dakarnA fI hI'aT
'aflAk al-^sams 'an bu`dhA al-'aqrab \aemph{nb nj}, wa-bu`dhA
al-'awsa.t \aemph{s}, wa-bu`dhA al-'ab`ad \aemph{sz r}. wa-'i_dA qasmnA
qi.trhA fI bu`dhA al-'awsa.t `al_A bu`d al-^sams .ha.sala qi.tr
al-^sams fI _dalika al-bu`d. wa-'i_dA qasamnA qi.tr\fol{.z 44 \mc}
al-^sams fI bu`dihA al-'awsa.t `al_A qi.trhA fI waqt mafrU.d,
.ha.sala bu`d al-^sams.

\clearpage

wa-qad tu.haqqiqu mimmA qulnA anA, 'i_dA qasamnA qi.tr al-^sams fI
bu`dhA al-'awsa.t, wa-hwa \aemph{lb lb}, `al_A qi.tr al-qamar fI bu`dh
al-'ab`ad wa-hwa \aemph{l _A.h}, _haraja \aemph{sb l}, wa-hwa bu`d
\VAR{al-^sams}{al-qamar \iscomplet{[\ma,\md,\mc,\me]}{[\ma,\md,\mc]}}
min markaz falak al-burUj
fI al-waqt alla_dI yakUn qi.trh mi_tl qi.tr
\VAR{al-qamar}{al-^sams \iscomplet{[\ma,\md,\mc,\me]}{[\ma,\md,\mc]}}
fI \VAR{al-bu`d al-'ab`ad}{ha_dihi al-bu`d [\mc]} fI al-ijtimA`At
wa-al-istiqbAlAt.

wa-'i_d taqaddm _dlika fa-_A.d` al-^sakl \VARC{al-.sanUbriy}{al-.drIr_A
  [\me]}. wa-la-takun al-^sams dA'iraT \aemph{a b}, wa-markazhA
\aemph{j}, wa-kuraT al-'ar.d dA'iraT \aemph{d h}, wa-markazhA \aemph{r}.
\VAR{wa-latakun}{wa-layakUn [\mc]} al-ma_hrU.t al-mu.hI.t bihA
\VAR{\aemph{a n b}}{\aemph{a r b} \iscomplet{[\ma,\md,\mc,\me]}{[\ma,\md,\mc]}}
wa-shmhi \aemph{r j}. wa-latakun al-qamar dA'iraT
\aemph{.t _A .h}, wa-markazhA \aemph{_A}. wa-latakun al-ma_hrU.t
al-mu.hI.t bi-al-qamar wa-al-^sams \aemph{a r b}. wa-nf.sl \aemph{r l}
mi_tl \aemph{r y}, wa-n_hrj a`mdaT \aemph{j b} \aemph{.t _A} \aemph{r
  h} \aemph{l m} `al_A sahm al-ma_hrU.t 'a`niy _ha.t.t \aemph{n j}.
\VAR{wa-ynf_d}{wa-nb`dhA [\md,\mc]} 'il_A al-jihaT al-u_hr_A,
fa-ykUn 'iq.tAr tilka al-kurAt.
wa-i`lam 'anna al-_hu.twa.t al-mArraT bi-maw.du` al-mumAssaT
min kull wA.hidaT min ha_dihi al-dawA'ir laysa hiya 'iq.tArhA, bal lA
frq baynhA li-b`d al-musAfaTi. wa-zAwiyaT \aemph{a r b} hiya
al-mu.hI.taT bi-al-^sams wa-al-qamar waqt \VARC{kawn}{_AkUn [\me]}
bu`dh min al-'ar.d _talA_taT wa-sittIn. wa-qad qulnA 'an qi.tr al-qamar
fI ha_dA al-maw.du` \aemph{l _A.h}, fana.sifuhu
\VAR{\aemph{y .t}}{\aemph{_Ah .t} [\md,\mc]} wa-hwa
zAwiyaT \aemph{y r .t}; wa-nisbaT \aemph{r y} (wa-hwa _talA_taT
wa-sittUn) 'il_A \aemph{y .t} ka-nisbaT jIb zAwiyaT \aemph{.t y r}
'il_A jIb zAwiyaT \aemph{y r .t}; fa-ya.sIr \aemph{y .t} ma`lUm"aN.

wa-.hisAbuhu, 'an ta'_hu_d jIb zAwiyaT \aemph{y r .t}, wa-hwa ni.sf
qi.tr al-qamar, fa-kAna \aemph{_Ah nA nd}. fa-.darabnAh fI \aemph{r y}
wa-hwa \fol{w 50 \md} _talA_taT wa-sittUn mn.h.t"aN. \fol{w 45 \mc}
fa-.ha.sal \aemph{_Aw l.t k.t mb}, wa-hwa _ha.t.t \aemph{y .t},
'a`niy ni.sf qi.tr al-qamar bi-mA\fol{.z 41 \ma} bihi
ni.sf qi.tr al-'ar.d wA.hid"aN. fa-.darabnAh fI nisbaT al-.zill, wa-hwa
`al_A mA \VAR{ta.haqqaqat}{ta.haqaqa [\mc]} bi-'ar.sAd"iN ka_tIraT
marratayn wa-_talA_taT wa-'arba`In daqIqaT fI ha_dA al-bu`d.
ya.h.sulu ni.sf qi.tr al-.zill.

wa-'ay.d"aN _ha.t.t \aemph{l r} mi_tl _ha.t.t \aemph{r y}, wa-_hu.twa.t
\aemph{l m} \aemph{r h} \aemph{y k} 'a`midaT `al_A _ha.t.t \aemph{n j}
fa-hiya mutawAziyaT; fa-_ha.t.tA \aemph{l m} \aemph{y k} .da`f \aemph{r
  h} alla_dI hwa ni.sf qi.tr al-'ar.d wa-.da`fh mi'aT wa-`i^srUn
daqIqaT; fa-'i_dA nuqu.snA minhu ni.sf qi.tr al-.zill
\VAR{wa-al-qamar wa-_dalika}{wa-_dalika
  [\md,\mc]\iscomplet{, _dalika [\me]}{}}
\aemph{sb .t m.t kj}
\VAR{wa-tamAmh}{wa-bi-mA bihi \iscomplet{[\ma,\me]}{[\ma]}}
'il_A al-mi'aT wa-`i^srUn daqIqaT
\VAR{hwa}{wa-hwa \iscomplet{[\md,\mc,\me]}{[\md,\mc]}}
_ha.t.t \aemph{.t k} wa-hwa
\VAR{\aemph{nr n y lr}}{\aemph{_Ar n y lr} [\md],
  .gayr maqrU' \iscomplet{[\ma,\me]}{[\ma]}}.

\clearpage

wa-_ha.t.t \aemph{r h} muwAz"iN li-_ha.t.t \aemph{.t k} fa-yakUn
nisbaT \aemph{r h} 'il_A \aemph{.t k} ka-nisbaT
\VAR{\aemph{b r}}{\aemph{b d} \iscomplet{[\ma,\me]}{[\ma]},
  \aemph{n d} [\md,\mc]} 'il_A
\VAR{\aemph{b k}}{\aemph{y .t} \iscomplet{[\ma,\md,\mc,\me]}{[\ma,\md,\mc]}}
wa-kanisbaT \aemph{r j} 'il_A \aemph{j y};
fa-'i_dA ja`alnA
\VAR{\aemph{r j}}{\aemph{r y} \iscomplet{[\ma,\mc,\me]}{[\ma,\mc]}}
sittIn daqIqaT, .sAra _ha.t.t \aemph{j y} ('a`niy bu`d mA bayna
\VARC{markazay}{markaz [\me]} al-nIrayn) \aemph{nz n y lr}; wa-baq_A
_ha.t.t \aemph{y r} (alla_dI hwa bu`d mA bayna markaz al-'ar.d
wa-al-qamar) \aemph{0 b .t m.t kj} wa-nisbath 'il_A \aemph{r j}
\VARC{al-sittIn}{sittIn [\me]} daqIqaT ka-nisbaT \aemph{r y} ('a`niy
bu`d al-qamar min markaz al-'ar.d), \VARC{wa-hwa}{nAqi.saT [\me]}
_talA_taT wa-sittUn, 'il_A \aemph{r j} 'a`niy bu`d al-^sams; fa-ya.sIr
bu`dhA ma`lUm"aN.

wa-.hisAbuhu: qasamnA bu`d al-qamar, wa-hwa _talA_taT wa-sittUn, `al_A
\aemph{0 b .t m.t kj} mun.h.t"aN _haraja
\VAR{\aemph{k.t r}}{\aemph{y .t r} [\md,\mc]}. fa-.darabnAhA
fI sittIn, fa-.ha.sala 1747, wa-hwa bu`d al-^sams min markaz al-'ar.d
waqt kawn qi.trhA mi_tl qi.tr al-qamar; wa-_dalika 'i_tnAn wa-sittUn
wa-ni.sf; fa-yakUn, \fol{w 42 \ma} 'i_dA .darabnA bu`d al-^sams
al-ma_dkUr fI sittIn
wa-qasamnA al-.hA.sil `al_A al-'i_tnayn wa-al-sittIn wa-al-ni.sf,
.ha.sala 1677 wa-sab` daqA'iq wa-_hums daqIqaT, wa-hwa bu`d al-^sams
al-'awsa.t `al_A \VAR{'in}{fI hAmi^s [\ma]} ni.sf qi.tr al-'ar.d
\VAR{wA.hid}{wA.hid"aN [\mc]}.

fa-'i_dA qasamnAh `al_A sittIn, _haraja bi-al-qismaT \aemph{kr nr r yb},
wa-_dalika .hi.s.saT darjaT min ni.sf qi.tr al-muma_t_tal, 'a`niy kull
darjaT minh ha_dA al-miqdAr. fa-qad tubayin 'an 'ab`ad bu`d al-^sams
zA'id `al_A bu`dhA al-'awsa.t \aemph{r r}, fa-'i_dA .darabnA .hi.s.saT
al-darjaT fI \aemph{r r} (.h.sala 198 \aemph{nh l _Ad kd}) fa-'i_dA
zadnAh `al_A bu`d al-^sams al-'awsa.t, .ha.sala \VARC{1876 \aemph{b
    mb}}{1876 \aemph{b mb _Ad kd} [\me]} wa-hwa bu`d al-^sams
al-'ab`ad, wa-'i_dA nuqu.snA _dalika min bu`dhA
\VARC{al-'awsa.t}{al-mutawassa.t [\me]}, baq_A 1478 wa-_hums wa-hwa
bu`d al-^sams al-'aqrab.

wa-'ay.d"aN fa-'in
\VAR{nisbaT \aemph{.t _A} 'il_A \aemph{_A r}}{nisbaT \aemph{j b}
  'il_A \aemph{j y} \iscomplet{[\ma,\md,\mc,\me],
    wa-kutiba fI hAmi^s [\me] >>nisbaT \aemph{.t _A} 'il_A \aemph{_A r}<<}
  {[\ma,\md,\mc]}}
kanisbaT \aemph{j b} 'il_A \aemph{r j} fa-ya.sIr \aemph{j b} ma`lUm"aN.
wa-.hisAbh: \fol{.z 45 \mc} .darabnA \aemph{k.t r} fI ni.sf qi.tr
al-qamar wa-hwa
\aemph{_Aw l.t k.t mb} wa-qasmnA mA .h.sala `al_A bu`d al-qamar wa-hwa
_talA_taT wa-sittUn, _haraja \aemph{r mb nj} wa-hwa ni.sf qi.tr
al-^sams bi-mA bihi ni.sf qi.tr al-'ar.d \VAR{wA.hid}{wA.hid"aN [\mc]}.

\clearpage
\noindent faqad \VAR{bayin}{tabayana [\md,\mc]} 'an qi.tr
al-^sams mi_tl qi.tr al-'ar.d sab` marrAt wa-_tul_tay marraT wa-ni.sf
`u^sr marraT; wa-muka``ab _dalika 459 \aemph{.h w mr mw kh _Ar}; wa-qad
tabayinu 'an nisbaT al-kuraT 'il_A al-kuraTi ka-nisbaT muka``ab
al-qi.tr 'il_A muka``ab al-qi.tr; fa-musA.haT jarim al-^sams bi-qdr
musA.haTi jarim kuraT al-'ar.d 'arba`mi'aT marraT wa-ts`aT wa-_hamsIn
marraT wa-_tul_tay _hums marraT bi-al-taqrIb.

wa-.hisAb bu`d ra's ma_hrU.t .zill, al-'ar.d 'an nu_hriju \aemph{l s}
muwAziy"aN li-_ha.t.t \aemph{n h}; \fol{.z 50 \md}
fa-mu_talla_t \VAR{\aemph{r n h}}{\aemph{r r h} [\md,\mc]}
\VAR{t^sbIh}{^sabIh [\md,\mc]}
bi-mu_talla_t \aemph{l r s} fa-nisbaT
\VAR{\aemph{n r} 'il_A \aemph{l r}}{\aemph{b r} 'il_A \aemph{r b} [\md,\mc]}
kanisbaT \aemph{h r} 'il_A \aemph{r s}, fa-y.sIru
\VAR{\aemph{r n}}{\aemph{r b} [\md,\mc]} ma`lUm"aN.
wa-.hisAbh: 'an _ha.t.t \aemph{l m} mi_tl _ha.t.t \aemph{h s},
wa-_ha.t.t \aemph{h r} alla_dI hwa ni.sf qi.tr al-'ar.d sittUn daqIqaT;
fa-'i_dA \VARC{nuq.snA}{nuq.snAh [\me]} minh \VARC{\aemph{0 mh l _A.t
    mA}}{\aemph{0 mh l l.t mA} [\me]}, baq_A \aemph{0 _Ad k.t m
  _A.t} wa-hwa _ha.t.t \aemph{s r}. fa-qsmnA `alayhi mun.hi.t"aN bu`d
al-qamar alla_dI hwa _talA_taT wa-sittUn, _haraja 260 \aemph{mr _A.h}
wa-hwa bu`d ra's ma_hrU.t .zill al-'ar.d min markaz al-'ar.d
wa-al-^sams fI al-bu`d al-ma_dkUr. wa-ha_dA yzdAd bibu`d al-^sams min
markaz al-'ar.d, wa-yanq.s bi-qurbihA.

\clearpage

\begin{center}
\normalsize fa.sl
\end{center}
'i_dA \VARC{a.d`afnA}{.da`afnA [\me]} ni.sf qi.tr \fol{.z 42 \ma} al-qamar
(wa-hwa \aemph{0 _Aw l.t k.t mb}) .ha.sala \aemph{lj _A.h n.t kd} wa-hwa
majbUr \aemph{lj _A.t}. fa-'i_dA qasamnA `alayhi qi.tr al-'ar.d (wa-hwa
mi'aT wa-`i^srUn daqIqaT), .ha.sala \aemph{j lw w}, fa-yakUn qi.tr kuraT
al-'ar.d mi_tl qi.tr al-qamar _talA_t marrAt wa-_talA_taT a_hmAs
marraT
(\VAR{wa-ksr}{wa-^say' [\mc]\iscomplet{, wa-kasIr [\me]}{}}
yasIr jidd"aN). wa-'i_dA qasamnA
qi.tr al-^sams `al_A qi.tr al-qamar, _haraja sab`aT wa-`i^srUn
wa-'arba`aT a_hmAs; fa-qi.tr al-^sams mi_tl qi.tr al-qamar sab`aT
wa-`i^srIn marraT wa-'arba`aT a_hmAs marraT. wa-'i_dA fara.dnA qi.tr
al-qamar wA.hid"aN, kAna muka``abh wA.hid"aN, wa-al-muka``ab al-kA'in
min qi.tr al-'ar.d (\VARC{wa-hwa}{hwa [\me]} _talA_taT wa-_talA_taT
a_hmAs) hwa sittaT wa-'arba`Un wa-_tul_tAni, wa-al-muka``ab al-kA'in min
sab`aT wa-`i^srIn wa-'arba`aT a_hmAs 'a.had
\VARC{wa-`i^srIn}{wa-`i^srUn [\me]} 'alf"aN wa-'arba`mi'aT
\VARC{wa-'a.had}{'a.had [\me]} wa-_tamAnIn wa-rub`"aN bi-al-taqrIb.

fa-yjib min _dalika 'annahu, mat_A kAna mujassam al-qamar wA.hid"aN, fa-'inna
mujassam al-'ar.d yakUn sittaT wa-'arba`In wa-_tul_tayn, wa-mujassam al-^sams
yakUn 'a.had wa-`i^srIn 'alf"aN wa-'arba`mi'aT wa-'a.had wa-_tamAnIn wa-rub`"aN.
wa-mujassam al-^sams mi_tl mujassam al-'ar.d 'arba`mi'aT wa-tis`"aN wa-_hamsIn
marraT wa-_tul_tay _hums marraT bi-al-taqrIb. wa-ha_dihi al-maqAdIr lA yumkin
'an yakUn 'aqall mimmA\fol{w 46 \mc} qulnA wa-lA
\VAR{al-'ab`ad}{al-'ab`Ad [\md,\mc]}, bal yumkin 'an yakUn 'ak_tar min _dalika.
\end{arab}

\begin{figure}
\begin{center}
\tiny
\input{sapin.pdf_tex}
\end{center}
\end{figure}

\begin{arab}
\resetlinenumber\pagewiselinenumbers
\clearpage

\begin{center}
fa.sl
\end{center}
wa-`inda b.tulamiyUs 'innahu, 'i_dA kAna qi.tr al-qamar wA.hid"aN kAna
qi.tr al-'ar.d _talA_taT 'ajzA' wa-_humsay juz', wa-qi.tr al-^sams mi_tl qi.tr
al-qamar _tamAniyaT `a^saraT marraT wa-'arba`aT a_hmAs marraT; wa-inna qi.tr
al-^sams mi_tl qi.tr al-'ar.d _hams marrAt wa-ni.sf, wa-jarimhA mi_tl jarim
al-'ar.d mi'aT wa-sab`In marraT. wa-'inna 'ab`ad bu`d al-qamar 'arba`aT
wa-sittUn wa-suds, wa-bu`d al-^sams al-'awsa.t 'alf"aN wa-mi'atAn wa-`i^srUn.

\begin{center}
tanbIh
\end{center}
sabab ha_dA al-i_htilAf fI ha_dihi al-maqAdIr hwa 'annA
_hAlafnAh fI ^say' yasIr fI qi.tr al-qamar wa-qi.tr al-.zill wa-qi.tr
al-^sams. fa-'inna qi.tr al-qamar `indahu fI bu`dihi al-'ab`ad
\aemph{lA k}, wa-hwa `indanA \aemph{l _A.h}. fa-qad _hAlafanAh \VARC{fI
  qi.trh}{nAqi.saT [\me]} bi-daqIqaT wa-_tAniyatayn. wa-qi.tr
al-^sams `indahu fI sA'ir 'ab`AdhA mi_tl qi.tr al-qamar, wa-nisbaT qi.tr
.zill al-'ar.d 'il_A qi.tr al-qamar `indahu marratAni wa-_talA_taT
a_hmAs marraT, wa-`indanA\fol{w 43 \ma} marratAni wa-_talA_taT
wa-'arba`Un daqIqaT.
wa-tukarriru imti.hAn mA _hAlafanAh fIhi
\VAR{bi-mu.haqqiqiy}{li-ma.haqaq_A [\md,\mc]} ha_dA al-fann,
wa-lanA 'ay.d"aN; wa-lawu i`tamadnA `al_A nisbaT al-.zill `indahu kAna
al-_hilAf 'ak_tar, wa-'innamA waqa`a al-_hilAf bi-sabab qi.tray
al-^sams wa-al-qamar. fa-i`raf _dalika.

\begin{center}
tanbIh
\end{center}
'i_dA usqu.tnA min 'aqrab qurb al-^sams ni.sf qi.tr al-^sams
(`al_A 'anna ni.sf qi.tr al-'ar.d wA.hid"aN) wa-_dalika \aemph{r mj},
baqiy 1470 \aemph{k.t} wa-hwa 'aqrab qurb 'aflAk al-^sams. wa-'i_dA
zadnA _dalika `al_A 'ab`ad bu`dihA wa-hwa 1883 \aemph{mw}, .ha.sala
'ab`ad bu`d 'aflAkihA; wa-fawqh smk al-muma_t_tal, wa-ta.htah
itti.sAl al-falak.

\begin{center}
tanbIh
\end{center}
qad _dakarnA fI hI'aT 'aflAk al-qamar 'an 'ab`ad bu`dh fI
al-ijtimA` wa-al-istiqbAl yakUn \aemph{sh y}, wa-'aqrab qurbh fIhumA
\aemph{nd n}, wa-'ab`ad bu`dh fI al-tarbI`ayn \aemph{s.h 0}, wa-'aqrab
qurbh fIhumA \aemph{nb 0}, ha_dA `al_A 'anna al-bu`d al-'awsa.t sittUn.

\clearpage
\noindent fa-'i_dA .hawwalanA _dalika 'il_A al-'ajzA' allatI bihA ni.sf
qi.tr al-'ar.d wA.hid"aN, .ha.sala 'aqrab\fol{w 51 \md} qurbh fI al-ijtimA`
wa-al-istiqbAl \aemph{nj 0}, wa-'ab`ad bu`dh fIhimA \aemph{sj 0},
wa-'aqrab qurbh fI al-tarbI`ayn \aemph{n _Aw}, wa-'ab`ad bu`dh fIhimA
\aemph{sh md}. wa-yjb 'an yazAdu `al_A _dalika ni.sf qi.tr al-qamar,
wa-hwa \aemph{0 yw l.t l}, ybl.g \aemph{sw 0 l.t l}; wa-fawqa _dalika
sumk al-muma_t_tal.
wa-'aqrab qurbh 'i_dA usqu.tnA minh ni.sf qi.tr \fol{.z 46 \mc} al-qamar,
baqiy \aemph{m.t n.t kA}; wa-'aqall min _dalika bi-itti.sAl al-falak.

\begin{center}
\large al-fa.sl al-_tAniy

\normalsize fI ma`rifaT 'ab`Ad `.tArd wa-al-zuhraT min markaz al-'ar.d
(bi-al-'ajzA' allatI bihA ni.sf qi.tr al-'ar.d wA.hid"aN)
\end{center}
qad bayanA fI hI'aT 'aflAk `.tArd 'an nisbaT 'aqrab 'aflAkh 'il_A
'ab`ad bu`dhA ka-nisbaTi 'a.had wa-_talA_tIn 'il_A tis`aT wa-_tamAnIn
wa-ni.sf, wa-'an nisbaT 'aqrab qurb 'aflAk al-zuhraT 'il_A 'ab`ad
bu`dhA kanisbaT 'arba` `a^saraT 'il_A mi'aT wa-sittaT. wa-qad bayanA
'an 'ab`ad 'aflAk al-qamar al-falak al-mA'il, wa-hwa sittaT wa-sittIn
m_tl"aN li-ni.sf qi.tr al-'ar.d wa-fawqah sumk al-muma_t_tal
wa-nufri.duhu darjaT"aN; fa-yakUn 'ab`ad bu`d 'aflAk al-qamar sab`aT
wa-sittIn, wa-hwa 'aqrab qurb 'aflAk `.tArd wa-'i_dA .darabnA _dalika
fI nisbaT `.tArd, wa-hwa tis`aT wa-_tamAnUn wa-ni.sf, wa-qasamnA
al-.hA.sil `al_A al-'a.had wa-al-_talA_tIn, _haraja mi'aT wa-_talA_taT
wa-tis`Un wa-_tul_t
\VAR{wa-`u^sr}{`u^sr \iscomplet{[\ma,\md,\mc,\me]}{[\ma,\md,\mc]}}
bi-al-taqrIb: wa-hwa
'ab`ad bu`d 'aflAk `.tArd. fa-'i_dA .darabnA _dalika fI 'ak_tar nisbaT
al-zuhraT, wa-_dalika mi'aT wa-sittaT, wa-qasamnA \fol{.z 43 \ma}
al-.hA.sil `al_A 'arba`aT `a^sar,
_haraja 'alf wa-'arba`mi'aT wa-'arba`aT wa-sittUn wa-'arba`aT asbA`:
wa-hwa 'ab`ad bu`d 'aflAk al-zuhraT. wa-hwa yanqu.s `an 'aqrab qurb
'aflAk al-^sams _hamsaT 'ajzA' wa-_tul_tay juz' wa-rub` juz':
wa-_dalika itti.sAl 'aflAk al-^sams.
\VAR{fa-tubayyin}{.gayr maqrU' [\ma]}
\VARC{imkAn}{an makAn [\me]}
al-zuhraT wa-`.tArd t.ht al-^sams, _hilAf"aN lil-mu'ayyad
al-`ur.diy wa-li-ibn afla.h.

\clearpage
\begin{center}
\large al-fa.sl al-_tAli_t

\normalsize fI ma`rifaT ab`Ad al-_talA_taT al-`alwiyaT min markaz al-'ar.d
(bi-im_tAl ni.sf qi.trhA)
\end{center}
qad bayanA fI hI'aT 'aflAk
\VAR{al-_talA_taT}{al-_talA_taT al-`alwiyaT [\mc]} 'an nisbaT aqrab qurb
'aflAk al-mirrI_h 'il_A ab`ad bu`dhA kanisbaT _tamAniyaT 'il_A mi'aT
wa-'i_tn_A `a^sar, wa-nisbaT 'aqrab qurb 'aflAk al-mu^stariy 'il_A
'ab`ad bu`dhA ka-nisbaT 'i_tnayn wa-'arba`In 'il_A _tamAniyaT
wa-sab`In, wa-nisbaT 'aqrab qurb 'aflAk zu.hal 'il_A 'ab`ad bu`dhA
ka-nisbaT sittaT wa-'arba`In 'il_A 'arba`aT wa-sab`In. wa-qad tuqaddim
'anna 'in 'ab`ad bu`d .hAmil al-^sams 'alf wa-_tamAn-mi'aT
wa-_talA_taT wa-_talA_tUn \VAR{ma_tal"aN}{mIl"aN [\mc]}
wa-_tul_tAn wa-`u^sr \VAR{mi_tl}{mIl [\mc]}, wa-fawq
_dalika smk al-muma_t_tal wa-nufri.duhu \aemph{w _Ad}, fa-ybla.gu 'alf
wa-_tamAn-mi'aT wa-tis`In: wa-hwa 'aqrab qurb 'aflAk al-mirrI_h
fa-'i_dA .darabnAhu fI 'ak_tar nisbaT al-mirrI_h, wa-qasamnA mA bala.ga
`al_A 'aqallhA, .ha.sala sittaT wa-`i^srUn 'alf"aN wa-'arba`-mi'aT
wa-sittUn: wa-hwa 'ab`ad bu`d 'aflAk al-mirrI_h. wa-'i_dA .darabnA
_dalika fI 'ak_tar nisbaT al-mu^stariy, wa-qasamnA mA bala.ga `al_A
'aqallhA, .ha.sala \fol{w 47 \mc} tis`aT wa-'arba`Un 'alf"aN wa-mi'aT
wa-'arba`Un bi-al-taqrIb: wa-hwa 'ab`ad bu`d 'aflAk al-mu^stariy.
wa-'i_dA .darabnA _dalika fI 'ak_tar nisbaT zu.hal, wa-qasamnA mA
.ha.sala `al_A 'aqallhA,
.ha.sala tis`aT wa-sab`Un 'alf"aN wa-'a.had wa-_hamsUn wa-suds marraT
wa-_tumn: wa-hwa 'ab`ad bu`d 'aflAk zu.hal, wa-hwa 'aqrab qurb
al-kawAkib al-_tAbitaT. ha_dA 'aqall mA yumkin; wa-yumkin 'an yakUn
'ak_tar min _dalika. \VARC{wa-al-ll_ah 'a`lam}{nAqi.saT [\me]}.

\clearpage
\begin{center}
\large al-fa.sl al-rAbi`

\normalsize fI maqAdIr 'ajrAm al-kawAkib al-_hamsaT al-muta.hayyaraT
\end{center}
\VARC{qad}{wa-qad [\me]} ra.sada 'ibar_hus
\VAR{wa-b.tulamiyUs}{_tumma b.tulamiyUs [\md,\mc]} iq.tAr
ha_dihi al-kawAkib, fa-wajadUA qi.tr `.tArd juz' min _hamsaT `a^sar min
qi.tr al-^sams, wa-al-zuhraT juz' min `a^saraT, wa-al-mirrI_h juz' min
`i^srIn, wa-zu.hal juz' min _tamAniyaT `a^sar, wa-al-mu^stariy juz' min
'i_tnA `a^sar; wa-lam ya_dkurUA fI 'ayy al-ab`Ad kAna ra.sadhA.
wa-i_htAr b.tulamyUs kawnihA fI bu`dihA al-'awsa.t, wa-i_htAra
al-muta'a_h_hirUn min mu.haqqaq_A ha_dA al-fann kawnihA fI bu`dihA
al-'aqrab, 'illA `u.tArd
\VAR{dUnihim}{fa-'annahum [\md], nAqi.saT [\mc]} i_htArUA
kawnihi \fol{w 44 \ma} fI bu`dihi al-'awsa.t.

wa-'i_d qad tqddm _dalika, \fol{.z 51 \md}
\VARC{fa-'innA 'i_dA}{fa-'i_dA [\me]}
qasamnA bu`d al-^sams al-'awsa.t `al_A qi.trhA, _haraja mi'aT
wa-_tamAniyaT 'ajzA' wa-ni.sf wa-_hums; fa-t.hf.z ha_dA al-`adad; _tumma
tqsm bu`d `u.tArd al-'awsa.t wa-hwa 130 wa-_talA_taT `a^sar daqIqaT
`al_A nisbaT qi.trh min al-^sams wa-_dalika _hamsaT `a^sar, ta_hruju
_tamAniyaT 'ajzA' wa-'arba`Un daqIqaT tqsm `al_A al-`adad al-ma.hfU.z,
y_hruju 'arba` daqA'iq wa-'arba`aT a_hmAs daqIqaT: wa-hwa qi.tr `.tArd
`al_A 'anna qi.tr al-'ar.d wA.hid"aN.

\VAR{wa-'i_dA}{wa-alA [\mc]} a_ha_dnA min bu`d al-zuhraT al-'awsa.t
(alla_dI hwa _tamAn-mi'aT wa-tis`aT wa-`i^srUn) `u^srh,
wa-qasamnA _dalika `al_A al-`adad al-ma.hfU.z,
_haraja _tul_tay juz' wa-`u^sr juz': wa-hwa qi.tr al-zuhraT `al_A
'anna qi.tr al-'ar.d wA.hid"aN.

wa-'ammA al-mirrI_h, fa-'innA, 'in ja`alnA
al-nisbaT lahu fI bu`dh al-'awsa.t, ru'y fI bu`dh al-'aqrab 'ak_tar min
al-zuhraT; wa-lam yUjid ka-_dalika, wa-'innamA a_ha_dnA ha_dihi al-nisbaT lahu
'i_dA kAna fI-mA bayna bu`dihi al-'awsa.t wa-al-'aqrab, wa-_dalika
\VAR{`inda}{nAqi.saT [\md,\mc]} kawn
bu`dihi min al-'ar.d _tamAniyaT 'AlAf wa-'i_tnayn wa-_talA_tIn marraT mi_tl
ni.sf qi.tr al-'ar.d.
fa-'i_dA 'a_ha_dnA min ha_dA al-`adad ni.sf `u^srahu, 
wa-qasamnAh `al_A al-mi'aT wa-al-_tamAniyaT wa-al-ni.sf wa-al-_hums, _haraja
_talA_taT 'ajzA' wa-_tul_tA juz' bi-al-taqrIb: wa-hwa qi.tr al-mirrI_h `al_A
'anna\fol{.z 47 \mc} qi.tr al-'ar.d wA.hid"aN.

wa-'ammA al-mu^stariy, fa-'innA 'in ja`alnA lahu ha_dihi al-nisbaT
wa-hwa fI bu`dihi al-'awsa.t, fa-'innA 'i_dA qasamnA bu`dhi al-'awsa.t
(alla_dI hwa sab`aT wa-_talA_tUn 'alf"aN wa-_tamAn-mi'aT) `al_A 'i_tn_A
`a^sar, _haraja _talA_taT \VARC{'AlAf}{nAqi.saT [\me]} wa-mi'aT
wa-_hamsUn; fa-tqsmhA `al_A al-mi'aT wa-al-_tamAniyaT wa-al-ni.sf
wa-al-_hums, fa-y_hruju ts` wa-`i^srUn bi-al-taqrIb: fa-qi.tr
al-mu^stariy mi_tl qi.tr al-'ar.d ts` wa-`i^srUn marraT.

\clearpage
\noindent wa-'in ja`alnA
lahu ha_dihi al-nisbaT wa-hwa fI bu`dihi al-'aqrab, alla_dI hwa
_tamAniyaT wa-`i^srUn 'alf"aN wa-_tamAn-mi'aT wa-'i.hd_A `a^sar
bi-al-taqrIb (li-'anna kawkab al-mu^stariy lA ya.silu 'il_A 'aqrab qurb
'aflAkihi allatI hiya 'ab`ad bu`d al-mirrI_h), fa-'inna qi.tr
al-mu^stariy ya_hruju mi_tl qi.tr al-'ar.d _talA_taT wa-`i^srIn marraT.
wa-yakUn \VARC{muka``ab}{nAqi.saT [\me]} 'i_tn_A `a^sar 'alf"aN
wa-mi'aT wa-sab`aT wa-sittIn, wa-hiya nisbaT jarimh 'il_A jarim
al-'ar.d: fa-jarimh qadr jarim al-'ar.d 'i_tn_A `a^sar 'alf marraT
wa-mi'aT wa-sab`aT wa-sittIn marraT bi-al-taqrIb.

wa-'ammA zu.hal, fa-'innA ja`alnA lahu al-nisbaT al-mu_dkUraT fI 'aqrab
qurbihi, wa-hwa mi_tl 'ab`ad bu`d al-mu^stariy ma`a ziyAdaT .hAmil
zu.hal: wa-_dalika al-bu`d tis`aT wa-'arba`Un 'alf"aN
wa-tis`-mi'aT\fol{.z 44 \ma} wa-_tamAniyaT wa-sittUn.
fa-taqasamh `al_A nisbaT qi.tr zu.hal min
qi.tr al-^sams (wa-hwa _tamAniyaT `a^sar), \iscomplet{\VARX{ya_hruju}{'alfAni
    wa-sab` mi'aT wa-sittaT wa-sab`Un. taqasamhA `al_A al-mi'aT
    wa-al-_tamAniyaT wa-al-ni.sf}{wa-al-_hums (al-ma.hfU.z)}{nAqi.saT
    [\me]}}{ya_hruju 'alfAni wa-sab` mi'aT wa-sittaT wa-sab`Un.
  taqasamhA `al_A al-mi'aT wa-al-_tamAniyaT wa-al-ni.sf
  wa-al-_hums (al-ma.hfU.z)},
ya_hruju _hamsaT wa-`i^srIn wa-_tul_t wa-_hums
bi-al-taqrIb: wa-hwa qi.tr zu.hal `al_A 'anna qi.tr al-'ar.d wA.hid"aN.

wa-'ammA al-kawAkib al-_tAbitaT, fa-'inna mA kAna minhA fI al-qadr
al-'awwal fa-qi.trhu juz' min `i^srIn min qi.tr al-^sams, wa-alla_dI fI
al-qadr al-_tAniy qi.truhu juz' min 'i_tnayn wa-`i^srIn, wa-mA kAna
minhA fI al-qadr al-_tAli_t fa-qi.trh juz' min 'arba`aT wa-`i^srIn,
wa-mA kAna minhA fI \VAR{al-qadr}{nAqi.saT [\mc]} al-rAbi`
fa-qi.trh juz' min sitt"iN wa-`i^srIn,
wa-mA kAna minhA fI al-qadr al-_hAmis fa-qi.trh juz' min
_tamAniyaT wa-`i^srIn, wa-mA kAna minhA fI al-qadr al-sAdis fa-qi.trh
juz' min _talA_tIn min qi.tr al-^sams 'i_dA kAnat fI bu`dhA al-'awsa.t.
fa-i`raf ha_dihi al-a`dAd, _tumma aqsam 'ab`ad bu`d 'aflAk zu.hal
(wa-hwa tis`aT wa-sab`Un 'alf"aN wa-'a.had wa-_hamsUn) `al_A al-mi'aT
wa-al-_tamAniyaT wa-al-ni.sf wa-al-_hums (al-mu.hfU.z), y_hruju
sab`a-mi'aT wa-sab`aT wa-`i^srUn wa-rub`: wa-nsmh al-'a.sl.
\VAR{fa-'i_dA}{fa-'in \iscomplet{[\md,\mc,\me]}{[\md,\mc]}}
qasamnA ha_dA al-`adad `al_A `i^srIn,
_haraja qi.tr al-kawAkib allatI fI al-qadr al-'awwal; wa-'i_dA qasamnAh
`al_A 'i_tnayn wa-`i^srIn, _haraja qi.tr alla_dI fI al-`a.zm al-_tAniy;
wa-'i_dA qasamnAh \fol{w 52 \md} `al_A \fol{w 48 \mc} 'arba`aT wa-`i^srIn,
_haraja qi.tr alla_dI fI al-qadr al-_tAli_t;
wa-'i_dA qasamnAh `al_A sittaT wa-`i^srIn,
_haraja qi.tr alla_dI fI al-qadr al-rAbi`;
wa-'i_dA qasamnAh `al_A _tamAniyaT wa-`i^srIn,
_haraja qi.tr alla_dI fI al-qadr al-_hAmis;
wa-'i_dA qasamnAh `al_A _talA_tIn,
_haraja qi.tr alla_dI fI al-qadr al-sAdis.

\clearpage
\noindent \VAR{fa-qasamnA}{fa-'i_dA qasamnA [\mc]} `al_A al-'a`dAd
al-ma_dkUraT; \VAR{fa-_haraja}{_haraja [\mc]} qi.tr alla_dI fI
al-qadr al-'awwal sittaT wa-_talA_tUn marraT wa-_hums wa-suds marraT,
wa-_haraja qi.tr allatI fI al-qadr al-_tAniy _talA_taT wa-_talA_tUn
marraT wa-ni.sf sub` marraT bi-al-taqrIb, wa-_haraja qi.tr
\VAR{allatI}{alla_dI [\md,\mc]} fI al-qadr al-_tAli_t _talA_tUn marraT
wa-_hums wa-suds marraT, wa-_haraja qi.tr
\VAR{allatI}{alla_dI [\md,\mc]} fI al-qadr al-rAbi` _tamAniyaT wa-`i^srUn
marraT bi-al-taqrIb, wa-_haraja qi.tr allatI fI al-qadr al-_hAmis sittaT
wa-`i^srUn marraT bi-al-taqrIb, wa-_haraja qi.tr allatI fI al-qadr
al-sAdis 'arba`aT wa-`i^srUn marraT wa-_hums wa-suds marraT.

fa-'i_dA ka`abnA iq.tAr al-kawAkib al-muta.hayyaraT wa-al-_tAbitaT,
kAna _dalika nisbatihA 'il_A al-wA.hid alla_dI hwa muka``ab qi.tr
al-'ar.d. 'ammA al-qamar wa-al-^sams fa-qad tuqaddim _dalika. wa-'ammA
`.tArd, qi.truhu 'arba`\fol{w 45 \ma} daqA'iq wa-'arba` a_hmAs daqIqaT,
wa-muka``ab _dalika _tAniyaT wa-sittaT wa-'arba`Un _tAli_taT wa-_hamsaT
wa-'arba`Un rAbi`aT wa-sab` _hawAmis; fa-nisbaT jarimh 'il_A
\VARC{jarim}{nAqi.saT [\me]} al-'ar.d kanisbaT al-wA.hid 'il_A
'alfayn wa-_hamsaT wa-`i^srIn bi-al-taqrIb.

wa-qi.tr al-zuhraT sittaT wa-'arba`Un daqIqaT; wa-muka``ab _dalika
sab`aT wa-`i^srUn daqIqaT, fa-hiya _hums_A kuraT al-'ar.d wa-ni.sf `u^srihA.

wa-'ammA qi.tr al-mirrI_h faqad bayanA 'annahu _talA_taT 'ajzA'
wa-_tul_tA juz' `al_A 'anna qi.tr al-'ar.d wA.hid"aN; fa-yakUn
muka``abh tis`aT wa-'arba`Un wa-suds wa-_tumn; fa-jarim al-mirrI_h
qadara al-'ar.d tis`aT wa-'arba`In marraT wa-suds wa-_tumn marraT
bi-al-taqrIb.

\VAR{wa-qi.tr}{wa-'ammA qi.tr [\mc]} al-mu^stariy mi_tl qi.tr al-'ar.d
tis`aT wa-`i^srIn marraT;
wa-muka``ab qi.trh 'arba`aT wa-`i^srUn 'alf"aN wa-_talA_t-mi'aT
wa-tis`aT wa-_tamAnUn, wa-jarimh qadr jarim al-'ar.d 'arba`aT
wa-`i^srUn 'alf marraT wa-_talA_t-mi'aT wa-tis`aT wa-_tamAnIn ha_dA,
'in kAnat al-nisbaT li-qi.trh min qi.tr al-^sams fI bu`dh al-'awsa.t
(wa-'in kAnat fI bu`dh al-'aqrab fa-`al_A mA tuqaddim qabla _dalika).
fa-i`rafh.

wa-'ammA qi.tr zu.hal, fa-mi_tl qi.tr al-'ar.d _hamsaT wa-`i^srIn
marraT wa-_tul_t wa-rub` marraT; wa-muka``abh sittaT `a^sar 'alf"aN
wa-mi'atayn wa-'arba`aT wa-tis`In wa-ni.sf wa-_tumn bi-al-taqrIb;
\fol{.z 48 \mc} fa-jarim zu.hal qadara jarim kuraT al-'ar.d sittaT
`a^sar 'alf marraT wa-mi'atayn wa-'arba`aT wa-tis`In marraT.

\clearpage

wa-'ammA al-kawAkib al-_tAbitaT, fa-a`.zmhA, wa-hwa alla_dI fI al-qadr
al-'awwal fa-qi.trh mi_tl qi.tr al-'ar.d sittaT wa-_talA_tIn marraT
wa-_hums marraT wa-suds marraT bi-al-taqrIb; wa-muka``ab _dalika sab`aT
wa-'arba`Un 'alf"aN wa-sitt-mi'aT wa-'arba`aT wa-_hamsUn majbUr"aN;
wa-jarimhA min jarim al-'ar.d ka-_dalika, 'a`niy mi_tl al-'ar.d sab`aT
wa-'arba`In 'alf marraT wa-sitt-mi'aT wa-'arba`aT wa-_hamsIn marraT
bi-al-taqrIb.

wa-'ammA 'a.s.gar al-_tawAbit, allatI fI al-qadr al-sAdis,
fa-qi.tr 'a.hadhA mi_tl qi.tr al-'ar.d 'arba`aT wa-`i^srIn marraT
wa-_hums wa-suds marraT; wa-muka``ab _dalika 'arba`aT `a^sar 'alf"aN
wa-'arba`-mi'aT wa-_talA_taT wa-sittUn bi-al-taqrIb; fa-jarimhA mi_tl
jarim al-'ar.d 'arba`aT `a^sar 'alf marraT wa-'arba`-mi'aT
wa-_talA_taT wa-sittIn marraT.

ha_dihi al-maqAdIr, `al_A mUjib al-u.sUl al-.sa.hI.haT, lA yumkin 'an
yakUn 'a.s.gar min _dalika; wa-yumkin 'an yakUn 'akbar, wa-lA
\VARC{yasta`.zimu}{tasta`.zimu [\me]} _dalika. fa-`i.zmaT ul-ll_ah
ta`AlI a`.zm, wa-qdrth awsa`, wa-hwa `al_A kull ^say' qadIr. wa-jamI`
al-mutaqaddimIn
\VAR{mujmi`In}{mujmi`Un \iscomplet{[\md,\me]}{[\md]}, ajm`UA [\mc]}
`al_A al-`aml bi-mUjib al-ar.sAd allatI 'addat 'il_A ha_dihi al-a^siyA'.
wa-qad tukarriru min b.tulamiyUs an \fol{.z 45 \ma}
qAla 'ammA al-ab`Ad fa-lA yumkin an yakUn 'aqall mimmA
\VARC{_dakarnA}{_dakara [\me]}; wa-'ammA al-ajrAm fa-hiya taba`
\VARC{lil-ab`Ad}{al-ab`Ad [\me]}, fa-'in kAnat al-ab`Ad
ak_tar \fol{.z 52 \md} kAnat al-ajrAm ak_tar wa-lA yan`akisu;
wa-laysa ha_dA bi-mustaq.s_A fI ha_dA al-naw`; wa-qad nAqa.da nafsahu
fI kitAbihi \VARC{alla_dI smAh \textbf{bi-al-iqti.sA.s}}{al-musamm_A [\me]},
fI al-hI'aT wa-fI al-ajrAm. wa-tasa'al l-ll_ah ta`AlI al-tawfIq
\VARC{wa-al-hdAyaT wa-hwa .hasbunA wa-ni`ma al-wakIl}{nAqi.saT [\me]}.

\begin{center}
tanbIh
\end{center}
kull kuraT qi.trhA ma`lUm, fa-dawrhA ma`lUm, wa-'ajzA' al-dawr
ma`lUmaT, wa-musA.haT basI.thA ma`lUmaT, wa-musA.haT jarimhA ma`lUmaT.
wa-kull miqdAr ma`lUm \VAR{bi-miqdAr}{fawqa al-sa.tr [\ma]}, fa-hwa
ma`lUm
\VAR{bi-kull}{kull \iscomplet{[\ma,\me]}{[\ma]}}
mA yu`lam bihi _dalika al-miqdAr.
mi_tAlh: ab`Ad al-aflAk wa-ajrAm al-kawAkib ma`lUmaT bi-miqdAr ni.sf
qi.tr al-'ar.d, wa-ni.sf qi.tr al-'ar.d ma`lUm
\VAR{bi-al-frAsa_h}{bi-al-farsa_h [\mc]} wa-al-amiyAl wa-al-a_dra`
wa-al-a.sAbi` wa-al-^sa`IrAt; fa-ka-_dalika al-ab`Ad wa-al-ajrAm
ma`lUmaT bi-ha_dihi al-maqAdIr.

\clearpage

wa-i`lam 'annA 'i_dA zadnA `al_A ab`ad bu`d aflAk zu.hal iq.tAr
al-kawAkib al-_tAbitaT, kAna _dalika ab`ad bu`d al-kawAkib al-_tAbitaT;
wa-jA'iz 'an yakUn ak_tar min _dalika bi-mA ^sA al-ll_ah ta`alI,
wa-.gayr jA'iz 'an yakUn 'aqall\fol{w 49 \mc} min _dalika, ka-mA `alamtu.
fa-yakUn
ab`ad bu`d al-_tAmin 'aw aqrab qurb al-tAsi` lA yanqu.s `an
\VAR{tis`aT wa-sab`In 'alf"aN wa-_tamAniyaT wa-_tamAnIn}{tis`aT
wa-tis`In 'alf"aN wa-_tamAniyaT wa-_tamAnIn [\md], 99088 [\mc]}
mi_tl"aN li-miqdAr ni.sf qi.tr al-'ar.d; fa-ha_dA hwa ni.sf qi.trh,
fa-'i_dA a.d`aftuhu wa-.darabtu _dalika fI _talA_taT wa-sub`,
.ha.sala dawr maq`ar al-tAsi`; fa-'i_dA qasama al-dawr
`al_A _talA_t-mi'aT wa-sittIn, .ha.sala
.hi.s.saT darjaT \VAR{wA.hid}{wA.hidaT [\md]} min
\VAR{mu.hI.t}{fawqa al-sa.tr [\ma]} maq`ar al-tAsi`;
wa-'i_dA \VAR{qasama}{qasamat [\mc]} al-darjaT `al_A sittIn,
.ha.sala .hi.s.saT daqIqaT wA.hidaT minh.
wa-qad .darabnA ni.sf qi.tr ma.hdab kuraT
al-kawAkib al-_tAbitaT (wa-hwa \VAR{tis`aT wa-sab`Un 'alf"aN wa-_tamAniyaT
wa-_tamAnIn}{tis`aT wa-tis`Un 'alf"aN wa-_tamAniyaT wa-_tamAnUn [\md],
99088 [\mc]}) fI _talA_taT wa-sub`,
wa-a.d`afnA mA bala.ga, fa-.ha.sala
mu.hI.t a`.zam dA'iraT yaqa`u `al_A sa.t.h al-_tAmin (wa-hwa musAw
li-maq`ar al-tAsi`): wa-_dalika 497124
\VAR{wa-'arba`aT asbA`}{wa-'arba`aT atsA` [\md],
$\dfrac{\text{4}}{\text{9}}$ [\mc]}.
_tumma qasamnA
_dalika `al_A _talA_t-mi'aT wa-sittIn, fa-.ha.sala 1380 wa-_tul_tAni
wa-rub`: wa-hwa .hi.s.saT darjaT wA.hidaT min dawr maq`ar al-tAsi`.
fa-qasamnA _dalika `al_A sittIn, fa-.ha.sala _talA_taT wa-`i^srUn
wa-ksr (li-mi_tl ni.sf qi.tr al-'ar.d): wa-hwa daqIqaT wA.hidaT.
wa-hwa bi-miqdAr mA
\VAR{y`d insAn sitaT msr`A}{\iscomplet{b`d insAn sanaT msr`A [\me], }{}
  y`dUA nisAn sanaT musr`"aN [\md], y`dUA
  insAn sanaT musr` [\mc]};
fa-yakUn bi-miqdAr mA \VARC{yqUl}{taqUl [\me]}
insAn"uN wA.hid, yata.harrak
al-falak mi_tl \VAR{qi.tr}{nAqi.saT [\md]} al-'ar.d
\VAR{marratayn}{fI hAmi^s [\ma]} bi-al-taqrIb. fa-qad tubayyinu 'anna
al-falak al-tAsi` 'i_dA ta.haraka darjaT, wa-hwa _tul_t _hums sA`aT,
ta.haraka bi-qadr ni.sf qi.tr al-'ar.d 'alf wa-_talA_t-mi'aT
wa-_tamAnIna wa-_tul_tayn wa-rub`. wa-'i_dA \fol{w 46 \ma} ta.haraka
daqIqaT, ta.harrak
bi-miqdAr ni.sf qi.tr al-'ar.d _talA_taT wa-`i^srIn marraT. ha_dA `al_A
far.d muqa``arh; wa-'ammA smkh \VAR{fa-mA}{fa-lA [\mc]} y`lmh 'illA
al-ll_ah
\VAR{ta`AlI}{nAqi.saT \iscomplet{[\ma,\mb,\md]}{[\ma,\md]}}
\VAR{`azza wa-jalla}{nAqi.saT [\mc]}; fa-yakUn musAfaT al-darjaT
\VAR{fI}{min [\mc]} mu.haddab a`.zam min al-musAfaT
\VAR{fI}{min \iscomplet{[\mb,\mc]}{[\mc]}}
muqa``arh bi-mA lA y`lmh 'illA al-ll_ah
\VAR{ta`AlI}{nAqi.saT \iscomplet{[\ma,\mb,\md,\mc]}{[\ma,\md,\mc]}}
`azza wa-jalla
\VAR{ts.hAnh wa-ta`AlI}{nAqi.saT \iscomplet{[\mb,\md,\mc]}{[\md,\mc]}}.

\clearpage

\begin{center}
tanbIh
\end{center}
i`lam 'anna al-zuhraT wa-al-mirrI_h lA yur_A qi.trhmA `al_A muqta.d_A
ab`AdhmA. li-anna ab`ad bu`d kull wA.hid minhumA a.d`Af li-aqrab qurbh; 
\VARC{fa-kAna}{wa-kAna [\me,\mb]}
yujib 'an yakUn al-aq.tAr \VARC{taba`}{ma`a [\mb]}
al-ab`Ad, a`niy 'an yur_A al-kawkab, fI aqrab qurbih,
a.d`Af qi.trh fI ab`ad bu`dh; wa-lam yura _dalika.

'ammA b.tulamiyUs fa-qAla: >>al-sabab alla_dI min
\VAR{ajlihi}{a.slihi \iscomplet{[\me,\mb,\md]}{[\md]}}
.sAra mA ya.zhuru lil-ba.sar wa-_Ata_hayyal
'ilayhi min `i.zm al-jarim laysa `al_A mi_tl nisb
\VARC{ab`AdhA}{ab`AdhimA [\mb]}, fa-ynb.gI lanA 'an n`lm anh al-.gala.t
alla_dI \fol{.z 49 \mc} yd_hl `al_A al-ba.sr min qabla i_htilAf al-man.zar.
wa-yatabayyan _dalika fI jamI` mA y.zhr lil-`ayn
(\VAR{wa-lA tufA.dil}{wa-tufA.dil \iscomplet{[\me,\mb,\md]}{[\md]}}
mA bayna al-a^syA' al-mu_htalifaT al-aqdAr, bi-`ilm li-nuq.sAnihA al-dA'im).
li-_dalika yur_A kull wA.hid min al-kawAkib qarIb"aN minnA
\VARC{ak_tar}{akbar [\me,\mb]} min .hAl .haqIqatah, li-in.hi.tA.t
\VARC{al-ba.sar}{nAqi.saT [\me]} 'il_A al-ab`Ad allatI
\VAR{qad}{nAqi.saT [\md,\mc]} a`tAdhA wa-alfhA. fImA
\VAR{bayanA}{.gayr maqrU' [\ma,\mc], baynanA \iscomplet{[\mb,\md]}{[\md]}}
\fol{w 53 \md} \VAR{li-_dalika}{ka-_dalika [\md]} al-.hAl fI al-ziyAdAt
wa-al-nuq.sAnAt allatI t`r.d lil-`.zm bi-.husb ziyAdaT al-ab`Ad
wa-nuq.sAnihA, fa-'innahA \VARC{takUn}{yakUn [\me]} 'aqall min
al-nisbaT allatI hiya lahA, li-`ajz al-ba.sr, ka-mA qulnA `an tamyIz
wa-'idrAk kammiyyaT \VARC{tfA.dil}{tfA.sil [\mb]} kull naw` mimmA
_dakarnA.<< ha_dA jawAb b.tulamiyUs `an _dalika, wa-alla_dI `indiy fI
_dalika:

-- 'anna
\VAR{al-kurAt}{al-kawAkib \iscomplet{[\me,\mb,\md]}{[\md]}} 'i_dA
qarabat min al-ba.sr, kAna mA ya.zharu minhA 'aqall mimmA kAna ya.zharu
ma`a al-bu`d.

-- wa-inna al-ajsAm al-nIraT lA ydrk al-ba.sr .haqIqaT
aq.tArhA
\VAR{li-istiqbAl}{li-i^sti.gAl \iscomplet{[\me,\mb,\md,\mc]}{[\md,\mc]}}
al-ba.sr \VARC{bi-^si`A`}{^si`A` [\me]} al-nUr.

-- wa-inna al-ba.sr ma`a al-bu`d lA yr_A al-a^syA' `al_A mA hiya `alayhi.

wa-mimmA
\VARC{yU.d.h}{nAqi.saT [\mb]} _dalika annah, 'i_dA fr.d jismAn kuriyyAni,
\VARC{qi.tr}{fI hAmi^s [\mb]} 'a.hadhumA .d`f qi.tr al-'A_har,
wa-na.zara 'ilayhimA min bu`d lam yumkin al-ba.sr adrAk .haqIqaT
miqdAr al-qi.trayn, wa-lA y`In an \VAR{qi.tr 'a.hadhimA .da`f
  al-'A_har}{'a.hadhimA qi.trh .d`f qi.tr al-'A_har [\mc]}, wa-lA
yumkin \VARC{ta.hqIq}{.haqIq [\mb]} _dalika bi-'AlaT"iN min al-'AlAt,
ma` al-`ilm bi-an qi.tr a.hadhmA .da`f qi.tr al-'A_har.

\clearpage
\noindent wa-in \VAR{.harrara}{jwz [\mc]} al-ba.sr taqrIb
miqdAr 'a.had al-qi.trayn min al-'A_har; _tumma
\VAR{fr.dnA}{fr.dA \iscomplet{[\ma,\me]}{[\ma]}}
baqA'a 'a.hadhumA fI makAnihi wa-ta.harrak al-'A_har .da`f _dalika al-bu`d;
lam ya.htamil lil-ba.sr i_htilAf mA kAna \VAR{.harrarh}{jwzh [\mc]}
ma` al-`ilm bi-_hilAf al-'awwal. wa-naw` 'A_har, law waqa`a al-ba.sr
`al_A .dU' ma.sbA.h min bu`d mafrU.d"iN, wa-tawahhum al-ba.sar lahu
\VAR{miqdAr"aN}{miqdAr [\md]} mA,\fol{.z 46 \ma}
_tumma qaraba minh ni.sf _dalika
al-bu`d 'aw ba`ada `anh bi-_dalika al-miqdAr, lam yu_hayyil
\VAR{lil-ba.sar}{al-ba.sar \iscomplet{[\mc,\md,\me]}{[\md,\mc]}}
\VAR{ta.gayur}{n.gayr [\ma]\iscomplet{, bi.gayr [\mb,\me]}{}}
_dalika al-miqdAr. fa-min ha_dA wa-mimmA
tuqaddim, yatarakkab al-jawAb `an al-mas'alaTi wa-`ilm .haqIqatihi, ma`a
al-bu`d `ajz al-ba.sar `an
\VAR{ta.hqIq}{.haqIqaT \iscomplet{[\mb,\mc,\md,\me]}{[\md,\mc]}}
maqAdIr al-'a^syA'. `ammA hiya `alayhi,
fa-innA njzm bi-'anna al-ba.sar, lA yumkinuhu 'i_dA waqa`a `al_A zId
wa-`umr wa-ma`a al-bu`d ta.hqIq 'ayyhumA a.twal min al-'A_har, wa-lA
\VAR{bi-'ayy}{bi-'ayyh \iscomplet{[\ma,\mb], bi-'i_trihi [\me]}{[\ma]},
  bi-atr [\md]}
miqdAr 'a.hadhumA a.twal min al-'A_har; \fol{w 50 \mc}
ha_dA ma`a al-bu`d alla_dI hwa bi-al-nisbaT
'il_A .gayrihi lA ^say'.% A46v l. 3-5
fa-'innh qad itt.d.h an ab`ad bu`d
al-mirrI_h sittaT wa-`i^srUn 'alf"aN wa-'arba`-mi'aT wa-sittUn
bi-miqdAr ni.sf qi.tr al-'ar.d. \VAR{fa-ysqu.tu}{fa-saqa.ta [\ma]}
.hikm al-ba.sar `al_A al-maqAdIr ma`a 'aqall min ha_dA al-bu`d
bi-ka_tIr; fa-hwa, ma`a ha_dA, ak_tar nfUr"aN `an ta.hqIq al-maqAdIr ma`a
anA nadruku i_htilAf aq.tAr al-kawAkib fI sA'ir ab`AdhA wa-_A_hisu
bihi ('illA 'annahu `al_A .gayr mA \VAR{yaqta.diyh}{taqta.diyh
  [\mc,\md]} \VARC{nisb}{bi-sabab [\mb], nisbaT [\me]} al-ab`Ad
kamA aw.da.hnA). wa-min hunA, yfhamu 'anna al-kawAkib ajsAm nyyraT nUrhA
min _dAthA, lA ka-al-qamar fa-inh jism ka_tIf wa-nUrh \VARC{`r.diy}{`r.d
  [\mb]} min in`ikAs ^si`A` al-^sams `al_A sa.t.hh. wa-bi-ha_dA
al-sabab 'amkan ta.hrIr qi.trh fI sA'ir ab`Adh min al-'ar.d, _hilAf
.gayrh min al-kawAkib.

\clearpage

fa-ha_dA 'A_hir mA qa.sadnA 'iyrAdh fI ha_dihi al-maqAlaT. \VAR{wa-ytlU
  ha_dihi al-maqAlaT maqAlaT _tAniyaT fI hI'aT al-'ar.d wa-mA
  yalzmhA}{fI hAmi^s [\ma]}. wa-nutba`u _dalika bi.hisAb jadAwil
ta`AdIl al-kawAkib `al_A muqta.d_A ha_dihi al-u.sUl fI maqAlaT
_tAli_taT 'in ^sA' al-ll_ah ta`AlI. wa-al-marjuww min muta.saffi.h
ha_dA al-kitAb an lA ynkr mA lA y.hI.t bihi `lmh, \VARC{wa-yslk}{wa-nslk
  [\mb]} mslk al-.haqq wa-al-an.sAf, wa-yatajanib .tarIq al-`nAd. fa-inh
min qAbil bayna ha_dihi al-u.sUl wa-bayna mA tklfh al-mutaqaddimUn
wa-al-muta'a_h_hirUn \VAR{fI _dalika}{nAqi.saT [\mc]} wa-slk fI
_dalika .tarIq al-.haqq, \VAR{.zhr}{.zhrt [\mc]} lah .sa.h.haT mA
\VARC{awrdnAh}{aradnAh [\mb,\me]} wa-wu.dU.h al-.tarIq alla_dI
\VAR{slknAh}{qad slknAh [\mc]}.

wa-al-ll_ah
\VAR{al-ma^skUr}{al-mtkUr [\ma],
  al-mas'Ul [\md]\iscomplet{, nAqi.saT [\mb]}{}}
al-ma.hmUd \VAR{wa-bihi}{bihi [\md]} n`t.sam wa-`alayhi
natawakal \VAR{wa-hwa}{fa-'innahu [\mc]} .hsnA wa-ni`m al-wakIl.

\end{arab}

